Disentangling Perceptions of Offensiveness: Cultural and Moral Correlates

Perception of offensiveness is inherently subjective, shaped by the lived experiences and socio-cultural values of the perceivers. Recent years have seen substantial efforts to build AI-based tools that can detect offensive language at scale, as a means to moderate social media platforms, and to ensure safety of conversational AI technologies such as ChatGPT and Bard. However, existing approaches treat this task as a technical endeavor, built on top of data annotated for offensiveness by a global crowd workforce without any attention to the crowd workers' provenance or the values their perceptions reflect. We argue that cultural and psychological factors play a vital role in the cognitive processing of offensiveness, which is critical to consider in this context. We re-frame the task of determining offensiveness as essentially a matter of moral judgment -- deciding the boundaries of ethically wrong vs. right language within an implied set of socio-cultural norms. Through a large-scale cross-cultural study based on 4309 participants from 21 countries across 8 cultural regions, we demonstrate substantial cross-cultural differences in perceptions of offensiveness. More importantly, we find that individual moral values play a crucial role in shaping these variations: moral concerns about Care and Purity are significant mediating factors driving cross-cultural differences. These insights are of crucial importance as we build AI models for the pluralistic world, where the values they espouse should aim to respect and account for moral values in diverse geo-cultural contexts.

==> sections/messages.tex <==
\begin{enumerate}

\item Oh yes we awful conservatives, only one solution. Put us all in zee camps und stoking up zee ovens.
\item All cats are stupid and mean
\item Oh and the Liberals never lied, LOL.
\item Especially given that they deleted your most excellent comment yesterday for no good reason.
\item Will67, histrionic is posting the same tombstone of bs in reply to post after post.
\item This is an extremely bright, ambitious, competitive woman who would love nothing more than to exceed her predecessor's time in office.'Sorry... you lost me after the first comma.
\item Typical Harper bullying....Seems to work fer domestic relations......Let's give 'er a go fer foreign relations......If it don't work we can run and hide......like at home. Get right on that John....why do you think I keep you around!
\item So f?hlt sich der Reichspropagandaminister stark genug, in seiner Position, die F?hrung der Partei die Nationalsozialistische Deutsche Arbeiter-Frage zu stellen.
\item Wow, Ultra Sensitive.....! And seems to be many assumptions. I take it you attended the party to know all these things you are saying?
\item It's well documented that you don't like Trump. The fact that you don't like Pence either is zero surprise to everyone.
\item 6 Canadians were killed in Burkina Faso not that long ago... they want to harm you in Ottawa, Ouagadougou, Nice, or New York.
\item Utter drivel and undeserving of further response.
\item Don't you just love the yahoos (not the native Americans) who refer to people as 'these people'?Yup, middle of the road attitude ...
\item Let us hope that the first casualty of the coming war will be the western mainstream media.
\item Its somewhat sad that many here confuse slant with fake. People should look up what people are talking about when the say 'fake news' before commenting.
\item It's about time.
\item Um no. If i can't eat, what good is school or a lighted street going to do for me? I know people like you in the PS won't go hungry but I will. Perhaps you should read the article in the Financial Post...
\item perhaps, dave. but then they move on to things other than directly into politics. or marry people smarter than them ...oh, wait.
\item DaleyI like the idea of ' getting over it ' with a Scot.. Maybe while we enjoy a three finger sampler of the national beverage.. And consider questions like... If I'm a white guy in Ontario will my kids qualify to be a ' national minority' Argh!
\item I am not sure what is silly, and if there is any story in what I wrote. You write about "deniers in the same tone as Inquisition spoke about heretics. Interesting. Just confirms my impression of climate change as new religion.
\item No - he does not dither - see Cuba - the GOP wont let him do a thing otherwise.
\item Joe, Joe, Joe... Try reading a newspaper or a book published outside Ontario my ignorant friend. Nobody cares about Mike Duffy west of Ontario - we just expect that kind of behaviour from the centre of our universe. BTW, have YOU tried crack?
\item If we left it up to all the Duggars families of world, what a mess we would have. Now those young girls will have to live with this incest all their lives.
\item There are approximately 1.6 billion Muslims in the world. If they all thought like ISIS, we would have been eradicated years ago.
\item Really? So basically only fire fighters are entitled to comment? Nope. Sorry. I pay the taxes. I want MY tax dollars going where it is actually NEEDED not wanted.
\item Oh...be serious ...who made it an issue... The Trailer Park.. made it.
\item Actually, he gave it away with the GST cuts -- the corporate tax cuts were simply a continuation of the plan initiated by the Liberals.
\item It should be remembered that ?Nations have no permanent friends or allies, they only have permanent interests.?
\item Yet again, the G \& M uses another female writer to promote legalization of prostitution to maintain male sexual privilege and entitlement.
\item This legislation would have no impact on Islamist males. It impacts woman, Sikhs, certain Jews above all. Are you saying one can only be Canadian if one denies one's religion?
\item The moderators are brutal; way to suppress free speech.
\item OH! What a marvellous idea!! All we'd have to do is firmly and strictly declare something like a War on Drugs.......Wait...
\item In this specific case it doesn't matter at what point you define the moment of death. The first volley of shots was lawful, even if it meant Sammy was killed by them. The second volley of shots was not lawful, even if Sammy had survived.
\item See how valuable an education is? Now you're able to accurately describe the poverty you find yourself in.
\item Weird how you say 'a Muslim male (never a female)' but don't add that same part in parenthesis after priests or rabbis when it can equally be applied there.
\item Hopefully, some of these more secular Israelis will end up in Canada.'Why?
\item Margaret Atwood bores a lot of women too.
\item Think you've 'done' it to yourself. Get some help, dude.
\item Mulroney's legacy whether you like him or not 1. North American Free Trade 2. GST if they are bad we had about 20 years to get rid of them so they must be good or we are lazy and incompetent grudgingly admit Mulroney left a legacy CHRETIEN left none
\item Itll be real interesting when Canadas Indians go to the Chinese government looking for reparations for loss of their homelands
\item They are poor because they are reliant on the drug trade and reliant on the drug trade because they are then poor. That cycle can be broken.
\item Margaret says the battle is over? Ask the bigots at trinity western, or the BC gov.
\item Take their guns away and these cowards wouldn't last the day.
\item President Dwight Eisenhower arrived at Union Station on a visit during the Second World War.'Huh? What was Eisenhower president of during WWII? The Elks club?
\item At last someone trotting out facts instead of armchair prejudices.
\item Quebec Nationalists are zealots. They don't care about finances. They care about politics of language and identity and that's it.....
\item Yet again with the personal shots without any substance to your arguments. One has to wonder about your abilities.
\item you are a closet idiot
\item https://www.whitehouse.gov/the-press-office/2015/11/06/statement-president-keystone-xl-pipeline No, he didn't.
\item That jobs in whch women predominate are lower paying is also part of the gender gap. Its not an either/or.
\item ...sure is a good thing CONs are spending our money monitoring these comments. the equallymonitored backbenchers are probably keeping tabs on here, too.
\item 'The Israeli snipers ( male and female) had a reputation for a lack of patients.''''Perhaps you are thinking of Israeli army doctors.
\item So you become more transparent by removing transparency acts. Got it.
\item Just maintain residency at your parents house. and come back and visit occasionally. Problem solved bleeding heart.
\item It's nice when a poster's punctuation mirrors the quality of their thoughts.
\item Rob Ford does not have the attention span to write editorials.
\item I've learned to look at it as more of a game where I am "beating" the traditional job market. I'm (op) only 28 and most of my friends have very little in retirement savings, few assets. They are just now getting out of student loan and auto loan debt. It feels great to know I'm living so comfortably compared to most.
\item ugh, put to rest that argument, it is so false. often people (well, me) will come to the site for the comments in response to articles and enjoy the knowledge that the sludge is not being ingested by everyone.
\item You probably really get off on the going's on in Congress. Serious stuff there.
\item Certainly not Wente, who only speaks for the Cons and their misogynist Bible-thumping puppet-masters.
\item Won? Have you been sleeping under a rock since 1975? And why would you want to change the culture? Nothing wrong with the Vietnamese.
\item Mr Paladin, the framers were, no doubt, well versed in the English language which you, evidently, are not. Try not to read things into a passage which exist neither in fact nor intent.
\item Rather a silly remark there, watchlist.
\item The whole article ignores the fact the \$3.1 billion figure is from the period covering 2001-2009. Who was in power from 01-06? Plenty of blame to go around.
\item Well we do have a surplus now. Perhaps we should give crack to all City Councillors.
\item How about the young getting off their butts and voting and/or ( gasp ) campaigning on behalf of their interests ?!The likes of Marx, Lenin, Hitler were also 'inspiring' !
\item Keep up the censorship G\&M, apparently only the Left is allowed to comment!
\item I understand the Liberal government will be bestowing two (2) taxpayer funded nannies each upon every wealthy trust fund family,
\item You claim there are gross exaggerations here. Yet, you do not cite a single one. Do you have a 'real case'? It would seem not, because you made a sweeping statement, then obviously deliberately neglected to back it up.
\item Not so much biased as clueless!
\item A truly twisted article by an obviously deeply wounded far right-wing academic.
\item It's the Pharmaceutical companies you should be watching over - duh!
\item But he is releasing his autobiography shortly so we will know what he has accomplished. It will likely be full of big words to make up for his short resume or what passes as deep thinking by JT.
\item Kevin O'leary Plays right in to the premier's hands. He may be loud. By She is much smarter then Kevin could even dream of being.
\item No country deserves someone like trump. However, the gop does.
\item Now happily the Conservatives can be consigned to their well earned oblivion.
\item Don't worry. You ARE wrong.
\item I don't agree with this (IMHO and all that, it ought to be done at the high school level) and, sorry, my comments do not exhibit 'the ugliness that ignorance produces'. I'll leave the irony of your comment to the reader to contemplate.
\item Love your grown-up, partisan-based emotional outburst! It has really helped move this comment board's mature, fact-based discussion forward. Take care.
\item if only we had a true head of state to slap hapers wrist. But we dont. We have a toad appointed by harper, acting as a rubber stamp for the other inbred rubber stamp who lives in an english castle and whose great grandson just pushed new teeth.
\item How is Harper going to take on ISIS from inside a closet ?
\item Short of taking selfies and spending billions on the world stage. Exactly how has he helped 1 Canadian? In order to get the god like accolades from fawning media?
\item I would happy see him at the end of a rope, in his spare time he was making bombs to use against Canadian forces, you do remember those pictures of him ? Want to tell that to some of our dead troops
\item  .. They invite criminals and inspire crime.... 'And without a casino there would be no criminals or crime ?!
\item Sorry to interrupt a good vapid pontification, but it's 'Sunni', not 'Suuni'.
\item what will happen to your race if you don't produce more children?'My race is the human race. There are 7 billion of us. I'm not worried./discussion.
\item Ya but in Ontario the LIberals only rip off the tax payer. The Kadhar family rips off the country.
\item who does the clown mulcair speak for then?
\item That's right, take your ball and go home... typical Con.
\item Many of you lefties seem to forget history. Martin raised EI premiums and passed all of the costs on to the provinces. You should get out more.
\item What a fool - Trudeau can try to put gloss over the obvious however the raw belly of Quebec society is showing.
\item Spoiler alert: long term consistent use of MJ can make you less bright and less motivated.
\item what a dull-witted nightmare.
\item Governments spending taxpayer dollars on terra projects in hopes it will change the climate at sometime in the future , what possibly could go wrong?........lol........
\item So the Reform party was 25 years ahead of the times? Pretty good for people the media liars referred to as Neanderthals.
\item Maybe it's time for the family owners to get off their lazy backsides and do the work themselves?
\item You think you're the only ones who deal with tragedy? There are lot's of others who make less than half of what you do. You simply aren't worth the price tag.
\item To M1717- Your ignorance of Alberta is hilarious. Oh well, if you ever become knowledgeable of Alberta you might still be welcome here..
\item I doubt anyone in Toronto has a brain, especially Simpson.
\item Trudeau: 'go ahead, watch me'Harper: 'Its too dark in here'
\item You're the second person in a week that has offended me, and many other rural people. It's B.S by the way
\item Please do not share facts. Right-wingers are uninterested. Although you can focus on his wig or how he is junior George W Bush. THAT they dot on.
\item Thats a sexist stupid comment.
\item PAS?' It doesn't need to be a physician. A nurse practitioner with a specialty in MAD?medically assisted dying?would do just as well and for less money. Whenever an article on MAD uses the word 'suicide,' I sense the menacing influence of religion.
\item So that encompasses whiny non smokers as well?
\item You can't discuss complicated things with simple voters.
\item You really don't get it, do you Patwant- or you choose not to. Do you actually read the articles that you comment on?
\item oops my bad, Little Boy and Fat Man.
\item Hi, dear Alborzagros, how are you?I woyld like just to say thank you, because you opened this page! See you soon! 
\item Ms Leitch is proof positive that having a degree doesn't mean one is educated.
\item Harper, the manipulator that he is, is using the lone wolf shooting to further his fear agenda... if you cannot see this-you are blind
\item Junior Trudeau keeps proving he is in way over his head. An attack ad wasn't necessary, Junior proves it time and again.
\item So, what are you trying to say?
\item If Grandma was a civic employee taking voting directions from a labour union, she deserves some blame for being so easily conned into bankrupting her children's cities.
\item David Smith another whiny Liberal.
\item A little levity at Xmas with animals getting into heaven , my father did not think that Protestants could get into heaven must be a strange place , wonder what time cocktails are served????
\item I wonder if Clinton will cry in public if she's ever indicted.
\item Is this a serious post?!?!
\item ; as expected you cannot read, understand and reason, or refuse to.
\item Kurds should have their right to self-determination. And if they do, Canada should support.
\item Rotherham. Try google. And then tell us who is enlightened and who are the primitives.
\item The French law has been used to stop Muslim mothers from helping out at school events and outings, and has resulted in them being ejected from the school bus in front of their children. How is that equality?
\item Gramps Maybe stay in your room with the lights out and you will feel safer.
\item You must be a new Canadian.
\item She's an empty shell... She has risen politically far beyond her abilties or intellect. She will be known as the 'Photo Op Premier' as a short footnote in BC political history.
\item Yeah, Harper can go to Helm.
\item Ken Maynard you've got some issues with reality
\item Uhm How long ago was Regan the President??? Oh wait you still gush over Trudeau I know!
\item gasoline price fixing, no way. you must also believe in UFO s and sasquatch
\item the Senate has a vote in this... HaHaHaHAAAAAHAAAAAAHAAAAArper!
\item Lefties want free speech and satire as long as the fundamentalist Muslims are not offended.
\item How about holding West and Saudis accountable.
\item Trudeau will regret his quote (said many times): 'Mr. Harper wants you to believe thereare terrorists behind every tree, under every rock'. Unfortunately, it just takes ONE treeor ONE rock to do serious damage. A boy in charge, how sad.
\item The NDP gave their vote of confidence to S. Harper to take out the Liberals.
\item Canada's evaluation process is really weak.
\item Oh so now it's their fault for being killed because they mocked a backward violent religion? Nice. Should we kill the cast members of Monty Python because they constantly mocked Christianity?
\item You were marketed to by the unions during the election. You bought it, and you're still buying it.
\item Russians have excluded themselves from civilization, by invading Ukraine.
\item There's always room for a second center-left party. Just no room for extreme right-wingers.
\item Obviously you aren't aware of the funding issues at the OTPP and all public sector pensions. Who do you think is going to fund these pensions.
\item WHAAAAAAAAAAAAAAAAAAAAAAAAAAAAA!!!!!!!!!'Stephen Harper doesn't like us after we lie about him every day!'Time for an All You Can Eat Hunger Strike!
\item 3P, how dare you confuse the issue with facts.
\item Is anyone surprised? There can't possibly be anyone still surprised by these fricken clown's antics.
\item Mor0nic post, Robert 320.
\item How can one work with 'silly'?
\item The Snake' is baaaaack. Listen and learn, suicidal lefties, why Trump will win. People care for their families. http://www.breitbart.com/2016-presidential-race/2016/09/19/trump-busts-snake-terrorist-attacks/
\item Right, real men scrape razor sharp steel across their faces at least once a day denying their natural appearance. Get over it already. Nobody is objecting to you wasting thousands of hours of your life shaving.
\item Valid question / accurate point.
\item What science degree does Simpson have? Doesn't stop him from pontificating on global warming.
\item Haven' seen the 'lisping ' insult for a while. Some posters seem to have a bit of a fetish around that.
\item The stories are because women are more thin skinned than men and demand to be protected from bad words. We must protect the women, women are weak and need protection. But they're also strong and powerful and can do anything a man can do.
\item If they return to Canada they can vote. If they remain abroad for 5+ years how is that 'valuable perspective' helping Canada?
\item Putin is really putting the sheep to work. At least it is gratifying to know that the Russian mob values Canadian perspectives.
\item Well you're presumably Canadian - so arguably it's not about you at all.
\item actually, it is you who is not objective Canadians voted the CPC a majorty based on this policy
\item Judging by your thumbs down, you must have touched a raw nerve with the Ontario Liberal apoloigists.
\item Rob The Cons have a 5\% advantage straight off because they their supporters get out and vote, unlike the Lefty supporters that sit at home and watch TV.
\item LOL....when was India's history so illustrious?
\item Canada also don't have to feed 20\% of the worlds people with 7\% of its farmland, and a hell lot less fresh water just laying around. Not comparable.
\item LRT Battle is lostmove on to fight other battles another day city and province and federal are now aboard the subway train don't waste leftist energy fighting futile causeslick your leftist wounds and get over it
\item No, I am saying PINK people like yourself still think you are better than blacks and other races... your are damn wrong.
\item In 20 years we can all end our comments, if comments still exist that is, with 'Allah is watching'. Cool, huh?
\item I can't believe this absolute nonsense from this newspaper.
\item WARD NEEDS ANOTHER DRINK
\item LOL the writer 'admires' these things about Canada.. but has chosen to live in the USA and continues to live there.. for 'some reason'even with the 'promising' PM Photo- OP..when she does not have to live with the consequences..
\item Rhodes scholars were chosen because their parents were well connected; go back through 50 years of Canadians who were chosen and then check their parentage.
\item Utter tosh.
\item I didn't realize that the conservatives lost the election on purpose. Thanks for that- I guess it explains the lack of a coherent plan, and so forth.
\item It's not calling a spade a spade that's wrong, it's putting huge numbers of very different groups under your spade that is the problem. And if you discard an argument as hooey you make a display of yourself as blind and deaf.
\item NDP thinks big with national daycare plan.... Didn't Jack Layton and the NDP vote along side with stephen harper against this national daycare program when proposed by Paul Martin and the Liberals ???
\item I don't think the journalists really care one way or another. A more accurate description is most Canadians are left wing and thus a PM who was popular here would probably liked by the New York Times not Wall Street Journal.
\item What is the G\&M's motive behind displaying 10 comments at a time? To inflate number of hits and extract more money from advertisers.
\item He wouldn't have to outlaw common sense as you already have none
\item I fart whenever I want........just cannot control it.....When you say, Wynn I fart....when I read Wynn, I fart, When I see Wynn on the TV, I fart
\item But it will be turned inside-out to please a few zionist financiers.
\item Boule sheet.
\item And aren't you just salivating at the idea of getting some kid of revenge. I invite any race or culture that has never 'sinned' to throw the first stone...
\item Natives don't need 'accountability.' Show us the money 'Apparently that is NOT what the bands' auditors had to say, but I guess they must be wrong and racist as well?
\item imagine actually being religious in 2019...did your parents not let you go to science class?
\item Trump supporters are the sorest winners around. This is what happens when you are the President elect and President. All your actions are held to account on a daily basis.
\item Who says it's impossible and when did your PM even TRY?????
\item Yup, and the Iraq people asked the Western Political society to use false premises and invade them. It has worked out quite well for them. Only 250, 000 Iraqi civilians have died post invasion. I guess this is 'public interest'
\item Aren't marriages arranged by the parents, since it is forbidden and considered sinful for single women to talk to single men outside the family?
\item A white supremacist symbol has been showing up all over the world for many years now, on walls, tables and especially school books. How can this epidemic be stopped?
\item The West tolerates China because they are the manufacturer of the world, like they tolerate Saudi Arabia because that country has oil.
\item Is that marijuana on your breath? Your fired.
\item Gawwwwwwd seeeees alllllllll
\item Progressives are guided by hatered.
\item Elect either of the other two nanny-state, tax \& spend jokers and, trust me, the economy under the Tories will seem like economic Nirvana! Lol
\item Somebody voted me down but provided no clue as to what Juneau said that Canada should have done. This column is an empty opinion piece to dump on the Liberals with no value added.
\item Wait, Harris had an idea? What was it? This should be good.
\item Well then that drops Kenny from your list of future PMs. But I bet you didn't realize that now did you?
\item It is to right wing fanatics. Adam and Even, tree of knowledge, original sin. It all makes perfect sense.
\item My how you add to the discussion.
\item Shhh, Liberals need no encouragement to print money. Wynne doesn't have her own printing presses that's why she's electing Trudeau, he's got the presses.
\item Wente shows naked opportunism. I don't know if she's noticed but all political parties seize opportunities when they come around.
\item The CBC is nothing more than a taxpayer funded mouthpiece for the left. Without taxpayer money, the CBC would be gone in a month.
\item Never. Progressives have a double standard.
\item Really - someone pays you to post this drivel or do you sit around all day waiting for inspiration? BTW - it's kumbaya and it means Come By Here (Lord). That song really should be right up your alley as you and Steve hold hands and sway.
\item Who is this woman and why is she in G\&M debate? Didn't we move on from State religion vs Secularism like a hundred years back? She likes state religion - let her move to Saudi Arabia...
\item My favourite Republican quote of the past week: 'Democrats haven't been this angry... Since we freed their slaves '
\item Columbine was actually a failed bomb attack. Interesting that almost nobody knows that.
\item copper5 - if you see this as 'done' now you are very, very naive.
\item Underlying racist assertion: First Nations history, culture, and philosophy are of no value.
\item OH! What a marvellous idea!! All we'd have to do is firmly and strictly declare something like a War on Drugs.......Wait…
\item Ah, death threats, huh? Where? I'm not able to scrape up a whole lot of sympathy for an entitled frat boy's poor choices.
\item The last thing we need is a national daycare program. Children raised and indoctrinated to behave as state approved, politically correct, liberal robots? Isn't the traditional family unit damaged enough already?
\item Popular? What is this.. 8th grade?
\item it was sad of harper to leave in the middle of a furneral just to make a stupid statement. maggie was glad to see him depart.
\item Not to mention being able to spell a little better, too: 'dilema'??
\item Is America better off and the planet safer?'Only a hack would offer up this question, as though some doubt might exist about the answer.
\item I strongly suggest you fire this editorial writer - he has no grasp of reality. See other comments for WHY!
\item For Canada?s foreign-policy elite....'Nice of you to put the straw man of your argument in your first sentence.
\item Try telling that to RMiller. Not that it will help the poor fellow.
\item Gee no hacks here...
\item The kids weren't allowed to speak their own language, much less harvest their traditional foods. Good grief, pick up a book, Bozo.
\item Those cities you mentioned have high paying jobs in industries like banking and law. Vancouver has developers, realtors, and baristas.
\item Yes, he basically said that ordaining homosexuals gave rise to child diddlers.
\item Its easy, the climate policy of BO is a complete FAIL. He does make Al Gore rich though.
\item Fine, let's see referendums across Russia. Maybe the Chechens would like out after the treatment they have received?
\item Another 'No Brainer' moment for the Harperoids.
\item andrea... what is your point ??
\item What nonsense.
\item Get the right team behind you, the answer is, Yeah, you can. "teamwork": it'll be nice to have a country governed by that again.
\item Typical Harper Hate Machine fear mongering.
\item Care to back that up with a credible link?
\item And that you mention Vietnam and the Phillipines in your list tells me you need to brush up'Not then. Now.
\item Orange wave is doable. People don't buy the alarmist fear mongering about the NDP anymore
\item We haven't had that big earthquake yet. And the proposed new KM isn't a 'twinning' as for the most part it's taking a different route. More PR BS.
\item I wonder how many of the people voting you down also demand we should be more like some Scandinavian country at every possibility. Like all those people who think a Carbon Tax is a great idea as long as they don't have to pay it
\item Why should someone have to pledge allegiance to the welfare queen, she doesn't even live in Canada
\item Good, timely open protest of federal government policy. Conservative supporters will unfortunately condemn the message as anti-Semitic rather than a legitimate cry for peace.
\item 30,000 guns deaths per year (2/3 are suicides), yet no reason to change? Tell that to the parents of the kids at Sandy Hook. I dare you.
\item Hilarious. Obviously written by someone who doesn't live in Polak's ridiing. She's a right winger through and through.
\item So now the american majority are 'facists' who have lost their way? Does democracy mean anything to you? Please remove this author and her negativity from this paper.
\item Taxrage 2 hours ago If you have a \$150K family income, why should you compete for a daycare space for a low-income single parent? ------ reminds me of JACK AND OLIVIA competing for co-op housing till they were exposed and run away in shame
\item Not even close. Trudeau cleaned house when he took the reins. A foolish move by any measure, but for this one.
\item 60 years of involvement and the politicians are all the same. The task of a new government is to find new ways of interfering in our lives. We are now a fascist country. Anybody want evidence?
\item A slang word blacks use to refer to police is racist if uttered by anyone except a black person and for their exclusive use? Seriously?
\item So, as long as Ms. Wente disagrees with the MP(s) being muzzled, then its okay. Like any of those anti-abortion legislation would have had a hope in hell of passing in the House, anyway.
\item Who suggested that prospective immigrants do NOT have the right to opinions about Canada?
\item Is this the plank or pillar of his platform? Way to get going Justin. Double dipping makes more sense if you are stoned however we are no oreo cookies. I'd rather vote for Big Bird.
\item Not only knew the game but tried to fix the outcome with the help of the MSM. It's the best measure of just how much Americans hate the Clinton mob
\item Killed by people who were safe where they were, but preferred risking the lives of their children out of greed.
\item Why is it that so many religious people can't distinguish between what's their business and what's someone else's?
\item Certainly explains his one and only policy idea of legalizing or de-criminalizing pot... I'm sure he has others but probably can't remember them.
\item Is this reheated leftover some sort of bellwether piece the Globe is floating to gauge their readers' interest in examining the 'Ford Fenomena'?It's no big mystery to anyone paying attention and it's been done to death
\item  . . . there will be tens of thousands of Canadians if not more who will identify with him. And they will vote for him in droves again and again.'You mean if you're nuts you'll vote Liberal?
\item Well KaelThas, good parents don't fight over their children. If you spent a fortune feeding some venal lawyer, you have only yourself to blame.
\item Politicians who speak of needed revenue from casinos are the vilest of spineless creatures.
\item Add Justin Trudeau to your 'doofus spawn' list.
\item So you have no problem with government employees advertizing thier faith in public? then you should have no problem with one proudly displaying a swastika while on duty either.
\item Any Canadian journalist or other critter who uses the suffix 'gate' to describe a Canadian scandal, is a sheep-like dunce.
\item How, exactly, are you impacted if new Canadians swear their loyalty to Canada rather than to the British monarch?
\item Yes it was funny but of course Canadians do not have a sense of humour. No wonder the Quebecois call us square heads.
\item That would be hypocritical! Harper put us another 170 billion in the hole.
\item You are out of touch with what most Canadians think. You speak only for yourself.
\item But the Oil Sands are not ignorant and washed up, like Neil Young himself...
\item Oh, I see now. The people passionately arguing FOR allowing the wearing of the niqab in Canadian society are in fact passionately trying to protect the constitution. I see that their intent is pure, and there is no other vested interests lurking.
\item How do you spell exploitation? This is a disgusting practice that sanctions abuses of fundamental rights and human decency. We cannot continue to condone it.
\item The Liberals were hypocritical in their decision making. You think their supporters would be outraged!
\item Thanks for the belly laugh, festina!
\item To voters that care about actual matters, like trade or not starting WWIII, being a "misogynistic bigot" is somewhere near the bottom of the list.
\item Now go write a post about the medical experiments and sexual abuse that Canadians subjected its minorities to. Or do you have too much invested in trying to keep it quiet from the rest of the world.
\item Huh? Where did this wing-nut Gray come from? the Athabasca has pulp and paper mills, coal mines, and naturally occurring bitumen deposits that it flows over. The lies are in his column.
\item You keep patting yourself on the back, confident that you're so much more, '. . . thoughtful, more unselfish, and more empathetic than are conservatives.'
\item girl'?'peggy'?Sexist enough Philly? Maybe we do need a woman in the White House
\item Brown, a pitiful case in point.
\item The post-truth posters didn't disagree with your post, FH. I there a hidden code word ?
\item He is as useless as teats on a bull.
\item Question: does this pointless wandering originate from Poloz or from the G\&M editorial board ?
\item And you are wearing yesterdays underwear? Yikes! Probably Depends.
\item Yah and while he is at it let's stop the Catholic Church from discriminating against women once and for all!
\item Perhaps she gets away with it because her view is correct? In m opinion it is, so chew on that for a while. And while you are at it stop inflicting your own 'twisted and warped opinion of morality' on us.
\item The most dangerous terrorist state is USA. Iran has not invaded anybody in my lifetime
\item Excellent, this is whats needed for all FN persons. The same right I enjoy on my land.
\item As a lifetime New Democrat, the day my party crawls into bed with the Liberals, is the day I'll tear up my membership card.
\item Nonsense. The same circular logic could apply to the other parties.
\item The idea that solar farms will deprive us of farmland is stupidity.
\item Yep, there is no middle ground with Wynne liberals, you are either for them or in the "dark ages," because they can do no wrong. And if monkeys had wings they'd fly out my butt.
\item Worse - Cruz
\item Islamophobia is no match for Islam's Christaeophobia, Judeaophobia, Buddheaophobia, homophobia, gynophobia, and xenophobia.
\item [brigade of Nazi Re-education Specialists] You are fulfilling Godwin's Law and I claim my five dollars.
\item Ha! Juniors first visit to parliament this year ended up with him asking questions about tricycles. I can't thank you enough liberals for not giving conservatives Garneau.
\item So, do you carshare? I've noticed a distinct tendency for green advocates to want everyone else to change so they can keep doing what they want to do.
\item Interesting reasoning. No doubt you feel we should apply it in cases of human suffering as well. When disasters strike, when famines hit, when wars are afoot... if there's too many victims to treat them all humanely, we should euthanize them. Right?
\item The Syrians fleeing to Europe are mostly pretty well educated. They were middle class in Syria and many of them speak more than one language.
\item fuck this man to hell and back, with a rancid cactus puncturing his ass along the way
\item the experiment is almost over, americans do not want another corrupt liberal government
\item A blue wall ?How about Trump finally has to face some educated voters ?
\item don't like Canada and it's tradition and laws. Lots of other countries to move to and mooch off the social security teat.
\item That depends on when the next suitable gender feminist martyr episode arrives.
\item The electorate of Minnesota elected Jesse 'The Body' Ventura as Governor of their fine state.
\item Tea party lover. Huh.
\item Anyone who has ever driven through, for example, Utica NY will understand why Trump succeeded.'Potholes???
\item iski99: The statement you quote is quite stunning and it's even more startling that about one-third of Canadians don't appear troubled by this at all. You have to wonder how much more of this government Canadians can tolerate.
\item Kind of like this forum, right? All I see is endless outrage here.
\item You tell those Russians Globe and Mail, you tell them......LOL
\item You're likely right... but will there be any evidence?
\item The further to the ' Left' a country or province votes the greater the disaster... look at France. Why is it that so many electorates, when unhappy and facing adversity, vote for the 'sounds good Leftists' only to find their miseries compounded.
\item Christy and her friends have pretty much just been looting the silverware for the last year.
\item Libraries are so important. They are among my favorite places. Hope begins again January 20th!
\item scr when you have time, explain this GGreaat business. no idea where you are coming from.
\item You just lost the argument.
\item It makes sense Canada should say no.
\item As long as the PC's have Hudak they have a losing situation. Try some real talent !!
\item Unfortunately the elites will survive just fine. It will the people who will suffer because the elites will make sure their oxen are not gored.
\item Wow, Moseby1 you seem hungup that I'm able to provide facts that counter the BS the antis spew. It's interesting that facts threaten you!! At least I use my real name and don't hide behind something that no one can identify!!
\item The US beat us to it, they gave up long ago, except for the guns.
\item brilliant broadcaster? I think not.
\item Who is the 'commie loving' poster here that's manipulating the thumbs on this website. Someone out of the 'BEJING' office??? lol
\item To speak the truth can be so immature and childish to those who refuse to think! To add some truth, you could have mentioned that Harpo's presence in the building is shameful enough!
\item 82\% of Canadians are ignorant, uneducated Conservatives?
\item D-girl1Hmmm.....Perhaps you're too young to get the point I was trying to make..
\item Why don't you tell that to the next firefighter, police officer or paramedic you see? Or do you just hide behind a keyboard?
\item It's whatever the G\&M says - LOL.
\item You are just silly. Not a word of what you said has any merit.
\item Says the opinion collected from voters at the advance poll and the strong trend toward registered democrats among the mail in ballots. None have been counted but it is a trend that favours the Democrats.
\item Imagine that he had to bow to absolute spectacles such as the always rabid and frothing at the mouth Pierre Polievre who was rewarded for his obnoxiousness with cabinet minister positions. Must have been a kick in the teeth.
\item If anything this piece suggest the immigrants are bringing the country up, not down,'Bingo!
\item what does robo-con harper say?
\item Interesting. That is exactly the same tactic used by the USA. Yo yo yo y'all!
\item Obviously you can't read.
\item Cynical, do you still call AIDS, GRID? Since you so much like to call things what they were called originally...
\item The highly rated comments are nearly unanimous in their condemnation of these hypocritical one percenter foreigners and their fuzzy thinking. Good job, Globe readers!
\item Sorry, but who the heck is Frances Wooley and why is her opinion worth attention?
\item You are incorrect. The firearms act does not require non restricted to be in a locked room. Maybe you should re read it before you post your B.S
\item Sounds like severe ladies' troubles to me, Pifco.
\item And how is TWU forcing their beliefs on others ? You have free choice which institution to attend. Your views on this matter are illogical and intolerant.
\item @tempsperdue If I were you, I'd put down the thesaurus and pick up a dictionary. It would make understanding language so much easier.
\item Looking forward to his slogans 'Stop the Lying Crackhead' or 'Respect for Moral People'
\item Talk about your 1\%er problems. Your kid got fired because she thought she was above the law. Wonder where she got that idea? Get over it.
\item Western countries immigration policies have ensured that we will be living with this growing disaster forever. Congratulations to our brilliant politicians. .
\item More garbage drivel from the Globe and Star.
\item Holy cow. Have you even been paying attention to politics for the last 10 years?
\item Mel, I don't like being identified by your binary labels, this is a safe space! (s)
\item Well I call him Mr. Senategate this week not the Emperor. Harper is fishing for consumer votes with the EU. Prices will stay the same as no one will pass on the savings to consumers.
\item That line is really getting stale chirp.
\item His emphasis was on 'small'. Sorry you missed it.
\item Free speech in Canada? You gotta be kidding!!!. Say the wrong thing that offends some minority group and you will be hauled before one of these 'human rights' tribunals.
\item because they have freedom of expression
\item ... you mean like the usual 'rants' that happen every Sunday at Churches for example ?
\item Please don't tell me you think any Quebec government has ever 'taken on the unions' . That statement is laughably incorrect.
\item a petty nation run by a petty Shirtless Selfie Shallow Silly Prime Ministerpetty indeed
\item @ReasonInsteadofReligionPrecisely. You hit the nail on the head. The values of islam are not compatible with the fundamental values of the West.
\item What? People spouting off about something they haven't read properly? On the Internet?? I never!
\item Yep, those child labourers must be hard to get rid of....and they grow up so fast too.
\item The epitaph on Klein's tomb should read, 'Dear God, let there be another oil boom and I promise not to pi\$\$ it away this time.'
\item ""n fact, we need to figure out how to manage population decreases."" LOL !!! See: ""World population stabilization unlikely this century"" at science. org.
\item In what way has the US 'taken responsibility' for the MSF hospital strike? What has it done, specifically, over and above what everybody already knew-- that they were responsible?
\item But I am far from ''sold'' and neither are many other Canadians. Enough, perhaps, to make a difference on the next national election day... remains to be seen.
\item What the Warmista's take away from your comment: You must really hate polar bears
\item The Libs in their infinite wisdom decided a shiny pony camp councillor was much better that a highly educated astronaut. Yup, the libs are always the smartest in the room.
\item That makes sense. So why did the author, who isn't stupid, make such a utopian argument?
\item Child brides have mothers. What are they doing about it? In the U.S., beauty pageants s*xualizing little girls have a lot of appeal for some women, unfortunately.
\item This province absolutely cannot risk another 4 years of NDP rule.'------Uh, when was the previous '4 years of NDP rule' in Alberta? How did I miss that? Did you cut those Modern Canadian History classes?
\item Brian is part of the corporate elite and we must listen to them!
\item you know what sucks about america's criminal justice system? if you're a woman and attractive you can drink all you want and never get a DUI. once I even saw it happen, cop just let her go. but a guy? oh no that'll be a year in the penitentiary and a few years supervised probation because it's your fourth offense in two years, fucking bs system.
\item Are you not capable of making your own decision?
\item don't forget to attend to the arrangement of the deck chairs while yer at it.
\item To tick people like you off. And it's not stupid, nor sarcasm. It merely points out the end result of applying retroactive laws.
\item This article is highly biased. People from ordinary working class are better off under Conversative than Liberal.
\item portia, Trump took quite an interest in young things.
\item Religion in the closet. Now wouldn't that be a refreshing change for once.
\item The good people of this country who have trouble making ends meet will have a difficult time with wealthy people who would fire their hard working employees to save a few bucks.
\item You digress ...
\item dream on-Bush's SAT score of 1206 correlates with a 95th percentile IQ or a corrected IQ of around 125that kid wouldnt even be closeHe got his mothers smarts ............not his fathers
\item Yup all those Wall Street tycoons, dyed in the wool leftists. Some times I wonder how certain people figure out at how to use a keyboard.
\item Yes, Siren, and Trudeau is Catholic; Paul Martin attended Catholic church every Sunday. I know, how dare some have a spiritual life? You 'progressives' are so closed minded. C.
\item What's the difference between your comments about Muslim refugees and Charlotte Whitton's views of Jewish refugees in 1939? Well done for exposing your true nature and lack of any Canadian values or characteristics.
\item If there was a free-for-all in the content consumption world, what role would the CRTC continue to have? I think that may be why the CRTC is flogging its dead horse -- to appear to be industrious and relevant.
\item Nope, Rob is number 1. They are a close second though.
\item Answer is easy- until they get divorced. Then they want to be looked after for the rest of their lives.
\item Stop accommodating them. Bring in the victims of Islam, not the Sunnis doing the persecuting.
\item Willad87'it seems I've heard that song before.....it's from an old familiar score'Can you back up your comment about refining locally not being profitable with some facts please?
\item Congratulations, you have the least popular comment on the entire blog. Perhaps you should reflect on that.
\item The only thing funnier than this scathing, witty article is reading the comments of Sun New's defenders. Read the lowest rated comments: comedy gold!
\item In no uncertain terms, this is the most mundane article I have ever read. Trudeau should stop global warming because kids don't play enough outdoor hockey?! Doesn't the Globe have an editor or something.
\item Corporatist'....the lexicon of a follower of Noam Chomsky....one of the dumbest people to ever walk the face of the earth (other than Karl Marx)
\item You don't seem to realize that Netflix isn't necessary for those with a life...
\item Shame on the Globe for writing this fluff piece in support of the F35 and sick and ugly procurement process.
\item American's used polite language and nuance to excuse years of slavery. Sometimes you have to call evil, evil. China and Taiwan are not the same country. Taiwan is separate. Time to acknowledge facts. No matter what the despots in Beijing think.
\item where is the Office of Religious Freedom on this? thought not
\item That's it Rio... stay klassy... DOOSH
\item Hudak is not responsible for the current financial mess in Ontario. Still journalists are after Hudak rather than the premier. They must be the pet-bull of the governing party.
\item Chimp, Please review...'' If it's wrong, it's wrong for both men and women.'' Again - if it's wrong, it's wrong.
\item You're totally ignoring the elephant in the room... population growth is occurring in the third world. What do you want done about it?Genocide?Forced sterilization?
\item You mean nothing was unprecedented and there were no records before climate change hit the scene? You mean, every day/year was like the one before?
\item The Canadian Voter - beleive me- was considered to be be a bunch of sheep who could be shepherded by the messiah Harper. now the truth is out in the open - the Canadian voters are not a bunch of sheep and Harper is a sitting duck.
\item Left of RightYou are proving my point by attempting to be dismissive. This is not about the fashion industry. It's about weak men still trying to put women 'in their place'. Like you.
\item I'll put my hours up against yours any day. Bet you \$100 that I work harder and longer than you.
\item Yes the Clinton pyramid scheme is soooo innocent. Pay to play politics.
\item First things first, but which are the first things?' Very good question, in fact. It seems the most important are cigarettes, dope, and Toronto. What a travesty.
\item Troll. Hey Harper isn't PM.
\item So why does the government feel it needs to force middle income earners to save? Can adults not take care of themselves? It should be a choice. Why does the government need to micro manage us? Generation Screwed...
\item @Needreason nice distraction. Care to defend your dear leaders retroactive law?
\item What bunk. It's gone from lets legalize pot because it's the right thing to do to how much can we make off it. Just legalize it now and work out all the details later. And Justin, in the meantime please call off your RCMP thugs.
\item No rational reason??? Are you kidding me!?!?
\item Actually I have, those who believe in fairy tales and other assorted biblical / religious stories are the ones drinking milk and eating cookies. Ba, Baaaa
\item I think you could say the same for Liberals and Catholics.
\item I'm not a supporter of Zionism, that's for sure. Want to blacklist me?
\item Which one of them was Globe poster Arimas involved in? Your comments are personal attacks composed of entirely unfounded allegations. They should be removed.
\item Where is the outrage from Danish tourist to this story?
\item I believe the author has hit the nail on the head. The Indian Act and the reserve system have turned the native youth into zombies. It's time to eliminate this system.
\item Why not? I would vote for a chimpanzee before I would vote for harper and I am not alone
\item As a Liberal from Toronto I don't really think about these things much. Once Justin Trudeau is elected Prime Minister For Life, we will have sunshine and rainbows forever! This is what the CBC told me at least.....
\item What's Jay Sherman blathering on about?
\item Pretty lame attempt to defend this pos.
\item If all you crave in a woman is a wet t-shirt or a bikini then you are a pig....sigh...hey buddy my eyes are up here...
\item  A rose by any other name smells as sweet....' Call them what you like. It changes nothing.
\item Red herring alert.
\item You poor sensitive soul. Perhaps you should confine yourself to a 'safe space'.
\item Are you expecting a guarantee that it should meet with your approval?
\item Far outnumbered by the misogynists.'---------------------------So if your not a feminist, you're a misogynist?
\item Got some bad news for your conspiracy theory. Obama has to exit the White House, anyway.
\item Not so soft hypocrisy - the Globe editorialists barely mentioned the issue when the Conservatives signed the deal. Now they are using barrels of ink to persuade us how the Libs screwed up. Nice try.
\item Great article. Big Pharma, advertising, commercials, books, chat shows, etc all focus on 'what's wrong with me/us'? it's all about making \$\$.
\item What about the presstitutes? Lets legalise them too.
\item I wouldn't bother defending your honesty with this crowd, Ed. They believe every hateful accusation against Muslims, and deny every story that might sympathize with Muslims.
\item Darn the truth, eh Joey and babbleon
\item We might as well just appoint him Prime Minister now. After all, he's leading in the polls. That would be the democratic thing to do.
\item Speaking of tools. It's arsenal.
\item All Europe, not only Sweden!!!!!
\item Actually it was developed by lefties to make fun of each other for the ever changing "correct" language in lefty circles. And just like Saul Alinsky, it was co-opted and turned in to a right wing meme and hobby horse.
\item Right on, D\_Peters. Sounds like fun. What a work ethic, eh?
\item Read the post and think a little harder, RW.
\item Where is death to Harper mentioned Lazy Beaver 1's chatter ? Death may only be in your ability to read and to reason. Not disgusting, just pathetic.
\item Also, Robert Nixon and Stephen Lewis (particularly) were gutless.
\item That's not even passable name calling. BTW by the look of this post, coherency is not your strong suit.
\item No more hate filled than you, for backing the wrong horse.
\item BS. What is your reference for this statement?
\item Well, Pierre Trudeau inherited a country that had the 2nd highest GNP per capita in the world (tied with Sweden) and ran it down to 14th or so. So there's competition.
\item You can't help it if you're ignorant of the law and one's legal rights - you're just one of the mob and need it to think for you.
\item hard core separatists who stay in Canada...?and what does 'arrogant to a distraction' actually mean? vraiment!!! You sound a little anti-francophone to me. Perhaps if Justin changed his last name to Waterhole you'd vote for him lol.
\item Very thoughtful post. Must take an IQ over 50.
\item Check out the guys record on truth of statements he makes. He is lying about 78\% of the time. http://www.politifact.com/personalities/donald-trump/
\item Dad, as he undoes his belt to deliver a (much needed) swat: go ahead and call them, son... the Liberals haven't made good on their vow yet!!
\item 2 different points of view is a good thing if only leftist rags would do the same
\item Putin may (as a statesman) want to take credit for Russia's entry. as his legacy. Merkel is a failure compared to such as Metternich and Bismarck. She's a Pentagon puppet, even uses their phones. 
\item only if you are a liberal or a dipper
\item Wow, only 6, actually 7 more years until we can start to get reliable information again. Thank God nothing important is happening in the meantime.
\item They'd have that money if they would drop their feeble attempts at comedy that are really cleverly disguised attacks on whatever government is in power (at all levels) in the form of satire.
\item Let bch speak if he./she wants to., logically presented arguments are rare here.
\item Unless you are speaking English. Then it's "Hail Harper."
\item You noticed that that page is empty? Very fitting.
\item While the right wraps itself in religion and claim to have a monopoly on patriotism.
\item cberk, Common sense - you should try it sometime.
\item Oooh boy! I guess you've revealed a lot about yourself in a single sentence
\item Oh, for pete's sake G\&M! The term Reformer-c*m-Independent is not worthy of moderation or censorship. Grow up!
\item A Sikh player wearing a sport turban does not in any way enforce his religion onto you. But you are pushing your bigotry onto him.
\item Well then stay under your rock.
\item I am not sure about this decision , I am afraid of 'mission creep' but once our forces are engaged every Canadian will back them and hope and pray there will be no body bags coming home.
\item The Rebel is not interested in 'asking the hard questions'. They are only interested in advancing their obnoxiously partisan point of view.
\item Have they really? I like Canada - I just don't like the bigots.
\item I agree that the status of women in China has improved a lot, especially compared to India, but1. it is still not enough2. it started before the Communism took over.
\item Every day Trudeau-lite proves how unfit he is to lead the country, let alone the Liberals, well, perhaps not he latter.
\item I disagree with your comment a lot as I don't think it really addressed anything I said
\item It's vindictive. Pure and simple. These guys run the country like the mafia.
\item LOL! well said.
\item I see a real problem with this article, if every minority is over represented due to political expediency we will run out of cabinet positions! No problem for the Trudeau liberals. Like Doritos, we'll make more.
\item Conservatives would win election on less votes than Liberals: July 2013 seat projectiondemocraticvotingcanada.blogspot.ca/2013/07/fpp-mockery-of-democracy-update-july.html
\item Poor Ricky, just more of his usual whining about those who do from one who never has!! standing by for his usual fraudulent or is it flatulent retort
\item How in the heck would anyone know at this time?? Lies
\item Another Toronto troll. Idiots like Simpson and wmk deserve each other.
\item Oh please tell us, g.d., about your photosynthesis delusions. Wait while I get some popcorn.
\item ...And his generation is out of touch with reality. They should all grow up.
\item Go work for the CBC. Your extreme left-wing bias will be more readily accepted there.
\item I forgot the world is flat and only 150 years old to you neo-cons.
\item TWF - mind your own business.
\item Maybe the thumbs down are for poorly-written and executed irony
\item What this means for Hillary is that she can finally dump that Arkansas Cracker she's been stuck with for the last four decades.
\item I think the main problem is the Catholic Church. It facilitates, activates and enables the corruption and ignorance that prevents knowledge, action and proper solutions being implemented.
\item if CSIS will only arrest you if you are telling the truth, you have no worries
\item It's nothing to do with the drought. It's corruption, incompetence and stupidity. I think that is fair.
\item Really, only one question. Given the fact that basically the only 'promise' this government has fulfilled is that we won't recognize Canada when Harper's through, why would anyone believe anything outlined in this budget?
\item On the other hand the defrocking of priests and nuns was a good move !!!!
\item No one is stopping you. please go
\item rick the CON will defend all CON crime.
\item You don't seem to know who appointed whom
\item If we don't sell them the ordinance, some-one else will, has to be the laziest ethical cop out argument. Why not just say we will sell them the ordinance. All consequences be damned, and the devil take the...
\item Really? Importing an American shop worn narrative into Canada to explain how this person 'forgot' where she was born? Really? Grow a few gray cells for heaven's sake.
\item Your view is distorted by your politics, and by trying to get a job at McDonalds....
\item And americans wonder why everyone hates them?
\item He's a robot spouting out his pre-programmed responses, and they clearly didn't upgrade his program prior to the debate. All the same lies, all the time.
\item Why don't you go loan them YOUR money hot shot? I hear they are offering a pretty good return on your investment.
\item more then 50\% of BC voters are saying yes. I don't know where your getting this no from.
\item Brilliant idea! We can go around together with the signup sheet, starting with Montreal. When are you available to start?
\item Adscam or 'pump-your-own-tires' scam... different out-houses, same smell.
\item How much longer will the sky be falling? Seeing suzuki on the Australian talk show really informs you how much this snake oil salesman knows, which is basically nothing. He is a large hypocrite though, I will give him that.
\item Or use their time to hang out with an MP dying of cancer in order to expedite their transition to government.
\item That's right. Don't fight evil. Let some other Country do it Jean. You are a cultural icon!
\item 30\% debt to GDP ratio1\% deficit to GDP ratioGreeece: Debt: 250\% Debt to GDP ratioDeficit: 10\% Deficit to GDP ratioYes, clearly we are exactly the same.
\item Hysterical: deriving from or affected by uncontrolled extreme emotion or relating to, associated with, or suffering from hysteria
\item Clinton is preparing for the debates which will be watched by millions. Far smarter use of her time. Trump just can't tear himself away from the ego trip to do the same. He will look like the childish amateur that he is because of his laziness.
\item Translation: Canadian Foreign Aid will be delivered by teaching Peruvians to rape their land for profit, which will be largely enjoyed by Canadian Mining Corporations. Steve also thinks there's a nice enslavable Native population there, too.
\item China apologist=======LOL I always say I am Chinese here. Why should I apologize for myself? Being a Chinese is much better than being a Canadian. We Chinese are just not used to be licking ...
\item You are wrong. It has definitely made an impact elsewhere. Get some new talking points.
\item Every single sentence a blatant lie. Good work, Peter1410.
\item What twisted logic. No one in Canadian media endorses or excuses these killings at all!
\item The Abrahamic religions (Christianity, Islam, Judaism) developed out of an old dispute between the sons of Abraham'.Now that's a weird interpretation, but I upvoted you anyway.
\item So we'll ignore the non-Christian historians like Josephus, who wrote 2000 years ago, and who talk about Jesus and his crucifixion. Even if you don't want to believe in him as God, there is a lot of historical backing that he was a real person.
\item So who are you to pronounce on what clothing does and doesn't qualify as modest for Muslim women? It's for Muslims to determine, not Canadian good ol' boys.
\item Yeah and Tory has the least credible plan....
\item sorry you don't have the capacity to understand that 'rich' resource is killing the planet.
\item I don't neccessarily disagree with any of that... but this article is about Trump, not Clinton or Obama, so how is your comment relevant? It isn't as far as I can tell
\item Bob Beal Nonsense, and you should not say such things.+++++++++++++++++++++++++++Actually, its utterly true and historically correct - they also engaged in taking slaves. Do some reading...
\item The corporations are mere amateurs when it comes to politicians pitching 'stupidity' wrapped up un the latest partisan mantra of FREE social services, health care, education, blah, blah, fiddle, faddle, jobs ... vote for ME ....
\item We give away that oversight when we elect governments whose main pitch is to serve public sector employees, for example Dalton McGuinty in Ontario, whose brain trust has now migrated to Ottawa in support of a doey-eyed political heir.
\item Why do the countries that lead in the War on Terrorism kill more civilians than the 'terrorists' do?
\item *Someone* wants a Senate post! Seriously though, this is a clickbait garbage article.
\item Whomever the next PM is will come out fine because of this episode. But Harper is toast.
\item typical victim mentality - always someone elses fault. The trademark of the socialist.
\item The federal people are too busy making selfies these days, so too busy to make decisions.
\item Harper's new law allowing him to steal what he wishes from the media for his attack ads could be turned back on him.
\item The author is probably very happy with this win! She gets to write her repetitive articles for the G\&M for four more years.
\item As will mine. The nonsensical editorial endorsement of the Conservative Party was pretty much the last straw. This just confirms it.
\item So you've missed all the information over the last, oh, couple of hundred years on the social construction of racism, sexism, classism, capitalism, ....
\item Bingo. I was appalled by their shallow and, frankly, predictable recitation of left-wing talking points Just completely missed the point didn't you? That figures since you progs seem to be quite full of hate for anybody that disagrees with you.
\item Though homophobia certainly still lurks in clubhouse culture, ...'Evidence please, or is it just presumed because it's all male.
\item Racist slime. Really?
\item Why the extremes with your thinking? It seems to me, with you its either conversion therapy or full on transitioning with no middle ground. Full on transitioning is in itself just another form of extreme conversion therapy
\item What if the terrorist wannabe plans to attack Egypt and is imprisoned in Egypt shall we also mind our own business and not provide consular services, which ultimately means more taxes too much of this going on lately
\item In my opinion, a nonsensical comment.
\item No truthful friend, but then folks like you have always had a problem with the truth.
\item Say, JD, maybe you can let also readers know what the Christians, the Jews, the Buddhists and the Hindus will be up to as well. Or stick to what you know, the bigots and fools.
\item You know the language you're using isn't even your own, right? 'Leftist elitists'? Step away from the hype, look at the situation for what it really is. Who are you defending?
\item Not sure how the PM can decide on any issues in our country......he's never here! He's a PM via text email or of course the odd selfie, he is a joke!
\item Rob Ford is far from perfect alright. He's drifting into the incompetent, way-over-his-head territory. But, on the bright side, his association with the prime minister has cost the Conservatives some support.
\item I just read the above. I am a scientist and this post is just total rubbish from an uneducated neocon moron.
\item As opposed to the regurgitation by Marcus Gee by repeating Deluce speaking points which are outright lies? You obviously did not read the City staff's report which overwhelming recommended deferral until a lot of unanswered questions get answered.
\item I think it's a concern about Canada, but go ahead with your continual, ineffectual baiting, as you always do.
\item The law only applies to some Canadians and not others. That is the joke. He's saying yes i know these laws are corrupt and unjust but we will keep doing.
\item Yes, I know. You have posted the same thing now for at least 2 months.
\item Buzzb .....Healthcare is a Provincial responsibility........Good...............than SCRAP the Canada Health Act and get Ottawa OUT of provincial jurisdiction..
\item As DT would say; Wrong
\item Like I said folks ... crickets from the establishment disinformation crowd.
\item Everybody must unite behind Hillary. Stop the fascist Trump at any cost. If he is elected billions of peoples lives will be in jeopardy! Vote for Hillary and sanity! Trump is racist, anti-semtic, Islamaphobia and homophobia!
\item There's something tawdry about a commentator urging a political party to do what is in its narrow self interest. Is Mr Flanagan looking for a job as a Liberal strategist?
\item Good call - not fond of mimes either. Too quiet.
\item Agreed Stephen Harper has been giving Conservatives a bad name ever since he quit the Liberal Party.
\item Bottom feeders ? It takes one to know one.
\item Really? This is how you interpret the Ghomeshi saga? You should google the Bavarian Illuminati. Now there's a conspiracy!
\item Boris is not the Lord Mayor of London. You aren't qualified to make comments when you can't even get basic facts right.
\item Sudia Arabia has behead hundreds of prisoners. But, we're allied with them.
\item Get a life!
\item and all of the people that voted for them (especially for Wynne, given all of her disgusting scandals in Ontario).
\item The UN is an ineffectual and corrupt organization many of whose members are dictatorships. We have democratic elections which are fairly won, even if some don't like it. The people of Canada decide.
\item Totally. I'm amazed that NOBODY seems interested in this basic, basic approach. Geez, people! Try something! Try anything! This isn't swabbing a mop around the floor. Cleaning hospitals requires very extreme, very high quality expertise.
\item I thought Margaret Wente was supposed to be the funny one! HaHa \& LOL!
\item "Look no one is suggesting that Clinton is perfect...." That's good because Hill is the most corrupt US Presidential candidate EVER...
\item [The US needs a change and Donnie has the diaper full to do it. ] The US is in trouble, no doubt. But Trump is the kind of change you go for if you've got nothing left to lose. America has an awful lot left to lose, and Trump will lose it for them.
\item Full moon having its effect, hmmm?
\item This may surprise you but Harper lies.
\item The EU was an economic failure. Its members would have all been better on their own.
\item If Lincoln could see the way we were behaving today he would be turning in his grave. The left has ruined the political process with their shrill idiocy.
\item Who's definition of 'better' shall we use? The nanny liberal socialist one, the wikipedia version or the persons involved's opinion?
\item Yes, and Mr Hitler was a good painter.
\item Publically funded faith based education has no place in Ontario, period. Why should Catholics be treated any differently than any other religion? The answer is obvious and simple, end the funding - or fund all!
\item You're going to give the provincial liberals a free pass? It's all Harper's fault? You can't be serious?... What a joke.
\item You left out these, all from comments on this thread:'fascists''unelected judges''Junior''LIB propaganda''in your subsidized apartment ''criminal's paradise''sharia law''Bob Rae'That's (ahem) 8 for me. ;-)
\item Yeah no shit, but the point is you'll be an insufferable pseud homosexual if you say it that way when speaking English
\item He only called Rosie O'Donnell a slob ? which will win the Donald a lot of votes.
\item We are talking about the UN. They would be able to provide as many reasons as needed to explain why Canada did not get the seat. Bureaucracies can explain any decision they make in a way that can sound reasonable.
\item Your infantile style is unmistakable -- I bet that you and your buddies miss your old playpen at the Sun.
\item No, they hate everyone else from outside their borders!'The immigrant vote' along with ridiculous language laws.
\item Yep, that's about what passes for 'leadership' out of the Conservative party these days. There are no standards of decency or intelligence whatsoever when it comes to this party of degenerates and fools.
\item Because she is a Dalton McGuinty Liberal.
\item Dunny why do you assume there is no conversation happening in class? have you ever visited a grade 2 classroom? All that happens is conversation!
\item The Work Farce does weird really, really well.
\item Tom Z should gaze at his own Canadian navel and not that of his neighbour
\item Not worth 100k/yr not even close, the way you lefties talk you have completely lost touch with reality. You know the starting wage for an engineer is 65-70k/yr.... Ask me how I know...
\item Alan, can you not go and find a tree to hug somewhere!?
\item Baird would be a nightmare as PM.
\item islam is the French underclass?
\item All of the intelligent people are behind Trump? Broad brush much?
\item Same drivel about low information voter, nobody buys that BS anymore, come up with something more tangible. What is unrealistic about building a wall? Again, spell it out.
\item Why do the Harperites all fail to address actual issues in favour of bashing their opponents? Oh, right - it's what you've got.
\item Not what I said at all. But keep trying.
\item Who are 'these folks'? Please, illuminate us with your knowledge of the Canadian Muslim community. And kindly stick to the facts.
\item Another person who thinks CO2 is plant food. Where did you get your science training?
\item a weaker democracy, a polarized electorate' remind me of Harper's government
\item Almost all murders and non-negligent deaths are caused by BLACKS
\item we are... but the system doesn't allow for recall of politicians/crooks...we have to wait til next election
\item I think you mean David Frum. Although he is a bit of glum and grim from which you perhaps get, Grum.
\item You sound like you need to bone up on your WW2 history to see what was actually happening. There is simply no current comparison for what was going on, and the bombing (nuke and non-nuke alike) was necessary.
\item I find the Calgary Flames name to be extremely homophobic and I am outraged. And don't forget about the Green Bay Packers!
\item I'd bet right now you'd have more success raising money to buy them plane tickets to send them back to Turkey / Jordan / Lebanon.
\item My goodness, your concern for Liberals is indeed heart-warming. What say you about a Prime Minster in contempt of Parliament (us), who cheats in elections and passes Constitution-violating legislation at every turn? Thought so.
\item The same brain dead liberals in this comments section that voted for Trudeau federally and for Wynne in Ontario are now saying don't vote for Trump. OK, got you.
\item Guess you missed the hatred during the referendum, conveniently so I might add.
\item There's 'no point' going from self-absorbed to a concern for the grandkids, eh kai2? Particularly if there are no grandkids to 'worry about.' Indeed, completely morally bankrupt.
\item As for Confucius Institute, it should be banned completely by all countries. It is the Chinese Teacher Union's vacation program, totally a waste of Chinese tax payer's money.
\item If I knew as much about anything as M Wente knows about everything I would be border-line genius. When it comes to Pot advise from Margaret. Just say No.
\item Did you just think that up yourself?
\item If one is a Con, why yes, one would honk. Loudly, repeatedly and in as coarse a manner as possible.
\item When one of the states has a motto such as 'live free or die', why would you want to move to a colony?
\item Assad's regime is murdering Syrians, aided by the murderous and imperialistic regime of Putin. We should nothing to do with either.
\item Quick, someone send her the news about Yoga Day from Vancouver, B.C.
\item Trump leadership suggest Russian roulette in Foreign Affairs is the way to go! Oval Office is not a game for Narcissistic Personality Disorder folks with documented Bipolarity limitations.
\item ahahahahahaha... I can't wait for the start of Donald Trump's presidency, it will be EPIC. I hope puts drama teacher, selfie boy in his place. Go Trump, Make America, and the West, Great Again.
\item NO one in this conversation wants kids smoking pot. Grow up Harperite - if you can.
\item Zero examples. And the Muslim countries you refer to are all 3rd world, poor - great.
\item Ascalepius: You should take a pill. You're irony deficient.
\item Congratulations Rmiller101, your dream of Stein winning is even more delusional than the Trumpster Divers. That was a tough hurdle to clear but you jumped right over the bar.
\item .Yes he did, and than the governments (US, UK, Russia and Canada) that make the decisions on the what, where, when and how sat on 'it', doing NOTHING) The UN does NOT make unilateral decisions, the nations that form the security council DO..
\item Your posting is classic assumption and a better understanding of a dictionary than the English language. You contradict the thing you wish to defend.
\item Mikey still has poopy pants from yesterday...
\item Nanakanda, you are the one expressing hatred.
\item What we need here are some salacious divorce records and a twitter account. And a few thousands posts on these comments sections. Then we'll see someone get smeared and attacked.
\item pretty jewish of you
\item The plan is similar to the Chinese encouraging Chinese immigration into Tibet: destroy the local culture and replace it with another.
\item Translation: Outside of legalizing pot we have no clue what our policies are going to be'You translated incorrectly, If the Liberals release their policy too early the Reform/Conservatives will steal it and claim it for their own.
\item But to most of us, it just makes him look gullible.'=====No. Not that. What a stupid remark.
\item When it happens in a 'Free World' like the US, then to the Lefties in Hong Kong, this is NOT a problem. Only when it happens in China it becomes a huge problem.
\item Define 'hypocritical scumbag'.
\item Russia was crucified by the warmongering of Putin and his supporters... just look at Russia's human rights, economy and status ...The billions could have gone to feeding the poor, but no... Putin and his zealots crucified Russia instead
\item The bigger they are, the harder they hit, best bring a taser.
\item Where is your evidence of corruption? That is a very serious charge. Please supply names, and details. Thank you.
\item Its scary that Mulcair and the NDP are offering up the more centrist, more thoughtful alternative than Liberals under the boy wonder and his communist leanings.
\item Small words. Short sentences. Celebrating ignorance. Living in a dreamworld. Welcome to Ford Nation.
\item Good article - about a career path that has become a monopoly enclave of overpaid professional whiners.
\item Feel free to add it to your bag of concern troll talking points.
\item To those philistines who don't know how to freaking spell. It's Israel not Isreal. Sheesh.
\item Dalton is not a crook!!! He is incompetent!!! Big Difference.
\item So the left does not trust judges?
\item Stop fear mongering like a neocon. Be happy climate change wasn't a real crisis.
\item Re: "if cake bakeries simply told gay customers how they felt" Sorry, but I came to buy a cake, not hear a sermon!
\item I think you are talking about the second amendment, but in any case just a stupid comment.
\item Trust me, Sanottava, master plumbers will not be digging that trench. But you will be billed as though they were. :>)
\item Monkey, If you think private money does not redistribute income and encourage inequality you are far more naive than I thought.
\item maximrw - what's backwards? THe coward's a Harper?
\item Sure - you just keep abusing the aboriginal people and bombing Muslims and Asians.
\item I wish there were more of this thoughtful eloquence in the current CPC. Instead, the best that they offer us is bigot snitch lines.
\item Sounds a lot like Russia and China as well.
\item This is looking like the anti technology column written on computers.
\item Posting on G\&M comment sites for pennies from the Liberal party.
\item Based on this editorial, but not just this editorial but the ridiculous opinions regularly put forth, editorial or editorially-directed, etc., this newspaper has gone batty, so politically correct to have lost all sense of common sense.
\item sorry cant feel sorry for the guy been sucking on the front tit for too long and the only reason he's at all relevant is our government allows french language laws to rule. Yes french spelled wit a small f.
\item It's idiots like you who are the reason the province is in such dire trouble.
\item The Globe is making a big deal of this 'Putin confrontation'.. I would think a Globe reporter would have attempted to verify it, afterall it was reported by the PMO staff so crediblity is lacking... anybody out there who wants the truth?
\item Clearly, containing the spread of Ebola is racist.
\item It's the best of all possible worlds doncha know
\item I completely agree with you. This government takes pleasure in turning the screws on refugee claimants but rolls out the red carpet for this convicted felon.
\item NO bloody excuse Eliza. If the police can't handle certain jobs, then take away their authority to do so and give it to an organization that can .... the army!
\item Do you want the OILSANDS shut down??? typical left wing stupid comments!!!
\item Really?And what kind of stores would those be? Walmart aims to be one stop shopping - which means there are precious few small business they don't compete with. Get a clue.
\item You cut-and-paste the same talking points in multiple messages on this thread. Who is paying you?
\item So a former Secretary of State and Two-term Senator is, in your mind, worse than a clown with no understanding of how the Government works and what the Constitution says. That soesn't say much good about your thought processes.
\item Well.... if I had the choice between the current, un-principled, Saudi regime or an overthrow like we see in Syria, I'll choose the former. One thing the world is learning, slow progress is better and less costly (in lives) than revolution.
\item how do you know the money wont be used to enrich shareholders first?
\item I smoke pot but not the very potent stuff. Too potent makes me paranoid. So BC should develop a reputation for potency; that brings recognition. But we should also offer Bud Light for those who like a calm stone.
\item Total nonsense. Is this a Breitbart theory? No evidence for your conclusions....
\item Go easy on them Mike, they are only atoms who don't get around to reading much. I'm glad that you and a few others do. Surviving the age of Rob and Steve would be good.
\item Ah Lars. I've missed your rants and pipeline support. Visit a reserve and walk in those moccasins before you speak.
\item Since he's a New York socialist I would lean towards sex offender...
\item Chiapethewise if you think Doug Saunders is a socialist you don't have any clue about the meaning of that word.
\item I agree that Islam is fantasy, but the offense is still very real. If two things equally offend, then does their grounding really matter, if the end result is the same?
\item He had to, otherwise he'd have had nothing to work with. When you look at the party platforms, nearly 70\% of Canadians agreed with most of it. Seems like thats Canadian enough.
\item What if they're attacked? Wouldn't you want them to be combat troops?
\item Two words....Bob Rae!
\item Funny; the one western separatist I know is also an Ontario transplant, to BC however, but in the oil business as a services provider.
\item personally I found recent coverage significantly slanted in favor of Mr. Dix and the NDP. Better luck next time.
\item Clearly you weren't around while western Canada burned up this summer.
\item That is fucking incredible
\item Margaret Wente's response to climate change? Do nothing. And she calls this a mature response to this crisis.
\item All of 'us' is a backdoor entry of United States.
\item Drive around Toronto for a while and you will see that the politeness of Canadians is a myth. You will see lots of grit though
\item A pickled ham wearing lipstick and an apple in its mouth.
\item Maybe we can create a huge "sense of identity" bureaucracy that we can funnel even more tax dollars into. That'll fix the problem of the odd nutjob slipping through the cracks.
\item Do you have any idea what welfare rates are like across Canada? You sound like you don't when you say things like that. You gave a nice sounding slogan but at best it is meaningless.
\item Worst PM ever, worst government ever. Zero respect. A nation embarrassed. Pathetic.
\item The Liberal Party is a fungus.
\item what a load of garbage. the western lunatic fringe took us all on a ride under harpers machiavellian manipulations. the rest of us westerners are finally seeing through it and are sickened by it.
\item Google 'New Brunswick General Election 1987'. Even though Richard Hatfield was the Conservative leader at the time, what happened to him and his party is the same thing as what's about to happen to Krusty the Klown and the BC Liberals.
\item The United States is a benign factor'Yeah, when they're not busy arming head-chopping and liver-eating jihadis to carry out their vile regime-change plans that are responsible for this whole conflict. Go Russia!
\item Make way people. ‘Real’ experts from the comments section coming through below.
\item Actually there is something the haters could do. Sign up as 'supporters' and vote for Garneau. marcgarneau.ca
\item Trump's 'hair' is the result of an overflow of straw in his cranium.
\item Who wants a nuclear deal with Iran when the military-industrial-security-banker-government-religion complex would profit immensely by a war on Iran and Artillery Hillary is waiting in the wings to become commander-in-chief with her very own war?
\item Your comment is beyond juvenile.
\item Neanderthals from Alberta is redundant. Just say Albertans.
\item Can't admit who was responsible can you - do you live in the GTA?
\item Your sunny ways is becoming more like the Dark Empire, lol
\item Wait, did this need a sarcasm flag?
\item Once a leader, Canada disappearing from the developing world'yes, Canadians are legends in their own minds..... this started with the Liberals under Chretien who decimated Canada's foreign aid budget not 'in the last 5 years' as Smilie claims
\item @ Reality\_Check (not) most Toronto firefighters \& police and most of the highest paid Toronto employees don't live in Toronto. So they aren't spending their high salaries in toronto. Check it out.
\item I think a councilor should be able to vote how he feels and it is inappropriate to robocallbutwhy is Doug Ford involved AGAIN! He is not the mayor and should not be setting policy or direction. I do agree these guys are bullies and yes liars
\item If Tabatha ever ventures off the overly politically correct shores, I would not expect anything more than the usual cookie cutter marzipan journalism, wrapped under 'How few bad apples scared Old Europe' title.
\item He could do worse than appoint Jim Stanford. LOL
\item I love the smell of lefty heads exploding.
\item Sorry, I must have missed the TV program is named after you.
\item Keep dreaming Liberals, but 'Le Dauphin' is not ready for primetime....
\item If you are Irrational, don't make stupid comments, make rational ones 'We will only pay for the who get sick through no fault of their own; the public should not be expected to pay for life-style diseases.'
\item Try using the same logic on Muslims and Arabs. You wouldn't last long.
\item Disgusting. Cannot believe this pay to play scheme is legal in Canada. Can anyone have faith in a Prime Minister and a Minister of Finance who endorse this practice. So tired of hearing silver spoons yak on about the middle class.
\item No, you've just demonstrated the 'God in the gap' fallacy: anything that is beyond your personal knowledge or comprehension must be 'God'. Apparently you could learn more from this episode with the coin...
\item and with any luck he will soon be the same inside Canada too!
\item The words of gutless surrender. Hard to imagine that this is what has become of the Vikings
\item Wow, two things that I can tell about you from your post: 1. You're young and obviously didn't live through it, \& 2. You have or are working toward an Arts degree.
\item On your way to delusionland remember who made Canada a one-trick pony of OIL OIL OIL
\item The UN has been the satrapy of the West-hating, Jew-hating OIC for decades. And as for Canadian Louise Arbour's toxic legacy, the UNHRC, the less said about it the better...
\item It's odd that the "lesser societies" are where everyone wants to emigrate to, Iranians included. Why is that?
\item What about you, Robbins and Summers? Coinpurses nice and smooth?
\item Somebody refusing to sell me a cake vs killing me. I will pick door \#1.
\item Overreact much?
\item Another ostrich with his head deep in the sand. Keep it there, business, you won't know what hit you.
\item The issue is that the university is not generating special exemptions for GLBTQs. That's actually equality, not discrimination.
\item Women are not sexually superior to men. They are sexually superior to immature boys.
\item The Globe replaces the letter from the former PM's et al with this partisan hack?
\item Ontario has one more disease to rid itself of, namely kathleen Wynne and her entire incompetent, corrupt liberal government.
\item Me too because PM Sunny Ways Selfie is a liar and a fraud and not very bright.
\item None of your examples suggest the 'utmost vile hatred' that you promised. You can find thousands of similar and worse quotations in the Old Testament.
\item Happy to hear that in being Canadian you became a better Muslim. How does that benefit Canada?
\item Moderator: Please investigate the meaning of this commentator's name. It is vicious and cruel. Please delete the account.
\item Yes, they certainly will increase our population quickly and easily. What do you know about population biology and ecology? Not much at all, obviously.
\item Bombast and nonsense' Principal tools of the Harper gang.
\item southcoaster: left to these clowns is anyone who does not think that taxes should be rolled back to 0.
\item why should I care what the catholic dinosaurs have to say? just one good reason please
\item So much for equality?.
\item Umm... did you not just read this article on a media website? Is this article what you consider 'anti-Harper bias'? If so, you really do need to lay off the Kool-Aid or re-adjust your tinfoil hat or both.
\item cjlawrie, you must be part of the Globe editorial board, because you are WRONG! http://www.theglobeandmail.com/globe-debate/editorials/ontario-election-part-4-for-a-conservative-minority/article19047636/
\item But we are only 0.5\% of the world's population. We are emitting FOUR TIMES the global per capita average. Including historical emissions we have contributed about EIGHT TIMES as much to this problem as the global average.
\item Who subsidizes your fire and police? Want a hint?
\item HAHA HAHAHA! Brilliant. But, of course, seriously, that stuff is dangerous. You can drown in it. It should be banned.......
\item i thought you might have some brains until this comment, buddy, this presentation was simpler than half of the senior engineering projects at my state school last year.
\item Excellent click bait for the legion of leftist hordes. Good job Mr. Martin.
\item It was a very good article until the last sentence, which I thought stupid.
\item Very good comment John, even if it requires fleshing out, so to speak, for the many commenters who don't understand the vacuous nature of disposable sex.
\item Well you seem pretty sure YOU know all about the case, although you've demonstrated you haven't even read the basic facts about it.
\item Miller, at least you don't whine like your buddy, Trump. You simply throw him in the trumpeter and move on your the next whacko. So it's Jill Stein is it? "Real Solutions go Working People" - wow! Inspiring!
\item Then why do Canadians go to the USA or Mexico for health care?
\item And anyone who resists cutting our carbon output has no care for the future or the kind of life their kids/grandkids will live. Get informed.
\item Religious child indoctrination.
\item Judy - you are Australian? Were you concerned with Australians killing Muslims in Afghanistan?
\item The fact that such comments can be made about any person shows you how low we have sunk in this country. You have no respect for yourself, let alone the Prime Minister.
\item Cherry picked history from the Wile E Coyote of Alberta politics
\item So you're talking about Greenland and Antarctica, as well as "the study area". What about the rest of the world? Or doesn't it fit your hypothesis?
\item Harperman, Harperman, November fourth, you're in the can. Justin's ready, his hair is nice, And he sure put you on ice.
\item I wish the person who voted against my post had explained why.
\item Seems to me that you are not thinking Konrad.
\item Logical thinking is not a strong point with many in the G\&M Commentariat
\item So what you're saying is 'people shouldn't overdose on opiods'? Very helpful comment.
\item Like his role model GWB, I call him an End Times Facilitator. I'm hoping there is a G-d, so She will intervene.
\item Are there any Moslem women reading this ?
\item Bitter and small-minded are appropriate adjectives to describe the Jones screed.
\item Voting Liberal? All you get is Harper-Lite?, plus endless income tax surcharges and sermons about a "middle class".
\item Please provide some evidence that 'Ford is working hard to save us money' - and by evidence I mean something more tangible than the woolly-headed thinking of you Ford Nayshunals ....
\item sounds good. let's disband the military and simply keep paying everyone's salary... that'd be the intreasts of the soldiers first
\item fewer obese people dressed in sweatpants.'... including the Mayor
\item The whole editorial - like the whole Konservative platform is putting the brightest shade of lipstick on the ugliest pig - and the back end of the pig at that.
\item Once the ultra-liberal PC crowd have remade society into their utopian wet dream, reducing every male and female into the more all-inclusive and androgynous 'Thing 1' and 'Thing 2', then maybe, just maybe, they'll be happy. Though I doubt it...
\item This must be sarcasm. At least I hope it is.
\item You're telling me Canadians are bipolar! They need their Lithium dosage quickly.
\item You know it really does get rather tiring when in the States it is always the race card for the blacks . Up here in Canada is always the race card with the Aboriginals. Seriously this is getting to be so damn sickening.
\item Personally, I feel that picking through human feces at a sewage treatment plant is degrading and unseemly, but I would never suggest that it should be outlawed. 'Perfect!
\item Muslims generally think it's a good idea for others to convert to Islam. The main point made in this piece is that Cathlolics now have doctrinal instruction no longer to try to convert Jews.
\item Have to laugh at the son of a Prime Minister who is made Prime Minister claiming to speak for a 'fair shot'. What a joke Trudeau and the Liberals are.
\item Why should the election of an undisciplined 12 year old affect America's future? You know, just because he is leader of the free world and knows nothing about world affairs.
\item Yes we have never seen such a bias media work so hard to drag this tired hag across the finish.'How come when I said the same thing in other articles against Trump I didn't get this many thumbs up??
\item She's not commenting on Brexit, she's doing something much more surprising -- commenting on the one-note media coverage of it.
\item Webbie, you are the problem now go away
\item you should get a subscription so taxpayers do not have to fund your fetish
\item How is it anti-Semitic? Does the state of Israel now represent the Jewish religion and every Jewish person in the world? By labeling everything you don't like as anti-Semitic you are diminishing real Antisemitism.
\item This, I don't know how it is in Latino and black communities. But in brown and what I can tell from the Asians. There is a lot of cooperation
\item The pensioners ARE the sponsors! Gt a grip, Art!
\item Asinine column Ms. Wente. Chock full of bias, straw men and appeals to populariy. STVis a much more democratic method. Look it up. Educate yourself.
\item skipping your English as a second language class again ???
\item Speaking of morons you fit the bill.
\item France is war mongering again.
\item Too right! What a drama queen.
\item Your opinion is extreme. I'm no fan of those two, but they don't qualify as extreme left-wing. Extremely incompetent, yes, but not extreme left-wing. More like, 'ideological nutbars'.
\item instability in Argentina -- who knew??
\item ah yes, Judge Judy. That bastion of informed, thoughtful, and insightful justice. Change the channel, will you?
\item This sounds like an ad from the Power Workers of Ontario.
\item Ever heard of wage cuts? Don't like it find another job.
\item Politicians are sheep, they fear easily.
\item Perhaps clever Canadian academics could be offering to help?
\item That people are forced by the government to sneak around to use it is completely distasteful to me. It's akin to forcing blacks to sit at the back of the bus. It's time for a change.
\item Saunders noodles about 'Canadian apartment dwellers' from his elitist rookery in London.
\item Yes perhaps we should show some love and remove these children from these 'hating' parents. If they resist, send the Swat teams. I'm sure you have nothing but 'love' for those who disagree with you.
\item JH....many of your posts are actually ramblings.
\item And we have two semi pretty blonde bobble heads that frame Harper and nod every time the great Dick-tator opens his mouth for the camera's
\item Good one. Allah help the peaceable, 'moderate' Muslin in France or Germany. Or Belgium. Or...
\item Tell me 'just tom' and 'you cant handle the truth' What bothered you more, my words or the fact that there is censorship/monitoring of Replies?
\item By supporting this bad bill, Trudeau managed to make the story about the Liberals too.
\item Your full of Sh*t. My FL rate is half of what my rate is in Ont. and I'm not even there
\item anything that is opposite of what the ontario libs are doing has to be better!
\item I don't think you understand how percentages, odds, or political analysis works.
\item Search the internet for Kal-Tec or Tavor TAR-21 or KRISS or Noringo 97.All currently available in Canada without a restricted license, all semi's, all 223 why all the fuss over the AR?
\item The majority of teachers are anti-gun and, at the college level especially, fascist. Use ex-military and/or police officers.
\item ...more learned liberal advisors...'Not only learned, but even 'more learned'? Where have they been hiding all these years?
\item HATE is not a strong enough word but I hate Stephen HarperHe is RUINING our country
\item Wrong assumption nakedeye1. Chinese and Indian beat English by many millions. Now, keep on displaying arrogance. It works well for your class.
\item I'd rather be me, than an ugly depressed manlet.
\item Leftists pee their pants when they see a handgun but stand up and cheer when someone gets their teeth knocked out in a hockey rink. Total hypocrites.
\item Clinton prepares for debates like any normal person unlike Trump who just can't tear himself away from the ego trip of the adoration of the "poorly educated", ha, ha, ha.
\item Apparently you are not well educated on what is going on in Canada and what exactly Kenney has done BESIDES NOTHING to stop it!
\item Here's your reality - Harper's gone (and good riddance!). Get over it.
\item How do you dream up the incessant nonsense? Harper is gone for good. Get over it.
\item This was a productive discussion before you joined in. Go back to sleep.
\item We should not be smug about this. Canada dodged a brown shirted future by getting rid of the Harper Government. In his desperation to be re-elected, Harper appealed to and promoted bigotry.
\item Boo! An Arab under every bed!!! Clutching a knife between his teeth to get ya!
\item Yeah, right. Merit as defined by whom? By males, of course.
\item In order to save this democracy we must stop people from participating!
\item Again Jack, embarrassing commentary. You bring nothing to the conversation of value. Please either up your game or stay home.
\item HaHaHa! The comment section of the G\&M has sure become the main message board for left wing numbnutz!. Far more balanced posting at the NP.'And you are here, Don. Welcome to the club, hahaha.
\item Nature recently published something on this and it clearly showed not all vegetarians are anemic, with a certain diet you and your sister can definitely avoid that
\item All colonialists, supremacists \& loyalists inCanada celebrate a foreign royalty today. God give us a republic ASAP.
\item Poor Hamas will have to stop shooting rockets into Israel, and also stop all other acts of terrorism against Israel
\item It seems that Ms Wente has brought her war on drugs mantra from the US with her. 1964 (year she emigrated) is a long time to harbor outdated attitudes in a country that knows better, save for Hasrpers gang
\item It's a train wreck waiting to happen, I'm happy to say ...
\item If the comments here are the true yardstick how people will vote , the Liberal will win a landslide election next time, and Harper conservatives will be wiped out from the map.
\item The BC Liberals have been trying to scare gullible sheep in B.C. since their old Socred days. Remember old Bennett's 'The Socialist horde is at the gate!'Famous fearmongers the whole lot of them.
\item Agreed, Donald Trump like many of those born with the golden spoon, share a common sense of entitlement. Vilifying immigrates, the poor and disadvantage will not put a halt to falling wages and standards of living for the rest of us working stiffs.
\item sure, and many prices have sky-rocketed. Friends of the government get the company and they give us the business
\item I completely agree with your commentary. It?s 2014 and contraception is an essential part of male/female health/lifestyle. It?s an issue one discusses with a medical professional. I wouldn?t let this physician treat me for a pimple on my butt!!!
\item Smoking marijuana relieves asthama symptoms. I'm surprised Stephen doesn't know that. Or maybe he does...
\item They have a soft corner for co-religionists.
\item Diverse canada? who are you trying to blow? Flotsam and jetsam of the third world. Call a spade a spade.
\item sara palin = fingernails on a blackboard
\item Indeed, russia is a pretty pathetic case for a country. I've been there a number of times - miserable, unfriendly, uncouth people and third world living standards.
\item another' that isn't the answer ' editorial written by someone who conveniently neglects to provide an answer
\item I wonder if Truth lives far from our increasingly foreign dominated banlieux?
\item It is time for Germany France and England to lead. It is time for Saudi, Kuwait,UAE to lead. The US should offer its full support.
\item How does an idiot like that manage to pull down \$107k a year?
\item Your clarification has as much relevance to people outside the absurd subculture from which the words arose as do the terms "bogey" and "birdie" to anyone other than golf enthusiasts.
\item A union economist? LOL! What the frig is that? Great at spending other people's money until it runs out and then asking for a grant to continue?
\item How's that real estate speculation gig workin' for ya?
\item David too bad you never got out of grade 3.
\item One World Government? Oh dear, you have been listening to those right-wing American radio talk show hosts a lot lately, eh? Watch out for those black UN helicopters!
\item Since we've been hearing about adscam for over 20 years now then by your logic it's only fair that we keep talking about Duffy for 20 yearsIs that what you want??
\item Moon, Do you *really* need it spelled out to you?
\item You know, right, that the first criteria to win a Nobel Prize of any sort is that the winner has to be alive?
\item Paul says "only the more simple minded among us would think so." Nice way to welcome a new Canadian. Typical leftist vitriol and thuggery from someone whose blue collar just covers his red neck
\item why would Brad Wall save Ontario? There is no need to. Let Ontario drop.
\item How about a Quebec federal red neck saying something stupid? Or a redneck from Ontario? Doesn't that bother you? It bothers me!
\item Not to mention the slur on Motley Crue, who do not deserve any association, wrongly perceived or not, with this Ship of Fools.
\item This guy never signed up for Econ 101 in college...
\item You got is backwards, it is Harper's opposition who has initiated this fiasco to show how the conservatives are against the freedoms of the immigrants....
\item He likely already has several diseases given...
\item Who wants to bet that the University of Ottawa will be the first to follow California? Exactly the kind of low level Liberal Progressivism that Alan Rock has built a career out of.
\item @Boogeyman3 - I wonder if Liberals lie about drinking at the ACC and insulting people?
\item I am not criticizing you because what you said is fact. However, such a fact is man-made arrangement and can be changed. Time to change.
\item Official' Documentary ?Whatta sucker .............
\item I don't care if he is successful or not in rehab. I just want him gone. I am long past feeling compassion for that waste of skin.
\item Far right conservatism in trouble, progressive conservatism isn't.
\item So people can never change to become more reflective, more responsible and more giving? Rubbish!!
\item Liar. The actual number is 17.5\%. See: http://www12.statcan.gc.ca/census-recensement/2011/as-sa/98-314-x/98-314-x2011001-eng.cfm
\item I used to think the WHO was a responsible organization. I used to think the Cancer Society actually wanted to cure cancer. I used to think there was no such thing as corruption. I used to think the Globe and Mail was a reputable newspaper.
\item 100\% accurate, unfortunately the liberal propaganda team will have this comment deleted like every other post that doesn't praise their god.
\item Much ado about nothing. In the grand scheme of things this hardly rates. All governments are corrupt. Only the degree of corruption is open to debate.
\item Wrong!
\item We elect governments that do not allow the 'market' to operate, we've been raised to be socialists.
\item ... and here I thought doctors went in it to help people first ... wow am I naive.
\item John, are you taking a break from your determined search for those WMDs in Iraq?
\item Nobody has a 'social licence' to commit violence, keith, and certainly not in the dubious cause of degrading our economy.
\item You haven't owned a Dodge Grand Caravan, bud. 10 more biweekly payments and this piece of junk is going straight into Lake Ontario.
\item Move over Stephen Poloz and Mark Carney. Here comes OldBanister: someone who really knows what they're talking about. LOL Holy s-8t.
\item yes, let's toss out rule of law ... so we can be more like ISIS.
\item sageantoine....if you believe hospital care is free... you are the one living in a fantasy. I gladly pay my taxes... i begrudge them being pissed away on foolish ideologically driven wastes of money such as carbon taxes etc.
\item Correct thing'? Maybe for people like you who have been out to get the PM from day 1, but not for me, nor for anyone else who can see clearly.
\item Are you stuck in the 1950s?
\item I'm all for black people expressing their grievances, but what has Gay Pride to do with those concerns? Gay people are not the ones oppressing blacks.
\item What was with Harper's use of the phrase 'old stock Canadians'? Sounds a lot like the 'pure laine' reference by extreme nationalists ion Quebec. A strong whiff of racism in that phrase. Too many Canadians not WASP enough for you Steve?
\item The appearance of Con support can be chalked up to cheating.
\item Harper censored all scientists, a far greater offense, and basically got a free pass.
\item The G\&M is a right-wing rag that gets called leftist whenever Simpson speaks the truth.
\item yes, I agree, Canada should give up its' thousands of nuclear weapons./sarc
\item Perhaps you should care about Tienanman Square if you are Chinese.
\item Truth in politics is an oxymoron - and to write abvout it seems redundant !
\item Good thing this did not happen at a Quebec university or the writers comments wouldHave been far more negative Robert tGatineau quebec
\item Many of history's finest examples agree with you as well; Po Pot, Stalin, Hitler, Chevas (sp), Castro....You hand-wringering, left-wing dingbats amaze me. Perhaps your rainbow unicorn has some legal ideas to suggest.
\item Atheism is a religion as well.
\item Well since I am smarter than you are. I understand that anti-Canadian movement of the left have done everything they could stop all pipelines from Alberta. Now go back and join your anti-Canadian movement and continue stopping any and all projects.
\item So why is Trudeau also falling into line? Is he as dumb and naive as everyone says he is? It appears that you think so.
\item With that attitude, you must work on Obummer's White House, eh?
\item Pure drivel. But keep believing yourself!
\item If there is anything the Press is very familiar with its the gutter.
\item Try actually reading the article.
\item A weird bit of illogic. Every citizen gets one vote, not many - obviously. You vote where you are obligated to register, which is where you live, or as an expat, last lived. Is that hard for you to understand?
\item Never trust anyone who predicts the future with such certainty. This article and woman are examples of why the British want and need to leave. Another globalist rant about how your average person is too stupid and inept to govern themselves.
\item Nonsense .. The U.K. wants the right to control its borders . If Germany wants to bring in millions of Arab migrants than go ahead but don't force the UK to feel the same
\item Media monkey!
\item Another dear leader that is more concerned with holding onto power than doing what is right for his nation. Reminds me of Rob Ford.
\item Hardly. Gibson is a life long Liberal with a capital 'L'.You certainly do not know Mr. Gibson.
\item People die if they are killed. But he probably didn't know that.
\item Amazing. Thank goodness the Clinton web of deceit hasn't yet taken over Apple autocorrect, Inspektor. Once that happens we know we are in deep deep doo-doo.
\item Im willing to bet that they're over ecological footprint is smaller than the average person.
\item This is an opinion piece. He is expressing his opinion. Got it?
\item I suspect at least 40\% of Canadians agree with you Bud. When a sober decision is made at the ballot box on Oct 19, 2015 there is only one serious option. Its the PM.
\item More like Trudeau's Fanzine.
\item I am willing to bet that the other common factor is that they are all poor.
\item I tend to agree. The biggest problem, as stated in the article, is that the union won't even discuss an evaluation process. Just mention it and we get a strike. Our kids are being held for ransom.
\item No, every Con played up the Liberal problems, like poor drunk Ralph Klein squalling about the NEP and transfer payments. Even as PM Harper played up the NEP. And the dumber members of Canadian society fell for it every time.
\item If you smell anything like you look, no wonder you have to spend most of your time posting on internet forums
\item Mr Simpson is disingenuous. He fully well knows that Parliament really does not exist in Canada. It has been fully castrated by the PMO, which is the real ruler.
\item 500, 000 unemployed in Ontario. 170, 000 in Alberta and so on . Why don't you go there and put those people to work?
\item The only racism displayed is your tolerance of old world sexism towards women.
\item Sarcasm at its finest - well done.
\item --well, --not\_quite\_no influence. Just enough to make us raise our hackles at the absurdities published at 'the Centre-of-the-Universe' in its' sublime ignorance of what's west of Lake Superior.
\item As if you know anything about terrorism or islamists. Get a grip.
\item Mark Shore - thanks for the context, that's very helpful. LoonerLander - your input is great. Not everyone would get around the censors with a llama manure reference ya know...
\item Instead of stopping people from taking the own lives why don't we actually address the elephant in the room for once? Why are so many people finding life so unbearable they chose to end it and what as Canadians can we do to help our friends, neighbors and our children.
\item A hateful Christian is an oxymoron
\item What a poorly written article. Does not say much for the University of Calgary. Like Harper he uses division for political gain.
\item Neo-Left Statistics - 60\% voted against Tory remember how many times sore loser leftists whined that 60\% voted against Harper 53\% voted against Ford so now we throw the whine back in their faces 60\% voted against Tory
\item Now if they would just add a contraceptive agent to the meatless meat then they could really solve the world's food problem.
\item lemme get this strait.... an academic from NB sez govt is great..... am I the only who sees a conflict here?
\item Moronic comment, Jimmie.
\item A WHOLE paragraph of NOTHING.......... I just wasted 15 seconds of my life reading your garbage
\item Who is not running for POTUS. Irrelevant R U
\item Who cares about the Reform Party or Back in the Day? If Back in the Day is so important to you why not dream about how your Liberals used to be in power and are now just 3rd rate also rans.
\item All true, but the real 'why' is that the others were loyal Canadians, while Harper is a traitor engaged in treason.
\item If you honestly see the deceitful Cons as the 'best option' available I feel sorry for you.
\item Straw man argument. Your wife doesn't pay income tax because she has no income. Sutherland make millions of dollars annually and pays no Canadian taxes on his income. Obvious.
\item Shia are not promoting international terrorism. I would even question if paying for the funeral of those murdered by Israel is really terrorism, but since criticizing Israel is verboten, many believe it to be so.
\item What a specious arguement. Are you suggesting that they wouldn't have freezed if those jets were parked?
\item Union membership is NOT a requirement of employment. You've never heard of the term "Rand formula" employee? Look it up.
\item Actually, the Central Canadian elites care more about bringing refugees into the country at the cost of several billion than helping our own Canadians first.
\item Harper is the Prime Minister for only the 30\% of us who still somewhat agree with his prejudices. For the rest of us (including the Chief Justice), he is content to be our Dictator, who will do anything to dictate his orders.
\item Stop it Avi, you're not supposed to comment on your own column.
\item It's too bad condescending wasn't one of the choices. Clark is an elitist without any elite qualities. Opportunist politician and talk show host don't make the grade.
\item For decades, the big frightening threat was fundamentalist Christians...
\item Yes, they will be much happier being Putin's slaves.
\item Thank you for you excellent statement. Unfortunately, these Marists/ Socialists change their behavior when they lose the luxuries of capitalism. They steal other peoples stuff.
\item Most people are hard-working, including people earning minimum wage. People living exclusively or largely off their capital still consume services like health care, and many others. They should pay their fair share for our defence, our policing, etc.
\item If I had a son who was an incompetent president he'd look like...
\item Most Americans did not hear, nor would not care what a visiting PM from Canada had to say... you over inflate how DC deals with these things...
\item Hmm. Sounds like maybe your brain is wired to dismiss the science/ignore climate change. Could it be the author is actually onto something? Nah, let's go with your conspiracy theory and call it 'logical thinking' instead. Yeah, that's the ticket.
\item It doesnt have to be hordes, a few as happened in UK, France, US. Deny all you want, they want to violently rule the world, or have you not been following what they are doing in Iraq?
\item Because to thousand of racing fans even having the welfare and EI fools out there losing to the slots is an embarrassment tot the sport of horse racing....why add to the problem?
\item Canada's PM is devious and manipulative. THe TPP deal is shrouded in secrecy but veils are the going concern with the Conservatives.
\item Another one jealous of the rich, did the toronto star send you over
\item I don't recall Canada dropping bombs on India before terrorists in Vancouver put a bomb on a plane and killed 268 Canadian citizens.
\item How about the distribution of armaments to countries you know are supporting some arms of the terrorist. Should they not be considered terrorist?
\item Human rights tribunals rival the Nazis
\item Now that you've climbed on your high horse and accused someone of being a bigot, please tell us about the family you've sponsored.
\item And How many jihadists and sharia law proponents in the mix?
\item Next time quote your research. Angus Reid polling shows the exact opposite.
\item  however, I think the guy needs professional medical help'Detox?
\item My guess is that Harper is more like Nixon than we realize - I bet that all PMO offices were bugged (audio and video) as well as all email and computer files regularly scanned and reported on. Harper is sick enough to set this up.
\item Erika from Amerika will use this forum to:1.) Tell us how dumb Canadians are and/or2.) Try to deflect or otherwise get defensive about anything that may have negative connotations regarding the U.S.
\item This rather predictable and innocuous article has drawn out an intriguingly large coterie of rightists to bray denials.
\item If you're going to quote, at least make an effort to get it right. ?? For me, pepper, I put it on my plate ?. ?
\item The world is addicted to a destructive energy regime and our pathetic response is: 'Hey, don't pick on us! We're just suppliers!'
\item you don't have to be one of the "useful idiots" to believe that this monument is a bad idea.
\item Wow, commenting on a post about anti-semetism, you post a racist comment. What a surprise.
\item It is particularly funny since Lawrence Martin is usually a Liberal hack.
\item difficult because there is no Party politics - officially but the weasel like NDP type of councillors hold a monthly "caucus" meeting 15 of them out of 44 this violates the spirit of Council
\item Oh please .....Sick \& tired of hearing about the 'noble' Jews. Israel; talk about a terrorist state - they are the paradigm.
\item Its a black mark on the feminist movement who think they can make up law on an ad hoc basis to suit their needs at any point in time.
\item And they can start with not listening to your sour attitude in your post. You don't like what men are doing..? TOO BAD FOR YOU..!
\item The HATER Jack trolling as usual. Dismal handling, could you provide some examples? Low oil prices?
\item We shouldn't have to deal with your horseshit here. 
\item ZZzzz.... Fill in the blank\_\_\_\_\_\_ have a right to be heard and respected. What a meaningless cliche!
\item I see you haven't bought into JT's 'new style of politics' rhetoric and prefer the standard Chr?tien liberal style of divisive partisan ad hominem attacks. I tweeted your comment to him. You made him cry.
\item That's nice, sweetie, you keep thinking that
\item Hmm well well comment after comment by Castro loverscomment after comment with distorted historycomment after comment of true believersall by the illusion filled extreme left...
\item Another Liberal boodoggle
\item Reminds me of Dan rather, the left winger making up fake news on 60 Minutes about George W Bush. He was forced to resign. It happens on all sides of the political spectrum.
\item Keep telling yourself that.
\item It appears ignorance is bliss in your case. Maybe you should take your own advice.
\item Anything a reader posts extemporaneously that shows disrespect for a PM, other than Harper, is abusive and must be removed.
\item actually he is from the university of guelph.. not in the GTA last i looked
\item Tory will not get re-elected. This and the DumbTrack will be a nail in his coffin. Buh buy Mayor Tory. You are no better than any of them.
\item If we have no right to call the language we speak French, you have no right to call your language 'English'.It is because of people like this that separatists exist.
\item I agree No too any Games, this group is not very trustworthy in any land!
\item The press did not cover themselves in glory on this one. The relentless cheerleading for Ms. Clinton was rather nauseating.
\item Lyle Lyle Crocodile it certainly does not include dingbats like u that like ms.wente's columns!! It shows the state of your non-existent brains.
\item No means yes, yes means anal', is a joke brought on by the stupidity of feminists. And I really don't care what your reaction is to that....
\item Yeah, because trying to force the First Nations to give up their culture has never had negative consequences for them before!
\item You do not question the Dear Leader! Our Lord and Saviour's word is Gospel and must be treated as such! Trudeau is ENTITLED by birthright to run Canada as he sees fit!
\item Actually all it takes is to say you are ( and of course label yourself a Conservative) and Harper's base will swallow it all hook, line and sinker.
\item You must be joking, right? The NYT recently published the home address of Darren Wilson, the officer behind the killing of Michael Brown. Talking about low class journalism. In a turnabout is fair play, the reporters' addresses have been published.
\item The voters in Ontario were faced with the choice between a liar, a fool and a thug.
\item Why, of course. How could I have been so stupid! They simply take 2.5\% away from all the teachers and then give it back. Thanks for clearing that up, Friggate! Now, back to summer vacation, you!
\item That long list of Harpers transgressions is pretty sickening. But consider just how much the Conservative party is now hated by a growing number of voters, and there's your answer.
\item And crooked, too. Look at the number of Liberals on the Beer Store payroll as 'consultants'. Of course the fix is in and we are all getting hosed, as a result.
\item So why, in 2005 did mayors of both cities invite and literally court Enbridge, so their individual towns could be the terminus of the project? Enbridge and their shareholders are owed an apology for this debacle.
\item A lifetime of improvement, yet you are still living down east. My My.(PS I know you think it is central Canada, but the dividing line is on the east side of Manitoba)
\item I found a bit of a "review" I guess... she is so right. All the conversation about muslim women revolves around those two things. There is so much more to it.
\item Your assertions are unsupportable and misleading.
\item Congratulations to Brad Wall. He listens to people \& is therefore smarter than the entire Liberal cabinet. Good work Brad.
\item Your post could have been written by the great con, Trump himself.
\item Can the Globe \& Mail please hire staff who can write proper english and doesn't do their due diligence from conservative election ads? Harper has delivered 9 deficits in a row and 2015 will be a deficit year as well contrary to conservative claims.
\item We did vote for sunny ways. We are getting what we deserve.
\item You never made it out of grade 3.
\item Not at all. The issue is they; re not too sharp and don't listen anyway.
\item If a chid gets sick because of not being vaccinated, their parents should be charged with child endangerment. plain and simple.
\item Trump supporter's r dumber than rocks
\item WOW, and they did it all by themselves without the interference of eco-hypocrites from the Green Party !
\item Straight talk, your ignorance is showing. Did you not know that for every murder by a terrorist in the United States, there are over a thousand murders by gun carrying good ol' American patriots? Look it up. You should.
\item If I wanted rip-off pricing for cheek by jowl housing surrounded by druggies, hipsters and foreigners in a polity collapsing from anomie I'd just move to Vancouver instead of trying to remake my own city.
\item Ontarians are going to have to choose to accept this damage to their lives, or get rid of these Green clowns once and for all.
\item How simplistic -- of course they don't accomplish what they promise, the world has a way of interfering. It was ever thus. What planet do you live on?
\item Agreed. Small money is for small minds. Prioritize accordingly.
\item That's not a very nice thing to say. You may lower self esteem...
\item If the boomers had paid their way we wouldn't have so much provincial and federal debt.
\item So what? Those are reasons for voting for Trump? Because, "It is possible that hostile actors ..."? Trump is the noxious product of Fox News, and a racist, delusional Tea Party. Even the GOP finds he has no redeeming qualities whatsoever.
\item killing terrorists is repulsive to the leftist pacifists indulging in moral preening
\item Google it you twerp.
\item Doug is a typical SJW defending his cultural marxist agenda by calling anyone against it racists.
\item Suzuki's Fish Story: opinion.financialpost.com/2011/03/14/suzukis-fish-story/
\item "...all scientists all agree..." Where do you get this guff from?
\item It's also the fault of those that voted for liberal governments too.
\item Those who play the drinking game based on CheeMiss writing 'union thug' in a comment . . . tend to get pie-eyed pretty quickly.
\item wrong questiondoes the Conservative party need Canada? harper and his evil minions were ready to send us into oblivion for their own selfish interests
\item Okay, I made this point, you agreed with me, and then you stole it.Please don't agree with me. You are behaving in a bigoted manner towards French-Canadians, and I don't support that.
\item He never did, it was all lies and uinnuendo that has yet to be proven. Now The Star is even trying to get the police chief to justify their slanderous accusations.
\item Shopping in a Wal-Mart store is not an opportunity, in fact, the 'experience' is more likely to remind a person that they have no opportunities.
\item This is the sort of drivel expected from a socialist rag such as The Globe.
\item If that ever happens, we should have no hesitation whatsoever in buying every single issue in the country and burning them all. What a statement!
\item ...but he's taller and handsomer than his father. Justin got his looks from the Sinclair side of the family. I never understood that 'Trudeaumania' when I was a kid. Pierre looked like a little twerp.
\item No, I'd say you are a typical Canadian.
\item Nothing? Is this action alone something? Try again?
\item LOL. PET continually ranks in the top 5 of Canada's best PMs!
\item SayNothing has just turned 13! Happy birthday, SayNothing! BTW, how's grade 1 coming along?
\item The barriers to mobility are caused by policies that cater to the 1\%, including lowering their taxes while raising them for everyone else.
\item To the author: Of course a friendly mutual hello would be nice, but we would rather have police who break the law actually face the same justice system we do.
\item "Deniers?" Me? Your handle says that you should know better, but it seems that you don't. I'm trying to get people out of "denial" about the population apocalypse, but it seems not to be part of the Prescribed Narrative.
\item Go back to your MRA goddess Christina Hoff Sommers.
\item Blacks don't get carded or pulled over for nothing in the States!? Who knew.....
\item An opinion columnist without their own opinion - how ironic.
\item I'm glad you are privy to the internal discussions of the Iranian government.
\item So has his brilliant cancer research been discredited by a bad joke? Should he take all his marbles, and cancer cures, and pack them up in cardboard boxes just because he's wrong about feminism?
\item Canada is an immigrant country, always has been and always will be - get used to it.
\item Who appointed the Commissioner and the Commissioner before him? The RCMP were politically controlled by the Harper government (TM).
\item Easy dear, just don't say anything
\item Congratulations, Wisteria, for being someone who votes looking through the windshield rather than through the rear-view mirror.
\item Like Mr. Harper, you failed to address any of the issues of concern.
\item >> pursuing an international criminalSo you fell for that one, as well.
\item Trump is the modern day leader of the 'Know Nothing Party.'
\item I've noticed that it seems to take longer for writers to come to the point the less significant the point is.
\item And was promptly voted in again by the Canadian electorate as PM. Swing and a miss there Bobby!
\item How does Raitt's appearance come into this? I judge people by how they behave, and seeing Raitt rescue May made left me with quite a different opinion of her that I previously held.
\item Baird needs to call Netanyahu to find out what he should do/say next. What an embarrassment!
\item You should be poisoned and murdered. 
\item it's a fact that 99 percent of people with red hair were bullied at school and can no longer participate in society
\item Progressive....I guess you can get away saying whatever you want in your world where facts don't matter and you feel that you are right because you keep repeating falsehoods. Mind boggling, really.
\item Bitter much?
\item Sure play the race car. It is not a racist policy because it applies to members of every race who are not citizens nor permanent residents of Canada. what is so racist about it?
\item But the point is, in this case, that didn't happen. Are you so incapable of distinguishing reality from fantasy? Lynch much?
\item Regular, If you're unhappy with the pay executives are making, buy shares and vote otherwise at the annual general meeting. Otherwise, it's none of your business what a company's board decides to pay its people.
\item You do provide good comic relief
\item Republicans opposed the measure across the board. Can you read?
\item Some people do not have the courage that freedom requires. They will never feel safe, not matter what security measures are taken. Have you considered a closet?
\item "cut your iPhone more than basic cable TV cigarettes booze vacation" 'And get off my lawn you lazy kids!! 1!'
\item You have not addressed a word the author said with your vile riposte.
\item Really. She reads like Patrick Brown's Communications Director.
\item Spin as you like. The undeniable fact is, Ontario has been "transformed" from a giver to a beggar after the 11-year ruthless abuse committed by the incompetent and yet very corrupted Liberals and Wynne is the worst of the worst, the rotten one.
\item To kevinThanks for the laugh ' leadership and commitment to transparency ' . There isn't one minister who has distinguished themselves with an iota of independent thought or action aside from kenney. The rest are sheep and incompetent.
\item Dopiest comment I see is "The science is settled," typically one of your favourites.
\item Tin foil hat crowd, if the shoe fits \& it seems to fit you well Jack.
\item As if you have brought anything useful to this debate either Looner but the same talking points as I have. Something your partisan brain can't accept. Merry Xmas to you too
\item In the 70's, girls wore tube tops and terry cloth short shorts and guys managed to graduate with good grades and no rape conviction.
\item Are school dress codes sexist and oppressive?'No.Show up to work at a professional office exposing your midriff, see how long you last.
\item Not sad, Pat. Pathetic.
\item Well then, Joannie, you must not have been pretty and smart if you think this.
\item What an ugly, purposely-demeaning term, "anchor babies". It seems ONLY to be applied to brown-skinned babies. Such prejudice is not something of which to be proud. 'Sounds idiotic to me.'
\item Which reminds me - they let Pamela Wallin moderate one year!
\item got re-elected doing it'Had Leopoldo Galtieri not invaded the Falklands, thatcher would have been a single-term prime minister.
\item Prove me wrong dicknuts
\item Please explain in detail the damage done to young Canadian men.
\item no different than anything else thrown out there over the years' - Yeah. By PCs introducing to Canada the worst aspect of US campaigning style. You can actually say this without feeling ashamed?
\item If that citizen hates Canada and its values he should be deported back to where he was born.
\item dude, im a Conservative making an argument that the CPC will win the next two elections with majorities. Perhaps you comprehension of writing is an issue here. Reread the comment, and save yourself a little dignity.
\item hey the Pope attacked the Donald first, the guy fights back. Good on him. I think a lot of Americans are tired of being so heavenly bound they are no earthly good.
\item Nullify their passports and revoke their citizenship, and problem is solved since they never be able to come back to Canada again.
\item The knuckle-dragging deniers on the right, in their reactionary ignorance, are the reason the modern world still needs real journalists and real scientists...
\item The terrorist calls himself Harper.
\item So Randy, if it's not 101\% effective, it no good at all?
\item no, feminism means one never feel shame for anything. Shame-shaming
\item Perhaps you will convince MLA's from the PC party to walk across the floor and join the Wildrose.
\item I suggest you read a few news sources outside of Canada, most of Europe is in the process of moving to the right not just in the USA.
\item A message from a Conservative, Nigel Wright must resign and be gone for good, this is not acceptable behavior for anyone at his level period!
\item Oh, you smug Canadians....Just wait until YOU get attacked....think it won't happen? Guess again. Then we'll see how 'tolerant' you are.
\item Learn how to spell, or at least learn to copy a word that is right before your eyes. They learn how to copy words in grade 1, guess you didn't get out of kindergarten.
\item @ MJT Do you think being fired for a legal non-corporate tweet is appropriate? If yes, please let me know where you work so I can be sure to never apply for a job there.
\item Sorry, By resorting to 'Reductio ad Hitlerum' your opinion is rendered irrelevant.
\item Hey Craig, why won't Nick Kouvalis run any relection campaign for Ford unless he goes to rehab??? This has nothing to do with 'Ford haters'. Folks don't like Ford because he is a clownish blow-hard who can't grasp his job.
\item Oh - so I imagine you have enquired about the curricula for each of the other subjects taught in our schools?
\item Cry SHILL!!!... and release the Dogs of Woo.
\item Sad how this paper rejects just about everything this government does, but will more than likely support Harper in the upcoming election. Globe and Mail double talk, as usual. If you don't support everything he does, stop being an accomplice to it.
\item Do you really expect people to read your book? Give us the Coles notes.
\item You counted the EU twice, and Germany three times. Was that an honest mistake, DUNDAS2? Carelessness, or deliberate deception?
\item pray tell. why is it 'cowardice'? see if you can do better than rona-approved and regurgitated talking points.
\item Trump? No problem. Ignore the bitter rants of those who miscalculated, got it all wrong, who bet on the wrong horse, who got caught with their ideological pants down.
\item Consultation is nothing but a sham... political window dressing, grip and grin exercisesproducing noting but sound bites and talking heads while the dictatorial Liberal scriptis being dusted off back in Bytown.
\item Come to Liberal Ontario - now that is the WORST government in the history of Canada by far..... sorry to burst your bubble.
\item Since when? A long time. Guess you don't remember chretiens big red book of lies. Your comments are foolish.
\item Pierre Poutine.
\item Hear, hear. The armchair spies are out in full force today. Doesn't matter what you think. This man has done more of significance for his country than either of you losers ever will.
\item I think your tin-foil hat is screwed on too tight.
\item You have never heard about Bill Clintons rape charges? Why am I wasting my time, you probably love Turdo also as prime minister.
\item Re: 'he is not a war mugger' [sic]You seem to have chosen to ignore his 'war' on Mexicans and Muslims. And on common sense.
\item You know the warmists are losing it when most of their comments are vitriol, Wente bashing, name calling...
\item No...It's not like you contribute anything....
\item Do you always celebrate amateurishness?
\item What a load of rubbish.
\item Ten years ago you would've agreed with nonsense, and now you speak it. Well done.
\item There was a time when one could expect most interactions with police to be courteous.'\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_\_If you are white, maybe. To the rest of us they have always been disrespectful, hostile, threatening, and violent.
\item Good for you. Keep collecting bums and junkies and try hard to be proud of them. 'Poor people' my foot...
\item There are more lead mines in Canada than in the U.S. Oh, I see a bit of humor. Doesn't stop you from your bi-monthly shopping trips across the border though, does it? Duck much lead during your trips?
\item Could we call it monolithic art and charge an entrance fee for viewing before it gets destroyed by the employed crew with jack-hammers?
\item Exactly. Even his comments yesterday are nothing new - e.g., Ann Coulter suggested bombing the New York Times.
\item How to get under Harpers skin, vote Liberal.
\item And yet some Canadians seriously think that we should be sending the CAF to Mali... Do you think that maybe we'll need them here at home?
\item What a laugh ... but apparently he's smart enough to lead our country ... how screwed up is that ?
\item Here you go again. Guess what: nobody appointed you to be the thought police.
\item "We" were not all involved in the collapse of integrity and reason, Chipreader. He's been "Steve" to me, ever since the murdering oilman Dubya dubbed him.
\item Yeah right......it was so balanced that it should get a journalistic award
\item Weaver is a Green Party hack. He has about as much trustworthiness as James Hansen....the fraud who was booted (finally) out of NASA.
\item And what good have you done, that would make you a judge.
\item And speaking of PR Ms. Wente, nice little PR piece for Israel. I'm not saying you're wrong about the motives of Hamas but I have a hard time feeling sympathy for Mike Tyson when he's throttling a toddler.
\item lets go............ the sooner we get rid of this piece of filth the betterTime to take back Canada and her democracy
\item Why do these politicians in Canada keep searching for money pits to toss taxpayers money into? Does anybody know of a way to reprogram these dolts?
\item Nobody competes on NBC except Americans... it's truly remarkable.
\item Jailed more like it.
\item Blithering eedjit.
\item Really?! This endorsement doesn't make any sense at all. Canadians have had enough of Steven Harper AND the Conservatives.
\item The tide has shifted, I know you Liberals are trying to whip up public support for more taxes but unfortunately that will fall on deaf ears for those not employed by the government.
\item Um, doesn't Donald have 'Big Hair'?
\item Merkel? How much time do you honestly think she has in Germany. Who cares what that traitorous scumbag thinks. She flushed her country down the toilet.
\item Please learn to read
\item This is a funny editorial. I guess the Globe lacks the ability to identify poor governance.
\item Correct, I have Harper to thank for the new boat and you to thank for all the laughs. Thanks!
\item Grampa, you're demonstrating your lack of knowledge of the US healthcare system. Seems you're relying on the nonsense you're fed by the CBC on a regular basis.
\item What ARE they saying then? Enlighten us, Mr. Comprehension.
\item The ads are simply meant to denigrate, degrade, humiliate, and intimidate.'.. by showing silly footage and someone's own words. Ooooooffff, you folks are in for a rough 2015 election night!
\item Ha. Good point on the cross; plain low grade masochism (turban) vs. gruesome and brutal sadomasochism (cross).
\item Are you saying no one in Canada has ever been attacked by wildlife?
\item What steve\_d1 said: What are you and your religion going TO DO about it?'Physician, heal thyself'
\item Is that a Drumpf endorsement, Ravensbud ?
\item Harper Conservatives are nothing if not radicals. Extreme in everything. Everyone else is either a terrorist or a child pornographer.
\item Mr. Walllace please check your false assumptions.
\item And that fcker McGuinty committed us to 80 cent per kilowatt hour solar!!! What an absolute POS.
\item Justice4AllTo answer your question, YES. In fact, IMO, there are 2 western leaders that should have already seen the front end of a firing squad.
\item Yes - a truly naive piece of scribbling !
\item What side? Both Sunni \& Shia hate the west.
\item So in your world only leftists follow the law of the land? My Ten Cents cited the Constitution.
\item Hey, at least the bigots on the right are self-identifying. That is what makes free speech a good thing!
\item Wow. Perhaps the most uninformed, inflammatory, and bigoted column in some time by the old hag down the block. Pathetic.
\item Odd advice, then, from 'right wing war supporters', Sirencall. Not exactly a clarion call to arms.
\item Carbon Dioxide is not a pollutant! It is a vital part of out atmosphere, biosphere and lithosphere. It is plant food. The level of science-illiteracy in this debate is astounding.
\item I agree with you regarding the new commenting set up. It makes healthy debate very difficult. As to the article, there is much to agree with, but those who buy it 100\% are somewhat lacking inn the critical reasoning skills; lol.
\item So everything is not hunky-dory in the big European family. Is this the group Scotland is so eager to join and young Londoners are so despondent about leaving?
\item No, Olivia Chow has nothing to do with David Miller's government or Giambrone's bathroom. You are making things up. Please construct an argument based on facts.
\item Mary Marxist Trash
\item The speech balloon above her head had to be saying 'Why does he get that great hair for free and I spend a fortune on mine',while her pancake make up was holding on for dear life.
\item Stop labelling and just make your point.
\item You already got yours so who cares about everyone else... A sadly all too common opinion of a baby boomer.
\item Onward Christian soldiers marching off to war... Anyone still wanna buy those F-35s,ah,ah,ahhhhh? This, is the price you pay... Highway of hero's??? More like highway of fools...
\item Sadly, they do refer to them as 'white schools'. They should be dismissed for such racist comments but are not.
\item Perhaps because it is neither propaganda or aimed at minors? Perhaps the better question would be why you support random gang violence and beating of people.
\item You got unrighteous doctors dealing drugs that will never cure your ills' - Bob Dylan - 'When You Gonna Wake Up?' - 1979
\item ROTFL.  So there are no black gay people then? Like there are no black feminists?   Gaad, where exactly is that world you live in?
\item Ali Ceste, please compare the status of Israeli women with that of women in the Muslim world and report back to us.
\item It might be a revelation, although many folks are already aware of it.  I don't think it would necessarily change the Church's thinking because (at least theoretically) all those gay priests, brothers, and sisters are living celibate lives.
\item I can't believe MPs can actually stomach voting for this. One would think elections would be sacred ground.
\item why are  all the poeple that get low income houseing .....WHITE...BLACK....LOITYNO.....AND WHY ARE JEWISH POPELE TOLD TO GO TO HELL WHEN THAY TRY TO GET LOW INCOME HOUSEING....??????MABY I SHOULD BUY A
\item Ah I see gay priest??
\item Lemme see. For the bible thumping idiots... Weren't the jews the ones that had the white mans jesus murdered by the parasites and leeches that made up the Imperial Roman Empire?
\item i would like to add that islam, xianity, and judaism are all goopy junk as well and  bring consequences far more serious than glitter on private parts.
\item No bigotry in you calling Conservatives Nazis, is there? A bit like calling Muslims terrorists if you were capable of honesty.
\item No, that's humanism. Atheism is the lack of belief in gods. That's it.
\item They didn't fail him...they turned him into what they are. And what tens of millions of fundamentalist Muslims are....
\item To Muslims  is there  distinction between Quebec City or Calgary  Quebec and Ottawa?  I suspect they will  all be   guilty to Canadian Muslims.
\item https://www.jihadwatch.org/2017/02/quebec-imam-prays-o-allah-destroy-the-accursed-jews-o-allah-kill-them-one-by-one 'Quebec imam prays: “O Allah, destroy the accursed Jews…O Allah, kill them one by one”'
\item Pocahontas lies.  She's a Muslim.   Undocumented Muslim.  Watch out, ICE is looking for you.
\item That's not shocking at all. 
\item Transgender - leave it to states. Weed - Keep it at federal level because states have no rights.
\item They are also extremely anti-Catholic, so it is quite amusing to see them defended by our rank and file right wing Catholic wing nuts.
\item It's not discrimination against transgender people.  The problem is that transgenders cost too much because they want sex change operations which are too  expensive and requires life-long evaluations and follow-ups.
\item Religious ideology as absurd as it sounds.
\item ...........................How shallow of you. But thanks anyway for your constructive POV.
\item In other words it's all the arabs fault. Isreal bears no responsibility for the suffering of the palestinians.
\item Self-hating liberal Jew - a stain on his brethren and his country.
\item Why not watch a NAZI film on the Jews before making a judgement on Hitler.  Sounds stupid doesn't it.
\item elevate your debating skills Why and Alceste
\item Yes, just like Islamopalooza went down bad last year.  Ctrl-left terrorists shouldn't be tolerated, remember when that Hillary supporter murdered 49 gays in Florida? Mateen and Hodgkinson were just part of a terrorist organization.
\item AS long as they do not join to get free surgery fine. If you are trans already and still want to join , do it. But can you do the job?
\item Honey?  Did you read the article?  She attacked Pope Francis for saying that countries should be welcoming of immigrants.  That is her whole platform.  That France would be better if she could kick out all the dark skinned people and Muslims.
\item Gotcha... you are on your way to converting me as well.... God would want it that way...
\item And the Germans didn't want the Jews so therefore they can just exterminate them   Pregnant women can always give their children up for adoption  Otherwise they suffer the risk if they don't go to confession of possibly going to hell
\item Yes, agree. All of these accusations of paranoia are amazing irony. Robert Reich is the fascist. Free speech for all except Christians and conservatives.
\item Raskolnikov, Your hatred of Jews has evolved over time in its manifestations and disguises and one can see all three forms in abundance here. Read some history and maybe you'll understand a thing or two about reality. Your antisemitism is disgusting.
\item That's OK. The United States will protect us again. Of course down the road they will want something in return...
\item LOL!   None of this medieval maneuvering has diddly-squat to do with any group of people who call themselves 'Christian,' i.e., followers of Christ.  It may, however, provide Dan Brown with his next stupid book and Tom Hanks with another bad movie.
\item Actually, Canadians acting on behalf of the government abroad must abide by the Canadian charter. the Canadian govt cant ignore the charter because they are operating somewhere else
\item Think about the nature of the fathers comments.. 'A good son. An educated son.' 'God will punish homosexuals'.. These radicals consider themselves instruments of God. How much longer will we ignore this kind of hateful rhetoric..
\item Torontonians were the aggrieved party in this sorry episode. Mr. Ford was in way over his head and became a public embarrassment, on a global scale. Nevertheless, may he rest in peace.
\item Meanwhile traitorous little potatoes flood their country out with Muslim extremists nobody asked or voted for!
\item Since the book of Wisdom is considered apocryphal by Protestants (like President-elect Trump)and Jews, it might not go over so well.
\item Thats the problem only Islam is being taught in schools. Muslims WILL NOT TOLERATE their children being taught any other religion
\item Just some inside info:  the 'you're a  pharisee' smear is from the 'beginner' section of Catholic commenting playbook.  High school, not graduate school.
\item What in heaven's name does your obsession with our new PM (maybe it hurts comparing where he is to where you are in life?) have to do with the topic Martin is discussing? Oh, right. Nothing. Off you go, now.
\item He?' It appears that your anti-transgender microaggression and degrading bigotry are exposed to the sunlight a bit, there. What I just cannot seem to spy behind all of that is your actual credibility. How hapless.
\item Yup. We be as quiet as a church mouse and we'll be safe. Yup.
\item That's not true of course, but I'm betting that you voted for Trump.  So facts don't matter.  Transgender people have served honorably in combat for years.  You know nothing.
\item They're just christian conservative perverts. Time to out them for what they are.
\item Racist Apartheid : Colonies for jews and for jews only. Trump's complaints about illegal immigrants are hilarious by comparison.
\item he was a nazi even at 14, and admits he didnt mind what they were doing, , get over it. facts dont change.  KROFT: Went out, in fact, and helped in the confiscation of property from the Jews.  Mr. SOROS: Yes. That’s right. Yes. KROFT: No feeling of guilt?  Mr. SOROS: No.
\item We over praise dads?  That like saying Hitler over praised Jews.
\item Disgusting! How, many more decades will it take for the Roman Catholic Church to wise up and do what is morally right? These obstructionists should be stripped of their power and put away in dingy jail cells. I'm ashamed to have ever called myself a Catholic.
\item Jews were not supposed to have guns in Germany after Hitler took over in the mid-1930s. They had damn few before the advent of that lunatic Schickelgruber.
\item As I've said many times before, sodomy is mostly practiced by heterosexuals, so there are, by far, way more heterosexual sodomites out there than there are homosexual ones. And the legal definition of sodomy, by the way, includes oral sex, just so you know.
\item most candidates of all parties are very poorly qualified.
\item Why don't you lecture Muslims about how they abuse trucks?
\item Is this what we want in Canada ? Stand strong Mr Harper. You must protect Canadians first. Trudeau and Mulcair will not protect us https://www.youtube.com/watch?v=R5L9SExquao
\item Not 15 years after we pulled the jews from the camp did they begin this genocidal immigration policy along with their cultural marxist policies that also destroy us. they need to go along with their browns
\item You left out a word: do whatever it takes to stop a gay man's right to HATE speech.
\item Right on Sarah Sanders!  She's not forcing anything on anybody--it's done silently and privately.  Psalms 14:1 The fool has said there is no God.  Which is in the Jewish Old Testament.   For the loud unbelieving Jewish friends.
\item I propose the WNBA all replaced with transgender women. Surely not a problem, no?
\item Attacks on Planned Parenthood, attacks on public schools. Gee, I wonder who could be behind this. Wake up people. There are religions a lot more dangerous to our freedoms than Islam out there.
\item This is right right out of the roundup of the Jews in Nazi Germany. Rise up. Rise up. Rise up against this FAKE president.
\item what a hypocritical statement by one who hates jews and other Asians.  if racism hurts America than you are one of those hurting America.
\item I haven't heard of any 'homosexuals' disturbing your religious holidays or celebrations, so why don't you and your 6-8 other people leave them alone during theirs?
\item Don't worry about GOP, the Democrats are not doing any better. They are becoming the party for queers and 'minorities'.
\item Don't want to leave anyone out.    Sandy Hook Elementary School - children murdered by a heavily armed JEWISH white guy.  There fixed it for ya.
\item The Jews in Germany would have loved to be treated as the Palis are treated. No ovens, no concentration camps, no genocide. No one is going to question support for Israel other than commie-pinkos, the chronic Jew haters, and assorted riff raff.
\item Not in the Conservatives family. You are not part of them.
\item Rubbish.  You ARE lying, and your 'faith' is certainly not Catholic
\item What about state right Donny Boy? That is what you said about transgender rights? This man is such a liar!!
\item Get lost with your stupid slave stuff. The Jews were slaves and they seem to be doing OK.
\item How does sharing a bathroom with a transgender person negatively affect your life?
\item When you start talking about muslim fascists, maybe ten we can talk about your concerns.
\item Comparing the treatment of pigs to the treatment of Jews?  You might want to rethink your unhinged comment
\item You have just raised the issue of religious misogyny (and not to mention hate and death among gays) that the MSM will not discuss nor are Canadians allowed to bring up in a multicultural society.
\item Churchill never mentioned even once the Holocaust of the Jews in his books on WW2 published after the war. Neithet did US generals Eisehhower \& others. Why?  Were they all anti-semite?
\item  white jew-god mind', well we know where 3d's head is at.  Bigotry and racism.  Must be another graduate of the Hawaiian Studies program at the U of H.
\item This seems a bit far fetched even if the Anti-Defamation League asked Trump to reconsider. Trump is not saying, 'America First...except for you Jews.' Maybe the ADL is being a bit overly sensitive...but then, that's what they do.
\item and someone wearing a cross around their neck also blocks your view of their face?
\item Personally I think transgender people should have the right to evidence-based medical treatment rather than being led to invasive procedures and heavy drug regimens prescribed by gender-identity politics.
\item You mean the 'Christian' who has repeatedly threatened to immolate 70 million men, women and children by deploying tactical nuclear weapons against the Islamic Republic of Iran? If Killary is a 'Christian', then so is satan.
\item Nothing but thinly disguised Christian Supremacy.
\item Why he is just a white, good ol' boy carrying his legal supply of weapons, disciplining his family members when they fail to obey the patriarch as religious dogma dictates.  No crime here, just performing his duties as white, christian rules apply.
\item if you are a Muslim you cannot be a Canadian as your values are incompatible with western society.
\item un autre qui n'a pas d't?te et il faut qu'il nous le fasse savoir
\item From Berig in RochesterPlease come join us in worship! No matter how un-Godly you may feel, the doors are off the hinges to receive you. Your lack of believe is natural, love awaits you, you're always welcome. Dig it.
\item Trump is right.  Let's hope this move prevents the USAs form becoming like France, where Salafist mosques are popping like mushrooms and hate against western values taught to millions of muslim kids.
\item The problem is much worse than simple indoctrination.  We now have parents who are working with the medical establishment to prevent puberty to 'help' transgender children.  So people who cannot vote, drink alcohol, or drive are being purposely mutilated.  This is child abuse.
\item @IvyW: and, besides being so full of yourself, how do you contribute to Canada that you think you should have a say in choosing its government?
\item Hilarious how the evangelicals tied their hopes to an atheist pedophile vile human like Trump. Sorry Mike Pence, no one buys the fake ass holy than now shit
\item The Muslim apologists, and the Globe has three of them as editorial writers, are in overdrive to distract from where the real threats lie.
\item Thankful for Canada's support of Ukraine and recognition of struggle Ukrainians have undergone for many years.
\item Because transgender people have been a tiny, tiny, miniscule number of people and their political agenda is not directly harmful to men, only to women, so MSM don't really care about it.
\item Unloving, yes. You would have us believe that God is as homophobic as you are. And, given that you reject Dignitatis Humanae, you are NOT faithful to Church teaching.
\item Love the tin hat crowd
\item Surely you haven't forgotten Pierre Poilievre. They've done a goodd job of keeping him in hiding.
\item It's mainly muslim hate for each other and everyone else
\item RobHave faith. Give people a chance to live like you do.
\item Wikipedia is written by people who have a wide diversity of opinions, but we try hard to make sure articles have a neutral point of view. Your recent edit to USS Shasta (AE-33) seemed less than neutral to me, so I removed it for now. If you think I made a mistake, or if you have any questions, you can leave me a message on . Thank you.    
\item THAT JEW IS ALL ABOUT PEACE DUDE
\item According to many of faith, it must be because of the lesbians. https://www.washingtonpost.com/opinions/did-lesbians-cause-hurricanes-irma-and-harvey-god-knows/2017/09/08/638efbca-94bf-11e7-89fa-bb822a46da5b\_story.html?hpid=hp\_no-name\_opinion-card-e\%3Ahomepage\%2Fstory\&utm\_term=.e5a3f348e31d
\item SCOTUS just folded on the transgender bathroom issue.
\item God bless you, and may He return the kindness that you have given.
\item He just said it because of the pressure that is being put on his administration to denounce the the violence and hatred that is being directed to Jews.
\item The article didn't talk about Viagra or the cigarettes they used to pass out, only the transgender.
\item Surely your not suggesting this man was invincibly ignorant of Catholic teaching or was compelled to behave in the way he did?
\item diverdave, why walk when you can fly first class, over that wall. any terrorists worth their vest will get anywhere they want to, anytime they want to. this is an anti muslim, fire up the base act.
\item Let's do a fun exercise here. Substitute 'transgender student' for 'Trump supporter student' as the topic in your critique. Should they be ashamed now? I don't believe so. We do not become inclusive by treading on the rights of others, especially in our publicly funded institutions.
\item Maybe the Aboriginal people could move to the Middle East? Your post is really really stupid. Do you think the Arabs care about Aboriginals? Of course not. It's just a convenient way of getting at Canada.
\item Larry,  Always bet on the Jewish Superguy.
\item There is no equivalency between the two. One group is evil and wants to do away with blacks, jews, etc... and the other, the antifa, wants to do away with the evil racists that think that way. Not the same thing.....
\item Anderson Stevenson: Even if you believe that sending priests 1500 years later is good enough, it's hardly a sign of omnipotence. After Jesus was resurrected why didn't he spread the message to the rest of the world?
\item From Russia with love...to Transgender in bathroom! Good move DJT.
\item Funny that you haven't mentioned the Viagra or the cigarettes they used to pass out, only the transgender.
\item one way to curtail fighting? Have law / act state it cannot be shown or commented on through the media - any media. If there was a fight and dead air or some replay the league intelligentsia would soon get the message.
\item When I was growing up transgendered people were known as in local vernacular chicks with d\#\#ks.
\item I would be more impressed if Trudeau would speak out against the Montreal iman who preaches death to jews in his mosque.
\item SMM: Electorate has spoken? When? You mean the 39.5\% popular vote for the Liberals? Craft a good law? How naive. For your sake, I hope you never find yourself in a situation where your life will be snuffed out against your wishes.
\item Ah, poor straight, white Christians. So persecuted.
\item Nope...not true. Beck retired before Osama was taken out.    And did not 'trans' until after leaving the military.
\item Jews only intermarry when there is big money on the table hence Kushner taking Trumps daughter.
\item Dear Mr. Hound38 Do I understand that, aside from the items you mentioned, you are a sound supporter of Mr. Harper?
\item From a 'fair work place' in a very short time, became, 'marriage, adoption, 'hate crimes' special privilege, and has gone on to 'transgender toilets' that we ALL must use, or be called 'haters'.  Call away then.
\item I have to wonder if your comments have more to do with Trump than any concern over transgender men or women.  You don't know that   'transgendered' is an inappropriate term that should be not be used.
\item And good on you for doing it, too - your commitment has not flagged, and now is when we need it most.
\item no sweetheart, they're going to slowly buy up everything you own, settle your lands and put you to work in factories and you'll be cheering them on
\item Islam makes for wonderfully tolerant, enriching and inclusive societies. It's not only a religion of peace but of joy as well.
\item that is a silly statement. the Jewish people had rules set out by God, and I am a gentile.
\item The Trudeau cabinet members and staff appear to have no sense of ethical responsibility. Brison's response is cavalier and shows he is completely unaware that this is a serious allegation of impropriety. Having a gay husband doesn't give him a free pass.
\item I am not anti-gay. i am for gay rights as long as they are not superior to rights of others. Neither of these two facts are evidence of support for the assertion of choice.
\item Maybe we should ask his Orthodox Jewish son-in-law and his daughter who converted to the faith  why he is such an anti-Semite.
\item The case of Sauve v. Canada was about the right of a person who is incarcerated in the prison system and does not address residency. In fact the decision refers to ' certain permanent residents' also 'citizens and residents'
\item According to NEWSWEEK, 'Border Wall Tied to Trump Transgender Ban'. http://www.msn.com/en-us/news/politics/border-wall-tied-to-trump-transgender-ban-report/ar-AAoSxVS?li=BBnb7Kz
\item Or maybe considering how it's ISLAM which specifically officially and quite repetitively commands the global genocide of all the non-muslim cultures, religions, and peoples of the world, it's only a legal, moral, and defensive stance? Unless you think 'muslims' are a 'race?'  ;-)
\item The future of the Catholic Church in this country is becoming more and more Hispanic.  That is one of the reasons so many white Catholics jumped on Trump's racist bandwagon.
\item Tabby Cat is using it in a disgusting offensive way and damn right it's a slur. It's a slur against every single non-transsexual person out there.    Wake up. The 'victims' of bigotry are now the bullies.   Tabby Cat isn't funny and should be dismissed for her hateful rant.
\item MEN OF CALGARY: GO GAY! It is the only thing that will save your skin. But in today's heated feminist empire, being gay may not be a defence from an accusation of sexual impropriety.
\item Martin is a homosexual and wants to be able to let everyone know.  Like all the homosexuals feel compelled to do for some reason.
\item Christianity at least is based on 'turn the other cheek'.
\item These are matters of facts, not belief.  You can certainly try to brainwash gay people into thinking they are straight, but it has not been shown to work very well.
\item I am NOT protecting or condoning the alleged behavior!  I'm pointing out the 'he did this because he is gay' bigotry.
\item Which 'Church' are you referring  to...the Roman Catholic Church  or the True Christian Church?
\item Well, if she's only gay at church...
\item [To those with the right shoe size:]  Surgery? A lie. Outgrow TG 'feelings'? Non-trans do. Trans children never, and when imprisoned in a strange body, the results are often tragic and lethal. This should be criminal? Depriving children of necessary, yes it's necessary, medical treatment for GD is already criminal, child abuse.
\item Here we go again - the rant about the Crusades, which were the Catholics, when people use this argument they simply showcase their ignorance.
\item Feeding christians to lions needs to be a thing again.
\item As soon as Freeland has NAFTA and the Chechen gay holocaust fixed I would like to see Trudeau set her on the little North Korean psychopath.
\item With so many people making the news today by claiming to be gay, it will not be many years before someone makes the news by claiming to be straight.
\item That is called a cilice, they are de rigeure for the Catholic in the know, paired with a hair shirt and optional chastity belt (now available in both male and  female styles), you will never go wrong!  Available at the nearest Opus Dei outlet mall!
\item Slavery killed a lot more Africans than Nazism did Jews.'  How did you calculate this?
\item Not all Republicans are racists. However, they are all collaborators with racists. They are like the 'good Germans' that never asked, where did the Jews disappear to? Today, they never question why cops kill so many unarmed black  people, including children.
\item The hypocrisy of leaning on Christianity as a crutch that dignifies and attempts legitimacy is front and center, in the past, present, and future. So much to look forward too.
\item But EWTN types told me that women have the important role in the Catholic Church doing all the menial grunt work that men don't want to under the 'leadership' of the more intelligent malefolk.  Sarc off/
\item It's tough being a gay guy these days.  LOL
\item Well - in Ontariowe they did what the politicians said ! How is that working for us ....
\item These women should spend a year in Iran, Iraq, Syria or any other Muslim country then tell me how oppressed they are in the US.
\item it's still male bones in there , be trans but don't try to compete with biological women, it's unfair . there should be special categories for trans athletes to compete against each other .
\item As Justin said about the arms sale to Saudi Arabia, one cannot interfere with the sanctity of a government contract.
\item I wonder how many people remember that Quebec was once the most difficult province to live in if you were Jewish.
\item Drake is half black. Being a Jew is not a race its a set of ideas like other religions. Ivanka Trump is Jewish because she converted nothing to do with this talk about race and other nonsense.
\item Mr. President, the  Chinese just invaded Taiwan'. 'Get Jew boy on it...I'm busy trying to come up with a killer tweet to put that nasty Samantha Bee in her place'...
\item I have heard the mothers of trans Americans often feel like they are 'transparent'
\item He is excited about being gay i guess
\item LOL.  Please tell me it includes the one that thinks that having boys do household chores turns them gay.
\item Trump speaks to solid Americans.  The ones who work hard for modest wage.  The democrats speak to special interests such as the gays, illegal immigrants, and rich narcissists who view themselves as better than their fellow Americans.
\item If Francis is concerned about the health of Vatican staff....what about the health hazards associated with gay sex (including depression, AIDS, suicide) and cocaine use among Vatican staff?
\item Literally the dumbest shit I've read in decades.
\item What a disgusting person.  How many offensive things has he said about other people and never apologized for.    What she tweeted happens to be true.   After all there were GOOD people chanting 'Jews will not replace us' at the white supremacist rally.
\item It's like giving a dying patient a transfusion with blood from his other arm.
\item All that is necessary for the triumph of evil is that good men do nothing. ~ Edmund Burke
\item And so a new orthodoxy was born.
\item Jews are whites too and whites are not the most advanced race either.
\item Not surprising Nikki, considering that millions serve and only a very tiny fraction are 'trans.'  It is using statistics to make a false point.
\item He wanted to hold an anti-lgbt rally right before the Pride festival? Disgusting. There’s no room for that kind of hatred here on the Harbor. It’s easy to believe the rest of the story when the owner’s actions at city hall show what’s in his heart.
\item Oh deer: Hitler really! I have nothing but respect for Jews, they are truly a remarkable people. It's you retread, left wing , tambourine banging, pot circle sloths I have no time for. Ps love your conspiracy theories, do you hear voices?
\item The modernity comment was solely regarding the sentence on transgender folks.  And that is a modern phenomenon. Not in terms of the existence of such folks, but of the familiarity of enough laypersons to raise the subject to the level of commonplace everyday conversation.
\item Well for starters, you're an excellent example of an off-putting individual, gay or otherwise.  Prefacing your rhetorical question w/an accusation isn't going to generate good will any time soon now is it?
\item Gary:  Are you a Homosexual??????
\item Nope.  Trump's campaign promise was a Muslim ban.
\item How do you progs become such extremists?
\item Glad he dealt with this because the issue of transgender soldiers in the military was keeping me up at night as one of the greatest problems currently facing the nation. (sarcasm)
\item colon7, you are partially right. Religion is the problem. A minority of one religion.
\item It was not immigrants that caused the carnage at that mosque.  It was not multiculturalism. It was not Islam. It was sheer unadulterated hatred. Pure bigotry. Revolting xenophobia.   Your attempt to justify the slaughter in Quebec is beyond repulse.
\item Part of living under Russian rule is that gays don't have rights. Perhaps you liberals would be happier living outside the USSR?
\item Because, in this instance at least, the Vatican is making a big deal over nothing.
\item Of course you did, Duke. You often do do. Your dour attitude and denigration of something as basic as human joy puts you far closer to the Islamists than to the rest of us. You deserve pity.
\item Most people that spout Jesus this or that are usually two faced hypocrites. Go back to watching your porn...
\item And I bet that in the day you expected your Jewish classmates to smile when you walked into that exclusive country club.  And you expected your black classmates to do the honourable thing and avoid using the whites only washrooms and lunch counters.
\item No, the Saudis are the largest funder of Daesh, which is a natural expression of Wahhabism. How many Christians, Jews or Atheists live in Mecca?
\item I wouldn't say that 'Being gay has nothing to do with being a pedarast.' Pederasty is a 'sub-set' of male homosexuality. So a pederast is a homosexual male while not all homosexual males are pederasts. So 'nothing to do with' is overstating it.
\item So you think it's un-Christian for a nation to have borders?  Absurd.  And since when are you a Christian fundamentalist?  Unless it's in the Bible, it's wrong?  Absurd.  Love requires we take in all the poor who manage to cross our borders?  Absurd.
\item I thought a fresh batch of trolls.  Probably from 'Church Militant.' Same crowd historically that favored slavery, lynched, segregated, slaughtered natives. 'Onward Christian Soldiers,' again; battle ready.
\item This is not shocking.  If women can do it, why not gays?  Now wait for 213 men to board the allegation bus.  We've known Kevin is gay for many years.  No big deal.
\item If he'd shot santa would it have been christian terrorism? Or 'just' a mentally ill person? Just sayin'.
\item These Scientists are morons globalists. We were in a doomsday situation until Trump won, now we can all relax. Not surprised one iota there is a Jew behind the moving of the Clock, Israel may be facing justice for it's crimes and we can't have that now can we. Marxist globalist BS.
\item And one can assume you lived at home - always a dividend, Orderkaos. Mrs. P has nailed it, with serious input from the real world by Mike. Margaret's experiences are of another age.
\item Infowars?  Congratulations on losing all credibility. Have another beer and watch more TV.  Obama made my frog gay with chemicals while cloning 9/11!
\item They are too busy fighting pro-choice, lgbt rights,  and making excuses on what Trump 'really meant.'
\item Hey Broom Closet, I see you haven't seen your doctor yet.
\item The irony is that those who support Ford's right-wing populism are exactly those who most benefit from social programs and the taxes that pay for them. This has been the 'success' of Canada's right wing: making taxation a dirty word.
\item Your concern would be touching if it weren't a canned talking point.  Nobody needs to be trans or a soldier to be in danger in these third world dumpster fires. If you walk upright you qualify.  The best solution ? Stay out of these 'heck' holes.
\item I take issue with 'the god of the Jewish Bible is a cruel, vindictive, angry assassin'.  In addition it appears to be unrelated to the article.
\item Lay off the Oxy, Von....
\item Just in -  Trump has transgendered from female rattle snake to spitting cobra!
\item The problem secularists seem to have with Christians is they mistake the Christian disciplines we impose on ourselves as being judgemental on their secular ways. People who are truly comfortable in their own ways don't have this issue.
\item You make no sense whatsoever. You're saying that it's perfectly rational to subjugate and dehumanize women, homosexuals, and Atheists?
\item He lamented that more children in the United States are raised in families led by unmarried mothers.'  We lament that, too, but don't put that one gay people.  Gay couples, in most cases, are helping children who were abandoned, as if they were strays.
\item Rest easy, Harper will win the next election and just like Benjamin Yahoo he will repeal this legislation and blame his Finance Minister for this stupidity.
\item Something gay went wrong
\item Don't remember you. Obviously no one cared what you said. 
\item We treat the 2nd Amendment like a death lottery and we are all potential blood sacrifices. How many of those concert goers thought they had bought lottery tickets? I thought Jesus made human sacrifices unnecessary. I'm sure a lot of those concert goers thought they were Christians.
\item You like to use the word Facist, seth. Do please tell us what you understand that label to mean. Then compare and contrast your 'notion' with reality.
\item While essentially agreeing with all the above, I'd suggest we not forget the striking history of anti-Jewish pogroms over the hundred years prior to the Bolshevik revolution.
\item Allowing perverted young males posing as transgenders to have access to female bathrooms will also have 'consequences'.  Rapes or suicides, what's your choice?
\item Oh, come on, Thatcher - you didn't even mention the current Jones/Infowars conspiracy theory that Jewish actors were impersonating the white supremacists, KKK and Nazis to discredit them. You're slipping.
\item There are very few people who are really transgendered with chromosomal abnormalities. Others who feel between genders would benefit from therapy..less drastic than genital mutilation followed by a lifetime taking hormone therapy
\item When a Christian performs a terrorist act, do you label it a Christian act of terrorism?  People of all religions engage in terrorist acts, most North American terrorist acts are perpetrated by Christians, because they're the majority of terrorists in North America.
\item Peter MacKay: He?s the Minister of Wrong Again... Why is it that everything the harper CONservatives do is WRONG ????
\item While we're sharing personal facts that have nothing to do with the column: My dog has a fluffy tail.
\item Trump's tweets expertly tilt the scales of justice against his Muslim ban
\item How is baking a cake for a gay couple exceeding his obligations?
\item The fact that transgender people need medical treatment for their condition tells it all.  Normal people come either male or female and require no medical treatment to stay that way.
\item uniquely Canadian' really means 'from Cana-duh'
\item Another way the Catholic Church can distract from the fact that they condone child rape.
\item If a military draft is necessary during war time is Trump prepared to give Trans-gendered people an exemption? Or do exemptions only apply to rich kids with heel spurs?
\item Science applied with your sense of the 'sacredness of the planet' and just a smidgin' of concern for one's offspring ?
\item Islam teaches hate. Muslims need to be run out of this country. They are a disgusting death cult
\item Lots of people are happy to live under a dictator as long as they feel safe.
\item globe editors.. stooping to new lows every day... Run along little editors... Harper beckons with more lies..
\item What is ridiculous is suggesting an equivalency between the number of attacks on jews in Canada and the number of attacks  on Irish people in Canada.
\item Of course Trump blames the black guy.  Hurricane Maria was the fault of Puerto Ricans.  The Jews caused Nazis.   Blacks force themselves to be abused by the cops.
\item A priest raping a child is hysterical.  Your comment history shows your reverence for the church and seems to be missing the teachings of Christ.
\item One of the hallmarks of a complex mind or a complex civilization is the ability to recognize, focus on, and address REAL problems. Which bathroom transgender people use, isn't one of them.
\item a Mosque is a Mosque is a Mosque Where else do they teach their Hate for non-Muslim's?
\item “don we now our gay apparel.” ? What is Kahle suggesting? Kahle is gay and his class mates knew he was? Or is Kahle sneaking in a homophobic slur and in the RG no less?
\item It is so revealing all these Republicans saying 'I have a wife, daughter and mother.'  You don't know any Muslims? Any Mexican immigrants? That in itself is deplorable.
\item its a jewish democracy, get over it, you and kerry are idiots
\item Refresh my memory, which religion killed millions of people in the name of imperialism or then thousands of people in Ireland or during the Thirty Years War or during fascist rule in Spain, Italy and Germany.
\item Chuckie isn’t the sharpest knife in the drawer
\item I always like hearing from a 'true - blue Conservative' as you have claimed to be on past posts. Keep it up......................................./sarc
\item Alceste, Paris voted 10\% Le Pen Paris is  20 \% Muslim ? 20 \% other immigrants ? 50\% urban leftists? - so why is that surprising?
\item Is that a slur on Burke's sexual orientation?  You have given the impression of being beyond that.  Gay jokes from an anti-homophobe.  LOL.
\item TO Blackfly and eCitizenfirefighters, police and ...teachers and TTCare examples of OVERPAID public sector UNIONIZED salariesthat people oppose but because Ford also opposes then the Ford Haters oppose Fordsort of cut off your nose to spite your face
\item ...are you talking about the Jewish 'propaganda movies' ? Anne Frank... about the Third Reich... about this...about that...on every chanels of the world... once a week...'when you run out movie ideas', eh ?
\item if you believe trannies are mentally healthy then you have lost touch with reality...it's classic body dysmorphia involving mutilation, self-harm, acting out...obviously this CG idiot needs to be fired and forced out of normal society
\item You have the disgraceful temerity to draw a moral equivalence between the Holocaust and the Jewish recovery miracle, and the Palestinian fourth generation, UN tit-sucking, Jew-hating refugee bullshit story. It's exceedingly charitable to describe you as a libtard.
\item Simple answer: people who don't like muslims care.
\item Freedom of expression should not include allowing women to be repressed or supporting Islamic extremists. i wish I could reference an article in the G\&M, written by two Muslim women as to why we should not support the wearing of the niqab.
\item More poverty for average joe hardworking taxpayer on a fictitious problem.
\item It's always a flukwing Jew, isn't it?
\item There is no 'peace' on this one princeed8.
\item Diversity should be restricted to the public sector, where merit isn't relevant.
\item It would be nice to see a transgendered black Latina beat Trump in 2020.
\item you are so naive.
\item When Lori has a PF named Persico he should really keep quite about issues gay.
\item As night fell Friday and Texas braced for a generational storm, Trump pardoned a racist political ally and ordered an indefinite ban on transgender servicemembers joining the military.
\item Forgive me for being ignorant, I really just don't know -- 'transgender woman', that means which way?  I mean ... well, what parts are there.
\item Compassion if necessary, but not necessarily compassion'
\item Agreed that Parliament should legislate the terms and limitations. But let's just wait until we have a real Parliament, not the current one, with its 34\% emperor...
\item They are the freakie new breed of drag queens. They can't even admit they are gay.
\item Oh yes let’s cut all social security pensions and healthcare payments and let people starve to death
\item Wyatt are you a transvestite, Transsexual, or just a Man that just hates himself for being what you are? Do you have a hard time competing against your gender?  Get real, look in your shorts Dude!
\item Exactly like the baker who will not bake cakes for gays, except no one fraudulently allowed him to discriminate.
\item Republican controlled only in theory even Republicans can't stomach Cheetolini your religious SAVIOUR ... lol ... 'christians' are foul and evil as is evidenced by YOUR President :)
\item Klastri, back to name calling when you can't explain a comment you made.  You said transgenders in the military is a civil right.  A sharp lawyer like you ought to be able to defend your position, so why can't you?
\item Wow, there sure are a lot of ugly posts here this morning.
\item Did you watch the videos? Only one side was chanting about killing Jewish people and listening to a KKK leader speak.
\item They have the same rights to life and security of the person as you do.
\item Just an excuse?' That's an interesting way to describe the targeted murder of six people. If it had been six Jews that were killed, would you have the same objection to a motion that condemned violence against them?
\item What a disgusting apologist stance!! G\&M endorsed Harper last election, and it looks like they have neither been paying attention nor learned anything since!! The worst accountability problems Canada has ever seen stem from the CPC Party!!
\item But no one can actually demonstrate why homosexuality is intrinsically degenerate. Not without relying on circular reasoning.
\item Yes because when I think of the PLO, Hamas, and Islamic Jihad the first thing that comes to mind is: law, morality, and ethics.
\item WTF?  He's Jewish and should be well aware that lineage is traced through the female line.  Second, what kind of message does this send to his daughters?  Sorry, girls you aren't good enough for me.  I need a son.
\item free trade, and unfettered shipping of jobs to places like india is what is pushing us into poverty, we have a moral obligation to help canadians before foreigners
\item Lori lives in an ivory tower and hasn't stepped out into the real world yet.
\item Ah, so it is only symbolic then ? ... how about the whole religion and all (man-made) religions are symbolic (i.e. created by man to suit his spiritual needs).
\item Gazans could have built a power plant \& a sewage treatment plant, but they decided that it was more important to build tunnels into Israel to murder innocent Jews.
\item Please post the stats on racial profiling and police shootings of Asians and Jews. I'll wait.
\item Typical looney bin democrat rent-a-mob.  A collection of neurotic women, homeless trans-whatevers and effete metrosexuals.  Yikes!
\item First of all. Modernism is passe. We are living in a post-modern world. SOme even say post post-modern.   Second, I stand by what I said.  Utter nonsense--specifically, the One, Holy, Catholic part. As far as 'outside of which' that is simply not provable.
\item Changing the subject...? Compartmentalizing is just another form of cognitive dissonance. Sorry I refuse to debate you any longer. You don't like your 'sacred' things being questioned, that's obvious.
\item Guy who wrote the bathroom bill loses to a transgender opponent.........delicious.
\item Ya you are probably right... getting rid of Islam would probably get rid of all those as well.... good point
\item The Nazis killed 6 million Jews, the Republican Party thinks nothing of attempting to kill 30 million Americans.
\item Or bakers not baking homosexual wedding cakes.
\item Rodney Howard-Browne is a heretic and an embarrassment to Christianity.
\item Lattes and Danish. The USA will protect us.
\item The Holy Bible is wholly babble. It's a bookfull of lies and ancient superstitions. The good news is the trend is overwhelmingly against religion and towards commonsense and science.
\item Trudeau is like all other politicians on the left. They have abandoned the LGBTQ community in favour of another community that persecutes and murders gays. Trudeau certainly wouldn't wish to offend his new best friends - the ones with the quaint cultural practices that offend most civilized people.
\item I am happy the community allows dissenting voices. I wouldn't subscribe here if all dissenting voices were banned like in other pathetic groups I've been in. 
\item If this insanity continues, one cannot help but wonder if Ivanka will eventually be forced to choose between her racist daddy (and his low-info racist supporters), and her Jewish husband.    Boy, do I miss having the adults in charge of things. Not surprising most Americans miss Obama.
\item This is silly.  Hardly any Catholics believe that contraception is wrong.   https://www.americamagazine.org/content/dispatches/us-catholics-hold-mixed-views-religious-liberty-issues
\item But it was okay to put drug dealers under house arrest so they could wander into the Eaton Centre and shoot it up, right? Wouldn't want a violent criminal with an illegal handgun in prison would we Liberals?
\item Moore’s candidacy points to what everyone should abhor:  Extremist Christian nationalism.  Elimination of the separation of Church and State is their primary goal.  (…and they get to define the official religion as whatever suits their agenda as they go along.)  Roy Moore is simply another psychotic whack right wing candidate.
\item Be careful what you wish for Jimmy.  Minorities are generally not treated well by republicans.  Who knows what will happen to you.  You might even be sent to Gitmo because they think you are Muslim.
\item Actually I do, but maybe it is you that does not? Do you work for the government? Seems so
\item so explain to us why Ford got the biggest funeral parade of any mayor in Toronto and I mean PARADE you should have been there to feel the love from the poor and the marginalized
\item You now accept Benedict as Jesus' Vicar.   LOL!!!  Five years ago you wanted to hang him.  Hypocrite!!!
\item Let me guess: M.W. ?Elizabeth is a gem among the Globe columnists.
\item Sir Tertullian also called women the gates of hell. So much for 'Christian values'. No, wait, that is the Catholic value.
\item Don't worry about African Catholics, they don't need our whitesplaining. They have strong voices that are rather uncomfortable to many European and American mostly white vatican elites.
\item If he had been Muslim, Mexican, Puerto Rican, or black POTUS would be frothing at the mouth \& tweeting uncontrollably.
\item Don't forget Infidel. It's not just the Jews they want to kill.
\item The fact that 52\% of US Catholics voted for Donald Trump would indicate that a lot of microphones in Catholic Churches aren't working at all. 
\item How many vegans are transgendered?
\item Being gay has nothing to do with being a pedarast, not to mention being a sexual predator.   So gross all around.
\item Arabs and Jews are both semites so maybe learn the right terminology if you are going to use it. You probably mean anti-Zionist but calling for equal rights is neither so you are just flat out wrong.....
\item Now that is laughable......If you heard nothing it is because you weren't trying to hear. I can't believe you would even imply something like this. Are you trying to imply this guy is a Christian ? A mass murderer ?
\item Amazing numbers. In 14 years, the Huston area paved over 54,000 acres of wetlands. Such hubris. Moreover, Texas is officially a climate change denial state. The whole disaster has been caused by gay marriage.
\item Not at the cost of the Human diginity of all women called to priesthood.  Justice First or we are not really Christian.  We are merely haters of women.
\item Garbage. The earth is entering thirty year cooling phase. The war on coal and oil will stop as soon as a Republican is in the White House. President Obama has been mislead by his science adviser.
\item This isn't Euro-weenie land, this is North America, where Ordinary Canadians and Americans don't give a rat's arse about this leftist propaganda, and happily eat our GMO food next to our steaks and ribs.
\item still synonymizing feminism with all that's holy and good. it's a theory, ideology and model. it's not goodness and justice itself. we can leave 'it' behind just like we can traditionalism and still be good people.
\item I think it is quite rational to be afraid of Islam. It's a violent, proselytising death cult. Just look at it's history over the las 1400 years.
\item Where was all the concern for persecuted Christians in the Middle East. Oh I forgot, Justin doesn't own a pair of socks with a cross on them.
\item It seems ironic that Trump worries them but the influx of Arab muslims and their murderous ways is oh so noble.
\item Obama allowed them to start serving in the final few months of his 8 year presidency. For some reason Transgendered soldiers became a priority for him after 7 years and 9 months.   Such fake outrage on the left.
\item Thanks for voting Liberal. Nice to see things working out so well....
\item Oh, Lord! Please stop citing Christianity to the exclusion of all other spiritual systems. There is so much in common with so mnay religions that it strikes me as exceptionally narrow-minded to attribute virtue exclusively to any one of them.
\item Is Richlynd Ketah-Guest, a transgender, taking hormone shots? Those aren't cheap.
\item Vote4Me: Sure, sure. No need to get too excited.
\item Rejecting homosexuality on religious and making a business transaction are not related.
\item I'm happy to see USA bombard ISIS. But if Russia used a big bomb there would be an outcry.  Let's unite to defeat Islamism and Islamic terrorism.
\item Bob, I know that you're not interested in facts but here's another report about the German 'green' jobs collapse. Don't worry, you'll hear more about this! http://greenzone.co/2014/02/26/german-government-report-urges-scrap-green-energy-subsidies/
\item That my comment has gotten under your skin with such little effort on my part gives me more pleasure that I can relay to you. Thank you. The bonus is that the quality of your comment proves Mill's point.
\item Another reason that I should be allowed to declare my cat as my dependent and/or spouse. Harper already was loosing me after he stopped home mail delivery... this just finalizes things. I will hold my nose and vote for Justin.
\item normal as in statistically so, which is untrue among clergy. True heteros left and don't join. priesthood Asexuals and gays do.
\item radicalized = reform, tea party, old testament, scarlet letters, Koch puppets
\item That's too ignorant to be worthy of a real answer.
\item they need to check the local rabbi for spray paint residue.  To identify the truly sick racists google: chief rabbi of Israel says only purpose of goyim is to serve jews, life of goyim worth same as donkey.  Netanyahu says this jerk is the greatest mind of this generation.  http://www.timesofisrael.com/5-of-ovadia-yosefs-most-controversial-quotations/
\item Our city celebrates slugs and trans.
\item Forcing your doctrine down the throats of ...'  Why do opponents of gay rights so often use this metaphor?
\item I wasn't actually sure of the intent of the letter writer, but some people seem to be interpreting it as trans = non human.
\item God bless, hope he makes you dreams come true.
\item And to think she was a woman does not guarantee Muslim terrorists women won't shoot  us or your kids. Remember terrorists. Not because they are muslim.
\item The Church does not teach that Mary 'never died'. Projecting your sexual issues, much?
\item Standing up to those who would eliminate you and your country is honorable. The only bullies in this conflict are the hateful Jew-hating Palestinians and their terrorist civilian-stabbing inhabitants whose goal is to eradicate Jews.
\item Grekoff, yes. The scientific evidence is that, for the past three or four years, the corporate media elites have been braying constantly in favour of transgender 'rights'.
\item More than a 'wink'  one  neonazi site said he had a Jewish gun to his head to make the speech.
\item And thanks to Alberta and Quebec before her, Canadians everywhere know it can be done. Let's go, Canada!
\item Really?  Does everyone really want to round up the Jews again?  I don't and I stand against racist pieces of garbage like her.  She even helped radicalize the right wing terrorist in Quebec who slaughtered six law abiding Canadians.
\item So tell me again about how loving, peaceful and tolerant Islamists are.
\item “alternative facts” that are spread about Muslims by anti-Muslim bigots.  --- There you have it: everyone criticizing Islam or Muslim societies practices are bigots and their speech is 'alternative facts' or soon hate.
\item This should be pretty simple for you to understand...
\item Her life partner Worth of 20 years.  Are they lesbians?   The vulture and the snake fighting for the \$200,000,000.
\item money is much more important than children.  no matter how many children are destroyed, faithful Catholics will always make more.
\item Exferrious....your post is the most ill-informed, misguided and bigoted comment I've seen on the G\&M boards for some time. Congratulations.
\item @Sher .. >> I know that a lot of people have .... Can you tell me what the weaknesses in western culture are? .. Why is it that people flock to live in Western countries - including immigrants from Muslim countries.  How many non-Muslims choose to immigrate to Muslim countries?
\item Very true John but obviously God-fearing Americans are more afraid of the possible threat from foreigners believing in a different deity than they are of sure death at the hands of an Second Amendment-quoting American born-again Christian. Better the devil you know perhaps.
\item Your post violates the first principle: Human intelligence in good faith. Jesus' maleness demonstrates only that 'He' was/is male.
\item KATO 50- 'still do wield enormous power in (Iran) to the point that they can dictate who runs the government.' You are talking about Mr. Harper aren't you ?? CAREFUL.
\item Could you explain how Obama was blatantly anti-Israel?  Lots of Jews inside and outside of Israel strongly disagree with the expansion of settlements but that does not make them anti-Israel. One can still support Israel and criticize their policies that appear to undermine a long term peace agreement.
\item Why should anyone bow to the progressive's demand that no one have any privacy?' Why should anyone bow to the conservative Catholics' demand to protect pedophiles, pedophile priests, the Pontifical Secret, and enabling Bishops and Cardinals?
\item As far as I know, Apple is the largest company in the world by market cap.
\item Great news now we can give out more medals for war heros. They will have as much success as the US had in Vietnam. At least we are full members in the war club now. So much for Trudeau standing up for his and Canada's beliefs!
\item The history of Muslim countries is one of violence, torture and war long before there was any bombings on them.
\item From a man that claims to be a Christian but doesn't have any Christian qualities very much like lots of his fake Christian followers . Greedy , spiteful, pompous, arrogant and a sexist .
\item Liberal dementia, a social disease void of intelligence, logic, and common sense, knows no shame. They negotiate just like Muslim terrorists, there way or no way.
\item At every level, public health doctors have the authority to communicate directly to the public, if needed, without political interference. You seem unaware of that.
\item Yes, most conservatives know these things, a small vocal number do not. But, do most liberals understand that not everybody who disagrees with them is a racist slob?
\item Paul Martin is the only former Canadian Prime Minister I can think of who has attempted to make a significant contribution to Canadian society after leaving public office. A great christian.
\item I would think, Andre, that the silence of the lambs in Gaza is due entirely to their known fate if they spoke out against Hamas. The Palestine Authority's leadership would likely suffer the same end.
\item Your post is both offensive and incorrect. Hitler did target the Jewish people.
\item Defense Department/Rand Corporation study finds the military spends five times as much on Viagra as it would on transgender troops’ medical care  https://www.washingtonpost.com/news/wonk/wp/2017/07/26/the-military-spends-five-times-as-much-on-viagra-as-it-would-on-transgender-troops-medical-care/?utm\_term=.06b4d712b1a8  Another study estimates that banning transgender service members would set the U.S. back \$960 million  https://www.nbcnews.com/feature/nbc-out/banning-transgender-troops-could-cost-us-960-million-report-says-n792466
\item Yes it does. It tells you that the discrimination against Jewish interests and institutions runs deep in the international community, just as the infamous Zionism is Racism resolution in 1975 did and as the continued and ongoing manifestation of international anti-Semitism, past and present, demonstrates and confirms.
\item I have met many homosexual priests.  none, I MEAN NONE  would have ever touched a child. THIS STATEMENT ABOVE IS SICK
\item And here are the biblical references to infanticide. https://bible.knowing-jesus.com/topics/Infanticide
\item cracking a smile and having a pleasant tone doesn't matter a damn when it comes to making the tough decisions and running a country. As was stated prior to the election this was not a popularity contest but it turned into one.
\item when you spread riches around, population growth slows down. you cant just dictate to the poor, you need to help lift them from poverty. then they will stop having so many kids.
\item But wait - it is the government who sets the work, not the bureaucrats who choose what they will do.
\item Thank you for sharing your sanctimonious rant.
\item Trump promised to deport eleven million people in this country because that's what his racist fans wanted to hear.  It is the duty of every Christian to stand up to ignorance, racism, and fear.
\item Jews will not replace us, Jews will not replace us.'  You down with that?
\item Human life begins when one makes the choice to bear that life into existence.
\item Liberal party has already been charged with illegal robocalls. Try to pay attention.
\item You know its not racism if it is the truth.
\item Actually there have been success's. Kobani and Sinjar to be specific. Sinjar and the close by mountain have split the ISIS held territory in half. ISIS will now have to retake Sinjar or re establish communications through the Desert.
\item How refreshingly void of content.
\item Interesting - I think those were the exact same excuses generals used in the past to keep blacks, women, and gays out of the military as well.
\item It was Catholics vs Protestants. How peripheral is that?
\item I did. And it's filled with the usual veiled anti-Islam rhetoric you've posted in the past.  If that's not the case then you need to explain yourself better.
\item Harper and Kenney are ideologues.  Kenney's campaign style is divisive and hateful. His party has attacked women, gays and minorities. But keep attacking the messenger.
\item Yrs, Ben Shapiro is a white supremacist.  You people do know he and his family are Orthodox Jews.  Ignorant people!
\item Can we please get away from gender,  transgender, race and other issues and  simply evaluate performances on merit alone?
\item No, gay or not, you should hate yourself if you are in a state of sin.
\item The international community must respond to attacks on gay men in Chechnya'  Such attacks are deplorable, but if we acted every time a columnist told us we 'must' something, there'd be no time to enjoy an occasional doob.
\item Trump is more like the anti-Christ. He literally checks off all the boxes that the Bible warned us about.
\item Who am I to judge?' means very little when you just got fired for being gay while working for a church.
\item Fuck, what a brutal story. 
\item All the examples you give, are civil servants. Thanks for proving our point
\item Who cares. Hamas and Hezbollah and the Palestinian Authority have continuously threatened Israel and its Jewish population with destruction and elimination and eradication.
\item Jews only marry outside of their religion when there is money on the table. If she wasn't an heir to Trumps billions Kushner wouldn't have even kicked her tires.
\item Yes, it leads to a Breitbart webpage. Pffft.
\item Couldn't agree more. My sympathies to Mr. Mason for having to write a puff piece.
\item No, it was right-wing evangelical hypocrite blowhard Jimmy Swaggart that was related to Jerry Lee Lewis.
\item In response to this, two progressive Catholics put a laughing face emoji below your post.  Both were totally unable to offer a cogent rebuttal, and masked their ineptitude with ridicule.
\item Given that Trump has shown himself to be a narcissistic, lying, sexist, racist bigot, he DESERVES to be attacked. Certainly, no Christian should support him. Do you really believe he gives a damn about abortion?
\item Terrorists didn't round up the Jews in Germany and systematically kill them: the state did. His message was crap, too.
\item So an unelected and unaccountable judge used his power whatever way he chose to exonerate an unelected and unaccountable senator. What a surprise!
\item There are scholarly/credible/etc. sources who say the gay priests, seminarians, bishops, et al. do NOT live celibate lives.  Why does it matter?
\item I can't believe the Denver Post published this witless slur against transgender people.
\item WE' have been trying to 'make things work' for 147 years. All Quebec has to do is to join us with a sincere effort to do the same. Throwing Queen Marois out is a very good step in that direction.
\item  A lesbian ,  a native,  and a Rabi are in a life boat ... '  Yadda yadda yadda
\item Kenney supports the corrupted catholics and therefore is incapable to unite Albertans.  Religions are used by politicians to divide societies.
\item Why should Trump receive a 'pat on the back' for enforcing equal protection for the LGBT community?  Trump's too far from the eight ball to receive any pat on the back.  A swift kick in the butt perhaps.
\item Protesting against Islamophobia?!?   Sigh...Alice, close your eyes, we've reached a new level of sheer stupidity.  I wish these same progressives would protest against antisemitism.  Or anti-Christianity.  Those darn white people just aren't as politically 'SEXY'   How about we protest against selective religious intolerance?
\item Does that make her an 'enemy?' Seems to me that she pays taxes like everyone else does. She is entitled to her opinion too. Or do Conservatives have a problem with free speech?
\item You might be the first NDP supporter I've ever run across who also supported the Fraser Institute.
\item Wrong.....2 shooters one muslim and one wannabe
\item So how do you classify Kevin Spacey?  He says he's homosexual not a pedophile.  The research you're talking about comes from the psychology arena that I spoke about earlier.  It's all biased, weak research.
\item Perhaps you should refer to the Hamas charter which lays claim to ALL the land and promises the eradication of all Jews.
\item \$ 40.00 Oil has already stopped Oil Sands expansion... what a weird article... so emotional
\item Would propose kicking Jeremy Christian out of your organization before he slashed the throats of three people or wait until after?
\item If I were transgender I'd say 'bah-bye' and be on my way, middle finger extended.  Trump is such a nothing.  And so are the people who support him. Just more to add to my personal list of 'undesirables.'   Ugh.
\item Liberals always march under the banners of 'Justice' and 'Equality', until they actually have to show up.
\item I support a voluntary \$100 fee.
\item People on the plane were allergic to an intolerant Muslim.
\item Alaska's Christians will continue to appear ignorant and vindictive to the rest of the world while the Prevos and Boykos of the world go on their merry way ruining innocent people's lives while the Carlsons of the world are forced into early retirement.
\item ruthmatthews, can Rob Ford find something more interesting to [do] except slander and scandal, slander and scandal? Isn't that the real question? (that you've conveniently chosen to ignore)
\item You didn't read the article. Free speech is freedom from government punishment for what you said, not from your employers/customers/partners/sponsors from reacting to what you said.
\item Steve Hewitt wrote that Islamophobia is a cause of Islamist terrorism.  What a perfect example of putting the cart before the horse.  It's far more likely that Islamist terrorism is the cause of Islamophobia.
\item So Hitler wasn't anti Jewish because he didn't kill all the jews?
\item You clearly have a rose-colored view.  Do you know what it is like to be an English speaking native of Quebec living in or visiting Quebec? ... Less fun than you'd think.  It gets even better if your mother, also a Quebec native, is Jewish.
\item I guess those Imam's in Canada who were shown preaching about killing Jews and non believers have been charged with hate crimes?
\item It's interesting how Jews can support someone connected to Nazi groups (Germany 1933).    Economic considerations almost always trump social and political interests.    Those Jews are less Jewish, more richish.
\item why, you want pictures?  numerous studies have shown that those who are vocally antigay are often closeted homosexuals that are secretly envious of those who are you publicly out.  is that why you are stalking me, you have a crush on me?   how special!  https://www.scientificamerican.com/article/homophobes-might-be-hidden-homosexuals/
\item What could be more clever than mocking the transgendered?   Are you 12 years old?  Pathetic.
\item Liberals being against ecumenism, who'd ever expect to see that. And 'traditional ecumenism' - what's that, 'Return to the Catholic Church'? How hypocritical: ecumenism is only ok with Christians more liberal than us. From Fr. '2+2 sometimes = 5'.
\item Trump calls for unity? I guess that means that all Americans should just accept the white supremacist Nazis, shouting 'Jews won't replace us', 'blood and soil'?  Capitulation to these lowlifes hopefully will never happen.
\item “[Progressive activists] were calling me a Nazi, a fascist, and an anti-Semite,” Dr. Gad Saad, a Concordia University marketing professor and one of the panelists, told TheDCNF. “I’m Jewish. So, they’ve lost the plot. It’s a form of lunacy that’s difficult to diagnose.”  http://dailycaller.com/2017/08/16/college-responds-to-hosting-panel-on-free-speech-by-canceling-it/
\item I am glad I am gay. The worst that happens  after a two guy have a night of drunken sex  is the guy doesn't leave in the morning , or if  he doesn't call.
\item Actually it's already covered by Medicare.  Besides, the Pentagon spends ten times as much on Viagra as on transgender medical coverage.
\item It's not a ban of all Muslims in the Universe. I know, hard to believe, but it is a ban on Muslims from certain countries. Are you simple?
\item The US has received zero terrorists from any of the banned countries, ever.  Not a single one.  Trump is playing the terrorist excuse to ban legitimate refugees, because he hates muslims.  period.
\item How long until somebody accuses her of murdering Servaas, her lesbian lover? I say 12 minutes.
\item Because at most they make up 0.3\% of the population? Clearly the left is in the next phase of making traditional Western culture disappear with their propaganda and social engineering. Next phase of the destruction of the west after 'Trans' is normalized will be pedophilia mark my words.
\item Good for you! Many can relate to this I think. Many, many worked hard, made sacrifices as needed and did the sensible thing, saving what they could. Now....let them enjoy it!!
\item quite the hypothesis... and now can you back that up with specifics? Naw, I didn't think so.BTW, I will take the wooden Harper to the pixie doll JT any day.
\item Gutless self serving politicians are afraid of losing the Christian vote so they will not do the humane thing to stop people from dying a painful death. Get rid of the useless career politicians.
\item You know who else was obsessed with perfect genes, right?   Hitler, who had Josef Mengele at his side experimenting on humans to find the perfect one, while killing millions of Jews.   The obsession with genes on the part of this president and his administration is really disgusting.
\item I was watching on HBO with candles and shouting your friends marching last weekend. They chanted the following: - 'the Jews will not replace us' - 'whose streets? our streets!' - 'Blood and Soil' an old Nazi chant This is outrageous and hateful. It was done by your side. Wake up!
\item I wonder what Putin's or Jung Un's policies are regarding transgender soldiers?  Do  they have their military forces  cover the costs of the operation and hormones ?
\item There's some justification for excluding the women carrying the Israeli flag. They should know that Israel is a devisive topic whereas being Jewish isn't.
\item How about a man who has transgendered into a woman.  Does he-she then become a qualified woman owned business?
\item You think your "expertise" is worth something? You uneducated rube! In the real world, what YOU think is exactly meaningless.
\item You obviously don't know what you are talking about. If you are a 'catholic', you don't know much about your religion. Nobody is playing dress up. And if you aren't Catholic, you should keep your mouth shut and hide your ignorance.
\item The president is commander in chief of every branch of the U.S. military.'  Since President Trump is also grabber-in-chief, is he going to issue a ruling on whether or not transgender people can grab?
\item Ever since they got their segregated Dyke March, Pride has been fractured and fragmented bit by bit, year after year until now, gay men are not really part of the festivities other than as spectators who are expected to shut up and buy something.
\item If you are annoyed by it, you don't really understand it.
\item My, what a cleverly SUBTLE example of Muslim-bashing!  I don't think I've been subjected to such a devastatingly articulate rejoinder since...possibly the 7th grade.  I-I-I think I might just cry...
\item Well put sir. Or Ma'am. And... these are probably birds from the same flock who still think of 'Jews' as a race.
\item Effeminate men are as likely to be asexual as homosexual.  Priests are as likely one or the other.
\item Where? Did I miss it? Damn. Besides, are you aware that Jared Kushner, Trump's son-in-law, and one of the most important and effective people on his transition team is Jewish?
\item Shhh, don't confuse them with facts...  Just like with Jesus, its much easier for them to celebrate the idea of the man, and ignore what he actually stood for...
\item NoinradClearly you are a 'believer', and no amount of adverse data will change your mind. You are the little kid with fingers in ears saying la la la can't hear you!
\item US/Saudi supported 'moderate' terrorist head-choppers' No, Islamic supported and trained... Countries don't train people to be head choppers, organ eaters and yell 'Allah Akbar while killing each other and innocent people.
\item Sorry Alexandea, any group that denies science and wants to trample over the constitution's freedom of religion- for all religions- is wrong. There are many beliefs in evangelicals 'faith' as well as Catholics 'faith' that are plain stupid!
\item It also executed gays.  Are you for that too.
\item I agree with those many trans-gendered.
\item The fact that gays find sex between man and woman revolting is testament to their intrinsic disorder. Tell the truth, for once, Bindner.  Tell the truth.
\item I think you should have used the term, empathy, instead of, compassion.
\item GE, I agree ! Why they we elect this lying liberal government 3 times in a row ?
\item I'm going to go out on a limb here and say the vast majority of Americans are not in favor of transgenders serving. Obumbler's policy change was stupid.
\item And Charlie Hebdo's editors routinely pulled cartoons that mocked Jews and Israel. Hypocrisy!
\item Meanwhile, in RC American schools gay students had better remain in the closet, or else!
\item Transgender soldiers follow the same rules as other soldiers and face the same consequences as other soldiers for disrupting good order and discipline.  What is your point?  That soldiers who dislike and don't trust transgenders might act out and disrupt good order and discipline?
\item To cut roots of terrorism, enforce the Rule of Law
\item 2 million? I'm going to vomit. Muslims have not built this country or any western country.  But they all seem to want to move to the west and then change it. Multiculturalism is proving to be a terrible idea.
\item Sara, here is a small sample from A.L., paragraph 259 'There are absolutely no grounds for considering homosexual unions to be in any way similar or even remotely analogous to God’s plan for marriage and family.” Emphasis on the 'and family' part.
\item Don't be over confident. Muslins that Trump tried to stop from entering the U.S. freely enter Hawaii. It's just a matter of time before we experience terrorists activities. No longer a question of 'if' but 'when' and 'where'.
\item I agree. But access to psychological help is almost non existent for most Canadians, unless they can pay for it privately, or have a good health plan at work.
\item A wonderfully expressive article that accurately encapsulates my feelings towards yesterdays events. Keep up the good work Ms. Wente, you just gained a new supporter.
\item If their an obese transgender, do they get in?
\item ...or the sexual abuse of children?  Jesus is a 'big boy', reputedly 'all knowing', etc. Children are quite another dimension.
\item I like the study showing lower IQs correlate highly with right wing tendenciesneed some certainty in your life? like authority? is thinking for yourself too much trouble? vote conservative
\item Note to Liberals: Bringing up the existence of Trump to in an attempt to shut up dissent about your insane immigration policies and your frantic rush to bring in Muslim refugees is pretty pathetic and insulting to anyone of intelligence.
\item It's because the editors don't know anything.
\item The Nazi went after German Jews and Aryan Germans later.' . The Nazis went after 'Aryan Germans' ?   Really ?  How amazing !!!
\item Muslims cannot emigrate to Japan
\item You are right, homeopathy has much in common with faith healing. Utter quackery.
\item M-103 is the discrimination. It's unnecessary identity politics. It's religious fools trying to get a foot in the door. It's complete nonsense supported by flakes and it should go in the trash bin where all religious con jobs should go.  Is that Islamophobia?
\item Why is Islam allowed in our schools?  It is much more than a religion, it is a comprehensive system - political, military, religious and dietary.  You cannot have Islam without sharia.
\item Trump also won because people despised the cabal that barnacled itself to Hillary: banksters, media owners, globalizers and the Republican elites they own, Democratic insiders, satchel-faced Radcliffe and Bryn Mawr psychopaths, Big Labour bosses ...
\item Valdy has a division of transgendered soldiers.   3,2,1 ... deleted
\item Leave the 'Hot Hatchet' alone, he is a victim and self identifies as a role model citizen!  Stop being Trans-existence phobic
\item depicts a fundamentalist society that treats women as property' A muslim country? Wait, I thought Islam was good...
\item I gather you have not been to Israel. It is a Jewish State and within the Jewish State, you can be Christian, Moslem, Bahai, or anything you want openly.
\item Let's see.. a group that supports children with very little funds is a bad thing. Attorneys helping the organization and victims, is a bad thing.  Yet the catholic church with enormous amounts of donations and funds can manipulate law makers to deny the abused, is OK
\item In the warped mind of the killer's father: Kallie is a good Christian girl from a good Christian family and the media (FAKE NEWS!) blew the story way out of proportion, so she should be let off. She's probably the real victim here.  GFY, Mr. Kuhasz.
\item This isn't about women in combat, its about transexuals in combat. The women in combat ship sailed long ago.  But hey, keep screaming on the dock if it makes you happy.
\item An interesting question, but one you're not going to try to answer, I see, slofstra.  I'll give my opinion on yours, though.  The fact that TWU would be the only law school with this rule makes it no better than a single corner store which refuses to serve jews.
\item The birth control mandate, if originally inserted in Obamacare, would have just as easily passed. Why? Because it is essential that Western Judaea Christian America continue to contracept itself into oblivion for a successful 'fundamental transformation' by the Godless left to occur.
\item Or a lawyer!
\item It is reportedly said that one of the Justices, Lebel, even talked about freedom from religion. If this is true here you have a justice totally misrepresenting the text of the Constitution openly. Really incredible.
\item It's about fuckin' time that a World Leader takes a stand against Evil Islam/Muslims.  Hopefully our White Trash Racemixing Liberal Govt. will follow suit, but I won't hold my breath.
\item It's called faith or believe for a reason. Logic is an attempt to either confirm or debunk ones faith or believe. To believe does not require logic.
\item I think the issue is more about being forced to stare at Mr. Winky at a female spa (no offence to transgender people).
\item When Trump moves the US embassy to  Jerusalem, the Palestinians will have to be very careful not to damage American  property when they blow up Jews.
\item Donald Trump is on the record for bragging about being a sexual predator.  U.S. Catholic Bishops have a long well-documented history of protecting sexual predators that otherwise conform with their positions.  No surprise that the bishops would overlook Trumps major character flaw.
\item You not only do not understand fascism, you do not grasp the conditions for fascism to flourish. And by trying to peg me as Jason, you have revealed yourself to be no more than a troll trying to annoy readers and commenters alike.
\item Trying to tie Christianity to white supremacy seems a real stretch.'  I'm told stretching keeps us limber. Just because I can't reach my toes, doesn't mean they aren't there.
\item Because then both boys and girls can get shot at equally !
\item Good find but it leaves one question unanswered.  Was that person transgendered, of was it simply a disguise to  commit a crime?
\item The Middle East conflict is not about freedom but personal security. These countries have never been free in the sense of democratic.
\item Who knew that anti Muslim vitriol would embolden violent racists to perpetrate viscous attacks. It just doesn't make sense.
\item Accepting and promoting are different things, whether you talk about legal homosexuality and a right to marriage or legal abortion.
\item Passer. You speak as though the Supreme Court was the highest power in the land. Who cares what they "require"?
\item None of the programs that Pope Francis is talking about discuss transpeople at length.  The French program that Pope Francis condemned is about gender equality.  The real issues is that Pope Francis wants women to be broodmares for Jesus.
\item Residential schools were Implemented and supported by the Government of Canada and  allowed the Catholics to do what they wanted.  Now Trudeau want's an apology from the Pope?  How about Canada  taking responsibility instead of pointing figures at others.
\item And in other news, anti-Jewish bigotry and incitement to violence given a green light.  Now get out there and a punch a Jew!  Oh sorry, punch a Zionist!!
\item Trump's surprise ban on transgendered people in the military is ridiculous. They were allowed before, identifying them is hard, they're not *nearly* as expensive as conservatives claim, and there's no clear instruction on what to do with the transgendered individuals already serving.
\item Muslims are the ones who wanted this passed dude.  Show some sympathy for the victims.  Amazing heartlessness in some of these posts
\item Whether you are guy, bi, trans, straight, nobody cares.  Using your orientation, as if it makes any difference, or because of that, your opinion counts more--it does not.
\item I doubt that President Trump knows what transgender is.
\item He supports people who have. He's against gay marriage, and for the right for companies and individuals to discriminate against gays.
\item Trump is not using race as an issue? You mean he is welcoming to Blacks, Latinos and Muslims to his rallies? What is the evil agenda that you speak of?
\item So imagine a white man making these racists comments about Muslims on campus. Would these same professors put it all on the line in defence of that white guy? The answer is no.
\item I am far happier and healthier post-transition than I was before.  So are lots of trans people.
\item Liberals just changed the game and dropped Motion 6 and are focusing on working together respectfully for all the people and country. memo for all MPs, sunny ways are here again, now back to work and voting like you are paid to be doing.
\item I find it odd that people think they can negotiate with a religion that wants to cut your head off because you're a Christian.
\item The column was amusing, well written, and written with affection -- which is more than I can say about some of the comments.
\item Some say Pride has always been about Politics NO Pride is not the United Nations it should stick to gay politics - fight for gay rights and not Israel-Palestine unless to support gay rights in Palestine (Israel already has)
\item i will lie to you, raise your taxes, increase the debt, and make sure you vote for me brother.
\item The simple fact is that self-identifying so-called Christians don't even come close to abiding by Christian tenets.  There's no apology for that.  That is better known as just what it is.    Blatant hypocrisy.  And there's no excuse for that.
\item The Dispatch uses every chance it gets to push their liberal agenda.  Showing a picture of  Kelter down at the gay parade .  Really ?  How pathetic .
\item We in the West need to concentrate on saving our civilisation. Let the Arabs take care of whatever revolution they favour.
\item All forms of hate needs to be eliminated. All forms of racism, Islamophobia, Homophobia, anti-semitism and laws discriminating against Transgenders. We need to get behind Justin, Obama, Hillary and Premier Wynne and fight all forms of hate which includes Trump!
\item Faithful Catholic wrote:  <<I will take Putin's useful idiot, thank you very much...>>  There you have it. Certain authoritarian Catholics are fine with Trump's entanglements with a murderous dictator.  It's disgusting.
\item You need to get a life. Really!
\item So this is the 'new wave' of anti-Semitism? Israeli Jews threatening their own around the world?  It never ceases to amaze me how much reality can differ from the propaganda.
\item That's your takeaway????No one is saying not to criticize her. Just don't advocate violence against women. That's the difference. And while you're at it, don't advocate violence against any male politicians either
\item but they can have 4 wivesmaybe it is the women that should have 4 husbands
\item He was teacher and a camp counselor. Those that can't - teach Perfect pedigree to run a convereted Muslim Communist country
\item @Gibson, you are paying more for Canadian milk, much much more. But you go right ahead. Not everyone wants to follow in your footsteps.
\item I can give examples of the peaceful Muslim missionaries murdering people 100 to 1 of your examples.  Islam is the religion of death.
\item Pope Francis talks about walls being bad and then defends Muslims.  Hmmm...
\item How about FUCK NO. If anything Canada should learn from America's example and start smartening up before this country is overrun by Muslims and Chinese who don't want to learn English.
\item Didn't you bother reading my post?  According to your criteria, my son did NOT honor the Church's teaching. He got remarried, and since he and his wife have children, has obviously had sexual intercourse with her.  He LEFT the Catholic Church specifically because of the laws on divorce and remarriage.
\item Believing in transubstantiation 'because the Pope says so' is just as stupid as believing the earth is four thousand years old 'because the Bible says so.' Both are simply political self-interest couched in supernatural blather.
\item Most military households say transgender people should get to serve
\item if a guy came to our Jummah and started spewing hate and being violent, he would literally have 300 brown and black kids jump at him.” --- Where were those 300 when the PDSB faith advisor hosted an imam calling for slaying of the Jews?
\item He's a man so that won't do.  I was thinking more along the lines of Theresa Spence now that she's looking for work but I'm pretty sure the CBC is hoping to cover all of their bases by hiring a non-white, aboriginal, trans gendered individual.
\item WOW  Jew hater nice
\item The same lefty loser 'activists' who 'March for Truth' can't bring themselves to say the words 'Radical Islam' and believe there are 71 genders.  (Or whatever the number is up to now.)
\item Every one of these hate hoaxes since the election have been staged by Jews themselves
\item Stop living in the '40s Matt. The rest of us have moved on from this a long time ago...
\item @ Nanakanda - Harper would never fund university education. He'd much rather let tuition fees go up. Harper doesn't like people who are smarter than him.
\item haters? you should have seen the FORD haters the MIKE HARRIS haters the HARPER haters Trudean Haters are meek in comparison
\item non-Muslim girls or women are not permitted in traditional costume during Burkini hours.
\item Extremists on both sides, left and right, are equally ridiculous, and capable of incredible hypocrisy and brutality.
\item That cannot be .... did you not know? :)) Only 'right-wing' (whatever that means) people can be 'populists! :))) Certainly not Obama, especially after demonstrating his great charisma in psyching people into a trans-like state with all the 'Yes, we can do' chants!
\item maybe you're gay ...try making out with another man , see if that helps
\item Why would people be posting about the liberals when Paris just had a tradegy? Can your partisanship know no end???
\item Firstly, Jewish is not a religion, it is a race. Secondly, the holocaust claims by Jews has been shown to have been a fraud to extort money from Germany. Google holocaust fraud and you will discover why.
\item What about Viagra? A 2016 study by the Rand Corporation found the maximum annual medical costs for transgender services would be around \$8.4 million. By comparison, the military spent \$84 million on erectile dysfunction medications Viagra and Cialis in 2014, the Military Times reported.
\item I really believe that Jews are sucking up way too much oxygen of public debate. Not one day goes by we don't hear about some grievance ..or need for special treatment.  All this clamouring for attention 24/7 leads to resentment.
\item  …or they've seen how hypocritical Christian act. . Sin all week long, absolve yourself on Sunday.  Rinse and repeat. .
\item I thought Asian's weren't considered minorities because they don't complain, do well in school and in business
\item If by "social engineer" you mean to correct misunderstanding, ignorance and eliminate bigotry, then engineer away.
\item Yes - anyone who puts his career and life on the line to stop North America from becoming East Germany is a hero and patriot in my book.
\item The underlying intent of EU is to destroy the white race, Christianity, and western civilization. Leave it.
\item That you would post something like this only underlines how you don't have the first clue about the crisis facing our veterans.
\item Bush used fake WMD's to go to war.  Clinton wrongly backed Muslim forces in the former Yugoslavia.  Two idiot tough guys who were also POTUS
\item No biases, thank you, just a realist.  Maybe he is biased toward Jews.  The fact is, he is ignorant and has a destructive agenda.  Can you imagine the rest of the world putting sanctions on us for destruction of the atmosphere using the Trump policies?
\item And the Republic party just loves its 'blood and soil', 'Jews will not replace us' core driving a car into a crowd and killing a woman. That's the Republic party's definition of a civil society.
\item I think we need to be careful of the old pupule about the Jews killing Jesus. Jesus and all his disciples were jews. It would be like saying that it was those evil Americans that killed Lincoln because Booth was an American.
\item integrityAnd yet it isn't in Canada's interest to be so one sided in this conflict-----yet if Harper were ONE SIDED in support of terrorist Hamas you would celebrate and not mind at alladmit it
\item Cry me a river.  What happened to the Syrian Christian refugees?
\item The Average Patriotic American does not like being called 'irredeemable deplorables'.  That is one reason.  Another reason is that the Dems spew hatred towards Christians, Veterans, White Males and anyone who disagrees with perverts showering with our granddaughters.
\item Why would I want to reject (or eject) a transgender cyber expert from my division as its supervising officer?  All military service doesn't take place in the proverbial 'foxholes.'
\item 1. Rubbish.  2. Flout, not flaunt.  3. The only 'homosexual advocates' are the ones that exist in your imagination.
\item I bet it was those radical hate-filled drug-free Christians. Again.
\item Doomed to fail? His communications director is the problem? How about our representatives? Maybe you should run and try to herd those cats.  Christ this is some horse shit.
\item That is an utterly ridiculous thing to say, since these poor people were specifically targeted because they were members of the LGBT community.  That would be like saying that Adolf Hitler targeted 6 million people for death in concentration camps in WWII, and failing to mention that they were Jews.
\item Is he attacking...Transgender individuals? No. The ideology that grounds transgenderism? Yes.
\item Sure, all newborns weight the pros and cons, and then make conscious decisions on their sexuality.   Don't you realize how ridiculous that sounds? What you mean is that you were born heterosexual just as those you judge so harshly are born as homosexuals.
\item A mouthpiece for the political party that attracts Blacks who hate Whites, Homosexuals who hate Straights, Feminists who hate Men, etc.  And if you don't agree with anything they say....burn and loot.
\item What exactly are Jared Kushner's qualifications for trying to negotiate peace between Israel and Palestine again?  Oh, right.  Hes Jewish.
\item Agreed. Those in the media are given undeserved adoration. They have bad breath, body odour and constipation just like everyone else but me. Hey, how come I'm not in the movies?  I coulda got babes for the ugly jewish man.
\item Propaganda of homosexuality should be forbidden.
\item There is precious little historical evidence for the actual existence of Jesus.' Ever read 'The Case for Christ' by Lee Strobel ? You need to. You'd rethink it.
\item Love is seeing yourself in others.' ~Eckhart Tolle
\item In private, however, he was living with Charles Chiarelli, his lover since 1965.'   That sentence says it all.  Fr O'Neil was an active practicing homosexual priest.  I don't think you should compare Fr Martin to this fellow Jesuit.
\item Paul - So when your teenage daughter is showering in the girls locker room at school and a teenage guy who identifies himself as a girl showers and walks around with his penis exposed, are you ok with that?  http://dailysignal.com/2015/12/21/why-these-high-school-girls-dont-want-transgender-student-a-in-their-locker-room/
\item How about keeping it to 'A nice Family moment' in a Disney film. Why does there have to be a Nice Gay Moment?
\item because Bud, if you don't come out it will be assumed you are heterosince most gays are cuter, handsomer ...this is like saying 'Ladies, I am not available... don't waste your time'
\item When will Justin apologize to sex workers for society looking down on them
\item Why would white racists burn the church and then write 'Vote Trump?' This is an act by the Saul Alinsky crowd. They drove down from New York in a Mercedes limo, committed the act of terrorism, then drove back. This is what we get if Hillary is elected.
\item Well Loonie, he's either a liar or extremely incompetent on the refugee file for a starter. He is saying the opposite of what his ministers are saying regarding the failure to bring 25,000 refugees in before 2016.
\item Does it say loser on it?
\item Very few people are transsexual. Trustin is just virtue signalling.  There are many groups who are being marginalized in Canada that need more help.
\item Maybe Harper can send you a free carton of cigarettes.
\item Anything that has the potential of taking seats away from the Harper gang can only be good for Canada.
\item The ignorant shall always be with us.
\item Whiteness is always changing, which further proves that it is dependent entirely upon social conditions. Greeks, Italians, and Irish were once not white. Nor were Jews until after the Second World War. Now it could be argued that people of East-Asian descent are on track to whiteness.
\item Support an independent CBC.
\item BS -- the whole 'transgender' kerfluffle is a minor, barely signifying blot on the national consciousness -- twitter is a perfectly appropriate venue for announcing the ban
\item As are homosexual tendencies.
\item Marx, your hatred of Jewish people is well known.
\item You're right. We should go full Orwellian. Great idea. Let's start with 24 hours cameras on YOU. Let's see what we can get you on. I think, at least speeding. And you probably swear once in a while too.
\item Trinity Western is not attacking. The ruling is a breath of fresh air to those who really do believe in freedom of rights. I think if you would read your letter objectively, it is you who is attacking.
\item Thank you Senator Schatz for standing up to this bully and racist.  I am proud that your represent Hawaii and in particular my views.  How can trump defend the crowd chanting, 'No Jews on the street.'  trump is unfit to be president.
\item ...and what about the Holocaust ?...'the PAST is the PAST. It's time to move over' Tell that to the Jew community and see 'the avalanche' of commentators you'll get!
\item Answers needed from the G \& MFor twice endorsing these turkeys.
\item excellent. I have a moral objection to hiring straight people and Christians. Time for them to go!
\item And you progressives equate Catholic social teaching with the evil systems of socialism and communism. Political conservatives (capitalists) have been improving the lot of mankind for centuries whereas socialism has usually brought poverty and enslavement in its wake.
\item Expect more trade deals like this in the future. Even expect one day we'll have a North American currency!
\item Some post Christian rubbish.
\item Evangelicals are the most gullible people in the country. They fell for extreme religion, lies, and will send their last penny to their millionaire preacher.
\item Do you deny the white supremacists want to be rid of anyone not just like them, and that they believe the deaths of Jews, Blacks, and Latinos would be just fine?
\item The NY Times has a history of being anti-Jewish and anti Israel.
\item Is it kosher to say I find the entire transgender thing slightly creepy?   But, hey, folks, you've been asking for social equality for decades. You got it.   What more can you possibly ask for?
\item Oh great, now we have a Toronto-based illustrator and textile designer telling Canada's snowboarding drama teacher Facebook Prime Minister Robin Hood how to run the immigration system.
\item Tory takes the subway to work- (but he gets there early- unlike the last one)
\item Assisted suicide ought to bring into sharp focus societies' role ensuring that all that can be done is done for the living protecting the sanctity of life.
\item Tarsand reveals no compassion for his fellow Canadians who have/ are suffering from a natural disaster... let's hope that a really big natural disaster visits Tarsand and loved ones.
\item Turns out that Milo fellow all the Republicans were falling all over themselves to defend is a straight up Jew hating foreign Nazi like the ones whose butts were kicked by our military in WWII.
\item In transgender, why do we assume the brain is right and the body is wrong?
\item St Paul was 'ex-gay'? That might be illuminating.
\item Because there's no cheating in the Olympics already. It's the transgender people who will start the cheating in the Olympics. OK.
\item I’m trying to imagine you with a personality.
\item All Muslims must take responsibility for the killings in Quebec. Ti was  for your  religion  these  murders happened and it is your religion that must change.
\item 100 million poor angry religious freaks.....this is going to end badly, IMO.
\item Yeah. Remember that Jesus told us 'Love your neighbor as yourself. Unless, of course, if your neighbor is gay; him you shall reject as intrinsically disordered.'
\item Then stop firing gays who marry. That is 'malice in action'.
\item Mucky wants a gay parade at every meeting in the country, eh,Muck?
\item Dear Ms. Wente, thank you for shining a light on the teachers' unions, and public sector unions in general. I wholeheartedly agree with everything you had to say.
\item If we spent more time looking after each other, we wouldn?t have to go to the government for support.'Excuse me mister Manning, 'we' is the government. Havent u noticed. Or it should be.
\item As opposed to so-called 'Christian' imperialists who murder millions 365 days a year.
\item That's just a silly statement in the face of the retreat of glaciers everywhere on this and other continents, brissy. But you don't 'do' google, right ?
\item RadirD, 'the agenda'?  To which right-wing conspiracy theory are you referencing?  The 'Deep State', the totalitarian 'New World Order', the 'North American Union', perhaps 'The Homosexual Agenda' or the overlords of the 'Liberal Mainstream Media' had something to do with this?
\item I love that people who have never studied journalism claim to know everything that’s wrong and how to fix it
\item However, he ( secretary of the bishops justice and peace commission) said that the Indian police, too, were at fault, because Islam had entered India without valid documents.'   Interesting tidbit. Hmmmmm.
\item Antisemitism suffers from the  same problem as this proposed law. Criticism of Israeli policies is not criticism of judaism.  All jews are evil = anti-semitism Israel,has engaged in illegal occupations = not anti-semitism
\item If Duffy can bring down the Harper regime, then in spite of his faults and errors, he would deserve a statue in Ottawa. It could go in the place of the ugly monument the Harper gang has planned.
\item The hypocrisy is worse if what your saying is true. Democrat Christians allow God to be removed from the platform in the name of politics.
\item Case in point: the person who equated a scarf-wearing muslim woman to a terrorist.' And who did that?
\item Palestinians may indeed defend themselves. Until they are serious about ending the rocket terror and their claim to the land from river to the sea, however, they will remain undeserving of the right of living in peace
\item That's funny.  Elsewhere the poster to whom you were responding claimed that 'quell' was a word used by anti muslim trolls.
\item I haven't mocked Mary.  The Church made up a bunch of falsehoods about her that reflected not her life and her sacrifice, but their own personal issues with women.  Aquinas, for example, believed women, which would include Mary, were malformed men.  How's that for mockery?
\item Rockin. You are losing on points so I'm a racist. Good argument.
\item Jim Jenkins, for a party that supported slavery, segregation, lynching, Jim Crow, and the current Jew-hating, anti-Semitic, anti-Asian left-wing Black Left....you sure have a big mouth.
\item Did he then stuff the transgender's penis after castration in the transgender woman's mouth with the head sticking out?
\item So brave of those who feel Bourque deserves another trial. I wonder how you would feel if you would lose a family member of your families. You would not give a damn about him of that I am sure.
\item Islamophobia to Muslims is anything that denies or resists the supremacy of Islam. Islam means 'submission' and not to submit to Allah is Islamophobic.
\item You just do not get it, dave. It is our right to democratic expression being tampered with and then controlled by exclusion.
\item Yay Alceste! Way to go!  Of course, some religions in Canada do warrant support because their adherents are less empowered in Canadian society. Thus, we as Canadians must do more to make those faiths more welcome than, say, tired, antiquated Christianity.
\item ....if only they could, but why would they when welfare (aka dumb canuck christians paying their \$\$!)
\item Would love to hear someone say they are sorry for all the Iraqi and Afghani families that have been butchered. Oh, I forgot ... U.S. lives are worth more.
\item you are so na?ve.
\item Isn't that the definition of the transexual  tribe? What is the address of this so called community?
\item this article reads like an entry in a political-junky teenager's diary. love the part about the evil Jews, too. THAT wasn't predictable at all, was it?
\item You may well think that but it's not Catholicism. The Commandments are not guidelines or ideals to be aimed for. And it's the deposit of faith these Cardinals are defending. Conscience isn't 'supreme'; the Truth is. Not even Pope Francis is teaching that.
\item You do realize that Iran and Russia are allies, right?.... and that ISIS is Sunni muslim and one of its top goals is to eradicate Shia muslims (which the ruling group in Iran)? ISIS and Iran are sworn enemies.   Educate yourself!
\item Are you aware that is illegal in most EU countries to mention the ethnicity of the subject on the arrest report or incident report?  Rapes are up dramatically, mostly by Muslim men.  But it's politically incorrect to say so.
\item Canadians don't want a lisping prime minister who's probably bisexual.
\item As this nation has gone way right of center in the GOP there is nothing worse than a Christian on a 'mission' and I don't mean Africa, I mean to serve as a US Politician.
\item One must remember that arrogant condescension and proselytizing is what has given fundamentalists and evangelicals a VERY BAD NAME.  One can't preach/practice bigotry and call themselves a Christian.  That's called being a hypocrite.
\item I respect your right to have a different opinion.
\item Better he survived to deprive him of his vestal virgins in Islamic heaven.  Let rot in the calaboose!
\item Serafim Saovskii, your hatred of Jews has evolved over time in its manifestations and disguises and one can see all three forms in abundance here. Read some history and maybe you'll understand a thing or two about reality. Your antisemitism is disgusting.
\item Tell that to all the children beaten by nuns im covent run schools a orphanages over the past 2000 years if the christian sects.  Women who beat children into submission....
\item Dear AlbertansYes, we feel your pain, and wish you well. Remember, misery never lasts for ever. This Easterner will never say ?let those western baaastards freeze in winter?. You are valuable to us in good times and bad. Get well soon. Best wishes.
\item Skeexix, Kinda like the TRANS people who mutilate their bodies..............
\item secularism is also an American concept. Sometimes we can learn from them
\item Motely, your recent cheap shots on gay people contain outrageous lies, misinformation, and zero evidence. You've convinced me to add another description to the growing List of Your Character Flaws - Racist, Misogynist, and now Extreme Homophobe
\item You can't mention Sharia law or you will get your account deleted.  People don't want to know that female genital mutilation, misogyny, and throwing gays off buildings exist under Sharia law.  It dispels the myth of multicultualism.
\item But you believe a few deranged Muslims represent the remaining 1.7 billion?
\item Interesting correlation, gay men and divorcees.  It kinda pains me to ask, but would you mind explaining that one?
\item The adamant atheist is no better than the fanatically religious. They both claim to just know.
\item Oh yes More Gun control is the answer right? I know we forgot that the Gun drove itself to the scene and met the shooter there.
\item Good point - but not so easy to do if you are an Anglophone in Quebec.....
\item I always find it amusing that non Christians are the first to demonize Christians.
\item Bathroom Bills' Pit Transgender Texans Against GOP  https://www.texastribune.org/2015/04/04/bathroom-bills-pit-transgender-community-against-g/  Get Ready for the Conservative Assault on Where Transgender Americans Pee  http://www.motherjones.com/politics/2015/03/transgender-bathroom-discrimination-bills   The growing trend of transgender ‘bathroom bully’ bills  http://america.aljazeera.com/articles/2015/4/1/transgender-bathroom-bills-are-a-statewide-trend.html
\item I hope everyone can find a home in the RCC.  They should also thoroughly understand the Church's teachings against sin, including homosexual behavior.
\item If all the left has to offer are homophobic and misogynistic attacks on Leitch, she needs to be very careful.  A protest banner will soon lead to possible hate crimes from this bunch of left wing deplorables.
\item The medical cost argument is just a distraction. DTs base followers just hate transgendered people and they don't care what the reason is as long as their hatred is somehow legitimized.
\item Cheetolini wants to ignore his duties, and is a racist pig.  Plain and simple.  He can't fake care like he does when he fake prays and gullible blind American 'christians' gobble it up.
\item I can't imagine a biological woman who is trans-gendering to a man feeling safe in some men's bathrooms...more potential for problems and don't we have enough of those already.
\item Poor baby. Those Kardashians have it so rough. Pretty soon Kanye will be announcing he is transgendered just to get attention.
\item Who else expects this to be the work the seventh century death cult known as Islam! Brotherhood of peace and love!
\item Nothing like starting the car and throw into gear right away at -20, this should do wonders to the tranny and engine.
\item Welcome to the 2000s. We will legislate to protect the stupid, instead of letting the stupid face consequences of their actions.
\item If their deeds do not match their words, their deeds show us who these hierarchs really are. They are not serious about dealing with the evil pedophile scandal. This is another reason why a future iteration of  Catholic Christianity will be one without  clergy.
\item Um liberal lies ... White extremists have killed twice as many U.S. citizens on American soil than Islamic extremists have. I wouldn't call it a 'liberal lie' either. When it's a documented statistic, it's just a fact. Please educate yourself, then you might actually contribute to society.
\item Pope F. certainly is not a pope to resolve clergy sex abuse of children in CI (Catholic Institutional)  church! Rather, he will help close down CI church! At this point, it will be better if he will do his job sooner rather then later, so people can start a new!
\item Oh please, 'Jews will not replace us' is false news. Listen to the audio, and then remove the pacifier.
\item Ah yes !! The G \& M elite's version of 'freedom of opinion'. Just a FEW times for moi as well !!
\item There is no freedom to dissent from church teaching on abortion, contraception, gay marriage, divorce and remarriage, sex outside of marriage, women's ordination, etc.'  Really, F.C?  So it is only the pelvic issues that really matter?  That explains plenty about the nature of your posts.
\item Transgender soldiers can kill just as efficiently as straight soldiers.
\item Just like your election of Trump explains the sharp rise in hate crimes against minorities, women, gay people, Dems, liberals and immigrants post-election.
\item I wish we could deport American Catholics who play censor on comboxes.     Censoring comments because you disagree with them....how incredibly lame.
\item You ignored skyofblue's point: that the groundwork for the now-accepted notion that every person has intrinsic worth and dignity was set by religious folks. The fact that Church hierarchy worked hand in hand with kings is another matter completely.
\item Overwhelmingly calls itself Christian.
\item LOL...yeah...you're right...there IS no swamp, North Korea is NOT a threat, Iran is NOT a threat, moslem terrorists are NOT islamic terrorists, the list goes on..... nice comeback.
\item Meanwhile back at the Ranch Wynne and Justin are stressing more diversity and the tricky subject of public washrooms (transgender issue).  Stay tuned!!!!!!!
\item And The Republicans have funnelled the \$ to their friends. With The Tea Party saying it's not enough ...A down turn and the cupboard is bare. Definately 'World Class' in the current political environment.
\item how many internationally famous musicians (violinist, pianists...)are jewishthey must be doing something right
\item You have absolutely no evidence that mortgage fraud is THRIVING in Canada. You have anecdotal evidence and even that is flimsy. It just a nice story that brings some drama to the business page. Not very responsible reporting if you ask me.
\item Again, your whinge is 'gay sex is icky'.
\item And remember, both ABC and WaPo are zealous Hillary supporters.
\item Why should I care that believers speak 'blithely' about there being a god? What does it matter? They can believe that to their dying day if they want -- and proclaim it -- and the rest of us will get on with our lives..
\item Calling yourself a patriot and talking like you do is mimicking Rush Limbaugh. Does not put you in a good light.
\item What a nice guy, how thoughtful of him! Lets go bigger, lets give him the Nobel Peace Prize.
\item People who have questioned Islam have been killed for it.
\item I think they do co-exist peacefully. It's other Catholics who seem to think it's any of their business that seem to be the problem.
\item Go to a volunteer force that are called in for bonafide fires while a core of say 4 professionals 2, 12 hour shifts to avoid the sleeping, who will respond to the medical emergencies and fire rescues. It would save millions and be as effective.
\item God Bless the Kid. Our nation was founded by young hardcore asskickers. Not liberal transgender pussies.
\item they tend to obsess over what we do so much, it is all in their heads.  they are the ones thinking about it over and over and over again.  way much more than we gay people do.
\item Anything I have commented on I have seen first hand. For the record my respect is earned... No doubt a foreign concept to a second nations supporter.
\item You and pretty much every person that is in favor of the baker discrimination do not get it. Political thought is not protected. In Colorado sexual orientation is protected.   Bottom line? You do not have to make a cake for a democrat. You have to make a cake for a gay person.
\item Yes...that explains why they are killing each other. I know if we in Canada were attacked, the firat thing I would do is kill my Catholic neighour. NOT!!!
\item Organize like the LGBTs did!? Are you serious? That's your best example? How about organized groups like Republicans for Trump, the KKK, Westboro Baptist Church and Anchorage Baptist Temple? Those groups are the ones I fear because they're hate-driven, not gay people.
\item Unless I am 'cis' and I have low T ....then I have no way to be competitive.   Why can't everyone raise their testosterone to a pre-agreed level?   . transgendered athletes are allowed to raise their testosterone - why not everyone?
\item Yes, there is no question that modern Muslim advances in the sciences have been suppressed and ignored by the racist Nobel committee.  To set the record straight I am including an exhaustive list of those breakthroughs below:
\item Of course you can, but know that in doing so you reveal your own personal obsession with the anus.  Are you gay?
\item Monica, there is an excellent treatise on sex written by two  non-clerical theologians: 'THE SEXUAL PERSON: Toward a Renewed Catholic Anthropology' by Todd Salzman and Michael Lawler. 'In short, say Salzman and Lawler: emphasize relationships, not acts, and recognize Christianity's historically and culturally conditioned understanding of human sexuality.' http://press.georgetown.edu/book/georgetown/sexual-person
\item Palestinians wanting peace? That's like ISIS wanting peace. Their resistance is in the toilet. Just look at their surroundings and what their resistance has achieved. Rubble and squalor.
\item Ascalepius, I doubt it. Hahahhahahahahhaaaaaaaaaaaaaa.
\item Sorry about not saying Islam is in no conceivable way involved in these murders.
\item St. Augustine has certainly messed things up regarding sexuality. Abortion is faced in the Catholic Church BECAUSE sex is ONLY for procreation!'  The better/best outcome of “sex” is “procreation” of life. Or, would you say it is not?
\item Lesbian nuns arise! Demand equal mistreatment, now!!!
\item Islam is not compatible with dutch values and i am pretty sure the dutch do not want to convert. It is all or nothing for the muslims and they will not stop until they have it all.  The elites refuse to except that reality.
\item Bottom line here:  Islam isn't trusted, so a Muslim-only cemetery is suspect.  No explanation needed for this lack of trust.  Most people know the 'why'.
\item Great?  2 homosexual males using surrogate mother(2) produce another homosexual male or lesbian or more homosexual males and/or lesbians.
\item Because it's impossible to align a transgendered individual's mind with their body.  Male and female brains are different - they're composed of different types of cells and they think with different parts of the brain.
\item Tell someone who cares Save Trudeau
\item i don't need your 'compassion,' thanks.
\item The idea of a homosexual orientation (as opposed to heterosexual men indulging in same-sex 'acts') is surprisingly modern, is it not?
\item LMAO! The Alberta Party is a bunch of extreme left-wing nutjobs. No one credible would ever associate themselves with collection of clowns.
\item Jews are scared because the terrorists lobbing bombs and launching rockets on Israel, are gaining ground in Europe.
\item Joanne... since you are a believer, what on earth are you doing using a computer? Turn it off and save the planet!
\item If you knew anything about the Bible you wouldn't make such a foolish statement.
\item What about christians sending drones to kill extra-judicially, with various collateral damage?  Or how about Sammy Yatim and others like him?
\item It was not a Sig Sauer Platform, it was a Sig Sauer MCX rifle. If people are going to discuss something, having the correct facts are a necessity... BTW...aren't pedantic people annoying ;-)
\item Change the childs mind about what? Being LGBTQ? Or just thinking that LGBTQ people don't deserve to be treated any differently than anyone else? And what 'real issues' are you referring to? There is nothing not 'real' about being LGBTQ.   Spare us your veiled homophobia.
\item It still seems to come down to dislike/hatred of Jews; not much has changed in Europe and it is the same here in Canada.  And the comments here are the nicer ones that have not been blocked by the Globe's civility policy.
\item Saudi Arabia is going to execute a man for being an atheist.  We don't need more 'Muslim values' like these here in Canada.
\item This is the second terrorist bomb to be set off in Manchester in recent years. If memory serves, the last one was set off by Catholics.
\item In other words: He's not gay!  Right?
\item Muslims are the ones who suffered this particular terrorist attack.  Six were shot to death by two gunmen while they were praying.  You should perhaps consider reading more than just the title of a news article.
\item You need a citation to a source that supports your very specific claim, that liberals (as a whole) like/love (whatever) ALL Muslims and that ALL Muslims treat women as property. Good luck!
\item Let's not forget that other adorable example of good Christianity, the Salem Witch Trials. Let's hang 'em in the name of God!
\item Oh Boo hoo, if we sound like armed hoodlums, it comes from a Place of Pain. Get yer hankies out, Albertie is a-whining again. I'm surprised they don't blame Jewish Bankers and the Masonic Lodge.
\item Thank you Konrad for an insightful article. Greece and Greeks, with their congenital hubris, are always quick to point the finger of blame at others.
\item Yes, time to move forward, respect right and the rule of law, not try to enforce a monoculture on other people.
\item Now we just need gay orgs to take responsibility for the fact that 4 out 5 church abuse cases were the work of gay priests abusing boys.  I call that fair play and honesty.
\item It's hard, well perhaps not so hard to humiliate a Jew hater. It comes with their mother's milk and their narrow education, and only serves to reinforce Israel's need for a Jewish state and minimizing the prospects of a terrorist state on its border.
\item Don't worry, this Catholic Institution will be dismantled before all other changes!!! You don't graft a new branch to a dead rootstock!
\item Mrs Gagnon never used the word ?madness? in her article in La Presse. Shame on the G\&M!
\item It's rich for a Muslim to call sovereignty a hate crime.  Muslims don't integrate well as seen in Europe. Why? They dont respect national sovereignty.
\item Transgender ban in service bad idea, say former brass' -  BUT 'Transgender ban in service bad idea, says former Enlisted Man, NCO'. Who Can You Trust?? Will a confused person make great Defense decisions, Not in my Book!
\item Dear Western Society: Hosea 8:7
\item Are you implying that it's appropriate that Muslims should be targeted in the USA because non-Muslims have difficulty practising their faiths in Muslim countries?
\item That any Catholic, Christian, or American would consider voting for a racist demagogue like Trump is shameful.
\item I would love to see you stand in the face of a transgender person and compare something as inmate as their identity  to having psoriasis or being overweight.  I could further pick apart your analogy but it's really not necessary because it's ridiculous.
\item Why did the music 'badly need change after VII'? Why is that? Just for the sake of change? Why should any Catholic Church ever allow something out of schismatic Taize to be heard within its walls?
\item Yes, I do have a question, franco prairie.  You call Justin Trudeau 'gender fluid.'  That sounds homophobic to me.  Can you explain it?
\item With 325,886, 603 people in the US (three seconds ago) and 'One birth every 8 seconds and One death every 11 seconds', one 'transgender' critter more or less is really irrelevant!  https://www.census.gov/popclock/
\item Ivanka, Donald Jr. and Eric have all married into the Jewish community.    All of Trump's grandchildren are Jewish.  Everything he has done so far has been self serving, why end at religious intolerance and bigotry?
\item It's cute when you try and do man things.
\item Trudeau much prefers the Muslims-as-victims narrative.  Indeed, his response after Muslim attacks has been to preach 'Don't blame all Muslims for the acts of a few'.
\item Mormons cannot possibly be gay.  We just can't have this, and that's the end of that.  /s
\item The Mormon  church is making itself obsolete. In the long run. This issue may cause a cysm in the church. Once side will accept homosexual and prosper. The other will die. Isn't this what the Bible says happens to sinners?
\item Imagine President Hillary, Commander in Chief of our transgender military, dealing with North Korea's nuclear ambitions. She might be selling us out to the Chinese for campaign cash for her 2nd term election, Yeah..she's that evil and power hungry. Thank God she lost.
\item Amy Demboski, your neighbors might be having gay sex. shouldn't you be putting a stop to that? thanks Eagle River, you're the deep south of Anchorage. the toothless inbred deep south.
\item I totally disagree with this editorial....looking after one's interest is not provincialism-whatever that means- it is realism
\item Absolutely so!  However, a transgirl is entirely different from your son.  Transgirls are insistent, persistent and consistent about their gender identity.  It is NOT a preference or a like for 'pretty things'.
\item It's not the politician's fault. We get the government we deserve since so many of us can't even be bothered to vote. Seems greed and looking out for your own self-interest is all that matters to a lot of voters. Sad, very sad.
\item Heck ya man! We gotta organize man, we do!! Lets get on board the CRUSH CRUSH CRUSH Truck! Honk ! Honk! Join our non-partisan facebook page Canadians Rallying to Unseat Stephen Harper. Toot! Toot!
\item The mayor's cooking the books is no surprise, he has lied his entire life about everything else so nothing new here, more people and institutions need to take this loser to task.
\item Just leave and go on with your life dude, wtf
\item Why the hell do Muslims want to come to Canada if we are such a despicable bunch of racist kurrs?  Oh but they forgive us and try to accept us.   How magnanimous.  How much of their objection to us is just taqiyya?
\item Errors on the part of individual priests' ignorance or poor judgment cannot be imputed to the Church's teaching or to Christ's divine command.
\item I've never noticed that kindergartners have (trans) gender hang-ups. If they do though, don't worry, they'll likely outgrow it once they've moved beyond functional illiteracy. How's that going for you, 4:20?
\item I'm not sure sending a Jewish guy to solve the ME problem is a good idea. Is that really going to be well received by the Palestinian side?
\item In 1944 18 year olds stormed the beaches of Normandy in the face of certain death to free Europe. In 2016 18 year olds need a safe place to protect themselves from getting their feelings hurt.
\item If you need to claim you're world class - you're not. Toronto pols haven't figured that out.
\item A gay person who supports Trump?  Oh, I forgot.  There's also that Milo guy.  The basket overflows.
\item  'Patriot'? What does that mean? '  'The ownership disqualifies it...' is what answers that. Levant is Jewish and 'patriot' is code for neo-nazi et al.
\item Utter nonsense. Only the religious ignore overwhelming evidence of the absurdity of their beliefs yet pride themselves on their blind faith.
\item so you read the contract or do you just make excuses for the sunny ways Justin?? He does have nice hair so I get your attraction to him but try to think on your own
\item If they're silent, they're not giving scandal, are they?  But that really wasn't your point.  I think you just wanted to remark that some priests and religious might be gay...  ..and being gay, of course (although you neglect to mention it) is NOT reason to deny a public funeral.
\item Nepotism, you think?  But his appointment would qualify as diversity since a lot of Trump's supporters do not consider Jews as white.
\item This is the new age Canada now, workers rights have been eroding rapidly.  Consider having a sex change, claim to be homosexual/lesbian or develop some deviant mental disorder if you want any type of workplace protection - sorry folks, I'm dead serious on this one.
\item Never read in any newspaper of a pervert dressing like a transgender and going into a bathroom for the purpose of molesting someone.  Most parents escort their child into the bathroom.
\item Islamic radicals, like mad dogs, bite themselves, along with everyone \& everything else.
\item ... liberals gently neighing as they seek to tax hard working Americans in order to pay for the sex change operations of transgender jihadists ... '   OMG, SD - please don't give them any ideas!!  =:-o
\item Fr. Martin is becoming Moses-like.  Pinning the snake of homosexuality and mounting it high on a pole.  Bringing it out of the darkness of unconscious fear.
\item Of course transgendered people could be a risk, as could anybody else.  Ask Edward Snowdon.   Linking sex to military security in the modern age is a huge stretch.  Blackmail is no longer particularly effective.
\item it is more a case of law in muslim countries.  Women cannot say anything about any man,  let alone the leader.  Get used to it. The ideology is marching unopposed.
\item I should add that I think it's immoral and a scandal to pressure homosexuals into pseudo-heterosexuality.
\item I'm more worried about my child sitting on a soiled (urine, feces, blood, etc) toilet seat than of a transgender person occupying same bathroom. Please get over yourselves.
\item Especially if that joy includes living your parent's basement. But then on the bright side, maybe their parents will have someone there to help them in their old age, although I wouldn't bet on it.
\item Go to a Muslim country and that's exactly what they do and they do it in public. Or if you are lucky they chop off your hand.
\item the hypocracy of the LGBT... advocates at womens shelters and related organizations who refuse to accept trannies born as males. apparantly only the trannies born as females get their (our)  financial and emotional support
\item And comes now Donald Trump being welcomed by major evangelicals of America, most if not all racists themselves, some even member of the Ku Klux Klan, to embrace and cheer each other on. Holy cow!
\item quiet honey, the men are talking
\item What would happen if the U.S.A. simply backed out and let the Palestinians, other Muslims and Israel sort out their problems?   Why does the U.S. government think it has to support Israel?  Why does the U.S. government think it's so important  to support Israel?
\item Easy! Get rid of the snowflake socialist stooges that whine about everything, and make little puddles on the ground when things don't go their way.
\item Ezra is an insecure, self-hating, Jew.  He looks for acceptance amongst the worst of society.  His heritage means nothing to him.  Most Jews have disowned him.
\item Allie, the transgender troops who served America well did so as men and women consistent with their sex at birth.   Allowing them to now serve in the sex with which they identify is beyond insane.  It is liberalism run amok.
\item The solution is simple. Open your eyes and your heart. It is not so hard as you think...
\item Dalton McGuinty was a puppet of the teacher's unions.
\item Yes of course. But will the natives actually give the AFN the authority to make binding agreements with the Feds ??? Not too likely !!! Therefore more of the same unending bullcrap forever.
\item Interesting take. I'm sure you won't have a problem with US track and field sprint/power events being taken over by trans women, then?
\item really, truly desperate. sad.
\item So trans-gendered people cannot defend the US and fight? Used to say that about black people and women. Discrimination is discrimination.
\item I don't feel like he represents me. He won't condemn those groups specifically, yet he has no trouble condemning foreign terrorists, undocumented workers, and Islamic terrorists. So no, he most certainly does NOT 'represent all Americans.'
\item The U.S armed Islamic psychopaths in Afghanistan during the 80's to fight Russia.  The U.S arms Islamic psychopaths in Syria during this war to fight Russia.  Nothing much has changed....
\item Especially the United Way and it's member agencies!
\item I am ashamed to be a Catholic today with this social activism gone wild.
\item Here is a thoughtful critique of the TV show in question from a trans blogger: https://sexdrugsmh.wordpress.com/2017/01/13/thoughts-on-transgender-kids-who-knows-best/
\item When the commander-in-chief says:  'After consultation with my Generals and military experts please be advised that the United States Government will not accept or allow Transgender individuals to serve in any capacity in the U.S. Military' - I believe that technically makes the President himself the credible source.
\item We agree then.   Although Trump says he is a Christian -he is far from it -  just another lie from the bully.
\item So Comrade, I guess you haven't heard about breitbart trying to boycott Kellogg's? Or RWNJ's boycotting Starbucks because their cups are christmasy enough? Or millionmoms boycotting Target, Penney's et al for not discriminating against gays? Yeah, it's just liberals.
\item You forgot gettingvthe sisters back into habits, getting sent to hell for a hot dog on Friday and all Catholics wearing at least one scapular 24/7.  Oh, and getting rid of girl altar boys.
\item When someone, especially an elected official uses their power to cause personal unrest to another individual or population by accusing them of being linked to Muslim terrorists, you've lost your right to free speech.  How's it feel to have your pants on backwards?
\item And furthermore, Jesus may have been dogmatic, particularly regarding hypocrites, but he never said a single world about homosexuality. Not. One. Word.
\item Free enterprise will always be with us
\item But...but...but...they are closed on Sundays and protest gay marriage.  They must wallow in morality!  This is surely a mistake.
\item Typical of Ms Wente....just pick the data that supports her point and don't bother doing any more research or analytical work than she has to.
\item I really hope you're right! I'm not a tech idiot, but this situation is making me feel pretty vulnerable.
\item Christ the Lord is risen again, hallelujah......'  Oh look!  Plastic eggs from a helicopter!!!!  He is risen!
\item The league is asleep at the wheel. Either way, this was going to end up in court, so instead of having to deal with controversial transgender politics, they should have simply disqualified Beggs on the basis of her/him using a banned performance-enhancing substance.
\item A lot of other people are also being massacred in the Middle East. They are called Muslims.
\item Plenty of white anglo saxon born again narrow-minded judgemental bigoted Christians have had their educations paid for by the same over-privileged white people. Stop whining and learn to be the tolerant civic-minded person this country is so proud of.
\item We need a politician like Donald Trump , who says what most people are thinking
\item ,,I take,, it you,, are a,,,Trump,,,supporter?!?
\item You were just as much as females who couldn't become firefighters because of the physical requirements.
\item The question should be is our military stronger or weaker with transgender recruits.  I vote weaker.
\item @Tron4000-  Yea people don't change after 40 years... Hillary opposed gay marriage for decades.  Chances are there was some point in your life when you used to call someone a 'fag'... by your logic you're homophobic.
\item Ah yes, the liberal architects of the oil war in Afghanistan, security certificates, Maher Arar, torture, rendition, etc... How nice, they have something to say on how not to do it.
\item Nothing ironic about it at all.  They hate everyone who isn't a greedy, lying, white Christian, old man.  They have never had and morals or values since day one.
\item They were chanting 'Jews will not replace us,' not 'You will not replace us.' Apart from the odious political message, I find the thought of being in a big, sweaty man-crush quite repellent.
\item Not sure if you're willfully blind to your attitude, or if you really don't know what condescension means.
\item I've had several people tell me they think Mike Pence is gay, although my gaydar never even wiggles when I see the man.  If gay, he must hate himself an awful lot.  Even more than Ted Haggard.
\item Trump is most likely homophobic due to a deep-seated embarrassment over his longtime homosexual relationship with his gay mentor Roy Cohen...
\item how many relatives have you lost to Nazi ? What the f... wrong with you ? How the hell you can compare Donald to Adolf ? Did he kill millions of Jews, Poles or Russian ?
\item So Hitler was anti jew because he left alone 50 percent of the Jewish people in the world? The KKK isn't racist because they leave black people in Africa alone? You have a high bar for discrimination.
\item Well, considering that her party hates Jewish people, she fits right in.
\item Good for them!  Thank you for being there, ladies.  Pence is a conservative Christian prig who likes nothing better than “keeping them barefoot and pregnant in the kitchen.”  Save us should the likes of him become President.....
\item That would be apostasy to question Islam,  and they would kill her  if she did that.
\item If it walks like a duck, quacks like a duck, chances are it’s a duck
\item every day now another puff piece of muslims
\item Noone cares what you think
\item The governing association got that part right but failed to realize that these transgenders are taking steroids to accomadate their sex change which also gives them a physical advantage. By not disqualifying herself this girl was basically cheating and being unethical.
\item Jews willnot replace us.'
\item YOU NEVER USE GOOGLE EARTH? DON'T USE GOOGLE. I GET ADS FOR TRIPS TO CUBA ALL THE TIME. AND OLD AGE HOMES. SO WHAT? YOU WANT THE INTERNET TO COST NOTHING? THERE MUST BE ADS.
\item I dont get it.  To date, all Israeli Jews; black/brown/white/Sephardi/Ashkenazi share a single space with separation between the sexes.  What rationale is there to demand being different and have a separate section for anyone or anything?
\item You obviously don't actually know any real liberals.
\item Pifco, You're so gallant, you'd look good even in a straight jacket.
\item It would seem that Globe readers - from reading this response to Doug's story - are the most easily misled on the planet.
\item Here ya go Paul...   Watch ''Jews Will Not Replace Us' in Charlottesville' on YouTube https://youtu.be/n12sjwk9FBE
\item Reagan wasn't arguing for an absence of government - but the belief by the left that the government should control every aspect of your life.
\item Every time I see those drama Queen adds of Justin. I send money to the Conservatives. Good job Conservatives, keep showing us how shallow Justin really is.
\item The Christian right should be up in arms, but they already made their deal with the devil...
\item Sure 90\% of Muslims will be patriotic when we are re-writing our laws to accommodate a 1\% minority! We treat them like Gods while ignoring the truth about Islam, we whitewash the reality of their religious text and their goals in our society.
\item I didn't see any females at any of our the Pride parades wearing a hijab, niqab or burqa.'  And none of the drag queen queens either, presumably. Clearly, the gay community hasn't adopted a diversity approach.
\item I wonder how many taxpayers know they paid for the tranny surgery because this little brat started a hunger strike and only would stop if they paid. What a real american!!
\item I'm 'avoiding facing the truth'. Someday, people like me will be assembled in stadia to face the truth in great climate change rallies. There, Truth will be presented on a very large screen while we hail those who have saved the planet.
\item The Harper Conservatives' hatred of muslims has lead us to this sorry state. Would have been no need for this large payout had Khadr been repatriated years ago.
\item If he is an example of what it means to be a 'recovering homosexual' (whatever that means. Can one be a recovering heterosexual?), then I am pleased to be a very proud UNrecovered gay man!!!
\item John are you suggesting that this government treats the opposition with such respect? Or ever would?
\item Trid, Many Muslims state that those who state that they are killing in the name of religion are using religion as a shield, not acting in the name of Islam.
\item If one can 'pray the gay away', then any sad cleric should be a few 'Our Father's and 'Hail Mary's away from bliss...
\item Hamas' founding charter calls for the annihilation of the Jewish State. Abbas has no control over them whatsoever. Negotiating with him is a fool's errand.
\item Kill urself
\item I'm an atheist and an anti-monarchist immigrant Canadian. I guess you think I shouldn't be here.
\item The BDS movement and the anti-Israel propaganda disseminated on our country's university campuses has unleashed the worst in people on the political left. The anti-Jewish bigots of the left feel emboldened as they hide behind the billowing skirts of Auntie-Semitism.
\item Ho hum.  Muslims being Muslims.  How boring. Tell me. Has there anything positive ever come out of Islam?
\item > If the Holy Spirit has been so assiduous in guiding the Church, then either the Holy Spirit is really bad at it or else has a very nasty sense of humor.  Please give an instance in which the Holy Spirit has lead the Church astray.
\item Jeez, you guys truly are delusional. The Republicans are rabidly antigay...whether it's passing  laws to allow discrimination against gays on religious grounds or telling them what they aren't allowed to do with their genitals.
\item Accurate headline, Yes they are up against the same obstacle - Catholicism!
\item And what is fair share? Who are you to tell others what is fair and what is not? Typical liberal.
\item Yes, the United Nations. Nothing more than an unelected world governing body that should have been abolished before it was ever born.
\item This sort of thing is precisely so many Canadians don;t want more immigration from Islamic countries.  We will be importing to Canada  our own destruction
\item So you approve of homophobia, dishonesty and misogyny in the Catholic Church, and this is what the people who run should be standing for? You think that 'pray, pay and obey' is the sole job of the laity?
\item It isn't illegal for an 18 year old to have sex with a seventeen year old' LOL. Good luck convincing a judge of that. In California, where the offense in question took place, the legal age of consent is 18.
\item Demographics would like to differ and tv ratings. Majority of blacks, Chinese, Jews and Flippinos prefer Basketball. These groups combined together represent a powerful force in demographics and  finance.
\item According to Trump's logic, blacks should share the blame for slavery, Jews should take responsibility for the holocaust and the protesters who were run over by the vehicle are guilty of damaging the car.
\item No, I'm showing the weakness of your position. You know that to argue against the transabled mutilating their bodies is to argue against the transgendered doing the same thing.
\item Do you seriously care about the rights of muslim travelers coming to Canada?  Why should anyone feel sorry for them?   Not our fault they live in failed states.
\item Justice, Very well said.
\item gtm, you're completely missing the nuance here... or not.
\item It wasn't mud.  It was aids urine.  Antifa is into some sick satanic stuff.  As far as any feces, its just a jew thing.
\item Mike, you are definitely gay. Face it.
\item So gay CIVIL marriages are not sacramental marriages. So what?
\item The kind sanctioned by my beliefs? Have you grossly misinterpreted something? I believe in monogamy and marriage. I believe in respecting one's spouse/partner, family, neighbor, other people.  I googled 'lesbian murdered bull dyke partner' but couldn't find the story you referenced. Link?
\item And don't forget to visit the gift shop for your asbestos bust of Dear Leader Harper and a glimpse at the \$127 billion deficit! All Hail Harper's Mother, Canada!
\item What a kill joy.  This man isn't a Christian, he's a Grinch.
\item Ok, so we've got Ben Carson masking his white supremacy by pretending to be black, and Ben Shapiro masking his white supremacy by pretending to be Jewish. https://goo.gl/LjQKTS
\item Well said. Ms. Henein is an exemplary professional woman and Canadian citizen.
\item I bet she uses poppers, like all the lesbians do
\item Right on.Free these journalists only doing their job as journalists. But both the Harper and Obama administrations have hailed the Egyptian dictatorship as a 'return to stability'.
\item Right back atcha!  Alinsky tactic...demonize the opposition and accuse that side of exactly what your side is doing.  Obama was great at it...just that most people saw thru it.  Great!  I'm glad you support Christian observances in our schools.  There's hope for us all.
\item There be no time for warning sirens when the Islam/Muslim fanatics steps out of their Trojan Horse and starts the slaughter in the name of Allah! yelling: Allahu Akbar!
\item Bishop Stowe's a nice, but catechetically under-educated man:  the Church, he said, 'has always opposed discrimination of any sort' (against homosexuals). No, Bishop Stowe, it hasn't: it opposes what it calls 'UNJUST' discrimination against LGBT folk. Can you spot the nuance?
\item Of course they do! Catholics like any other religious group have a constitutional right to raise their children in accordance with their respective faith. If you do not think sex as taught in public schools is not based in a particularly ideology, you are not paying attention.
\item No, they just give Islam a pass and they will again for this latest attack carried out in the name of Islam .
\item I don't think hitting yourself on the head with a hammer counts but it might explain the hairdo.
\item ya but how many Gay Parades has Trump been to.
\item Females soldiers do not received tax-payer funded abortions.  Why should transgenders be provided free tax-payer funded sex reassignment surgery and treatment?
\item Joe, your rhetoric is about 30 years behind the times.
\item Author of this hitpiece is a Jew. Enough said.
\item Hey military hater, join up, become a REAL MAN, are you a transgender freak? military does not want you; not sorry.  be quiet............................ :)
\item Sounds like they sold their souls and principles
\item Oh yes, the time of the Crusades was very secular and Democratic!
\item Haint y'all never heard tell of that place called 'Jew York'?  My preacher said hit be plum full of them there Jews!!!!
\item Why not send them to canada ????  And if there are any gays, then even better .................
\item How nice! whiskycharlie crawled out the the cesspool to post.
\item \$84 million on Viagra and Cialis, \$8 miilion on Transgender according to a Rand Corporation study conducted in 2016.
\item We should rid Canada of elections which are basically a referendum of the current government since people are so easily swayed by empty rhetoric, hence we end up with leaders like Trudeau.
\item I must admit that compared to Harper anyone would look very/very good. But, that said, this government is doing very well delivering on their agenda. Now it must push forward aggressively with electoral reform.
\item The. Transgender pervert republicans need to be sent home , replaced immediately !
\item uh... "thoughtful"? when she didn't even bother to read the book?
\item What about the Establishment Clause leads you to think Trump has the constitutional right to ban Muslims? (which is what the order is)
\item Yes. 'Intrinsically disordered' is an insult thrown at gays to prove that the institutional Church has rejected them.
\item This is a day of miracles.  For the first time, I agree with you about something. Aside from being a total sleaze bag and hypocrite, Joel Osteen is a faux Christian. He disgusts me.
\item No I'm only obsessed with the Jewish holocast let's get forget about it  Your a loser  No that's bullying  Go cry baby Go to a real college and gain an intellect
\item Most of what I've seen in OCP's publications is not what I would call .... Music fit for a King.  Exactly who are we trying to please here, yourselves  or the Lord. Garbage, Garbage, Garbage. No wonder Catholics can't  or won't sing.
\item Could Pius XII have done more? Perhaps. He did take action to the Jews of Rome, though he made no public statement.
\item Did I mention that France is one big gun free zone?  Only the police are allowed to have assault type weapons.  Oh, and radical Islamic terrorists.
\item what blows my mind is how black slaves adopted the religion of white European slave owners, and abandoned their African American religion/culture. As the son of a Native American I have been baffled by members of my family who adopted Christianity that tried to genocide Native Americans.
\item These transgender folks have a method to their madness.  They want the government to pay fo their body alteration.  The costs of this type of operation is costly and they feel the tax payers  should pay for it
\item Some Canadian milk producers - you do know that cheese is made with milk ? - are going to be squeezed.. And the Europeans want nothing to do with hormone beef. Strange people over there, eh?
\item Glbalsoul, you need to research Agenda 21 (Sustainable Development) because that's the global geo-strategy you are so misinformed about. I'm willing to bet that your first instinct after this is that I'm a Harper supporter, right? Get informed!
\item Why would anyone be surprised as the recent influx includes many (Peace be upon them) who consider Judaism something to be eliminated? Hint: pay a visit to Paris to get a preview.
\item Since Tennessee is a red state, climate change does not exist there, but Godly punishments do. Gatlinsburg is probably being punished for not hating gays enough. Like New Orleans was with Katrina and NYC was with 9-11. Just Baby Jeebus' way of helping The Donald Make America Straight gain.
\item and your post take first prize for absurdity.
\item Passer - if they have commitment they will become citizens. Simple. You show commitment by becoming a citizen.
\item David-G2-regardless, it's the government that set the rules. There's no way the IESO would want anything to do with pain in the neck solar and wind if it was up to them.
\item Veritates, if you hometown is in Ukraine perhaps you should go over there and do what you feel necessary - dragging Canada into this issue is irresponsible.
\item In some circles, Christianity for example, a death in a dysfunctional society diminishes me as much as a death in a peaceful, prosperous society.
\item I recall Iggy's eloquent dialogue about how the Liberals are like Puffins who clean up after themselves by burying their skat. Harper's pooping puffin hate ad will go down in history along with the Liberals soldiers in the streets classic.
\item Jewish terrorism arose as self-defense against Arab terrorism.
\item If Scaramucci is indeed a good Catholic (Christian), then I must be on the road to sainthood.
\item When are Indians going to join the American Tribe and stop whining about the past? Jews have a similar or worse past yet seek to integrate not segregate themselves.
\item All forms of hate needs to be eliminated. All forms of racism, Islamophobia, Homophobia, anti-semitism and laws discriminating against Transgenders. We need to get behind Justin, Obama, Hillary and Premier Wynne and fight all forms of hate!
\item What is Harper afraid of ? Let the prisoner speak. He was a kid when he killed the American man in military uniform in the heat of battle. They were both enemy combatants.
\item The Bible makes minces no words--slavery is okay, so is stoning homosexuals, and committing genocide. The only false equivalence is your brain.
\item No, republicans are far more likely to cheat, lie and persecute others who aren't white Christian heterosexuals.  Republicans through years of lies are turning this country into a fascist theocracy.
\item Thank you for your very thoughtful and helpful response. I wish you good health and continued support from those who love you. May you find the balance you seek.
\item Why would anyone allow publicly-funded Catholic schools to promulgate  the church’s perverse and dangerous views on sex?
\item With respect and the deepest gratitude I remember and thank those veterans for their sacrifices.
\item I'm trying to figure out how old you are. I mean, I'm not young, attended Catholic school, and all we talked about was sex.
\item And it's not Christian either. Sickening how Trump's phony  'Christians' turn their backs on Christ's teachings.
\item I think both camps have been strengthened. However, I seriously hope it won't go the way like American politics, where you'll have 45\% going very hard one way, 45\% very hard the other way, and 10\% kind of wishy washy.
\item What does this have to do with the corruption talked about in the article?  Are you saying that the entire US Navy has been corrupt since 1967?  Why do you hate Jews because of what President Johnson did?  Was he Jewish?
\item LazeelinkLOL!!!!! is right. Your talking about Executive Orders, I'm talking about Executive Action. There is a HUGE difference!!!!.
\item Sins are sins because they make our lives harder to live, not because they anger God.  They anger God because we are unhappy.  Homosexuality, at least on the male side, is naturally occurring at a stable rate.  The bias toward procreation is idealism, not nature.
\item Trump's election on support from racist and white supremacist feelings, especially among Catholics and Evangelicals is the primary evidence of how far we yet have to go.
\item Drop pot, not bombs! ISIS needs hugs, not bullets! -JT
\item My, my.  I bet you kill other living creatures as well. You're really bloodthirsty. A typical arrogant human predator. The worst of the worst. Hitler used the same 'reasoning,' lies, biases and hate in his quest to eliminate the 'vermin' Jews. You're a lot like him.
\item Agreed. A parade of self-loathing gay people, ephebophiles, gay rights advocates plus MSW and Andrew Sullivan does not an argument make.
\item I agree.  Gay men shouldn't be around children.
\item I agree with the sentiment and the respect shown. And it maybe notable that two of the three national Leaders are Montrealers.
\item Hatred of Muslims  See how easy it is to define?  Easy peezy
\item An Islamist?  What a shock.  I thought it was an American angry white guy.  Our spud Junior has hatched the same future for Canada by allowing in 35,000(!!!) Syrian 'refugees' without proper vetting.
\item No we didn't. A fresh platform, new ideas. The same old same old would be austerity, for instance. Lots of new faces in among the seasoned veterans and an smart, tough, energetic, kind-hearted, optimistic leader who has proven himself truly worthy.
\item The gay men of Toronto had established a good rapport with the cops despite what BLM and the womyn o Pride  say. Many gay guys like the sight of cops in uniforms, even if BLM said it disgusts them.
\item Who cares?  She didn't win because she was transgender, she won because she '...focused on jobs, schools and, with particular fervour, northern Virginia's traffic congestion.'  Politics is a contest of ideas, the best of which have nothing to do with what's between your legs...
\item It is not headscarf.  It is the philosophy of subjugation of women (four wives, genital mutilation, unfair inheritance), hatred against homosexuals, and despising secularism..
\item David Thomson and Galen Weston Sr. And all along we get told by anti-Semites and their ilk that wealth is a  Jewish attribute.
\item Free Speech. No to M-103.  Stop spreading of Islam in Canada. Stop converting Canada into an Islamic country.  Limit Muslim Immigrants into Canada. Limit Mosques in Canada.
\item There is no such thing as transgender! You are either male OR female!  You are born what you are, this transgender stuff is a big lie!
\item What if they gave a war and nobody came?  Cheeto Jesus should invite Lil' Kim for a beer at the White House.
\item Oh and its nice to see that my earlier post calling Yakabuski out for serving up lightweight drivel got censored.
\item Wow, taking the 10 seconds to reply is quite the heroic feat. 
\item The public is stupid. Thank God for leaders we have leaders like Justin Trudeau that can do all the thinkin' fer us.
\item If you believe this girl you are utterly naive.
\item Where are the stories about retail businesses owned by homosexuals(or LGBT)? They have to be raking in the money.
\item No, just Diversity. It's all he thinks about: Diversity, Diversity, Diversity, the answer to everything.
\item Ask the people of Paris who the real enemy is. JT would to get to the root cause of ISIS hatred. Well duh!
\item So Eugene IV's Cantate Domino is still in full force. It says that Jews are automatically going to Hell. No ifs, ands or buts.
\item America's version of the roundup of German Jews by the jack-booted brown shirts in the 1940s has begun. There won't be a good ending to this white power charade.
\item We shouldn't have to deal with your horseshit here. 
\item Mel, this is an adult discussion. Get somebody to press play on your Dora the Explorer DVD for you.
\item FOX News is left wing now, is it? Methinks someone need to re-assess their own biases.
\item Except he hasn't put any fiscal brakes on. Go look at the numbers yourself instead of listening to the spin.
\item How sad, you show us how Catholic values can be twisted and skewed. Your comments are consistently sickening.
\item Muslims do not assimilate. Muslims infiltrate. It is called 'Hijrah' (jihad by immigration).
\item Sure more immigrants. But none of the religion that dare not speak its name. Their numbers are starting to change the culture of the city for the worse. Ask any woman who dares to ride the metro after sunset.
\item Another Islamic attack, and still Obama and the left want to blame the symptom instead of the root of the problem. Come on Obama you can say it, let me help you: I-S-L-A-M-I-C    T-E-R-R-O-R-I-S-M
\item Yet these same groups look the other way when islam teaches it is O.K. to beat women, to rape women for not dressing properly, and allow the raping of non Islamic women!  The hypocrisy is staggering!
\item BLM has created a situation  where  gay white  men who show up  will be accused of being racists, If  gay white men don;t show up,  they will be accused of being racists.
\item There will be a bloodbath in Israel of Jewish blood if the UN gets its way.  The Palestinians will make ISIS look like rank amateurs in how to kill lots of people.
\item Yes, this is outrageous what happened and the response, but to think that the differing reaction to similar acts by Muslims is hypocrisy is to ignore the fact that Musims don't vote for Trump while white bible-thumping hillbillies do.
\item But why did the truck hate all those poor defenseless swedes.  Terrorist trucks could be lurking anywhere.   Thank goodness the truck wasn't Muslim.
\item It's pretty sad that the Assistant Police Chief seems to accept that the scope of the term 'terrorism' is confined to terrorism carried out by Muslims.
\item Lesbian trapped in a man's body!  Been one my whole life.
\item True. Unless of course the skinhead said he was gay. Then it's bake baker bake.'  It's been explained too you multiple times by multiple people why this argument you keep attempting is false. So why do you keep attempting it?
\item RD, so anyone who disagrees with you is 'slope headed?'  I haven't seen the geometry of your noggin, but, what ever it is, it hasn't helped you make logical, honest, or Christian posts.
\item Dress up an invasion any way you want, tovarich. Are you still upset about our winning Eurovision song?
\item Democrats, RINO's and atheists won't be happy until they have destroyed conservatives and christians.
\item What does Harper have to do with Trudeau not bothering to even show up a a service for 6 Canadians who were victims of a terror attack because they were white Canadian Christians? Trudeau's supposed to be in charge right ?
\item This is a great example of how badly catechized too many Catholics are.   And yet it doesn't slow their typing.    A 'liturgist'.
\item Your prejudice is showing. Rather blatently. And perhaps you need to search the net before making statements. A Google search of John Hopkins and transgendered surgery states that as of last year, starting a program for transgender surgery. I guess they don't agree anymore with Dr.McHugh.
\item If they feel hurt by it, why do they keep on doing it? Is peer pressure actually that overwhelming that it turns off the brain?
\item I am sure they are just like other government workers, doing their jobs at the pleasure of the government with no obvious political stance in their work, but I guess being non-partisan is not really in your vocabulary.
\item Name one Islamic country where gays can live as freely as they do in Western countries... including the ones with large 'evangelical' populations and I'll call you a liar.
\item Religious people are supposed to be snide, base their presumptions off of feeling and not fact, and try to cram their beliefs down everyone's throat.  Oh god, I just described the Transgendered movement
\item Transgendered need treatment, NOT political correctness.  No matter how hard you want to be to be a male…after operation after operation…and what your family and friends do to collude with your fantasy....if your DNA says, female, you are FEMALE!
\item Women like men who can take care of themselves. Like Justin laying a beating on the Con Senator . Women like to be protected they don't care for cowering hiding in closets wimps. Seems like you do .
\item The world just laughs at Vancouver
\item Harper is dismantling the peace, order and good government that once was, he is guaranteeing that the left can never put it back together without natural resources extraction. Harper is very much remembering his base.
\item Deficits funding transgender operations and military transgender policy studies.    Great.
\item How wrong art thou? Let me count the ways:  (1) Qur'an doesn't order Muslims to kill people on the basis of belief (2) Qur'an says nothing about 72 virgins (3) Dismissing a book you haven't read as 'evil' without reading it--you clearly haven't read it--is stupid.
\item 1 white guy, 1 muslim dead = WORLDWIDE HEADLINE NEWS  many muslims, many dead = shhh
\item American evangelicals, oddly, seem to love people getting killed.  But only after they're born, of course.
\item Liberal party agenda. raise taxes. increase spending pad our pockets screw the middle class
\item No.Not according to Obama himself, the Pentagon spokesman and John Kerry. But perhaps you have quotes from them to the contrary that support your absurd contention that you can share with us?
\item What do you expect from a Liberal media shill.
\item And Strom Thurmond fathered a child at age 22 with a 17-year-old black girl.....and yet most would still consider him a racist.    Besides, it is possible to have no racist tendencies towards Jews and yet still look down at blacks.
\item She is a 'blogger' not a journalist. This last piece will definitely not go 'viral'.Yawn...time for a popsicle.
\item Canadians tend to keep up with what is happening ... all over the world, but especially in the US, much, much more so than Americans do about the rest of the world or Canada. P.s. It ain't 1975 anymore, either.
\item Didja notice how Cohen is a 'Jew' first and then an American?
\item The Priestly Society of the Holy Cross is an association of Catholic diocesan priests which is integrally united to the Prelature of Opus Dei.'  Integrally united to  OD.  Same dangerous difference. A cult.
\item Homosexuals see 'intrinsically disordered' and see it as applying to them. Not some amorphous 'homosexual tendency', but to them as homosexuals.   You are now spouting the tired old 'gay sex is icky'. If you don't like it, then don't do it.
\item No, trans folks are not having surgery in combat zones, but apparently a whole slew of men are taking ED drugs...to the tune of 84 million a year.  Why isn't the GOP demanding that little tax perk be shut down?
\item You've asked for another office to be set up.  How nice.  Let us know when that happens.  Some Catholics are young enough they might still be alive and even give a d***.
\item Defund organizations that discriminate against Love Saxa. It is a Catholic Institution and should follow Catholic tenets. If the priests in charge, do not enforce this, summarily remove them
\item When BLM accused the white gay men of Toronto , who started Pride in 1981, a bunch of racists and oppressor class white supremacist, NOBODY came to their defense.  Being gay is one thing, but being white negates that.
\item Right next to the part that says gays and lesbians can marry.  And right next to the part that says the word 'Penalty' means 'Tax' in Obamacare.
\item She looks transgendered.  So they let her get away from robbing 2 banks and still walking? Wow.
\item Absolute nonsense.  Where do you get this stuff? Trump has as much to do with White Supremacy  as Obama with radical Islamic terrorists.
\item The PM's role is leadership, not facilitation and not equivocation. His father understood that. Pierre cared not a whit what his critics thought. You may not have agreed with him, but no one doubted he was in charge.
\item David K: I agree, what a manufactured issue....
\item The time has come to profile in London as well as the United States.  Israel has been profiling for years and the incidents of terrorism has dropped significantly.  The Muslim ban must take place until they can be vetted properly and carefully.  It's just common sense.
\item The rabid right have done most of the crying and screaming this year...it's how Trump got in. He convinced the voters that the US was in terrible shape, and that white Christians were an endangered species...
\item Sorry to fill you in on the big secret Jill but transgender issues are not about race.
\item And why would anybody with a high calibre of leadership and knowledge touch Ontario with a ten foot pole ?
\item Cassandra: Now that you are mocked in the Trudeau stories, I see that you are hanging out with your second love i.e. jew bashing
\item You can put lipstick on a pig, but it's still a pig. And boy, is there ever a lot of lipstick on that pig! And rouge... And foundation... And hairspray. Even Carrot Top points at Harpo and laughs.
\item Take away his security clearance. Fraud and lying was used to.obtain it. He should go back to slum lording business. Does not belong in WH staff. NO,absolutely NO diplomatic experience.  Oh wait,he Jew.
\item They are no more united than the EU is. They are nations and each has its own way of looking at things, just as any other nation.
\item Which is why we shouldn't give this right to any state. A government will always act in its own self interest.
\item All form of hate need to be eliminated racism, homophobia, Islamophobia, Anti-Semitism, discrimination against Transgenders. We must get behind Justin, Obama, Hillary and Premier Wynne and fight Trump and this racist Quebec law!
\item I know! ISISists are EVERYWHERE!! Don't forget to check under your bed! (Harper has your broom closet covered) (lol)
\item gender inequality, intolerance,'You espouse these views yourself, whenever the topic of gay rights comes up.Kinda makes you look like an idiot, defending intolerance then supporting it.
\item I hope for your sake that your na?vet? is feigned.
\item Just as pseudo Christians/ pseudo conservatives have destroyed the GOP, political correctness has destroyed liberalism.
\item More often it's Jews looking for more victim hood.
\item Try reading one of the many excellent books on the history of oppression of people under communist regimes and reflect privately Will China be front and centre as an oppressor? It's a terrible idea. What next, a monument to the victims of bullying!
\item Any republican claiming the moral high ground because they oppose gay marriage and abortion should be reminded that they voted for a man who bragged about grabbing women by their pu\$\$ies and whose wife has posed naked for a lesbian photo shoot!
\item SNC lobbied the Prime Minister, the Prime Minister pressured the Attorney General. The Attorney General said no. The Prime Minister removed this Attorney General. Enough of this political Mumbo jumbo.
\item So Hilary accepting millions from countries that still stone women to death, and kill people who are gay is acceptable? Again who is the whore in the house?
\item Aren't Porta Potties transgender?
\item Between radicalized white males and radicalized young Muslims we will have our hands full.
\item The only thing I'm worried about is if Malina goes home too early will tRump keep his hands to himself and not be grabbing under the table, or shoving his uncontrollable appetite into the women's bathroom.  Hey, he might get ahold of a transgender.
\item Geeez, you're thick, Rhyner.  It's the CHILDREN and their accepting parents that were interviewed by Oprah.  You're afraid of what transgender children have to say about their own sexuality?  Haha
\item Need a lot of help? Aren't you of the Con school? Shouldn't people be paying their own way for their choices?
\item Uganda had the death penalty until 2013 when they moderated their stance and only sentence gay people to life in prison now. So, I guess you win, Duque, don't you?
\item Just as I think that having to pay to give churches tax exempt status and pay for catholic education is a bloody disgrace. Unfortunately neither one of us gets to dictate what out taxes do and do not pay for. Its called a democracy.
\item Yippee!  What about questioning Trans Marxist kids? It’s all about inclusion.
\item And how is your covenant of marriage ruined by the existence of gay marriage? Please elaborate on your persecution and oppression.
\item Do the one million GOVERNMENT WORKERS care? They delude themselves that they saved 100, 000 jobs from cuts If Wynne cannot decide to cut the credit ratings agencies, creditors and lenders will decide for her And it will hurt more when they do it
\item Preventing or opposing Jews from living in other territories or countries is racist, just as the Germans attempted to do. Palestinians claim that Jews will not be allowed to live in a future Palestinian state. Their racist bigoted endeavor should not be allowed to prevail.
\item The United States has never been a Christian nation.  The racism, bigotry and hate that exist here make that very clear.
\item That was ...... gay lol what are you woot wooting about???? Find some candy in your pocket?
\item That is textbook Grade 10 Marxism, and silly.
\item Right on! The Bible says bless a Jew and you will be blessed. Outremont may not know it, but they are very blessed by having the Jews in their community.
\item Another attack by Islamists today in Pakistan killed at least 40. Comments are open in the article but my comment (which is perfectly civil) was deleted. Happens a lot. The censorship in this newspaper is being noticed by more and more readers. It's beyond ridiculous.
\item Personally, I don't agree with Kenney's politics or social values, but it would be interesting to see Alberta with its first gay Premier.  Definitely something to talk about.
\item well well well, look what the cat dragged in
\item What a rancid apologism for hate.  The two faccts 'omitted' are common knowledge, so why would hte article have to even mention either?  You, meanwhile, 'omit' mentioning that Russia hates gay people and treats them horrifically. So, that must mean your post is 'fake news', too, using your ... er, 'standards'.
\item This little piggy should have stayed home
\item I did not write the Gospel.  Take it up with God.  I could state a person who suffers sexual attraction to children is nature, not choice and love is a right of nature.
\item Sir SAMUEL de CHAMPLAIN The (real) 'Father of Canada' (aka New-France) First Canadian Scientific (Premier Scientifique Québécois)/  Explorer/  Navigator/  Cartographer (he made the first accurate map of the coast)/  Geographer/  Ethnologist/  Diplomat/ Draughtsman/ Soldier/  Chronicler/openly Gay in Huronia Nation (Ontario)/  founded New France and Québec City in 1608  CHEERS to de CHAMPLAIN !
\item So what's up Scott, I guess this thinly veiled threat of violence is cool too since its directed at a trans person and not a real human.
\item The RCC is simply an institution bent on profit and power.'  There is a special place for those who malign the Church that Catholics hold dear, and a special ignominy in being once a Father of Church and saying such things.
\item No but it is funny that the Islamic terrorists are for the most part right wing followers.  They are conservatives.  Fact.
\item Didn't stop 'em from murdering millions of German Jews and Gypsies, however.  I quoted Goering in my previous post.  Like I said, the TRUE face of 'animal rights'.
\item The obvious irony is that the slave trade was controlled by Jews and Jewish households were much more likely to own Slave's than non Jewish households
\item No matter what party each of us is from, no matter whether you agree or disagree with the nannies issue, can we all, together, please focus on important issues? There are so many, let's pick one and start working as a proud nation.
\item Why aren't their islamic brothers taking them in?  Since when is it the West's responsibility to save muslims?  We can see around the world how well it works out when you allow islamists into your country!
\item Be thankful this isn't in the states... Some bleeding heart liberal would be screaming the anti-bullying law infringes on the freedom of speech
\item Trump is implementing his Muslim ban in steps.  This is 17\% toward a Muslim ban.
\item It's not just at the college campuses. How many newspapers are shutting down their comments section? How many comments are eliminated even though the comment makes no threat of harm.
\item right on, but privileged haoles moving to hawai'i maybe have more in common with colonizers than they do with an historically oppressed people like Jews.
\item Canada was built on the 50\% +1. Check out the history on how Newfoundland joined Canada and you will see they won the referendum with a 52\% majority.
\item You mean it was Richard's venue.
\item If my memory serves me well, it wasn't even legal back then when this happened for homosexuals to marry.
\item I think the biggest gay concentration is in Toronto not Montreal but that doesn't matter,because in Justinians mind doesn't concentrate on the foul taste in his mouth just take a deep breath and savor the sacrifice for the win.
\item Aw the child porn lovers come out to defend Flanagan, how touching..
\item There is an Alt-Left, the extreme left that sees 'racism, ethnophobia, islamophobia, misogyny, homophobia, transphobia, etc.' under every bed.  Both extreme fringes make the moderates look bad by association.
\item Since when is being trans gendered a sin?  There are no laws against same-sex marriage in the US anymore.  That ship has sailed, sister...
\item Being respectful toward other people has been labeled 'political correctness' by those on the right. You have misunderstood the point.
\item Actually, gender reassignment is neither cheap nor easy. But what do you care? You have decided that psychological knowledge has not advanced in 50 years, which combined with your easy dismissal of the transgendered shows that you don't actually care about real people with real problems.
\item Voting for Hillary and being Catholic is an oxymoron .  Abortion is an abomination in the eyes of God.
\item I suppose you are right, DMOnt1. We could fall into that less aggrandizing, idyllic skill set where we say no Jews are still too many, and send them all back to die in the Holocaust.
\item All things are equal to all others'- you agree with that, you shouldn't even have children
\item Meanwhile, on the military transgender front...
\item This minisster is NO friend of the majority of taxpayers. Watchout please!
\item as a lesbian, a new parent ...' How is that even possible? Good God, don't tell me.
\item I believe the close race has a lot to do with Hillary being a woman; not because many people can't stomach electing a woman president but because she's being judged by a different standard than if she were a man.
\item What was it Jesus said to 11 other men again? - 'You will all lose faith.' Those 11 went on to show themselves to be weak, cowards, unbelievers and..... the greatest saints of our Church.  'Can anything good come out of.... Germany?'
\item Another conservative family-values politician goes down again.  Interesting how almost all of these conservative family-values people eventually get caught with their pants down.  At least  he was  only a Baptist Deacon and not a Catholic priest or Catholic Bishop sexually molesting innocent little boys.
\item Back to the Supreme Court of Canada. The judge was correct. Make the Catholics pay for their own faith-based religucation.
\item So who are you to determine what forms of correction are legitimate? You must have some qualification beyond being a busybody liberal.
\item Trump’s Navy Secretary On Transgender Troops: ‘Any Patriot’ Should Serve
\item ...Trump's hateful ban of transgender troops weakens our nation...'  1st, his ban wasn't 'hateful'.  2nd, his ban strengthens our Military. 3rd, what the ban does weaken was the damage Barack Hussein Obama's hatred of our Military wrought.
\item There is no proof that this is the alt right.  It is equally possible that it is the  alt left.  Both groups hate jews. Furthermore, the latter hates Trump and would be happy to set him up for responsibility..
\item Oh, they will still blame the Jews, lots of their propaganda from the 1940s and beyond reminded people that the people who came up with communism were Jewish.
\item As a guy I have no problem who is using men's  washroom, but I can imagine that ladies may have an issue with it.  Realistically, the percentage of trans-gendered people is so mall that you have almost a zero chance of bumping into one in a washroom.
\item Right and wrong actually exist. Comparing the systematic murder of over 6 million Jews alone to Elvis is beyond foolish. We don't need any 'dialogue' about Naziism.
\item This is like those folks who disown any of their fellow religionists who get caught doing something wrong as 'not real Christians.'
\item And Satan's spawn using a church for the meeting no less. Church of Evil, from the sounds of it. Fake Christians. Death-dealers.
\item You'd feel safer in Afghanistan or Iraq or Pakistan than in Kansas?  The Vegas shooter was motivated by Christianity?   Or was Dylan Roof?  Just stop.   There is no Christian extremist movement on a crusade of killing people.
\item ZayWhat, No harm to society as a result of open use of pot. But slow death for an economy based on slave wages.
\item thoughts and prayers', yeah that'll save a lot of lives
\item Lesbians can only get pregnant with help from a MAN. You know, like one man - one woman?
\item Are you bothered by imams preaching anti-Jewish bigotry in Canada? Probably not.
\item Hahahaha, you're quoting a right-wing Republican vice-president forced to resign in disgrace.     And stayed in disgrace: 'In 1976, he briefly reentered the public spotlight and engendered controversy with what Gerald Ford publicly criticized as 'unsavory remarks about Jews'.'
\item Wednesday May 17 is the international day against homophobia and transphobia, I encourage everyone to do something in their community to raise awareness of this issue!
\item liberals don't care about life, it is money and power
\item More importantly to be Canada's head of state you must have greater loyaLty to another country ,the UK.Sounds kinda crazy to me.
\item Good point, Javan. So very similar. A transsexual woman needing to pee or wanting to re-do her bouffant hair do is very much like a (presumably) straight man following little girls down the street.
\item Mel... educate yourself before posting drivel like that. The US didn't start the war in Vietnam, it was long started previously by the French.
\item Ya that 60\% efficacy rate (at best, most years, slightly higher this year) will do wonders to keep everyone safe. I'm in favor of the flu shot for most, but nowhere near stupid enough to believe that it keeps me, and everyone around me, safe
\item You're right about that.  Such good Catholics, they're as tribal as the Bundys.
\item Diversity! In everything but thought...
\item The worst hate mongering  apartheid countries  are Muslim.
\item Well, thank you, for identifying 'socialists' as the only ones who care about human rights. You could be right.
\item Believe me, the gay community is not recruiting.  We have enough problems with our own voting liberal every chance they get.  If you aren't gay, don't worry, there is little hope to make you gay.  (But if you are a liberal, please become a conservative!)
\item dome:  You are describing a he/she or she/he or Trans something.
\item The Liberal Party of Canada thanks you for your loyal posting.
\item Good!  White Christians are evil.
\item B.C. citizens have finally seen the Right. That is, the so -called fake Liberal Right. Ontarians have seen the Right, too.
\item Your lack of Christian charity always amazes me.
\item Are you a muslim Alceste?
\item Another minion of Satan. Bergoglio (Lord Of Flies) Continues his usurpation. All who help the anti-Christ who currently occupies Saint Peter's throne, will answer for this blasphemy.  Repent or be damned.   in nomine eius
\item Belief in god is dying fast. Thank god.
\item The North Korean 'people' really don't have much say now, do they?  But yes...when we have a draft dodging, chickenhawk, wanna-be tough guy saber rattling and gambling with the lives of our military men and women...transgender, straight, or whatever...it doesn't help the situation...
\item Patrick D'Aloisio aww! Are they making fun of your Imaginary Friend?
\item Very na?ve, I'm afraid.
\item Pandora, just because you suffer from the delusion that women are not second-class citizens in the Catholic Church does not mean that others share your folly. These women were protesting an injustice. What is awful is your objecting to it.
\item Paranoid'? People pointing out a clear advantage FOR this individual in a field of competition are 'paranoid'? Fairness is taught in ALL fields competition. At all levels. From youth to professional. There is clearly something wrong here. Otherwise create a transgender division.
\item Drug addiction is a malady, so compassion is warranted.
\item It's no myth. Not only do they get paid quite well in Alberta but they are paid as 'independent contractors'-------------------------Ah. Not all tradespeople live in Alberta. That probably surprises you, though.
\item @MMackinnon Yes in the Chretien and Martin years there was a more peaceful world... Terrorists would not have blown up WTC in 2001 just a few miles south of the Canadian border.
\item There are other ways to protect your home - martial arts, for example
\item They still throw gays off buildings and stone women.
\item Members of one religion bombing members of another...just as Christians killed Cathars or Catholics killed Protestants (and vice versa) years ago. Maybe absolute certitude that you are hearing the true teachings of God is not always a good thing.
\item Excuse me, people of Jewish descent are not asian. That is absurd.
\item That's not exactly the reason why you were suspended though, is it?    From what I read, it was because of your open and supportive stance for gay marriage in defiance of Church teaching, your Twitter comments and activism....not because you are gay.
\item An amazing shot when you consider that the person who took it is a transgendered aboriginal.
\item I presume a combat rosary saw service in Iraq or Afghanistan.  While Mary loves all the troops, I am not sure that Mary the Palestinian Jew would approve of any foreign occupation by an imperialist power, speaking of that other kind of Americanism.
\item I don't think you can compare Trump wanting to keep criminals and illegal migrants out of the country to Hitler's disgust for Jews. Btw, how many Syrians has Israel adopted?
\item Earlier this week, 56 retired generals and admirals came out against Trump's ban on transgender troops, arguing it would be disruptive and degrade military readiness.
\item Why would the daughter of a draft dodger, who has just slapped the face of every serving American transgendered person be chosen for a ceremonial task of honour?  Time to for the government to remove her from the guest list.
\item I didn't know journalism degrees come in crackerjack boxes. This girl no doubt got hired for her looks.
\item Damn that Trump!  Now he has turned blacks against Jews.
\item Those pharisees said Jesus was a cafeteria Jew.   I don't know why, cause  Jewish food is delicious (except that gefilte fish, oy gevalt, it's shreklekh).
\item Nobody should be force to speak french it is ridiculous. | Canada needs to be split into four separate countries: French, Native, Catholic and Agnostic.
\item Cannabis has been used to treat addiction to hard drugs -- might work for Nicholson and Toews as well ... we could only hope.
\item GDP grew during the financial melt down of 2008 and onwards? Now who's drinking the coolaid.
\item Sure you want people to be damned. If you did not want it, you would reject Canatate Domino and accept Dignitatis Humanae.  Your God is a bigot. He sends Jews to hell for being Jews. How does this differ from the Nazis sending Jews to Buchenwald for being Jews?
\item Catholic social doctrine is not owned by the 'left'. The Church was established by Christ as a hierarchical institution, not an egalitarian one; and was empowered to determine right from wrong based on revealed truths, not epistemic relativism.
\item hes way too smart. (the bar is low)
\item No right minded person would want to enter those places, unless they were Muslims, what they call a place of worship is frankly a place to breed fear and judge people.
\item Shame, indeed!  But Christians don't think laws apply to them.  You know, 'religious freedom' and all.  'Render unto Caesar. . . '  Oh, never mind.
\item Target still hasnt recovered since their stock tanked after implementing their store's gun free status, and Obama's transgender bathroom nonsense.  How could this 'news story' ignore that 10,000 pound elephant in the room?
\item Utilitas, you keep insisting that all Trump voters are not racists.  Yet you are saying all Muslims are terrorists.  Do you see a problem here?
\item Anti Muslim name????? How exactly is defending France against invading moors in 729AD 'Anti Muslim'?
\item When you start worrying about the 'human rights' of terrorists.................
\item Yes that's right. Only you and Fanfret know the path to truth. Which of course is why we dont need a referendum. Because we have Liberal Party hacks and spinners like you guys to design a new system for us.
\item The truth hurts, don't it, Barry?
\item If Trump's goal was to ban all Muslims, why does his executive order apply to only 1\% of the Muslims in the world?
\item Don't think all black gay guys agree with BLM.  But because of the colour of their skin they are ignored by  media politicians and even BLM.
\item More treacherous than Nixon?  Yet, the outgoing tyrant called white, christian, conservative a domestic terror threat.  Hey, Berstein, GPS!
\item No, because Muslims don't let their women out of the home.  They also don't have gender fluidity.  Therefore, the only option is a manhunt.
\item Canada was established on Biblical principles.
\item What Quebec wants is Chinese immigrants who drop off half a \$-million on their way to Vancouver.
\item True, we can just ask gays their experience and then trust them when they provide it. Sexual morality is for them, not for God. What bothers you more is not their morality but the public authority of the Church hierarchy, which God does not care about.
\item He was getting fresh with the transgender woman, and she said 'Cut it out!'
\item The fact that this person is transgendered shouldn't matter. The real question should be, can she do the job?
\item I think Mr. Khan covered it pretty well.  In later interviews, Mrs.Khan addressed Mr. Trump's claim that she 'was a Muslim woman and, therefore, wasn't allowed to speak.'  Mr. Trump reminds me of the old 'Limbo Rock' lyrics..........'how low can you go?'
\item If probably more than half the priests are gay why are they against gay people and their marriage rights? Are they angry they can't gay marry?
\item Liberals are still crying over the fact that Mateen wasn't a white Christian.
\item As a Canadian trans woman living from time to time in the US I am feeling very vulnerable, and very angry. Thank you for stating this so well.
\item OH NO! The snowflakes will have to pay for their education of black studies, women's studies and transgender studies! Oh the humanity!  The good news is that a degree in transgender studies will ABSOLUTELY help you get into a profession paying \$150K year.
\item Seth.. Good comment. I am very happy to see that there are some honest, capable people out there trying to help Ontario save itself from the largely left wing disaster called renewable energy.
\item Don't worry. Trump has already played the transgender card to please his base. He's got GLB remaining, as well. If the heat gets too high for Trump, if he's not feeling the love, he'll make sure Hillary Clinton does the perp walk. The ratings on Fox will be yuuuge.
\item Gay rights are more than marriage. But yes, if you are against gay marriage, you're a bigot. And you are a bigot. Roskell.
\item Why not post the names of the adults? Must've been another Christian hate group.
\item Ad absurdum much? 6 million Jews, not arguable. 6 billion sperm? very arguable.
\item Great writing. As an ex parrot... er.. christian - it's good to hear of good sense in amongst the adoring patness.
\item I think the G\&M gets these 'articles' for free - and the authors thereby obtain a soap box for their pet diatribes, mostly uninformed !
\item Such clubs fan the spirit of victimhood and nurse self-focus.  Never a good thing to do.  I can't see St Maximilian Kolbe (feast day today) starting a club in Auschwitz for 'condemning the bigots' who gassed the Jews and himself.  Instead, he used all of his time very well...serving others.   Argument emptied.
\item so basically you're fantisizing about getting a legal reason to kill someone. You are a horrible person
\item Hey, don't sweat it.  We kill thousands of Muslims every month over in the middle east.  We're well ahead in the body count.
\item He didn't take action with the Jews in Rome.  He actually let them be rounded up.
\item Most of us have grown up and no longer refer to gays as icky.  Time to move into the 21st Century.
\item Was this story written by a jew? The import tax is now 300\%. Tell you what Globe, cancel my fucking subscription. Period.
\item GOD has changed?  Say what??  I doubt you studied Catholic theology on a graduate level; but if you did, get a refund.
\item Funny, no parliamentary motion to quell the Quebec imam who preaches for the extermination of the 'accursed Jews.'
\item The press is trying to jump on every major and minor misstep Trump makes but many admire his politics. He has a very good chance of becoming the next president even though many, especially the establishment, do not like the idea.
\item The fact that religion is based completely on faith alone does not necessarily make it 'unequivocally' crazy. Your well-written comment would have been much stronger (for me, at least) if you had chosen a better example.
\item Trump is their savior.  They said so.  If a protester is run over  by a car will Trump even speak about it?  The wery good people chanting “Jews will not replace us”.  What a disgusting pos
\item And here I thought we were doing so well, with not a cathouse or casino in town. I forgot about the homosexuals. No wonder we're being smitten.   (That was sarcasm, if anyone misunderstood.)
\item Thank you for your service and may God keep all our military service members SAFE.
\item Star\_Chaser - 'The most bigoted people I have seen here are the Harper haters.'Just like Israelis and Jews who oppose the policies of the Israeli government are 'anti-Semites'? Your attempts to criminalize political opinion are pathetic.
\item Canadians won't be in a position to say 'we have made amends' for at least a generation AFTER the government has demonstrated it is treating aboriginal people with respect. That has only just started after a decade of going backwards.
\item Gee the geniuses at the Glob of Muck are just finding out that Trudeau is just your garden variety lying Liberal ..brilliant !
\item Transgenderism and other politically correct stupidity will be the downfall of Western civilization.  Sorry if this offends the minority, but most normal people are tired of this nonsense.
\item Ruling government' !! That says it all. Like yourself, Harpo appears to think he was elected to reign over us.
\item Which military commander is saying that transsexuals are good for the military?  Name one.
\item Sure it was, HM, but the shooter was born in the USA. A Muslim ban would have changed nothing.
\item A 'post-American era'--what is Hillary a secret Muslim like Obama?
\item Shias, Sunnis, and all other Muslims as well as Christians, Buddhists, Hindus etc. can find a safe haven in Israel. Just stroll around the streets of Jerusalem and see all the various worshipers freely observing their religious practices.
\item Oh boo hoo! Another sob story from the liberal Kool-Aid factory attempting to make us feel sorry for the most hateful, misogynistic, homophobic, racist group in Canada that produces the vast majority of terrorists. Not that the Globe is taking sides or anything...
\item A transgender identy child has suicidal tenancies???  May want to inform the parents then.
\item Let me get their logic straight: Jesus was a pedophile, so it's ok for Roy Moore to be a pedophile?  Wow.  Just wow.
\item Pizi It makes no sense to occupy a strip of land partially occupied by and surrounded by your enemies. Nothing to do with ownership of the land.  If Jews bought Palestine, their reception would be the same. It makes no sense to..........................
\item CDNWorker writes: 'Honesty and integrity do matter.'=============The recent Ontario election demonstrated that these two things are not particularly high on the list of voter concerns.
\item I could also ask why left-wing Catholics supported an amoral philanderer conman like Bill Clinton.
\item Don't you find it is becoming rather monotonous and predictable? It may seem to be parodying traditionalists but in reality it is a mockery of the Catholic Faith.
\item forwhatisworth, When these people started 50 years ago to want to kill all Jews and continue to think like that instead of negotiating a settlement they deserve what they have. Terrorists are terrorists and desrve to live in ruins.
\item Yippee! And the point of this is what exactly? To trivialize homosexuality even further? I'm thinking opening the first all-gay lawn care service. That will make me 'courageous'!
\item So the children graduating from Catholic Schools have actual knowledge that the Catholics Imaginary Supernatural buddy is a fraud and public School Grads do not?  Private Schools do better because they can refuse or expel problem students, or ones that require more resources.
\item Russians didnt like Hilary Clinton, Israelis hated Obama (Bibis government) Both Russians and Israelis meddled in the election. But everyone is very quiet about the Israelis. Putin and Bibi hooked up last week never mentioned in mainstream media. I guess being Jewish has its privileges !
\item The ACLU says an estimated 8,800 or more transgender people currently serve in the military'. Are they referring to actual transgender, or just grouping as queer. 8800 sounds a bit high.
\item Nothing but fears and jeers, Gay.  Keep whining.
\item Trump's banning of transgendered people was certainly arbitrary but I don't think it will have a drastic effect on LGBTQ rights, especially not in Canada.  Their rights are too entrenched now. They have become unshakeable like the rights of women.
\item That will be happening here in Canada very soon.... as a matter of fact, it may be going on right now.  In Richmond Hill there is a Muslim-only housing community where it's forbidden to walk your dog on a public street.
\item Or the incompetents that are running the liberal party now.
\item How about the rights of working Canadians who pay \$14 BILLION a year in funding they get with no accountability?
\item What about your RoboCall Scam and the investigation and muzzling election Canada so they can't ask questions of the scammers? That doesn't bother you eh?
\item the price we pay, low as it is, mostly goes to the middle man and not to the sweat shop workeryet progressives, leftists, socialists, Marxists in the West keep on buyingforgetting their public pose as advocates of Social Justice
\item No, he's not proTrump, but only because Trump is anti-Muslim. And unless you're a Muslim, Minshall has no use for you.
\item Redford yet again shows She is more aligned with Her bretheren at the UN than Alberta... Lawyers do that, it's called Weasel words... used in an Election, then do something else altogether! One hit blunder this one...
\item Freedom of the press belongs to those who own one'It's the internet age. DIY, start your own website and let the comments fly. It's never been easier.
\item ... it really is only about 20\% support this monster.  What is SAD is that 80\% of THAT 20\% consider themselves Christian.  Disturbing!!
\item sorta like the anti infidel hate practiced by the Muslims.
\item Joey, it's not the gay agenda, it's the black agenda. Membership has been declining since 1974, when the Boy Scouts were forced to integrate blacks into their troops. Equal rights are ruining the morally straight....
\item Oh they know, they just love having this as a stick to poke LGBT folks with.
\item When it calls me a 'rag-head' I disagree.  Guess since it's a tranny should be OK for me to punch it out without being accused of 'hitting a woman'...
\item Neither is Bernie, but Bernie is also trusted by the people.
\item Forget the prejudice junk. And forget the neighbors junk. Practicality and economics.  And if you don't think an openly transgender in a barracks with 100 men isn't detrimental to the military mission then I give up.
\item  I don't see the death of Western Christianity as a bad thing ' .  It doesn't get much more pathetic than that.
\item Baloney! Separate school boards in Alberta feature prayers and Catholic religious courses. Holidays at Christmas and Easter are Christian celebrations. You'd do better to hide your prejudices and keep your shallow thoughts to yourself.
\item if you are browsing these comments, you are definitely a divorced, unemployed loser. get a life
\item We need a cohesive plan to get paid for our resources in cash in envelopes.
\item These people here regularly hold up Westboro Baptist, the Catholic Crusades, and the Catholic Pedophilia as a model for Christianity, which is ludicrous, they only demonstrate their own ignorance and bias.
\item I don't know about 'constitutionalizing'. Parties are most certainly already legally recognized and given great power by both law and Parliamentary Rules.
\item Your equalization money.
\item Can you provide proof that the number of reported hate crimes against jews has been falling?
\item Not like the right wing was obsessed for 8 years with the secret-Muslim, non-American, baby-killing Obama, no?
\item Check the FBI and CIA sites for information on the religious affiliations of terrorist groups. There are definitely Christian-affiliated (self-identified as Christians) terrorists.
\item Pedophilia? Hmmm? Catholic much?
\item Catholicism certainly. They were expert terrorists.
\item Yup, conservative politicians like Kenney who still can't force himself to say that lgbtq rights are legitimate, that gay support groups in schools are a good idea..
\item Get used to it. Liberals believe that they have a God given right to tell all of us how to live their lives.
\item Thank you for such a fine article! I particularly listen up to the parallel between raw anger and raw empathy.
\item Bravo !  Hispanic Catholics are like Italians or Irish of a century ago....the next big winners in America's economic lottery.  Why Hispanic Catholics would ever want to copy-cat the Black Protestant Democratic Party disaster never made sense to me.
\item I don't subscribe to a religion, but to a relationship with Jesus. I think for myself and strive everyday to act decently.
\item Muslims are the worst Islamophobics of all . Ancient hatreds and wars of extermination between Kurds, Shiite, Sunni, Wahhabi, Druze and other Islamic sects are worse than anything expressed in the west, even by Trump.
\item What trash, Tridentinus!  There are many who leave the Church for other very important reasons, the sex abuse cesspool for example.  Your rigidity reflects something entirely different from the Church of the Gospels.
\item You have to admire Margaret for her willingness to take on sacred cows, whether you agree with her or not.
\item Your post is very short-sighted and uneducated......trans-gender restrooms has got to be just as important to the council.
\item Right on! Each time Harper opens his mouth, I?m reminded of, ?I did not have sex with that woman,? and ?It?s not a crime, when the president does it.?
\item Get ready for more of this nonsense.  Once transgendered rights are elevated to the point of disallowing any thoughtful criticism, the lunatics will use their new found powers in ways that make 'self serving' an understatement to say the least.
\item don't shoot the messenger Skeptical - if you all you have is insults and abuse, you have as much as admitted you don't have a position you can defend and the other right.
\item No, we do not. You've had your day, get lost, buh bye.
\item He'd feel as safe as he did in the broom closet.
\item Perhaps if you avoided hard liquor this early in the day, that may make a difference in how you approach the subject matter?
\item Fair points on Adams and Blair.
\item They're the intolerant and authoritarian type of people that are like this towards minorities. The authoritarian mentality has reared its ugly head in recent years using Muslims as the current scapegoat. In time, they'll drift away to other groups...
\item So who's the bigger threat to Americans??? Islamic Terrorist or American Terrorist killing thousands of Americans in places like Chicago??? \#MAGA
\item The hierarchy of the Catholic Church in the USA are a rigidly politicized group. Their alliance with far right anti-gay forces, and their intellectually dishonest embrace of a phony notion of 'religious freedom,' makes them inevitable enemies of gay people.
\item Paprocki is denying people in same sex marriage funeral rites, not gay people.
\item Learn to spell and/or proof your comments before posting.
\item I (don't) know why, please inform me! That is why I posted my comment. It is not due to gay issue because the Boy Scout USA had already agreed that the Churches  can exclude Gay troop master's if they want to.
\item You're just mad because we are the world superpower and have accomplished more than you, and you have nothing to say for yourself.
\item You look into people's eyes
\item All women are strong and are able to become leaders if they want to
\item Of course, Naomi Klein's not arguing we should force the third world to pay for emissions reductions, but keep tilting at that windmill Ms. Wente.
\item It's almost certainly ISIS or other Islamist terrorists.  A nightclub = booze + fun; Nightclub on the European side of Istanbul; Nightclub frequented by foreigners.  ISIS and other Islamists hate Europeans, booze and people having a good time.
\item Trudeau needs to talk about the millions murdered by Muslims. The fact their religion does not respect human rights.
\item Jewish fundamentalists (Haredim) in Israel would prefer a rabbinate rather than democracy- a Jewish version of Sharia law.
\item Another, Want to ease the suffering of your working life? Don't suck up to your corrupt corporate employers and don't kick down on ordinary working folks.
\item Some ex-Jews are so fed up with the false equivalence of Judaism with Zionism  that they have decided that they are not Jews. Don't dare speak out publicly, but can quietly avoid ticking the 'Jewish' box on the census.
\item Dare yourself to travel to those banned countries, anytime? Be aware that not only americans have got killed in those places, but also europeans, and other non-muslim foreigners who happened to be there.
\item The UN is sacred and all things Holy to Canadian liberals, never forget it.
\item I'm more curious about the reaction to 1k gay priests saying 'We're gone!' More than a few have already gone to live their vocations in different pastures, and probably a few more will move on because of this.
\item According to the author, to be in favour of human rights and against occupation and colonisation is 'pro Palestinian'. So logically support for Israel is........
\item Transgender is a mental disorder. Doesn't matter if your liberal or conservative.
\item So transgender does not include looking post-menopausal, huh?  At 66, real women do not look like this.
\item How about answering the question asked rather than throwing up a smokescreen?
\item We must build a wall to keep these transgendered sheep-lovers from invading the Homeland and forcing their boiled food on us!
\item Justin is a devout Catholic, it's no wonder he believes the earth is flat and only 6000 years old.  If he's into cupping, perhaps he's into other forms of fakery.  Has he burned any witches at the stake recently?
\item Admitting we have a Muslim problem would be the best staring point.
\item Gee....when I bought a house in Anchorage in 1980 I thought I'd moved to Alaska.  Searched through your link.  Didn't find a reference to 'sex', or 'gender', or even the part word 'trans'.
\item  "the racists and the bigots have always been there... appeal to the lowest common denominator"
\item RD, wrong again.  Obama's was an effort to revet people from a country known to have terrorists.  Trump's is a ban on people from countries that just happen to be Muslim and where Trump has no business dealings.
\item In fact, most people interpret what the CDF said as meaning that homosexuals are 'intrinsically disordered'. Homosexuals do almost unanimously.
\item I suppose that white men might also be transgendered so...
\item Gender based? Just male-female?  . What about transgender?
\item It's not hard to find out that Saudi Arabia would not exist without US support.
\item This isn't racism. It's the truth. It is what it is. Unlike you, I'm not so arrogant as to believe the truth will never offend anyone.
\item In other news, a person with a penis  is demanding the right to attend a women's only event where nudity is common. See: http://www.metronews.ca/news/toronto/2017/06/14/women-only-spa-s-no-male-genitals-rule-ignites-transgender-debate.html
\item It takes a lot more integrity to grope women .................. and spy on 16 year old pageant contestants changing into their bikinis.
\item Ask Marshall, the loser. His campaign went negative or Roem being a transgender woman. Ask Trump why he wants to throw all transgender people out of the military. Ask the 'family values' crowd, they equate being transgender with being a sex offender.
\item lies-vast majority of Christians support ay marriage
\item I think you'd get better luck with dogs! At lease they have loyalty.
\item Soros is the money source for almost all the muslim travel ban lawsuits. That's why Saunders and Alceste love him.
\item Hey my fellow Christian person, I'm happy to pay for healthcare like Jesus commanded us as soon as we make abortion illegal and outlaw homosexuality. Oh yeah I forgot this isn't a Christian nation unless it's convenient to commies.
\item True. Unless of course the skinhead said he was gay. Then it's bake baker bake. The Little Guy
\item Not a cent....period.....sadly our rather stealthy government will probably funnel money to this and hope no one finds out, just like Khadr, just like bringing in the Gays secretly.
\item You yourself hate Western principles. What's your opinion on gay rights? If your comments on here are any indication, exactly the same as the Muslim point of view!
\item Ah, the SJW industry. Is that anything like the gay agenda?
\item If the Holy See quietly vetoed a homosexual representative, then why do they appear to be willing to work with a heterosexual mistress \& her adulterous spouse?? Could it be all that GOP friendly K of C money??
\item ...And how are the French doing on integration of their Muslim minority...?
\item Racist drivel from a commie and Islam loving rag and liberal propaganda machine!
\item CG cutters used to have sonarmen, depth charges, and torpedo tubes. They don't have those anymore. But they probably are all kinds of cool with transgendered issue tho!
\item Another arch Liberal blames someone else for his hate speech. It's not unlike Hillary blaming the women her husband abused. Or Barack Obama  when he blamed White people for Black crime, or when he blamed Americans for Muslim terror.
\item Lots of so-called Christian suckers. The same people who give to these hucksters vote for Trump and believe his lies.  As Lincoln said, in a woderful euphamism for fools, 'You can fool some of the people all of the time.'
\item Yes, Mike Pence Is A Calculating Gay-Bashing Koch-Toady, ...But You Knew That https://www.newyorker.com/magazine/2017/10/23/the-danger-of-president-pence “When the conversation turned to gay rights, Trump motioned toward Pence and joked, ‘Don’t ask that guy — he wants to hang them all!'”
\item I'll bet you were first in line to decry obomba mandated transgender bathrooms.
\item Pathetic to hear you think Christ died to end poverty; pathetic to hear you mock the idea that he came to save souls.
\item So the Church employee was fired for entering a gay marriage.  You expect the Church to continue to employ someone whose conduct is in the face of the Church's significant moral teaching?  Why should it?
\item Conservatives generally and this President in particular have made 'Christian' just another word for self obsessed \& hypocritical worshipper of war.  Merry Christmas.
\item Mr.Simpson you are wrong about tax policy and justice there will in the longer haul be a trend of reversal for the better. Not all of the people have such shortsighted views of society as the Conservatives have
\item I'm not so sure that Islamists problems are public relation based as much a ideologically based...it's now 9;17, I give this comment 10 min.
\item Not even a tenth of one percent of students are transgendered.  D I S T R A C T I O N
\item I just refer to everyone as 'a**hole', everyone male/female/trans has one, so it fits.
\item I don't believe you know what you are talking about. You just don't.
\item Ah. The gays are threatening your straightitude, huh? Your neighbour, mowing his lawn shirtless, makes you question your life choices?  Maybe you should seek out Mike 'Get out of my uterus' Pence for his conversion therapy.
\item Letting people make their own decisions hasn't been in the plans of most Canadian governments since the 60s.
\item We very definitely are not in a holy war with a million peaceful Canadian muslims.
\item I hope that this will be a good time to move away from only victims of Catholic priest predators and include other ministers, school teachers, scout leaders, coaches, and others in positions of trust and authority who have abused children in their care.
\item Known for his controversial views, Drollinger has said of Catholicism: 'It's the world's largest false religion.'  Christiantoday.com  Catholics who jump in bed with fundamentalists might just be really, really deceiving themselves.
\item It would not surprise me that Stephen Harper oversee the demise of Canada, and be a key determining factor of Qu?bec independence. The perfect legacy for a man who has no idea what 'Canadian unity' is about or how to govern a country.
\item Trans people have a condition that requires the regular use of drugs to maintain their physicality. Diabetics are not enlisted either - are you going to claim that the CiC is not supportive of diabetics?   Military is for fighting, not a support group for medicated people.
\item a catholic priest molested children?  Surprise, surprise, surprise.
\item So the transgender members of the military in other countries have never fought and died  for freedom in the name of their country.
\item It is a human rights issue for the  'Human' fetus.   It is synonymous with the Nazis sterilizing Jews.
\item Please continue living in your bucket, that is the best place for people whose eyes remain closed to other cultures.
\item No more niqqers nips spics or Jews
\item I think NCR actually self flagellates Catholicism more than the fictitious 'Opus Dei monk'from that silly Dan Brown book.
\item filipino psycho killer!  filipino and filipina pride!  life long filipino catholics are life long atheists.
\item Dude so she spelled yer name wrong get over it snowflake. Bottom line I'm Jewish and I don't appreciate the dumb jew comment. Clean up yer act.
\item Jews breathing in Israel 'upsets the Arabs'. Women serving in the IDF 'upsets the Arabs'.  It's time either some people put their adult pants on and stopped being upset, or the rest of us just ignored their constant offense and rage
\item They don't understand how Catholicism works and have a rigid and superficial understanding of it as well as bringing their bad Evangelical habits with them like their worship of far right politicians and love of the culture wars.
\item Missouri LIBERAL JOURNALIST charged with Jewish bomb threats, you mean, WaPo/ADN! Funny how they are saying it was because of his girlfriend now.
\item palestine has 0 jews. Israel has 20\% non jewish arabs and plaestinians and others. It is plain who the problem is.
\item Coates is an overt racist himself as evidenced by the position he stated in The Atlantic that whites are an 'existential threat' to the world.  That's the kind of rhetoric the Nazis used against the Jews.
\item Are we safer with transgender recruits?  Is the expenses warranted to keep our country safe?  Does a .005 or less of the population warrant so many drastic changes to our military?  If you answered 'no', you are in the MAJORITY of the population.
\item Probably transgendered. He does look a bit prissy. Does this mean Trump will be pro Xwoman? Life is funny.
\item Typical liberal Jew. Has he forgot what nation ended the Holocaust? Total disrespect of the office of the president. Who's the malignant one?
\item I thought that only trans genders shop at Target ?
\item Thank you for this article. For the lucky people not exposed to family members in the grip of addiction, it is harder to be empathetic on this issue. Addiction is a medical issue rather than a moral failing or crime
\item Now there's an example of the sort of civility 'progressive' Catholics are known for, eh? Unlike those terrible, awful right-wingers.
\item The Arab sycophants who regularly find fault with Israel have suddenly gone silent. No Jews involved, so no need for them to comment.
\item I thought he was gay from the start but I did nto care one way or another.  It is his personal business.
\item The Church is now in a full-blown civil war over doctrine.'  A headline from a Catholic paper not pron to hyperbole or click-baiting.  http://www.catholicherald.co.uk/commentandblogs/2017/02/15/the-church-is-now-in-a-full-blown-civil-war-over-doctrine/
\item some kind of relationship?'  NO, they were, and are homosexuals, just say it.
\item A hopeless state! Same old tragedy, over and over. It's their guns that are doing most of the damages, not Muslim immigrants.   Idiots elected a morally corrupt party and president.
\item I loved that line from Powells email pointing out ho her Hubris touched everything she did, and messed everything she touched. And he was a supporter!
\item Get with the times, Pal! Russia, non-Communist, is our ALLY in fighting ISIS, unless, of course, you are a proponent of innocent severed heads. Why don't you extol the Catholic virtues of faith, hope, \& CHARITY!
\item Republicans state they don’t hate gay people.  Moore wants to lock them up.   Horrible people.
\item The US military spends more on Viagara than on transgendered persons. Should it put a hold on males with erectile dysfunction from joining the military?
\item Do you remember when Canadians were too smart to trust Steve with a majority? Oh, for the good old days.
\item they are counting on more hugs from the sheep
\item Jews weren't flying airplanes into buildings and slaughtering thousands of innocent people in the 1930s.
\item How clever of Kenney.  He hates gays and so he found a way to put them back into the closet.  Brilliant indeed.
\item CTV News Montreal headline today: Visiting imam denounced for calling Jewish people 'evil' Where are the voices of protest and uproar over this ???  And one questions why there is Islamophobia  ??
\item I see that you, Motley, care more about semantics than facts. You can always find an angle that justifies white racism. You would make a 'good German'. They never asked where the Jews disappeared to.
\item How to know if your child is transgender'  The real problem for grownups is how to know if that hott person you met at the supermarket has the correct parts for what the spaceship pilots call 'rendezvous and docking.'
\item It's true Harper was a devout Christian and he was a disaster.
\item Both Climaxica and colin7 are right. Faith and fantasy feed the soul. Science and the reality of mortality feed the brain.
\item So, you feel that WORKING FOR the people running the death camps which were killing communists, Russians, Jews and other undesirables was preferable to STOPPING those deathcamps from committing even more war crimes and mass murder? With friends like you, Freeland needs no enemies.
\item Many trans-gendered agree with you.
\item And they absolutely LOVE them some muslims who DO treat women as property! A sort of hero worship.
\item Adam Lanza... Dylann Roof... Jeremy Christian... . To pretend that one race isn't contributing to the problem is just plain ridiculous.
\item I've heard that one before 'I have a lot of Jewish/Black, etc. etc. friends. ' And they are almost as good as 'real' people'  is the sub-text.  'Shanty Irish' and 'Lace Curtain Irish'  equals the 'N-word'.    Pure Bigotry.  https://en.wikipedia.org/wiki/Lace\_curtain\_and\_shanty\_Irish
\item In the interest of 'firsts' and political correctness, I won't be satisfied until we get Hawaii's first transgender Tongan-Vietnamese midget as police chief.   Hiring a regular white woman is such a huge disappointment.
\item https://takingnote.blogs.nytimes.com/2015/06/19/lawmakers-push-to-end-military-transgender-ban/ Lawmakers Push to End Military Transgender Ban Congress has the power to do what Congress did. President Obama signs legislation. He couldn't and didn't over-reach his powers as the fascist Trump is attempting.
\item There deserves to be a war on orthotoxic faux Christianity.
\item Indeed. When she visited Ukraine she did not pay homage to the victims in Baby Yar . They were Jewish massacred by Nazis and Ukrainian collaborators.
\item Interesting how this 'cosmic, Jewish, zombie' keeps our kids from killing each other.
\item 2 of the 5 were native themselves, one of them was gay.  Many of the people in the ' indigenous' ceremony were not even natives but Social Justice Warriors of all races.
\item Typical Marxist Pfleger. Has he ever sought the conversion of any non Catholics to the one true faith. The 'violence' of damnation is far worse that that which the gun or knife can inflict.
\item So you are a neo-nazi using a meme from 4chan by calling other non-jews Goyim?   Do you find satisfaction in running down other ethnic/religious groups? Do you not have empathy?  I know you are probably trolling, but seriously taking the Nazi road is pretty dumb.
\item What happens when transgendered people go off their hormones? How does that affect their fitness for active duty?
\item The murder of transgenders this year has been one of black men killing black transgenders.  Great denial out there in GLBT and BLM community on this problem.
\item Gay promiscuity and fornication is wrong, which is why, because some kind of sex is moral for them because they are differently ordered, not disordered, the Church should offer a marriage right, or rather reinstate the one it had in honor of Bacchus and Sergio.
\item Once again an attack on Christianity.   We are about to change Canada and there will be no turning back.   SAD
\item I have herd of bone heads but those that oppose Trump's desire to stop Islam should take not f the following and please put a cork in your poorly educated brains DO A STUDY OF ISLAM FIRST !  https://www.youtube.com/watch?v=axe\_NcIEfsU  http://jesus-is-savior.com/False\%20Religions/Islamic\%20Muslim/islam\_exposed.htm  http://www.informafrica.com/afrikan-consciousness/religious-slavery/exposing-islam-religion-the-quran-and-barbaric-muhammad/  http://www.exposingchrislam.com/  Deception  http://www.meforum.org/2095/islams-doctrines-of-deception  http://islammonitor.org/index.php?option=com\_content\&id=4394:great-lies
\item The anti-Semitic hatred has been unleashed by elements of the political left who hide their anti-Jewish bigotry behind the supposedly respectable label of anti-Zionism.
\item Isn't it really a three state solution? Jordan is about 75\% Palestinian heritage and Jews are not  to live there so with a Palestinian state in the West Bank with no Jews there will be two Palestinian states.
\item So as a Muslim what have you done to help your religion move away from extremism, other than posting here that is?
\item Ghetto Hill doesn't realize that Trump has a Jewish son in law, convert daughter and Jewish grandchildren. Also a black friend named Dr. Ben Carson. Not the traits of a white supremacist bigot.
\item They are in this case - do you seriously think that only religious rights are at stake here?  In fact, that was the concern - Christian intervenors allowed, LGBTQ, not so much.
\item Jews are the worst people on the planet. They lie, cheat, and destroy entire nations. They have no boundaries, moral or ethical, when it comes to dealing with the gentiles. They only thing they worship is the almighty fiat money. Those are facts.
\item his call to temporarily ban all Muslims from entering the United States.'  I guess he needs to watch Blazing Saddles again and listen for the comments about the Irish.
\item how would a gun registry have prevented attacks by these muslims ?
\item The power of the LGBT gang is terrifying. If transgender do not identify themselves it is deceptive to a person who is hoping for a normal opposite sex relationship. The surprise and embarrassment that would come after unclothing is shocking!
\item Agree.  Can't see what all the fuss is about having a gay scene and gay character.  Especially when the main theme of the movie is beastiality.
\item Canada has no balls when it comes to collecting on taxes. This is why despite all its problem the USA is still world power \#1. They collect taxes based on citizenship not residence and they don't mess around.
\item Breaking News:  Donald Trump opens fire on 5th Avenue--several wounded; in a strong show of support, pro-life Catholics rapidly come to his aid.
\item my, aren't we a special snowflake?
\item Ford's biggest strength was his stand on family values, which immigrant communities supported.
\item He is another gay one and they wouldn't touch him with a ten foot pole.
\item The Human Rights Watch report linked in the article is a must read.
\item Maybe you should try using water bombers instead of F18s...
\item Christians, especially evangelicals, are, almost by definition, gullible. It is  not surprising at all that so many support Trump.
\item If this woman was black or brown and a Muslim the jury and the courts would impose an immediate, maximum sentence.
\item So what are you proposing - other than more flooded basements.
\item That’s racist, xenophobic, islamophobic. That’s the extent of debate from you and your ilk. I’ll now gladly just call you mentally retarded and move on to someone with the intelligence to Debate in the first place. That’s what happened to debate.
\item Between this gang and the Catholic church, there isn't much respect for organized religion these days. At least they aren't sexually molesting innocent little boys like the Catholic church.
\item That's one reason the conservative muslims  murder others to try to convert/ 'align' rest of world to their views.
\item Your comment about the closet is getting old. Any leader in the western world is protected when attacked.
\item Oh Yes - The Media IS FILLED with account of Christian Terrorists blowing up planes, people, launching Jihad etc. etc. etc....While we are at it, PLEASE share some stories of Christian Polygamists and Beastiality as well....Yes, that is what we thought.
\item Well said, Heckler!  And I believe you are on to something important: whatever difference there may have been in the past between a murdering, marauding Muslim extremist and a murdering, marauding Democrat Party extremist now would appear to be approaching the vanishing point.
\item .  Hitler/Nazi supporters and racist white supremacists. These people are legally allowed to march (armed) through the streets of America? Because of free speech?   If they call on their supporters (as they often do) to kill all Jews and destroy the State of Israel, is that free speech as well?  .
\item I personally see the sexual offender registry as the digital equivalent of the pink triangles that were used to identify homosexuals in prewar Germany.'  ===  I'm pretty sure Mr. Wilde didn't just equate a heinous felony, a choice to violate another human being, with homosexuality.   Did he?  Nah, couldn't be...
\item Will the bishops who advocate the denial of communion in other matters, I wonder, recommend the same for racist Catholics?
\item It'll deteriorate, as it already appears to have done, into usual Catholic cultish 'Religious freedom for Me but not for thee.'
\item Better to brainwash them about Jesus Christ, the evils of s-e-x, the need to keep guns, the horrible things Obama has done, the damage illegal Mexicans cause, etc etc etc?
\item You must think it is un-Christian to carry a gun.  But when did Christ say it's impermissible to kill in self-defense or defense of a third party?  He didn't.  In fact, the Catechism correctly says that such self-defense is a duty.
\item Come in your car, come on the bus, crawl out of your box, every tranny, woman, and cisgendered male has a claim on the impeachment of this fool!  Just bring your own hypodermic needles
\item Maybe Muslims should consider their plight in today's world and realize that they are a foul philosophy and should change there ways and stand up and denounce the killings and atrocities of their own doing first....Just do not like the crap they are spreading in the world...
\item Trump is under the opinion that transgender 'bathroom rights'  is an issue to be regulated at the state, not federal, level which I believe to be correct. The Feds have many issues to confront, where a child goes to tinkle at school shouldn't be one of them.
\item So apes officially have more rights than unborn humans. Way to go...
\item I'm pretty sure no matter what your views on transgender athletes, it's never ok for a grown man to ask to see the genitals of a teenager.
\item SO MUCH PROPAGANDA!!!!!!!!!!!!!!! Even the NyTimes reported how Soros and Clinton-financing Soros funded these marches, the man who was a Nazi Collaborator who saw his 'fellow' jews get sent off to the ovens. He is insane, mad and driving much of this madness to overthrow actual democracy.
\item Of course you'll agree that it didn't cost Putin a dime. And, you'll probably also agree that a good portion of the 52 billion actually went INTO his pocket.
\item I'm also sure that the Dem support of bathroom options for transgenders didn't help.  Biological males have no business being in female-only spaces.  No means no always - no exceptions.
\item You mean the pope does not specifically command the President to outlaw abortion and gay marriage but very ecplicitly references the poor and outcasts?  Trad brains must be exploding!
\item Change it to Jew hating crowd then you cannot evade what I mean.  What a dopey reply.  'Antisemitism (also spelled anti-Semitism or anti-semitism) is hostility, prejudice, or discrimination against Jews. A person who holds such positions is called an antisemite.'
\item You have my respect and thanks. (Oncologist in Ontario)
\item Right because that's what being transgender is. Just waking up every day and claiming to be one sex or another depending on how the mood strikes you. That is exactly how it works.
\item The truth is that Roman Catholics and Protestants have more in common theologically than they have differences; this needs affirmation and celebration. The differences are predominantly (if not only) ecclesiological. It is ridiculous to allow ecclesiology to dictate relationships...at any level.
\item Hirono, who serves on the Senate Armed Services Committee, said, 'Transgender Americans serve our country with honor and distinction.''  And their names are???..........
\item Supplemented by the Jewish truck drivers attacking Christmass parties
\item White Catholics were very narrowly in favor, 50 percent-49 percent.' How wonderful!  Really something to be proud of -- in the true tradition of Jesus who always said that those who worship differently ought to be cast out.
\item You fail to mention Ruse is listed by SPLC for just this type of behavior and actually much wirse, including stalking gay bloggers to leave obscene comments. What Ruse did with Martin is mild. Ruse is totally obsessed with gays.
\item I have been a member of the Catholic faith my entire life.  I am sorry you find the Catholic Church so disappointing.
\item Why would the smiling, lying, Christian crusader Mike Pence need a lawyer for...............for lying?
\item http://www.independent.co.uk/news/world/gay-lesbian-bisexual-relationships-illegal-in-74-countries-a7033666.html  You're welcome.
\item the real victims are the women.' Yes because they are wearing hijab, a women demeaning and subduing Muslim custom imposed by inferior Muslim macho men.
\item What does the Church's TEACHING authority have to do with pedophilia? The 'sex abuse problem' has nothing to do with 'clerical control' other than the lavender mafia admitting far too many homosexuals into seminary.
\item SDPW - problem is, they were elected to serve the people of Canada, not to serve themselves.
\item Black Pride = being black and proud Gay  Pride = being gay and proud White Pride = NAZI!
\item No mention of the religion that preaches hatred of Jews in their places of worship.
\item The globe and Mail, where Wentes opinion keeps on crashing and burning. Good for a laugh though...
\item wolfhall, If Obama's politically correct capitulation to gay marriage was his greatest 'accomplishment', it's no wonder liberalism is dying in the US just as it nearly died in Canada under Jean Chretien.
\item Anti-Semitism in America is coming from all those useful idiot undergrads and their professors.   They hate Jews and love them some Palestinians.
\item I guess that they now know that being fellow Muslims counts for nothing when dealing with extremist and criminal elements.
\item I was brought up catholic, and the church was quite clear, masturbation was a sin.  It wasted life.  I guess the priests in your parish were a little more uhhm open than in mine.
\item Thanks for that reasoned opinion. We should also gear post secondary education funding to employment opportunities.
\item because she's black \& a tranny
\item Really?  They're not focusing on transgender bathroom rights and strong-arming universities to hire more women?  What will Justin talk about?
\item Dude was an atheist who hated Christians.
\item >> But they didn't kill the Jews by the thousands or millions  They didn't? What kind of 'Hindustan' math are you using?
\item Right. A racist, sexist, bigoted, adulterous liar of a president should be supported, and those who voted for him praised.  Previous conservative presidents at least gave lip service to their Christianity. Do you really see Trump doing even that?
\item You have to admit the man is two faced. Witness the Alberta comments. He is above personal embarrassment.
\item I want everyone to know, when I get busted for my next big felony, I am a lesbian trapped in a man's body and want to go to the woman prison. (Not the man's - yuck)
\item Yes indeed. The New Black Panther Party is a virulently racist and anti-Semitic organization whose leaders have encouraged violence against whites, Jews and law enforcement officers.
\item Ontario Liberals are not BC Liberals.
\item Looking forward to Russell's next installment, which will mock Jews, suggest watermelon spritzers for the next BLM activity, and feature a picture of him making slanty eyes while standing in front of a statue of Buddha.
\item Trudeau and his feel good government are weak kneed. The Americans will walk all over us for the next four years.
\item last time I looked the charter applied to the forces, unless your friend Justin changed it - Justin is into Diversity not white males unless they are gay and march in Pride Parades
\item Dude, don't point out supposed grammar mistakes if you don't realize that 'unnavigatable' isn't a word. Unnavigable, my man. Unnavigable.
\item The picture in the newspaper is interesting.  A presumably black, gay female officer is now excluded from a parade that BLM has really nothing to do with.  Amazing!
\item It is a matter of free choice. If the public believed women choose to be covered from head to toe then it would be ok. But, it appears most women have no choice. We can't allow that in a free society.
\item Subaru website says 1500 pounds.  To be safe with the tranny I'd say 1000 pounds!
\item Does the Catholic Church force nuns to wear uniform, and don't they force nuns and priests into celibacy.  To me that is more repressive!
\item Yes. All those over 60 should be denied the right to vote, anywhere, for anything. However, they should still be required to pay taxes.
\item I wouldn't want to be expected to take orders from a transgender dude/lady.  If they can't make up their mind on that stuff, will they be capable of big decisions?
\item Those socks look a lot like those worn by the wicked witch of the West in the original Wizard of OZ.  Any transgender serving in the armed forces is guilty of fraudulent enlistment.
\item Will he defend the transgender bathroom guidance that Obama issued for  public educational institutions?  He said during the campaign anybody should be able to use whatever bathroom they wanted, so one would think he would defend this in court.
\item If the Nazis are eliminated then the Jews are OK.
\item How do you know the flu shot made you sick? Just because you get sick after the shot does not prove it was caused by the shot.
\item how shameful, a jew practising eugenics
\item You're so rad. What's the point of being Catholic if one can't angst over one's salvation?! :)
\item The financial sink hole of the UN makes the Wynne Government look positively Thatcherite in its austerity.
\item Political power has been restored to its natural place: Central Canada.' Ugh. What a load of rubbish. Mason, in what world is that kind of attitude acceptable?
\item Was Scott Ostrem a Muslim?  They should deport his family and execute him.
\item Re: 'People who claim to care about spreading hate in the name of religion are remarkably silent when hate is spread in the name of Allah.'  No more nor less so than they are remarkably silent when hate is spread in the name of the Christian God.
\item Obama and Kerry have been happy to 'stand idly by' for mass murder, decapitations, burnings, sex slavery, ethnocultural cleansing, etc, etc, etc. But put up a Jewish subdivision and all of a sudden they're not going to stand idly by, no sirree.'  Mark Steyn
\item You really are the definition of stupid. Try reality sometime... you'll like it.
\item I greatly admire both Mr. Flaherty and Mr. Martin. Both were very solid, competent Finance Ministers who recognized the importance of balancing budgets and keeping Canada's debt-to-GDP in check. Best wishes to Mr. Flaherty.
\item Patience is a virtue.
\item Trump supporters are people who follow only Fox News (not about news), Rush Limbaugh (was convicted of sending his maid to buy thousands of prescription pills for his consumption), Gordon Liddy (convicted as one of the Watergate burglers), etc.
\item So you equate being transgendered with pedophilia? Do you think transgendered people should be put in jail? Anyone notice any inconsistency here?
\item It has always been thus.
\item Jews were not engaged in terrorism against Germans. Palestinians are engaged in terrorism against Jews.
\item I thought he had. Did he not say he felt that Canada would be more helpful as the coalition partner that would help the refugees in the camps?
\item I am a great supporter of well-paid jobs IF THE WORKER DESERVES ITMerit and educationNot well paid just because it is a government union job
\item where did he blame the victims?  He's blaming a clash of ideologies and cultures.  The victims were individuals, not a culture. . although I suspect you would blame western culture for fostering an environment that leads to muslim terrorism Alceste.  Am I wrong?
\item Once upon a time, America ignored the slaughter of Jews. Once upon a time, America put Americans in concentration camps. In the present, America is supplying the illegal drug demand that fuels the killing and violence South o our border. In the present, America is the force causing the violence.
\item McHale, since you are in schism with the Roman Catholic Church, how do you reconcile that with your extreme interpretation of extra ecclesia nulla salus? You are proclaiming that you, yourself, are damned.
\item It is tough to get by all the censors when commenting, but one must respect that the Journalists do have bosses and sometimes those bosses do not always want too much 'truth ' to get out there.
\item thats literally just a fancy way of saying 'muh women rights'
\item Yep, this is thanks to Bush-era nonsense put out there as red meat to the Christian Taliban. IIRC, this is hardly the only case like this.
\item My bank has the same policy.  I told them I would comply when they insist Muslims do the same.
\item AlwaysThere:  Great Point, where is DHS anyway???  I believe DHS is looking the other way.   As you stated earlier,  the TRANS whatever folks are at the top of the PROTECTION LIST...................
\item Malcolm:  We know that a 'lemon party' is an Orgy for old gay men.  I'm old, heterosexual, and seldom go to any parties.  I've flagged this post as a crude, ad hominem attack.  Gary Crum
\item They are Muslims.  Trump sees them as people with no worth.
\item The American Alpine Club has created a Sherpa Support Fund that will raise funds to assist the families of the Sherpas who died. I encourage and challenge anyone who has climbed or tried to climb Everest to donate. Www. americanalpineclub.org
\item And just imagine if you are a teacher, school secretary, or janitor looking for a job.  Those without the Catholic church membership card are not welcome to apply at these schools.
\item But there were quite a few Jewish scientists in the Manhattan Project so blame away with irrelevancies.
\item There is no logical argument for outing gay teenagers and there is no logical argument for withholding factual information related to sexual health and wellness.  The UCP are revealing themselves as a group of anti-science dinosaurs hiding behind out dated religious concepts.
\item Super fakey bigot racist sexist 'christians' dont like to think too hard or deep ...
\item I won't bake you a cake because you are Jewish.  Take your business to the baker down the street.  He serves your kind.
\item Oh me oh my THE SKY IS FALLING THE SKY IS FALLING! Watch out for Andrew Scheer! btw how can he ruin our country since Turdeau already has.
\item Fair point. The sexes are equal. Women has strived for decades to be treated equally. So suck it up when someone treats you equally, but unpleasantly. It's less about your gender, and more about YOU as a person.
\item Apparently some of the trans-soldiers feel like they were fired via tweet. In any event, these sorts of communications are not fitting of a true leader. I find them shameful.
\item You should try using punctuation. It makes you appear a bit smarter, even when you make a claim that no one can substantiate.
\item It would be fair enough to do so if large numbers young non-Muslim French men started saying they were there to 'die for Jesus' or the Napoleonic Code while committing crimes.
\item An ignorant comparison !!! 6 million Jews exterminated just for being Jewish. Truly entering the mind of the left is an exercise in madness.
\item Entirely different subjects. You might as well blame Jews for Hiroshima because of Einstein.
\item The mainstream Jewish organizations in the 1940s were brown-nosing the British. The Irgun drove them out. But as I said, the 1940s are not analogous to today; there are no similarities to today.
\item grizzled'? all journos and columnos, including Ms Wente, should retire at 65; hey it's 2016!
\item I would presume this move is to stop the transgender from joining the military for paid sex changes on the public dime.
\item Choose? Are saying that being gay is a choice? That's been debunked decades ago. When did you make your choice as to your sexual orientation?
\item That was Brennan, under Obama, not our good American, Christian president.   You really should not make baseless statements to fuel the dopes who believe this nonsense.
\item You asked who the parents complain too. The answer is the school district.  'The Association of Alaska School Boards is also urging school districts across Alaska to adopt transgender policies. The school districts have to get into the nuts-and-bolts policies.”
\item You draw your brush too broadly if you believe that 'Gerson's God'(particularly the Catholic one and the Baptist one) supports abortion or anti-capital punishment, just to name a couple of issues which don't match up to your interpretation.
\item dear scottd  Pride gets public funding for gay pride and gay rights  yet allows non-gay politics to march like Queers against Israeli Apartheid and Black Lives Matter  is this not incompetence? using public money for purposes the money was not intended for
\item Don t forget to invoke the saints!  Surely the saints in heaven will support you in your support for breitbart news, which is a bulwark of christian ideals and veritable font of truth.
\item That's all baloney nicky/truthhurts/retiree. You have no proof for any of that. You also need to watch your mouth with the insults. Oh, and try going back to public school to see if you can finish this time.
\item your days are numbered there is blood on your hands!
\item That claim is false. Ultra-Orthodox Jews have mounted terrorist attacks on Palestinians and foreigners since before Israel was created in 1948.   https://en.wikipedia.org/wiki/Jewish\_religious\_terrorism
\item Pass the salt and pepper please. Democrats like road kill too, kaine threw himself under the bus by signing on with the witch. Debbie Was A Man, transgender meat ala cart.  Bon a petit
\item Obviously it must have been Martians who gave him a majority government.
\item Neither the Gay Community or BLM deserve any respect for excluding uniformed police officers.
\item Climatism is a religion with amazing similarities to Catholicism. It has original sin, fires of purgatory, the flood, pestilence and the plague of locusts, sinners, sin and repentance, redemption, guilt and forgiveness, indulgences, incantations, hypocritical priests, agnostics, faithful and the unfaithful.
\item A ridiculous article.  ...'it was an existential attack on the entire LGBTQ community, particularly gay people of color.' Ohhh Pleeease!   As  Xavier\_Malcolm stated: '...we’re not buying into the drama of the BLT-GQ pity party.'
\item Direct Quote: And Spencer made it clear that white-only means Jews aren’t invited. They have their own identity, and it isn’t white-slash-European, and that’s that.  “Jews are Jews,” he said.
\item It's cardo212. You get real with your crazy, paranoid views about transgender people serving in the military, the ACA, and the Paris Agreement.
\item I'm not even going to read this. I know it's transphobic 'hallelujah jesus' drivel.
\item (((they))) are the problem, nothing changes.  Its tribal.  Open your eyes.  Its the jews, they are all jews
\item Poor people in third world countries are under attack by 'christians' every day---maybe it's time you get your head out of the sand and start paying attention...
\item Having spent time in a number of Muslim countries please allow me to add to that:  For Muslims 'It's ALWAYS someone else's fault'.
\item And when justice is done, we must accept it. Whether we like it or not, even you Zoe101
\item Inspiring!! First transgendered woman in the pagent!
\item For The Globe's editorial board to stop being so schizophrenic? I agree with you there.
\item The police do need evidence of the motivation other than the victim being transgender. The evidence is not in this article so nobody can judge the police's motive from just reading this. Motivation is also hard to come by and is not needed in a clear cut murder case.
\item why does this old hag of a writer hate visible minorities? Her columns are reliable for taking cheap shots at marginalised groups. Try attacking the Jews in the same fashion and see what happens.
\item I wonder if Ms. Kinworthy would find it 'educated and reasonable' for the ASAA to adopt the NCAA's policy regarding transgender athletes participation?
\item Is the author suggesting that it is OK to align with the  USA that has invaded Iraq, Afghanistan, and drone attacked Pakistan and Yemen etc and a new president who has very racist views on Mexicans and Muslims.
\item If a poll were taken of most black people and most gay people, the police would be welcomed. A tiny minority of hardcore black racists like BLM Toronto should not be running our city.
\item Was the Jewish community invited to send representatives to this conference?  If not, they should have been.
\item Lefties are stupid then... because crazy people don't ever get an AR and shoot up San Bernardino or gay nightclubs...  which makes me wonder why are these shooters always LIBERALS?  Grow up.
\item The only way a Muslims will reach out to embrace Mormons or any other religions group is from behind around the neck.
\item Complete disdain and hatred towards Canadians born in Canada WHERE IS YOUR EMPATHY FOR US! NOWHERE BECAUSE ISLAM DOMINATES AND CONTROLS OTHERS THROUGH RAPE AND MURDER, A FASCIST IDEOLOGY!
\item Man oh man am I glad 'bible thumping' is not part of Canadian federal politics.   Evangelicals are as bad as sunni wahabbis.
\item They're not Christians, they're ChristianISTS. They wish to spread their religious beliefs by force.  They're religious radicals in the same vein as the radicalized Islamists who bomb everything.  It's just unfortunate that you rarely hear Christians condemn the radicals in their midst...
\item For all the issues that divide Americans and Canadians, there is one thing that both these countries can agree upon, and it is this. Tory times are indeed sorry times.
\item You invite a guy into your house and you don't know he's Jewish? You just met him at the mall?
\item I remember in Canada it was not a civilized discussion, but rather rearguard action. The anti-marriage side didn't want civil unions either, until it looked like gay marriage was coming in, and then proposed civil unions as a 'compromise'.
\item All the issues with men harassing me have been the white men who have voted for Trump.  Working class types who don't seem to follow basic ideas about manners and common decency frighten me more as a woman than some vague scary foreign Muslim threat.
\item Everyone should be upset with the little potato doper and his billions blown on Communist Chinese 'schmoozing' and flooding the country with Muslims that no one asked for or voted on. But no money for the health care system and citizens in need.Pathetic!
\item Until feminists take on islam and how it treats women, the entire movement is a total farce!
\item What do other countries do about this ? Or is it just the US that has this transgender nonsense?
\item Our best friends are democracies and among those Britain, Australia, New Zealand and United States (sans Trump) stand out, still.
\item Are you Obi Wan Kenobi? Is your next line to tell us that we will never find a more wretched hive of scum and villainy?
\item When asked if he were a Muslim, the son should have replied: I am an American, my religion is none of your business.
\item By JewsJuice I meant the holy wine offered as blood sacrifice on the altar, as well as by McJesus bits I meant the flesh of Jesus in the form of little, round, baked waffle pieces.
\item We've got to get these assault trucks off the street. Nobody needs an automatic truck....especially one with 18-wheels.....4-wheels is enough for anybody. Only the military should be permitted to have 18-wheel automatic assault trucks.
\item There are more important things to worry about instead of bathroom laws and transgender rights. Once again, USA  is the laughing stock of the world.
\item Scientific American cites studies saying that the additional medical cost of transgender soldiers is between 2.4 million and 8.4 million per year. That is literally nothing, less than the cost of toilet seats. https://www.scientificamerican.com/article/cost-of-medical-care-for-transgender-service-members-would-be-minimal-studies-show/  https://www.theguardian.com/us-news/2017/jul/26/trans-health-cost-us-military-budget-pentagon
\item "Canada is regarded as extremely well-governed ..." By whom?
\item I disagree. It is true that a belief in gods played a big role in how the world developed, but there can be civilization without gods....perhaps one day we get there.
\item What your weird hypothetical has to do with this election is a mystery.
\item Including the terrorist-supporting Jew-hating Palestinians and their Hamas brethren, right?
\item The ideology of Islam is in direct conflict with the constitution on many counts. It is unconstitutional to let muslims into the US.
\item You can be as angry and insulting as you like, but I will choose to obey God and demand that my church do the same.'  ...yet, American Christians are so incredibly hypocritically selective in obeying Gods word(s).
\item I fail to understand how calling God 'hir' insults trans people.
\item It shouldn't be a surprise, it doesn't take crooks long to figure out loopholes if their commission depends on it.
\item Then I would respectfully ask you to substantiate your arguments with proofs. No where is it taught that women are secondary to men, rather there are differences that have to be recognized. They are equal in justice.
\item As a 'christian', super fakey 'believer' in the Flying Spaghetti Monster, do you ever wonder what the hot burn of HELL will feel like when you die ... ?!  Your voting record alone will put ya there ... since you 'believe'.
\item Quebec independence is coming. God knows they deserve their freedom. After 250 years. The dream will never die.
\item The best thing the Ontario Liberals have going for them is Tim Hudak, the master at campaigning for opposition leader.
\item Just another evangelical Christian extremist being a bigot based on what he thinks his imaginary god tells him to think. I wouldn't step foot in his bakery.
\item It's just hilarious how blind the progs are. To bad it is so sad.
\item Written like someone who has an all powerful protector to deal with the cares that every other country has to deal with on its own.
\item ...Move on and solve the issues in your community and stop seeing yourself as a victim.,,' same for Jewish community ?
\item It's great how liberals think our own government is more evil than muslim terrorists. Go ahead, give all your jihad friends my money if it makes you feel better while sipping your wine at night.
\item tick tock tick tock..... time is running out for you lot!!
\item Fake news. Check other sources for what was really happening (see link below).  The protest was against  imams within the mosque preaching death to Jews and infidels.  http://www.therebel.media/the\_other\_side\_of\_the\_toronto\_mosque\_protest
\item Probably the easiest thing for the government to do would be to stop the practice of using faux private member bills to advance its agenda with minimal scrutiny.
\item To identify the truly sick racists google: chief rabbi of Israel says only purpose of goyim is to serve jews, life of goyim worth same as donkey.  Netanyahu says this jerk is the greatest mind of this generation.  http://www.timesofisrael.com/5-of-ovadia-yosefs-most-controversial-quotations/  ,./
\item Dude, those lies don't work anymore. The world is onto you. Israel is a democracy for Jews, discrimination for Palestinian Israelis, and apartheid for the West Bank and Gaza.
\item Adolf Hilter was actually left wing. The Nazi party was very socialist.'  If you knew anything about the history of Nazi Germany --- persecution of Jews, intellectuals, communists, social democrats, etc -- you'd realize how ridiculous your statements are.
\item Jews dont have honour killings of women who don't cover their heads.
\item Oh, look at you, making fun of the way Jewish people talk, thinking you're making a funny joke, that isn't.
\item This makes me want to weep for the government that could have been.
\item How about Trudeau apologize for his Pro-murder (aka Pro Choice) and gay marriage stance??
\item You're a cockroach. look sharp
\item Muslims...driving the wedge into the log, one stroke at a time.
\item You are partially correct.  I looked at the charts again and indeed, racial crimes against blacks did exceed crimes against jews.  However, your assertion that  hate crimes against wiccans exceeded  hate crimes against jews is laughable.
\item And if the business owner didn't want to serve a gay couple, you would be the first outside screaming and crying about it.  You want the right to discriminate but do not want to extend the same right to the business owner.  Typical hypocrite libs.
\item If that many!  I guess this is a lot like that 'one drop' rule in the old south.  Just one gay marriage will destroy all heterosexual marriages in the whole world!
\item Oh, I see. My freedom of religion is an affront to their guilt. Thanks for the clarification. Refusing to 'celebrate' gay marriage is some kind of ban. OK.
\item Marx, That is obviously not true, and it says a great deal about you to even suggest it.
\item Oh no -- are they doing that stupid Pokemon thing too?
\item I wouldn't pay a penny to hear Trump's personal bidet regurgitate Tony Perkins gay snuff porn fantasies.
\item Steven - If it is not gay marriage or abortion, I would count of silence.
\item Dan - Fair enough.
\item Transgender persons suffer from a medical condition and require extensive, expensive treatments that are not compatible with any deployed forces. Many other medical conditions are excluded from service for the same reasons. It is not that they are morally unworthy. Most Americans haven't really thought this out very well.
\item The only troll is Azira herself, trolling for Islam and for western civilization's submission to the Koran. Her hijab is the sign she handed her fate to Allah. Giving up free will is just one thing Muslims ar expected to sacrifice for their religion.  3rd  posting.
\item Trump is an atheist who manipulates poorly educated evangelicals to his own advantage.  I find Trump easy to see through.  He is a cynical TV entertainer and shibai artist.  So sad to see any Christian fall for his nonsense.
\item He is no orator and no speech of his will go down in history... his delivery is stiff and halting and when TelePrompTerless he wanders off topic and makes remarks that he regrets later as he did after his red line in the sand speech.
\item Wrong. Oh, yeah, they're every-ready, to govern, alright, at the drop of a hat (or a writ) But the questions are: (1) Do they deserve to? (2) Are they able?
\item We don't need life without parole. We need the death penalty.
\item Coming from a person with an ethnic background steeped in Jew hatred, your comment is not surprising and entirely predictable.
\item If Jesus intended to establish NO priesthood and did not--then there is no problem and no argument.  If Jesus established no priesthood and had nothing good to say about it, the problem isn't that the Church won't ordain women, but that the Church is ordaining men.
\item Orthodox Jewish women are not at risk of being stoned to death or drowned in their car driven off a cliff into a lake  if they disobey.
\item Last time I checked there wasn't any Jews shouting death to Americans
\item No mention of an under the table boycott of Target for it's ever increasing leftist policies culminating in outright anger at their transgender bathroom policies.  Not sure what the affect that has been but should have a clearer picture after the others report.
\item Those events exist. Look at 'black bike week' in Myrtle Beach and all the gay cruises. There is absolutely a double standard. Just try setting up a whites only 'Ivory Awards' to the corresponding blacks only 'Ebony Awards' and see how that would fly.
\item Indian are probably the ones who will bury the west once for all, just look at the pace all stuff are outsourced to there, even English.
\item So the transgender troops expect the military (meaning taxpayers)  to pay for their conversion surgery.
\item A nice Jewish lad... but no actually the 6 pointed star is associated with the Gangster Disciples and their affiliated gangs.
\item Go easy on the Salt Ms Wente, we need you healthy and vibrant.
\item Agirl:  Congratulation.  You've sunken to a new low.  First you accuse President Obama of being a closet homosexual.  Then you belittle Michelle Obama as a 'cow.'  Have you no standards of decency?  Gary Crum
\item The many, many postings from the PMO here show their desperation. They're all over this editorial like they're cligning to a life raft.
\item light stepping Jesuit priests'  RD has to insert his fear and loathing of gays even into this comment.
\item Is it OK to call people homos?  Trump hasn't been sworn  in yet.  In any event, I would bet \$100 on one of Trump's sons killing the last gorilla in the wild.  Just one more accomplishment for those swell guys.
\item I don't think the big deal is that he is gay, the big deal is that he allegedly forced himself on to a minor.
\item Yes, predominantly white christian america is afraid of being invaded and colonized by another race, and/or religion.  Welcome to my world.
\item Homosexuality is a biological issue and not one of ideology.
\item I'm not surprised Barry got close to a guy making big donations.  Republicans would have done that too.  What is really telling are the close ties not associated with money.  Bobby Titcome and the tranny arrest?
\item If you have a better (or even a correct) answer why didn't you put it forward? But yeah, my assuming that 'Jamish Mafia' references 'Jewish Mafia' is just an assumption. Since 'racoon' didn't produce an answer what other options were available to me?
\item ....Shorten the track to citizenship for immigrants who agree to the same....'Similar programs already exist, and they simply do not work.
\item The face of evil, another super fakey 'christian' doing their best to cause harm here on earth ...   Her brother started Blackwater, nuf said.
\item Try rampant violence in the gay community....   https://www.lifesitenews.com/news/cdc-gay-lifestyle-fraught-with-violence  Try out of control disease in the gay community...
\item Tell that to the ashes of the Jews in Auschwitz etc....
\item Sure.  Why let facts and reason get in the way?  It's always better to argue a case from a platform of complete ignorance.  Just ignore the fact that transgender people have served for decades.  Why think?  Let me guess .... you're a Trump voter?
\item Sorry you lost your job, friend.   If you were female, gay, or a visible minority, I'd give you a free selfie!
\item Right on. G\&M is accountable for helping to elect the least democratic gov't I have seen in my lifetime
\item Another Communist Jew.
\item If someone has testicles they are NOT a 'transgender woman' but a male pretending to be a female. End of story...stop the PC lunacy.
\item everything is a protected class now a days.' Except the beleaguered white, christian male, amirite?
\item You do realise the Jewish people essentially dont believe in the new testament, right.  The messiah has not yet come?
\item @denglish4 Wasting all the young precious life in pointless praying are disturbing. Teaching them people that have different faith than Islam are stupid/Infidels/evil are disturbing.
\item You have our sympathy and support.
\item Not at all.  Transgender troops have served America well since the 18th century hon.  Trump's orders will be ignored by the Pentagon.  He is a nasty, truly immoral President who has set us back decades.
\item Surely not the worst we see online. The worst has been from those oppressively against gay men.
\item Empathy. Compassion. Intelligence.
\item Broglio 'backs transgender ban, but says human dignity must prevail'.    So he backs banning an entire group of human beings, albeit in a humane, dignified manner?!  Jeepers, they looked better fighting for glutenized hosts!  I'm so ashamed.  This is not a 'religion' worthy of supporting.
\item It wasn't any shadowy international ghosts who have been trashing Jewish graveyards here.  And the white nationalist lingo identifies you as one of the tribal followers.
\item Anyone who ascribes to the will of Islam and carries out the evil deeds of ISIS is the very definition of *'terrorist.*'  This maniacs ignorant family has no clue what radicalization tactics Muslims use. This animal was killed by good guys with guns, and the sooner they're gone, the better.
\item New travel ban makes sense to me. If the Country cannot provide relevant information they should not be allowed to enter, Muslim or otherwise.
\item How many non-Muslims fear for safety ?  How many non-Muslim women fear to walk in some parts of European cities because of the clothes they wear ?
\item At least we don't have to worry about transgender bathroom issues on those airplanes today.
\item To help with Ebola DONATE to Doctors Without Borders (MSF) www. msf.ca
\item Proud Boys, sounds like a gay porn movie.
\item From the first comments on this thread saying there were too many muslims shown and mocking Trudeau's 'ramadan socks' to the latest claiming Trudeau spoke too long and too loud and disparaging 'teepee' comments - there sure are a lot of miserable people here on a long weekend.
\item yeah, it reminds me of the rock band 'the who' kept coming back for another 'farewell' concert. We all love Justine
\item It would be easier to understand transgenderism if advocates could provide a definition of what it now means to be a man or a woman. What criteria would someone use to self-determine whether they are male or female gender?
\item You know, I have seen a lot more stories about U.S. Congressman misbehaving in public bathrooms then transgender people.  Perhaps they should be the subject of such an ordinance.
\item Furthermore this has NOTHING to do with hiding taxable income from the U.S. This is absurd. Where are you getting your information?
\item Yes, yes, yes.  He is slandering his confreres and fellow Christians to build himself up.  '*I* am not like *those people*.  They criticize; I think you're good just the way you are...'  The age-old patter of chatlatans and womanizing cads, but applied to a different problem.
\item Homefront support' is purely a social construct with no basis in reality for the vast majority of men. What's obvious and measureable is where the real support is - meeting the needs \& wants of women.
\item The burkini is not a political project'That's what you want people in Canada to believe. Europeans have finally woken up and know it is a political project. Segregated swimming pools for muslim women only are also part of the agenda.
\item I will also never forget the Shafia women who were murdered by their family members because they just wanted to live like Canadian women. This is where my 'Islamophobia' began.
\item And that a religion is misogynistic, treats women like property and throws gays off buildings.  That is not very nice either.
\item I'm a strong advocate of freedom of speech, and the right to practice your religion......unless it's Islam.
\item I'm starting to think Trump will be a great president after reading drivel like this from the G\&M. Don't you have more opinion pieces on transgender washroom selection?
\item Thanks for reminding us all to stay open to life, and all it has to offer us, throughout ALL of the ages of our own existence. Well done.
\item I don't know why he's so focused on the travel ban; we have the birthers, the neo-nazi's, the white supremacists, Russians, deplorables, evangelicals (the holy liars), the Real Americans, and other problem citizens he needs to be aware of......aoha and enjoy all the Fake News \& Fake Facts......lol
\item Jason Kenney has declined to comment on his own sexual orientation, as is his prerogative.  I hope he will accord young gay people that same right.
\item And the next time a Christian (Dylann Roof, Robert Dear (the Planned Parenthood shooter) and so forth) decides to commit a terrorist act against innocent individuals lets not sugar coat it by claiming that they were simply 'deranged individuals' but lets call it what it is - terrorism
\item You know what happened to me? I nearly converted to Islam in my 20s and then studied Islamic Law and came out of it horrified.
\item most jews have moved on  it is ypu marxists who keep the fear and  sadness alive becuade you feed your agenca off it.  you are  the true evil in our society. you divide  in the  hope of enslaving us we see you
\item Please come to Canada and run for office! We need to hear more of your voice. Bless you.
\item I point out Purg generalizes all gay men from the odious Milo, and my comment gets voted down? What the heck, readers.
\item Canada is a Christian country, there has long been a witch hunt against nonChrisitans, secular and agnostics.  Look at the long list of victimless crimes, the evanglalist PM Harper has created.
\item (Sigh) There never was absolute unity in the Catholic Church.  We are not, never were, and never will be a doctrinal monolith.
\item Oh no, this isn't about the kids. This is about the parents fulfilling their responsibility to care for their children themselves.
\item I just don't find her a very good representation of the transexual community. She just seems so self-absorbed \& concerned with such superficial issues.
\item So if a parish priest obeys the directive and refuses burial to a married homosexual, he is to bear the blame, not the diocese.
\item You've  got to be kidding! Judy Lamarsh? Shelia Copps? Jeezz. I'm waiting for the first transgender who-knows-what to get their face plastered on one. Mind you, at least that way, you'll have both sides covered.
\item And a ban on Muslims, you forgot that.
\item So you are a sane young black ( or non-white ) liberal college educated atheist woman ( or LGBT )...? ... or  were you born an insulting  ( mentally  challenged  ) tard. Oooops...turd.
\item Reminds me of an old Don Rickles joke. 'Why do jewish men die before their wives?.....Because they want to!!!'
\item Are you claiming that straight married men are 'homos?'
\item https://www.youtube.com/watch?v=PeXVP7TlSxY  Muslim Feminism for real.
\item Go nuclear. The Chinese are. We are being ruled by scientific enviro Luddites, so we will not.
\item I think a four-hour erection would be a greater distraction while on mission than the trans person that has to wear the same combat gear as every other man or woman in the unit. Why are we paying for this?
\item No. I know LGBTs who have been chased out of the Church. It was made abundantly clear to these 'intrinsically disordered' people that they are neither wanted not welcome in the Catholic Church.
\item Bookies in Vegas are offering 500 to 1 against the driver being a Christian.  I wonder if Obama would like to place a small wager?
\item Islam triumphant. yeah,  Oh boy.   Liberals, feminist, natives, LGBT  and socialists will love that.
\item Just another church scandal. At least this time it's not the Catholic church molesting innocent little boys again. Is there no end to what these 'people of God' keep doing?
\item Shakespeare was a transgender squirrel with an alien brain transplant. Most people know this already. I'm so tired of hearing distorted facts thru conservative 'Fixed News' channels!
\item So, he was simply a devout Muslim.
\item So transgender folks are like everyone else?  There's hope for you yet...
\item Not involving the issues of religious freedom, abortion or transgenderism.  He has my praise on those subjects.
\item No Catholic Church should ever shield illegal aliens.  This gathering is a toxic cancer.  This is the sort of left-wing Protestant nonsense the Church needs to not touch, it's a political tarbbaby.
\item you mean a transgendered horse.
\item Actually, the DNA testing shows that Palestinian Arabs and Jews (at least Sephardic Jews) are ethnically  identical. This makes sense if you consider that most indigenous Palestinians are the descendants of 'Arabized'  indigenous Jews
\item Bay Anderson go take your meds granny
\item This would be an appropriate time for Trump to admit that he lied about seeing thousands of Muslims celebrating in the streets on 9/11.
\item equal? worthy? What planet do you live on?
\item What will help the Muslim community be accepted, and feel accepted, by the larger society in Canada is if we don't discriminate against them. Quebec's law does discriminate.
\item Her Catholicism was warp and woof of her writing.
\item HAHAHAHA.... Clinton and 'progressive'.... Good one, sanctimonious one.
\item No, it/she is hiding in shame.
\item Just blame born again American Christian fundamentalists . They get blamed for everything one way or the other.
\item Can someone name ONE Muslim dominated country where things are just fine?
\item He wasn’t asked about Transgender troops.   He made a statement in general that cannot be argued with but that is completely unrelated to the discussion at hand.
\item Monica, not really. I am just being a realist. The Catholic Church is not really Catholic anymore. I'm stating a fact. Do you REALLY believe that the Catholic Church is any different than the myriad mainline protestant churches? What do you think, I'd be interested to know. I respect your insights.
\item Yep, that's sanctimonious, Sanctimonious.
\item It's also about time that you and your parents and relatives who have settled on lands belonging to the native peoples begin to evacuate and leave just as the UN resolution demands of Jews living in the West Bank. Get moving hypocrite!
\item You should be ashamed for writing such a hateful post and quoting the bible is particularly vile in this case.
\item Anyone who thinks that two men or two women masturbating, sodomizing, or fellating one another constitutes 'marriage,' and calls himself a 'Catholic,' is living in a web of fantasy too deep and dense to be unraveled by any natural means.
\item Nothing but spoiled little children raised in an artificial world of make believe.  When the war with Islam comes they will be the first to die.
\item There are lots of nationalist/sovereigntist movements that are not dirty words ... in Scotland, Catalonia and Quebec, for example. That's because they're not right-wing, ethno-nationalist, racist movements. Now white or Jewish or Islamic nationalism/sovereigntism on the other hand ...
\item I presume were talking about the 'poor, innocent' transgender Latina who stole a car and got shot? Has she stolen anyone else's hard earned personal property lately? No? Sounds like a win to me.
\item Now what? How about waiting until the legislation is actually tested by people with the authority to make a ruling?
\item One can see a thread of Islam-worship in this article's description of women.
\item Thank goodness for that. Now if the could only remove Catholic from their name and all would be well.
\item And let me guess. Your proposal for people being gunned down in their place of worship is that Muslims should leave Canada.
\item Its war on men  Hallelujah Its war on men AMEN ! No guy is never,  Ever gonna be  Not FOUND TO BE  NOT GUILTEEEEE Its war on men  Its WAR  War war war  ----------------------------- Thank goodness I;m gay and I dont have to deal with that stuff straight men have to deal with.
\item The Executive Order banning 'not-Muslims' is taking effect, even if it may not be what Trump anticipated.
\item The wrong-winger hysteria over transgenders needing to use public bathrooms will end up just like the anti-same-sex marriage ban. Kaput :-)
\item Because I wanted to and it fits the argument maybe? Read it. I was responding to the guy who brought up the anti-gay baker who refused service to a gay couple.
\item Nope, but I can read. If you and others would take a moment to read and research rather than knee-jerk 'muslim! ah! islam! bad!' every time a terrible crime is committed by someone with a name you have trouble pronouncing, you'd look much less ignorant.
\item It does teach decency, good morals, and respect for others. Have you read it?
\item Do it yourself then....if you dare.
\item No faith is required to not believe in fairies. No faith is required to not believe in unicorns. No faith is required to not believe in Apollo or Zeus. And no faith is required to not believe in your god either.
\item Russell,statistically homosexuals don't prey on our children. Pedophiles do. And statistics do show that pedophiles have a high propensity for recidivism. Do you have children?
\item STAGE FOUR: ISLAMIC THEOCRACY The Qur’an and the Sharia becomes the 'law of the land. ' All non-Islamic human rights cancelled. Freedom of speech and the press eradicated. All Religions other than Islam are forbidden and destroyed. Enslavement and genocide of non-Muslim population. Destruction of all evidence of non-Muslim culture, groups and symbols in  country.
\item The fundies I know think of the Vatican and Catholicism as a pedophile ring.
\item I also heard that women in Quebec can have prostate surgery, just so they don't feel discriminated against.
\item You are more likely to die in a bathtub than be killed by a Muslim.  Therefore your fear of taking a shower is rational too.
\item Jews culturally appropriated it -consider it NYC pidgin.'  Oy vey, now that's not kosher:  https://www.youtube.com/watch?v=NQhwNtY3N2k
\item Bannon has already returned to harassment of Jews.
\item But under the law. a gay baker could not refuse service to someone on the basis of religion, national origin, race, color, or sex. The law should treat EVERYONE equally.
\item Why  don't you ask your buddy Fred? He wrote the very first comment about 'gay sex and male genitalia.'  I just assumed you two are an item.
\item Absolutely. RCMP now to allow women to wear the hajib. Is this what Canada is becoming? A country dictated by immigrants how Canadians must change to suit them?
\item My reading of the statement at issue is that the Roman Catholic school board condones a man forcing his wife to have sex, because marriage trumps consent.
\item Haitians, El Salvadorans, 'Dreamers', Hondurans, Gay Chechyans etc. bring them all, there are over 60 million left to come worldwide, and fortunately for them, Canada's borders are open!
\item Hey, Foo, Bannon eats Jewish?  Great!  But no Neo Nazi or Fascists friends, please.  They kinda, you know, take over.
\item Due to lack of Muslims Hawaii is not so dangerous YET.
\item Contempt for the military?'  Damn straight.  How'd 'the military' discover they weren't going to add any more transgender'd personnel?  The same way, at the same time, everyone else did: through a Presidential tweet.    I'd hate to be a member of the Joint Chiefs right now.
\item Do these girls face genital mutilation as they do in Islamic cultures?
\item Trump and his Jewish son in law will never give the Palestinians an even footing. Allie is right on this one.
\item So substitute 'gay' with 'colored'
\item Many eye-witnesses do not corroborate the officer's story. If fact they say it was the officer who attacked Brown. And yes it does add up. The police have started to kill unarmed innocent civilians at a alarming rate.
\item Yup. Why did the Church stop talking about sodomy (homo- and heterosexual) as sinful?
\item Great perseverance story.  Not sure what relevance being gay has on any of it.  If everyone was hetero would they have even mentioned it?
\item Keith D LaRiviere are you referring to the trillion dollar give away, please sit down and read
\item self hating jews I guess. There are millions of jews  who are anti-zionists which must make things awkward at times for the non semitic zionists who currently run things in Israel
\item Remember: empathy is what inspired the shooters in Dallas and Baton Rouge.
\item Ah the Christian taliban speaks!
\item Like these black-clad fascists that attacked a gay man's right of free speach. https://medium.com/@trentlapinski/the-berkeley-riots-were-a-cowardly-act-of-domestic-terrorism-2bcafbb32ff0\#.rlbjjb1np
\item All that needs to be done is an end to medical payments for any transgender care in the military.  That will reduce the small number of transgenders in the military from pursuing gender transition.
\item Trump is right on the money!  We don't need or want islamic terrorists coming here!  These people hate the West, our way of life and the simple fact we are not muslims!  That does not make for good citizens!
\item Yes, jots and tittles, crossed Ts and dotted Is. This is a bishop who wants simultaneously to single out the gay members of his local church for specific opprobrium and distance himself from the directive by which he's doing it.  Deplorable.
\item All are nasty nasty jews except for colbert, but he is married to a jew-- nasty people
\item No Duke! The Liberal are on the ground training the Kurds fighting against ISIS. That where they are needed most. Did you have your coffee yet? lol
\item A historian of the Shoah... how appalling. Imagine a person of power said to a jewish student 'This is your Obersturmbannführer... can you smell the ashes?'
\item I lost what little respect I had for Mulroney when he stood by Peladeau as he announced his ambition to separate from Canada. With Brian, money always goes before integrity and honour and loyalty. I am sure he will do well - for himself.
\item Isn't it disgusting? These people commenting, and the Liberals clearly don't know how to use a dictionary. None of this makes any sense. Everyone wants to protect the religion of Islam, and they care nothing about the muslims. That's exactly what I see here.
\item Coming up soon? Trump executive order that all Jewish centres remove the Israeli flags from premises.
\item you seem like a real likeable guy! No wonder your mum abandoned you at birth
\item I think I understand you now. It's only free speech if a paper publishes what you can agree with. right?
\item It's not a function of cultural relativism - gender equality, secularism, and personal freedoms are better than cultures that subjugate women, have draconian religious-based laws, and restrict personal freedoms.
\item Fine, rid all evidence of Christianity from Canada. Just remember, this must result in all religions being expunged from the public school system. No more prayer rooms for certain members of society.
\item In fairness, the COUNTRY isn't second class. Just the current government, and I'd say calling them second-class is a compliment of extravagant proportions. Really, they are class-less, as in devoid of all class.
\item Hey Darty! The vet abusing party is slipping, look: http://www.thestar.com/news/federal-election/2015/10/08/liberals-move-back-into-lead-new-forum-poll-finds.html
\item Is you blatant racism meant to be representative of the views of most Catholics?
\item Yes, I agree with your assessment, good job Obama in destroying any voter base the democrats once enjoyed among jewish American voters for the next few years or longer.
\item Interesting that they would target an event that was overwhelmingly being attended by women and young girls.  There are virtually no male victims of this gruesome terror attack.  What does this say about these reactionary Muslims who believe in Jihad??
\item As you read the gripping reactions of the Jewish survivors of the Holocaust, it makes the idiotic and insensitive remarks made by Sean Spicer on Passover even more grotesque as he refers to the camps as Holocaust Centres. Like somewhere you would gather to for a spa day.
\item Just wait for FN to have a confrontation  with Muslims over land (like for a cemetery)  and not  enough  white people left to come to FN defence.
\item Because nobody believes these nutcases have anything to do with mainstream Christianity.
\item MGWhat do you think of Canada attacking a completely innocent Muslim country? Would retaliation surprise you? It seems most appropriate that Muslims would try to disrupt the source of the invasion, namely Parliament Hill.
\item This marine died because of the gay pride parade in Waikiki took extra resources from HPD.   How stupid is the HPD brass to take away manpower away from a high crime district?
\item Bloggins, who pays you to spew such rubbish. You come across as a fool.
\item The Vatican pundits called cooperation between Catholics and other Christians, largely for the sake of prolife issues, an 'ecumenism of hate.'   Might just be the wackiest thing out the Vatican since HV.
\item The larcenous crowd at Queen's Park has virtually ignored Don's World.
\item Donald Trumps states people should “use the bathroom they feel is appropriate.” (April 2016)  Donald Trump revoked landmark guidance to public schools letting transgender students use the bathrooms of their choice. (Feb 2017)  So which news is fake Donald?
\item When does it end when people like you stop the hate and bullying and killing Transgender humans and learn how to be more for Human rights
\item And, if you even bothered to read the diagnostic criteria (which you didnt), requires anxiety and distress resulting from misidentification of gender at birth due to psychological, behavioral, and biological causes. Transgender is not a disease or mental disorder under any clinical diagnostic in the US. Period.
\item Only sexist men think feminism is an organized religion. Feminism is for people who believe in equality of women. You clearly don't.
\item A LIBTURD APOLOGIST HIMSELF DALLAIRE  .HOW MUCH DOES ONE GET TO TAKE A FEW MUSLIMS DOWN  FOR FUN  MUST BE WORTH \$25 M
\item More men with 'mens plumbing' have harmed kids sexually in Richard Rhyner's church alone as compared with all Transgender people combined
\item It's like saying 'I don't hate Jews, I hate Judaism'. Fools no one.
\item Yes, your claim that only Jesus is God is rubbish, and I'm glad you have recognized and, hopefully, repented.  I hope you will next discard and repent of the idolatry of worshiping a man-made institution as Divine.
\item Yeah that was the remark that offendedme most. Trivializing malfeasance andelectoral fraud among other things is sotypically arrogant of Ms. McDougall.
\item It's over, Trump won because the Democrats put climate change, anti-American activist groups and transgender bathrooms ahead of the hard working middle class. It's as simple as that. Russian activity had no influence, whatsoever.
\item like baird stepping into a coffee shop in east Jerusalem semantics or establishing falsehoods as facts on the ground semantics?
\item Did you read the article? Can you read and comprehend?
\item If I understand your comment correctly you are right.  'Strident professed militant Catholic' is their self proclaimed mission.  The group think is on their part and it's powerful in keeping them in the fold and donating money.
\item From some of the comments it would seem that Canada's historical behaviour towards , say east European, Irish and Jewish immigrants, should be copied here as well. Let's not do the knee jerk conservative values thing again. It doesn't mean we have to be idiots, just not mean spirited psycho's.
\item good point. call us back the next time we get a Christian  shooting tourists in the US or Canada, or calling for authors' heads to be cut off or...you get the point
\item Ah yes. The poor, neglected, downtrodden civil servant. Please pass me a tissue ... I feel a tear of sympathy welling in my eye.
\item Tony, how u feel about the ontario liberals. Interested in your point of view. Do u think they are more corrupt than Harper?
\item Trump is an honourary Jewish President  3 kids 2 married Jewish 1 married half Jewish  Goodbye Obama's anti-Israel - not very subtle
\item I recommend to the parents of Ontario to take Scrimbro's advice. Stand together, organize a volunteer network, and create a system of alternative education for your children.
\item The bottom line is that the Security Council countries see the rest of the world as Muslim dominated with demonstrated terrorist aspirations, and have opted to feed the Muslim crocodile in the hope of being eaten last.
\item An order of the commander-in-chief on a ban on transgender is just that -  an order from the Commander-In-Chief.   This is the military we are talking about where orders from the top do not contain even a single information on how to accomplish the task.
\item the conservatives do not have to embaress trudeau, the shiny pony is doing a fine job all on his own
\item trans gender people need counselling not washrooms, there are only 2 genders, male or female anything else is a fantasy of belief
\item Nope, Chris from Ottawa’s tranny ego Cassandra. The incredibly boneheaded sjw duo.
\item Kinda like what is happening with Muslim terror immigration. As we lean more and more about the plots by Muslim terror immigrants to hurt us. You all support further Muslim immigration Something very sick is in your heads
\item There is nothing to reconcile. The two are intractible, church: 'intrinsically disordered' and LGBT person: 'I am'.
\item The fact that you cannot think of a single homosexual who has been lynched is quite revealing.
\item When one works with the Nazis, dresses like a Nazi, greets like a Nazi and hates the Jews, this person is a Nazi, even this person calls him/herself a 'Ukrainian Nationalist'
\item Yes, pity the Muslim woman who accepts second class treatment.
\item Just a matter of time for all women to be obligated to get covered up and hidden up veils to not offend Muslims. They are winning .
\item Ah yes. Trying to mock him for being an amazing family man. How will he recover.
\item IRT FastEddie, agree with your post.  The Congress must repeal such nonsense where citizens (tax payers) must pay for any transgender surgery.  For some reason Congress and Hawaii born ex-president Obama created another human form besides a man and a woman.  Auwe.
\item Up vote me if you would love to see someone (woman, man or trans) come forward with a previously buried sexual harassment claim against Boy Justin next.
\item Not all Muslims are terriost but all terorist are Muslims!
\item I don't mean to be contrary, Wavemaker, but historically the Jews have  in fact been forced to give up their homelands and relocated to live in camps, ghettos and the like.
\item More than 80\% of the country identifies as Christian, but go ahead and cling to your persecution complex in the face of all evidence to the contrary.
\item Only academics and journalists think killing our enemies is a bad idea. Normal people know otherwise.
\item Understood,  I would prefer Pence. People hate him because he is a Christian, but that goes with the territory. It's Amazing closed minded people can get.
\item Me too Neko.  Good Lord the gay brings out the worst in some 'TradCaths' understanding of Christianity.  And yes, I am definitely making a distinction between Christians and self proclaimed traditional catholics.
\item Islam is a common denominator for Terrorism. We will not be silenced. Free speech in not hate speech.
\item They do and have been for a very long time. Look it up lmfao
\item What about Catholic  prelates telling us we can now disregard those 10 commandments?
\item tories will never give compassion instead of contempt, but it would be nice if they recognized the points you make here. Harm reduction is a much better approach than shaming and demonizing.
\item It does not matter which name you use john, joannie, JOE or maybe ???, the result will be the same unless you change, namely purgatory, probably preceded by psychological problems.
\item They want God to bend around their will.'  When you say 'they', RD, are you including yourself? As when you show your basic misunderstanding of and contempt for the transgendered.
\item To me accommodation of religion and culture is a Canadian value as enshrined in our Charter of Rights and Freedoms.
\item Before Trump got elected I would have agreed with youBut its impossible to imagine Trump doing anywhere near as good as Obama did on foreign policy
\item My interpretation of Trump's decision is based on the financial burden placed on taxpayers for the gender transition. Here's an idea, start a go fund account to support transgender transition for those in the military, that way taxpayers won't have to pay for the enormous medical expenses...everybody wins.
\item Don't forget a value added tax (sales tax) of 23\%. But yes, very well spent, and I would be happy to pay it to see those around me well cared for and disparities in social class minimized.
\item How much land does Arabs need? It's not about the land but murderous hate towards HaShem's chosen people...The Jews. The Lord has set a blessing(Torah) and a curse(secularism) before us...Choose wisely!
\item I hope they build it. Then I'll get to see it blown up too. These morons sure know how to show off their bad taste. It is beyond embarrassing.
\item well when is the homeless jew going to get the \$12,000 that he needs to buy a house......he is 36 ....and has lived his hole life in phovertity and prison and jail......he would get a job but prison and jail made him to crazy to work.....
\item Why?  He's not gay.   Huh?  She's a woman?  Now I get why Bill did it....
\item It is more socially acceptable to be gay than to be white or male. Ultimately being a white male gets me accused of being racist by the BLM Pride Committee (with the tacit agreement of Tory, Wynne Trudeau and Wong Tam)  despite being gay and non malicious.
\item We have had easy access to  weapons for a century. Shootings like this are a new phenomena denying everyone what has been our Constitutional right because we have crazy people and radical Muslims is a poor answer.
\item You can stick a fork in the roasted pig!  Pretty comical actually that it wasn't the Muslims, Mexicans or tax issues.  Just being himself.  Clinton should cancel the rest of her ads.  Save the dough, she's home free.
\item I feel the same fear for the gay members of my family.
\item Well there you have it. The Globe's most worthy apologist for this tarnished govt. Konrad, you should be ashamed of yourself for so heavily buying into the party line. Flanagan would have said the same, but perhaps with just a hint of 'mean' to it.
\item The mainline Protestants ARE VALIDLY BAPTIZED!!!!! And they are recognized by the Catholic Church as Christians.  Furthermore, the Catholic Church, at Vatican II recognized that Catholics, Protestants and Orthodox comprise the Church, not just Catholics only.  Lumen Gentium, 14.
\item No, it wouldn't. Again, he didn't want to bake a cake for a gay wedding. The issue wasn't serving them at all.
\item Terrorism Is a real threat … but try to keep in mind only a small percentage of terrorist attacks carried out on U.S. soil over the last couple decades where carried out by muslims. Lesser yet Somalians muslims.
\item In a way to be concerned about your safety yes. To be left wing quite often is to champion those who would want to kill you.
\item “Ivanka Trump calls for tolerance following threats on Jewish centres” ----------------------------------------------------------------------------------------------  I wonder if she realizes the irony and the hypocrisy in her call. Her father stoked the fires of racial and religious intolerance and filled his cabinet with like-minded bigots, but she remained silent until it impacted her own religion.
\item You're full of it Quibly. I travel a lot and people have nothing but good things to say about Canada.
\item That is how early Christians destroyed the ancient Roman civilization,: by smashing one statue at a time.
\item Don't confuse the US with 'English speaking nations'. The use of f----t to mean male homosexual was basically unknown in the UK and Ireland until the last decade. It is a US import - seemingly the same in New Zealand where I am now.
\item There aren't Nazi's silly. Certainly not ones making bomb threats to Jews. The fact you think that demonstrates your susceptibility to propaganda.
\item We pedestrians should start making citizens' arrests of all cyclists who ride on sidewalks and hold them in place until the police arrives. This way, everybody will be safer and happier.
\item Lorna, what is your take on the story of the great deluge? In that scenario god euthanized most of the human race for being 'sinful'. Whether you consider it literal or allegorical it doesn't say much for the sanctity of human life by your creator.
\item You're okay with demeaning Islam for people that radicalize it, but are totally okay with a religion who's leadership actively covered up child sex abuse?
\item I agree......Jesus had cigars and bourbon with jazz playing for the social hour after the last supper......how quickly some folks forget.
\item I'm with you, Mike.  But I would use the terms: same sex 'behavior' or 'homosexual behavior.'  The other words (sodomy or sodomites) sound caustic to modern ears.
\item one thing I will remember about Steve Poutine and this subject: when he said that ndp 'supported' hitler and of course vicious attack adds smearing opponents. I cannot imagine respecting anybody among robo call crew. sad story about Canada
\item You couldn't pay me \$1000 to go see the head of the Christian Taliban!
\item The Globe promotes ghettoization.
\item Why is it America's issue that Muslims hate Israel?  Weren't you paying attention during the inauguration?  It's all about America First, baby.  Israel is a nuclear power.  They can take care of themselves.
\item Rifleman 1010 writes:  ' ...the 'alt-left'........Much like the Alt right and ISIS.'  --  Any calls lately by the 'alt-left'  for Jews to be rounded up?  Any lynchings?  How about church bombings?  How about beheadings?  .
\item Aren't all gays female friendly?
\item That only works when vermin like Muslims aren't involved in the mix.
\item One thing you have to understand is that RD's actual knowledge of transgendered people is nil. His knowledge of feelings is also nil, so he has decided that they count for nothing.
\item What utter, hyperbolic rubbish. As if Obama carefully plotted this to outrage the Jewish faith.
\item ... but no one wants one Jewish state with disaffected, disenfranchised Palestine...'  Unfortunately, that is precisely what the Israeli right wing want (assuming they can't get rid of the Palestinians altogether).
\item That's like saying a racist doesn't hate black people, he just hates the color of their skin. Or an anti-Semite doesn't hate Jews, he just hates their religion. Or a misogynist doesn't hate women, he just hates their gender.
\item 4) Hinduism worships gods that are not the God of the Bible.  Why should money spent on a Catholic school facilitate paganism/polytheism? My Catholic university spent money to buy idols for their worship services.
\item Don't bother.  Rio rarely posts except on any jewish or Israel related story. He clearly has an agenda. Don't feed the troll.
\item You just might be a racist. How do you know who is an Arab,  anyhow? Someone who looks just almost like a Jew or an Italian?
\item China is an interesting counter to this kind of barbaric uncivilized thinking.' Really? Have you ever seen this? This is how the government in China operates. https://www.youtube.com/watch?v=V3XfpYxHKCo
\item There is no comparing a Canadiam prime minister with a US President. A president is head of state, commander in chief
\item Psychiatrists talk to gays with infinite affirmation, while gays continue to kills themselves at 4x the base rate of the population (CDC numbers).   time to rethink infinite affirmation.
\item why were you at catholic school?  i don't believe in Gesus either... and did not goto a gesus school..  you should sue your parents for suffering you through a catholic school.
\item Islam is as much a political movement as it is a religion. Like global warming.
\item The fact is that the Trump regime is white supremacist Christian Republican extremists who hate everything our country stands for.
\item Quick question for ya Corporate: what is the age of the earth? A) 6 - 10 thousand years B) 4.5 billion years
\item Well, this pretty much explains the lack of intellect and rationale in the typical Con post.
\item Check out some of the people who helped Trump get elected. National Policy Institute--OR--white supremacist 'evangelism'--you make the call. Either way they're racist kooks.  https://youtu.be/1o6-bi3jlxk
\item The Muslim religious culture is so far from our Canadian values that it is impossible for most Canadians to believe that our supposed multicultural society can ever accept their religious culture. The solution is obviously that we should very much limit the number of Muslim immigrants.
\item Long long before the Jesus fantasy, ancient man marked the shortest day of the year and the return of the sun with festivities. Christianity took that even more ancient belief and mixed it with their belief system. No harm no foul.
\item JJ: You forgot to acknowledge that Lesbians also murder their SO's just like Hetro's, Homosexuals, and  all the other groups do,  and Democratic Men Cheat as well.  Lets not leave out any pertinent ones.......
\item Reality has a Liberal bias...
\item I missed that part of his speech where he used the three words he blasted President Obama for not using, please point me to the time in the speech where he directly used the term 'Radical Islamic Terrorists'.  Thanks :)
\item On which moral or scriptural foundation will the law abiding majority of Muslims stand to address the issue when everyday they pray from precisely the same document as the terrorists, which contains the exhortation to and legitimization of the terrorists' acts?
\item A disproportionate number of Nobel Laureates are Jewish, does that mean that non-Jewish people are incapable of abstract, complex thought?  By your logic, that's exactly what it means.
\item To identify the truly sick racists google: chief rabbi of Israel says only purpose of goyim is to serve jews, life of goyim worth same as donkey.  Netanyahu says this jerk is the greatest mind of this generation.  http://www.timesofisrael.com/5-of-ovadia-yosefs-most-controversial-quotations/
\item What a load of unmitigated racist drivel. How do the these views square with the success of the Jewish community in Canada - particularly in academia?  People of colour I know are not shrinking violets who have to be coddled by reverse-racist policy.
\item Heterosexuals\_tend\_to\_find\_gay\_sex\_icky.\_It\_is\_part\_of\_being\_hetero.\_All\_are\_wicked,\_gay\_and\_straight,\_and\_it\_has\_little\_to\_do\_with\_sex.
\item Amazing that every serving transgender member of our military doesn't suffer from 'bone spurs' isn't it? 'Bone spurs'  is a symptom of  'P\_ssy  running away because people shooting at me is scary!' disease.  Comes with complementary yellow stripe on back
\item Not really - there is something SERIOUSLY rotten in the PC party though.
\item Now this helps to bring the country together! What tripe.
\item .  A victory for intolerance.  The Muslims who have been so rejected by these people should be, and probably are, already looking for a place where hatred doesn't determine who rests where.  .
\item The POTUS is charged with keeping the military at is strongest, and Transgender soldiers in any capacity will weaken it, regardless of what you think his intentions are.
\item once she is President' ?? Getting ahead of ourselves aren't we?
\item The only troll is Amira herself, trolling for Islam and for western civilization's submission to the Koran. Her hijab is the sign she handed her fate to Allah. Giving up free will is just one thing Muslims ar expected to sacrifice for their religion. 10
\item Las Vegas mass shooting: 'This is the price of freedom...'  'Gun control is more of what doesn't work' New York truck attack: BAN MUSLIMS!!!! This country has dementia.....
\item A walk-in clinic is not a family doctor, no matter what they advertise. Trust me, I've done both. There's no comparison.
\item Theres plenty of fat to be cut from our medical community. Start with anything to do with transgender issues
\item Jerome would rather advocate for transgenderism to kindergartners like they do in Washington.   http://www.k12.wa.us/HealthFitness/Standards/HPE-Standards.pdf         page 29
\item Ward1 in Springfield: I don't think there is any evidence that the recent threats made nationwide against Jewish institutions originated in Eugene or even in this country.
\item How sad.  Now where else is Harvard going to find another TT (trans traitor)?
\item Quebec still remembers the FLQ, so why should they take a chance on potential terrorists, which all these Muslim brought here by Trudeau could turn into some day soon!!
\item Even now evangelicals and conservative Christians are among Trump's staunchest defenders.  Jesus wept.
\item If this guy was truly a hero, he would have stopped the Muslim terrorists from carrying out the London Bridge attack. This is simply lionizing by the leftist press based on opinions, not fact.  Nothing but a daily dose of fake news.
\item Islamist' terrorists, please, Guest997. Amid the carnage, butchery, and ignorance, we must use accurate terms and remain politically correct.
\item JHsassYou are free to volunteer for the 14 year prison sentence.
\item I am concerned that, whether they are conscious of it or not, the white men who would vote for Trump have never fully accepted women and people of color as equals...'  Not only these, but also LGBT folks and Jews, two other groups many of these white supremacist types hate.
\item When POTUS Trump speaks to the Boy Scouts it's political but when the left shoves gay propaganda down their throats it's educational.'.... Dinesh D'Souza.
\item In America anyone is allowed to opening mock something as dumb as Christianity.  But that is a waste of time. Let’s get back to mocking draft dodging cowards.
\item For the rest of the population it  mean doors are closing and opportunity are being taken away if you aren't part of the favoured group.  Muslims want to be served by Muslims and not by Kafirs if at all possible.
\item Better yet, It's time to wound old heels - get lost Brian!
\item Oh good, Jewish conspiracy theories. Given that Trump's statement on Holocaust Remembrance Day was praised by neo-Nazis for its 'de-Judeification' of the Holocaust, I'm going to say I don't give a fuck who his kids marry, he's empowering anti-Semites.
\item As long as you like Liberal party propaganda.
\item Uh, plenty of women have learned how to pee standing up. And after surgery, trans women no longer have a penis.  Why don't you do a little research on the subject.
\item Why not add Saudi Arabia and North Korea to the list? After all, one finances half the Islamic terrorists in the world, and provided 15 of the 19 hijackers on 9/11. The other recently killed an innocent American, and threatens to nuke US cities.
\item McInnes is a public anti-Semite if you go by his video about why he hates Jews, posted on The Rebel.  It is important to call these people out for who they actually are.
\item You get the government you deserve.
\item you sound like a jew.
\item This is the Christian equivalent of Sharia Law.
\item Parental Rights' is just extremist Christian code for their version of Sharia Law.   In Jim Minnery's perfect world, all women and girls would essentially be slaves of their fanatical fathers, just like in all extremist patriarchal religions.
\item How gallant of you.
\item I'm pretty sure Jack Phillips said he would, and has, served gay couples.  Serving is different than making a specific kind of cake.
\item not a prince, just a tranny gold digger
\item The extreme ideologues inhabit the NDP and environmental movements. While the Tories and Grits have some that are out there for the most part they are mainstream Canadians.
\item Address religion head on. It is nothing but tribal mythology, manipulated to control the ignorant and utilized by the heinous. It has been so for millennia. Radical Islam is just another symptom of the virus.
\item How ignorant! No wonder Catholics are leaving the church.
\item Regressive-Leftists are out in force I see.  ISIS claimed responsibility. ISIS are the invading imperialist, colonialist Islamists in Syria and Iraq. They killed tens-of-thousands of Muslims to take-over Syria. It's a joke if ISIS is blaming British colonialism. Even more ridiculous from our own commentators.
\item will thay let the homeless jew work there......with his long voilent crimeal record????
\item Christians today are like Thor Johnson.  They like to beat up on  non-Christians.
\item It was a poll done recently by a liberal jewish group and it was all over the news. Among the jewish youth: it was about 80\%. The same jewish group support the UN resolution
\item there is no such thing as a 'peacekeeping mission' when dealing with islam
\item Well, I think we can rule out the Christians!
\item I think Marx doen't understand the meaning of 'civility', constantly decrying perceived 'Jew hatred', while making the most offensive comments about everybody else.   I suspect he's had more comments deleted than anyone else. What could possibly lead to such hateful views?
\item No one would dare say that the Prime Minister endorses unethical activities...'I'll say it...loudly!
\item Moral/ethical values are intrinsic to humanity and a Darwinian survival mechanism. Religion is merely one manifestation thereof, and not necessarily superior.
\item Spacey pulled the gay card to avoid the pedophile angle.' ============ He just didn't 'pull it out of thin air.'  Apparently there has suggestions, allegations, and rumors that he has been gay for decades. He finally is confirming it all. Besides the 'homosexual-pedophile' angle is hardly better than the 'homosexual-pedophile' angle.
\item .  'The whole notion that somehow we just say no to more Muslims, just ban a whole religion, goes against everything we stand for and believe in.'   Dick Cheney  ----  Wow.  When Dick Cheney  calls you out for being intolerant and anti-Muslim, you know you have to be one grossly sick POTUS.  .
\item You must not have 'been there' in the 50s or 60s when tenure was needed to protect people who were working to advance civil rights. It's needed now to protect people from Harper's anti-science agenda.
\item The evangelicals' support for Trump glaringly displays their complete moral bankruptcy. They are not Christians.
\item Hear, hear! One law for all Canadians!
\item What a bunch of gobbledegook.  Followed to its ludicrous conclusion, Christ (who did't actually 'ordain' anyone) only 'ordained' Orthodox Jews. Therefore the only men eligible to be priests are Orthodox Jews.
\item hard to feel much sympathy you get what you vote for, you make your bed and sleep in it.
\item Yes - exactly - how many police officers in the U.S. have been shot by black suspects - is it at the rate of 1/day as black suspects shot by police? - not sure where I saw this in the past couple of days on which website (Globe,BBC,Yahoo,Huffington)
\item i know cayjaybird, you'd rather have a p**** grabber, who is vindictive, a racist, a thin skinned,, untrustworthy liar.  You are so forgiving, an evangelical perhaps?  lol
\item Says the greatest homophobic poster...
\item kind of like lawyers, eh?
\item And yet another progressive Catholic who is calling half of America 'Nazis.'
\item On yesterday's show Spanish film director Pedro Almodovar talked about gender roles in his films. He began by explaining how his scripts always depict men as abusive and violent towards women.
\item Boots and I are waLKING all over the beaten Trump.  The truth is the terrorists are already here and they aren't Muslims.  Checks the stats guys and wake up!
\item Actually it calls for the death of all Jews in the world.
\item Only the informed globe drive writers can show us a picture of a heavy duty 2500 truck then go on to describe a 1500 with a V6 engine. Globe writers should go back to writing what they know best about, like transgender people and their washroom problems.
\item Precocious doesn't mean what you think it does. Look it up.
\item Obama has defecated on Israel repeatedly.  Why would any Jew give him the time of day?  Iran has pledged to wipe Israel off the map and Obama gave them the means to do it.... nukes.
\item I though gay marriage was going to control population growth.  I guess I was wrong.
\item And a boot smashing a human face, forever.
\item I agree. Stay out of it. Russia and Muslims (of all stripes) were fighting Wayy before Bush thought he was king. They have lots of crap going on that North America and even the UK won't understand.
\item Israel and AIPAC OWNS our congress, as evidenced by the 30 standing ovations netanyahu got.  Yet these jewish left wingnuts in the fec are 'horrified' by a russian vodka ad on drudge.  This is total friggin clown world here.
\item I would not vote for you as that would be a vote against the country and our cherished belief system!  Now go to your transgender room and close the yap!
\item I would like to see a program that tried to integrate armed forces personal into the fire department. 6 months working with the fire department would seem like a vacation for Canada's true heroes.
\item Steve Jobs wasn't eleven years old! This is about the rights of children...
\item Honestly I am dumb struck. Of all the issues facing the Church, this is the one a Bishop concentrates himself with?  Most days I'm proud to be Catholic. After reading this I can safely say that today is not one of those days.   Fr. Neil Pezzulo
\item Shouldn't the title read 'Muslim extremist wrecks havoc on innocent students'?
\item This must be what Harper's minions on the back bench do to stay awake.
\item So much ignorance in 9 little words, kmedland1. That 'girl' has 'M' on his  birth certificate.  You seem utterly unaware about trans folk.  Google 'Buck Angel' and tell me she belongs in the 'women's room'.  Good Christ - this is the kind of ignorance we have to put up with.
\item If only they will stop crying and exaggerating every small incident!!!!!!! I read this news article the other day about Quebec Muslims crying that they have never felt this unsafe before, yea right, maybe you should move back to where you came from if you find this unsafe!
\item You're confusing 'cajones' with racism.  White Neo-Nazis chanting 'Jews will not replace us' are 'very fine people.'  Black athletes quietly kneeling are 'sons of bitches.'  Rote patriotism is not an ideal of this country.
\item Konrad isn't going to get an invitation to the inauguration of anyone even if it's held in Wilno or Barry's Bay!
\item remember 'wacky' should be the rallying cry against trumpkins and westelca.
\item I guess you think that baseball enjoyment is more important than social justice.
\item Funny how these brave feminists have no problem with how islam treats women?  Only Trump is the bad guy!
\item You assume that mist lesbian or gay male couples yearn for recognition and blessing by the leadership of this sect. Those I know, me and mine included, do not.
\item Obama and Trudeau think transgender washrooms are YUGE important matters of state
\item By the same token, Catholic students should not have to pay for atheist an other non-faith based schools. Why do I have to pay for heathens and infidels to receive state based filth?
\item ...she rolls out aseries of her so called attacks on faith....none of which attack Jesus, or Mohamed or Budda etc .... the pope's the church, aand her aunt....that's not attacking faith
\item Jews won't replace them. Instead, these losers will be ignored, cast aside, forgotten. They're whining because whites have 70\% of the power, instead of 90\%.
\item The cognitive dissonance is amazing. Mitch McConnell extends the Senate session determined to pass a so-called health care bill depriving millions of access and Christians cheer? What?
\item If we could only listen to each other respectfully without getting each others backs up, progress could be made in solving difficult challenges facing this country. True collaboration.
\item The question IS about baking a cake.  Please read: https://www.nytimes.com/2017/09/16/us/supreme-court-baker-same-sex-marriage.html.  'Mr. Phillips shut down the conversation as soon as he heard that a gay couple was getting married.  “I’ll make you birthday cakes, shower cakes, cookies, brownies,” Mr. Phillips recalled saying. “I just can’t make a cake for a same-sex wedding.”
\item Thank you for the great Christmas cheer.
\item I wonder if the Jews thought that as they were being prodded into rail cars by men with guns..?
\item Good article. Gay marriage was also about portraying gay men as monogamous seeking individuals, rather than the reality of promiscuity and HIV infection that still exists in the community.
\item why then funding them partly is ok?? is that make it only half wrong or half right? it is either right or wrong. make your mind up.
\item You actually read that rant?
\item tea Party'--a scattered group of American patriots who believe in fair taxation and smaller Gov't.--what is it you people don't get.
\item This has all been a great exercise in how to whip up a crisis where none exists.
\item Islam is no more deserving of respect than any other idea or philosophy. People deserve respect. Islam, like other religions, is tribal and destructive. I will not be silenced in my criticism of these archaic and barbaric ideologies.
\item Merkel is neither intelligent nor knowledgeable.  She is a puppet of Islamists, supporter of gay-rights oppressors in Riyadh, and does not know that Obama bugged her phone (though the whole world knows it)
\item Only in America. Society, rules, laws, boundaries are torn down, thrown out, tossed aside, and discarded as being outdated, unfair, anti-immigrant, anti-gay, anti-anything.
\item The problem with all this is that Trudeau and his government are dealing with someone who is probably mentally unstable. Witness Trump's rant against the judge who overturned his travel ban against Muslims.  Maybe the best accompaniment for Trudeau will be men in white coats.
\item I think the percentage of Canadians he is offensive to is higher than your estimate. Even white males like myself are offended by this man.
\item I disagree with you about the nature of transgender people, but ...  Welcome aboard!
\item if this terrorist problem isn't solved peacefully now , that is ,  by muslims, then it will be solved violently by other later
\item Beware the Gay Mafia.  They are the BIGGEST group of self-centered hypocrites \& thugs on the planet.
\item Not all transgender people have gender reassignment surgery.
\item I remember that period as well. Since everyone in my father's family was Anglican, and my mother's family were all Jews, it seems they were all damned.
\item According to Trump voters, this interstate compact agreement is a no-no. Think Aurora theater shooter and the Muslim sex offender named as a suspect in Clement's murder. Of course, the rules and law (rule of law) only matter when it favors their agenda.
\item You do realize that Jews read the bible too don't you?  Just the Old Testament part.  It's so funny that people are so obtuse about this fact.
\item Interesting.  But since no one has ever  been fined for refusing to bake a cake for a gay wedding.  I can't see how it wouldn't be.
\item I thought Jesus is dead.  Oh yeah-- I forgot he got resurrected and has been hiding out ever since, but a lot of you seem to know what he's thinking and feeling -- how convenient for you and self-serving.
\item I support religious liberty AND Thomas Jefferson's great wall of separation between church and state. No religion should trump equality under the law. Period. Good fences make good neighbors. Why does fundamentalism target gays rather than ALL persons who violate biblical morality like divorce and living together etc.?
\item That power argument is a big joke, applicable only when the victims are pre-pubescent.  This is about homosexual sex acts and the preference for younger, near-pubescent age men/boys.  Married men without same-sex attraction, no more altar girls, and a lot would be resolved.
\item Playing the victim card once again, what's new?
\item Fortunately you are not a Christian.  Otherwise you would need to care about your fellow man (or woman).
\item I bet if she was a Nun you would have more respect.
\item Admiral Zukunft says 'I will not break faith' with transgendered members of the Coast Guard, but apparently has no problem disobeying the President of the United States. He should be removed from his command forthwith.
\item Now that is a load, it has been Obama and Kerry in full out attack on Israel,   Trump is Jewish you fool
\item Mel, The world is swinging left, baby. Heeeyeahhhhhawwww!!!!! First we take Ottawa then we take Moscow!!! Power to the people!!!! The people united will never be defeated!!!!!!!!!!!! Hoooo Hawwww!!!!!
\item A Catholic Women's Strike is one of my dreams.  I would envision all the women, nationwide, refusing to do any work of any kind for the church, including attend Mass, starting on a Thursday and ending on a Monday morning.  Pick a date, I'm in.
\item The true fascists are those who seek to silence any open scientific debate surrounding transgender issues. As it stands now, qualified professionals asking too many questions risk their livelihoods and reputations by questioning the politically correct wisdom surrounding the issue now
\item That murderous sociopath who claim to be religious are killing people.  Christians meanwhile profited from enslaving millions of Africans over hundreds of hears, occupied these nations then propped up dictators in the war against communism
\item This is not a justification'  Really?  If an entire city taken over by Daesh affiliated terrorists raising the filthy Daesh flag over churches while taking priests and Christians hostage isn't then what is?
\item If there was anything to reinforce the perception of the Catholic Church as a fetus-fetishism cult, this would be it.  Just ghastly.
\item Mom you are a hero and I applaud you. I also wish all the best for your son and we are so blessed having people like you in this world. Definite prayer for you and your son at church this Sunday!
\item There are probably valid moral arguments about banning transgendered persons from serving in the military.  This is not one of them, and reeks of adolescent moral reasoning. I'm surprised the Denver Post chose to publish it.
\item Wow. a few months ago you were a stalwart defender of women when you feared transgendered people in the restrooms.   Now you wholeheartedly support a guy who brags about sexual assault.  Strange guy.
\item Blowing ISIS off the face of the earth might be their worst fear. our tolerance and some Liberalism just make them hate us more.
\item the jews fleeing the nazis.....where deniend the right to come to the usa.....becouse thay where from germeny....and the usa said that thay mite be nazis.....
\item I hear you Canada1. I don't want a Leader. I want representation.
\item Married men with children are less likely to be the molesters of boys that homosexual priests have turned out to be.'  Absolutely not true.  Look up the statistics. I'm not doing it for you.
\item What is there to hurray for? Pulling out of the Paris Agreement? Trying to take away health insurance of 20 million Americans? Banning transgender people from serving in the military?
\item The Right: Always more than willing to be dishonest!!!
\item Quick, name a better Central Banker.....let me see most cons always admired Greenspan, the Aynn Rand groupie.....but surely you see what a joke he was now....so name a better one?
\item w kingIf you cannot comprehend international law, why not just start thinking about basic human respect for other human beings?
\item I can say 'Orthodox Jews'  I can also say Sharia law, burka, honor killings, Assad soldiers raping women, Isis raping women
\item No, it is largely the institutional Church showing a lack of compassion for gays.
\item It's just really hard to find an Indigenous Asian Female who's transgendered lol
\item And here is another progressive Catholic who's against free speech, and ignores the recent murders of innocent Christians in Egypt and elsewhere.  It's so strange.
\item I hope the cake guy wins.  The gays and their drama...
\item ummmm no  To find the hate for homosexuals, minorities ( infidels), women you need to visit a mosque.  Merry Christmas
\item National Catholic Reporter is the best newspaper in the country, Catholic or secular.  It deserves the support of all of us.
\item When wrong is committed in the world, it is right to sanction it. As a Christian, I say it is high time that Christians stop defining themselves by what happens in the bed. It is time to define ourselves by our generosity to all of our fellow man.
\item A quick google shows many examples to contradict you. 'Black Lives Matter blindsides Jewish supporters with anti-Israel platform' 'BLM activist advocates white genocide at Harvard - YouTube' ...
\item AS BAD AS THAT IS IT IS BETTER THAN HALF BREED MUSLIMS!
\item A Trans man is a man that wishes he was a woman. Grasp the concept
\item ....sharing of the blog post and discussion on her show led to 'Islamophobia and hatred toward Muslim people.'  I think 9-11 had a lot to do with that, not sharing a blog.
\item Is the cosmic Jewish zombie baby snow white, or did they bother to find a doll with some color?
\item Love drama, but the kind done by professionals not your crybaby antics
\item The Muslim youth unemployment situation has more  influence  on radicalization than devotion to Islam.
\item We're being told there are no differences-it's how you 'identify'. Fine by me. When will the US Olympic team be allowing transgender women sprinters? No big deal, right?
\item You will absolutely love the women's rights perspective of those deluging Europe now. See Sweden the rape superpower with Germany catching up.
\item Most intelligent statement to date on this subject, destroy the ideology and you destroy the movement. Muslims have done this before, they must do it again. Bombs do not work.
\item Klastri, Muslim ban?  Why do you make up such stuff?  Where in the EO does is religion mentioned?
\item The policy of the church is that gays or straight clergy are to be celibate---no sex with anybody, even themselves.
\item I remember the Conservatives raised not a peep when another popular PM spouse, Mila Mulroney, was provided with office and staff, yet they have done a 180 now. Hypocrisy? Nah.......Let's stop being so mean, small-minded and cheap
\item From a policy perspective, the endearing thing about Trump is his incompetence. Pence is sufficiently coherent that he could put in not just a Transgender ban, but a full LGBT ban.
\item The exclusion of 'outsiders' and emphasis on 'purity of the race' is very much a RIGHT wing trend. Just ask Hitler.
\item A classic counter terrorism operation. Deny the Moslem terrorists their support base.  Seems to be working as the terrorists have declared a truce while they re-organize their logistics.
\item The lady in the burqa at Canadian Tire also did it for Syria.  She lumped all white Christian in one basket and committed a hate crime. but she will get away with it.
\item Nothing like being gay and hanging in Gaza City town square.
\item Is the G\&M going to report on what certain Imams at this mosque were promoting? Death to Jews anyone?  Of course not, it doesn't flow with the narrative.  G\&M: A newspaper with an agenda.
\item and so do many americans believe the same way.   Why NC can't even accept trans bathrooms.  Come on..............
\item It's really clerical homosexual pederasty that was/is the issue.   We see it flare up again with Milo and George Takei.  It existed with Oscar Wilde.   It was a HUGE problem in the last 50 years with homosexual priests.
\item Yes, she always manages to find a way to explain outrages committed by Muslims  in a way that directly or obliquely blames the west.  Which warms the hearts of the moral equivalency crowd.
\item You mean the pussy grabber? How could you evangelical far right Taliban style Christians cast a vote for such con man? Explain that and then tell us again how LGTB pose a risk to your rights as a citizen.
\item and therefore, you do not have the right to force your aberrations on others. should a christian butcher be forced to make a moslem sacrifice? NO. should a christian physician be forced to perform an abortion? NO. shameful.
\item Nice article by 3 Lesbiens
\item The military will refuse to follow Trump without the authorization of Congress. They've already refused to listen to him on the Transgender ban...
\item Trumptie duped the voters and once again they fell for it.  The Christian voters always get duped.  The Tea Baggers too.  He drained the swamp to make room for the jackals.
\item If you work with 4 Catholic priests you should be able to readily get a precise definition of the term 'Invincible Ignorance'.
\item Cinnamon Hitler'? Yes, Trump is exactly like Hitler, what with his half Jewish grandkids and the millions of people he's sent to concentration camps and the world war that he started. Idiot.
\item So....Jewish kids should be blown up in their school...is that your point ?
\item And before Vatican II all the Latin American countries were 90\%+ Catholic. Maybe the bishops should focus on why they are losing so many Catholic who are seeking to get their spiritual needs met elsewhere over material concerns?
\item Yeah, and Breitbart is pro-Israel and run mostly by Jews.  Come on dude, spend more than 2 minutes at a site before you make an idiot of yourself.
\item Or a few drunk lesbians.
\item what good have the millions of fake Christians ever done for anyone?
\item Yes I'm sure doing mushrooms and eating berries requires massive intelligence.
\item Oh, so you have no problem with you son looking at a man in a locker room and sizing him up, or your daughter looking at another woman, it's natural.   It's just trans-gendered people who bother you. Got it.
\item Of the 4 posters above I would lay money most are gay activist!
\item That's hysterical! The alt-right ARE the barbarians.
\item Transgendered bathrooms ? We pay for this madness ?
\item islam has had a terrible impact on the western world. Now there is someone in a position of power that recognizes the danger and is willing to do something about the spread of it in the US.
\item Social and economic equality work amazingly well in social democracies like Norway, Denmark and Sweden.
\item Much like the Pharisees who conspired, colluded and crucified Jesus Christ. 'Close-minded ideas.' Yes, you hit the rusty nail on the head.
\item You speak for your wife, do you? I guess you white Christian men know how to keep them under control, no burkas required!
\item The only status that matters is being a Canadian. Remove all other status designations and let us move on as one nation where everyone is treated equally.
\item And Jesus said, 'Enough!  Put away your sword. Those who live by the sword, die by the sword.'
\item I never would have guessed you were a closeted gay male based on that jacket you're wearing..or maybe this is just a really good disguise after all.
\item Between apologizing for all generational misdeeds of the white man, meeting with Muslims in mosques and catering incessantly to LGBT, our man Trudeau seems to have a full agenda. Maybe in year two he'll make some time for the average Canadian who has bills and taxes to pay.
\item Inshallah,  it is God's will.  At least that what they say when they blow up Christians.
\item How about a pm who tells the truth, shows respect for parliament, does not put corporate profits ahead of everything else, and actually cares about Canada. We don't have that at the moment.
\item The only troll is Amira herself, trolling for Islam and for western civilization's submission to the Koran. Her hijab is the sign she handed her fate to Allah. Giving up free will is just one thing Muslims ar expected to sacrifice for their religion.  5th posting
\item Israel's military does not appear to have suffered by including transgender soldiers.
\item I'm starting to like this guy. Refreshing. Ford in 2014 !!!PS Ainslie is a goof.
\item Every sperm is sacred? The little whimpers of each sperm must make you cry
\item No one knew of homosexuality? ! Were you raised in a bubble?
\item I know this decision will hurt feelings but it is probably the right one. Until society in general comes to terms  with transgender disorder there will be too much drama playing out to have it effect national security.
\item Von, But, you see, spirituality isn't religion. My idea of spirituality is quite the antithesis of religion. It's more about the shared reality of people in the here and now, not the unreality in the hereafter.
\item You're either utterly ignorant or totally incapable of telling the truth. Trump's VP is viciously antigay...  http://www.businessinsider.com/mike-pences-most-controversial-stances-on-gay-rights-abortion-and-smoking-2016-11  https://www.theguardian.com/us-news/2016/oct/04/mike-pence-led-anti-lgbt-backlash-trump
\item You dont see the difference between being concerned about immigration and wanting  it slowed or stopped and calling for the death of of Jews and Blacks? You must be blind.
\item AUGUST IS PERSECUTE A CHRISTIAN MONTH IN THE USA,THE SOUTHERN BAPTISTS DESERVE PERSECUTING THE MOST FOLLOWED BY THE MORMON FREAKS
\item It is interesting to note that Womens Netball is quite regularly seen at primetime, live on New Zealand television. Further, both men and women are supportive of rugby teams of both genders.
\item I would rather share a bathroom with a transgendered person than a sanctimonious bigot.
\item Huh, maybe that's why lesbian sex is shown in straight porn and not considered homosexual porn.'  And you know this how?
\item People get the government they deserve'.
\item The first step on a long road to restoring democratic institutions and responsible government based on the rule of law and respect for the governed comes on October 19th. Carthago delenda est!
\item For all the liberal supporters that says she should get help, why not pay for every member of parliament spouse also? After all if their spouse is doing something for them, why shouldnt they receive money also? Or is it just for SGT?
\item Well, Clearthinker. I wasn't aware that gays can force people to give them baked goods for free...
\item You've just called the innocent Canadians he murdered Islamic terrorists.  No surprise.
\item The world must stand United in fighting all forms of Trumpism which leads to Islamphobia, racism, anti-semitism and disgracing the transgender community.
\item Burly123: Mr Birch hates Chinese, Muslims and Black Canadians too.
\item Are you changing your lifestyle so it is not reliant on petroleum products or are you like Leonardo Decaprio and will continue to preach about the evils of the oil industry while you drive your car by your self 1 hour each way to work
\item Hawaii Dems proposed the resolution.  So let them take the complaints when the Con-Con results in a Constitution that outlaws gay marriage and abortion.
\item Funny how the author uses Jews in this column, but he is rabidly anti-Israel and pro-flooding of Europe with Middle East migrants.  This is so transparent. His fake sympathy to Jews is sickening.
\item We must be submissive Marian broodmares for Jesus.  Duh.
\item Watch this video and weep http://canadians.org/energyeast
\item They certainly weren't invited by the Chinese government. They were invited by House Christians as opposed to state-sanctioned Christianity.
\item Canada is a cesspool, used to be the nicest country on earth, now it is a cesspool of 3rd world immigrants and parasite politicians that have sold Canadians out to keep power. This place is SH.
\item Sadly, it is the sanctioning of bullying OF homosexuals that comes about as the result of how the Church deals with homosexuality - another reason gay teens suicide.
\item Support for Donald Trump in Canada is strongest in Alberta. Go figure!
\item You left out one trait, they are also Jewish.  But if she had said older, white Jewish men, oh the outrage.
\item Especially those that are lesbian phobic and dead from the neck up.
\item So is Jason Kenney. No one today thinks that being gay and conservative are mutually exclusive persuasions, nor they should be.
\item Frankly I hope that it changes Britain for the better, and we make sure the Muslims know that if thye want to live amongst us.. they better stop this nonsense, or a lot of them are going to suffer real pain.
\item Good question. I am sure the answer is not because Christianity is better than Islam. I think the answer has more to do with politics, economics etc.
\item No one should ever trust a Catholic priest or bishop after what they have done to so many innocent little boys. No parent should ever let their children alone with one.  As for this lawsuit, it sure sounds fishy as 'ICEEBEAR' so succinctly put it.
\item And we still have plenty of people who want to see more Muslims here.  Sickening...
\item If you watch the latest John Oliver video you'll see Ms. LePen at her very best, spouting anti-Semitic threats of tossing a few more Jews into the ovens, etc. She's a thoroughly disgusting person.
\item that example is retard tier regardless, even you should get it straight away
\item You don't know any Catholic heterosexual males who like classical music?  More's the pity.
\item I tried to reply to you, but it seems citing published peer-reviewed studies on rates of Personality Disorders  among patients who also identified as trans is considered offensive.  ....which kind of goes to proving my point, that this legislation will be weaponized by high-conflict individuals suffering from personality disorders.
\item What am I missing here? The Chinese government going after Falun Gong ain't no difference than the US government building a Mexican wall and keeping out Muslims.  It's all a gong show seems to me.
\item Plenty of difference. Palestinians stab innocent Jews in Israel who are going about their day-to-day lives.
\item Try marching down to a stripclub respectful places and everyone has a price what's yours? Just cause someone is different then you doesn't mean protest it. I didn't protest that Obama couldn't say Muslim terrorist even though every time it was just that.
\item Maybe better than lying and cheating
\item Have you ever tried to get into a University with the same GPA as a black, gay, woman with a limp?
\item same as gay marraige ........ cowardly unprincipled politicians scared off by a small vocal group who want to impose their unfair peticular religious dogma onto others...throwing the common sense of my 91 year old WWII vet dad out the window.  Cowards!
\item I have no issues with these types of individuals. However it is unfair to the genders that were born female. This transgender may be a female now in physical appearance but still maintains the strength of a male through
\item Ran gas chambers?  You're defending a mob including organized Nazis who were yelling anti Jewish slogans at their rally.  Darn right people like that used to run gas chambers, so why are you defending them?
\item I'm a white Evangelical Christian. I proudly cling to my Bible and my guns. I am a member of the NRA. I am a proud American.  I am your worst nightmare. And there are about 100 million of us.
\item That quote does not imply morality originates from Christianity. And the West's morality is dominated by Christian morality. Are you going to deny history? Our past is overwhelming Christian.
\item Huge scandal'?   That would be the hundreds of gay priests who molested children.  That was a huge scandal the church may never fully recover from. The burial of gay parishioners isn't something that most people care about, so it  hardly rates as a scandal.
\item Pay the firefighters by the call. Only when they are doing the job. Not while they are waiting for the 'work' to show up.
\item The islamic kingdom asked for more cupholders and a backup cam next year
\item Just the Kid can not protest against a Muslim leader.  That will be Islamophobia.  Hahaha.
\item You miss the entire point of the article and seem to want to besmirch any female leader you believe is on the left. Yours is a political, anti-female leader rant.
\item Yeah, the very one's that like to practice sodomy in the privacy of their bedroom but deny it to gay couples.  Tee hee.
\item I find it near impossible that a true Christian could be a republican.  Republicans have abandoned their values and are today frauds.  I am talking the national level.  I think there are a few good republicans in Hawaii.
\item Yeah let's focus on Shumuer. Let's FORGET that Donny is the most incompetent president in US history...
\item You have to admit that the blacks have had it harder than the Irish, Jews, Ukrainians, etc. You see, if any of the above changed their names, you couldn't tell they were different. A black person can't change his name and look like a white person.
\item The 1\% in this country are largely liberal Democrats.  Most of them are liberal Jews and liberal WASPS.  Watch FoxNews sometime, you'll learn new things !
\item Next year he can book passage on the Sliverseas cruise ship as it does a Northwest Passage cruise and save taxpayers money.
\item Isn't that we they thought in 2008 and 2011. Some seem to think they are still the natural governing party. The Tories are not the natural governing party, but neither are the Liberals.
\item I wonder how the hermaphrodites feel about this? Seems the tranny community is getting all the ink.
\item Russia as a whole is hostile to homosexuals.
\item Clueless! I see you still are!
\item Muslims were here before cars and airplanes. Again, it's somebody writing in asking a question. What does SJW have to do with it?   We should all be concerned about border officers targeting/harassing people for no reason.
\item Not to worry.  Obama is importing millions of Muslims to replace the Mexicans.    Mr Trump, build that wall.
\item 1 in 3 billion?  were the 2 Boston Marathon bombers 1 in 3 billion?  was the Florida gay nightclub 1 in 3 billion ?  was 9/11  1 in 3 billion ?
\item You and your ilk should be duly processed and charged with promotion of Hate against Jewish people!
\item She swears she wasn’t doing it when we were together and it was only pills that she was doing when I kicked her out the last time plus I haven’t fucked her in 2 1/2 years but I still feel like I should get tested for every disease known to man.
\item The military is being abused........by the freaks that the 'Hoodrat' let in.......transgender freaks of nature.
\item Whatever the reasons, they are still dumb. Don't want to show your face?don't become a citizen.
\item Were you quivering in your perma-virgin rage as you typed that out?
\item Never thought I would ever agree with Mr. Simpson on anything. I do on this however. A very good description of what's wrong.
\item Thousands of transgender members are CURRENTLY serving. And, in a tweet, Trump just ordered all of them to be thrown out.
\item Oh sure Ben, it was just about opportunity, because these priests were on an island where there were no females.  Is it really true that gay people think heterosexual men are attracted to boys?  What a strange idea.
\item This is among one of the most ridiculous lies spoken to date: ' discriminates against homosexuals '.  From the 2016 GOP convention speakers: Mr. Thiel : 'I am proud to be gay, republican and American' Mr. Trump: 'I will protect our LGBT citizen's from hateful foreign ideology'.    https://www.youtube.com/watch?v=lSVLpzGseXw
\item Only problem is we now have two little dictators and one will feed the other's narcissistic needs.   Trump's daughter Ivanka converted to Judaism so it will be next to impossible for him to be remotely impartial in this dispute.   This will not end well.
\item You declare that homosexual acts are immoral and evil.  I declare that you are evil for trying to devastate a group of people just for being who they are.  So whose declaration should carry greater weight?
\item I support your cause 100\%!But at the same time, I support political and economic autonomy for aboriginal nations. I think Canada running the lives of aboriginals is completely wrong.
\item Women and children first. Helping those who are most vulnerable first isn't discrimination, it's the right way to do things.
\item At least we don't have to worry about transgender hottie hottie issues on an airplane today.
\item Those stories about gay sex orgies aren't welcome at NCR.  NCR delights in blaming the Church for what gay priests do, and when referencing stories of abuse, adheres to a policy of gender agnosticism re the victims of these priests.   That is, if these victims are male.
\item when speaking about people like the clintons, nasty is simply being kind
\item There will be civil war, too many people don't want to go along with this 3rd world genocide, there will be a war to separate and form normal nations like we used to be, not these 3rd world cesspools that are being forced on us now.
\item What's any of that have to do with this story about Trump's guy who's a wife beater, hates Jews, and may have committed election fraud? (Remember when Republicans used to care about election fraud? lol)
\item Trump says this is not a Muslim ban. He lies about his motives.
\item The women came out because he is a hypocrite, a child predator.  Comeon trumpers,  defend the child predator Christian, lol
\item Only the GOP extremists believe in God -- what a ridiculous comment. Seems the right-wing extremists wouldn't vote for Christ Himself, calling Him too socialist.
\item Hundreds of thousands of Hawaiians who are Christian know that stones are not sacred.  Christ is and Christ alone.  Stop making the ignorant bow to strones while the rest of you go about your regualr business.
\item dershowitz is a loud mouthed hook nosed jew scum who is loyal to israheil.  we can only hope that the brain cancer spreads quickly.
\item Compassion is for the person who does the wrong...' 'A person who does a criminal unjust act needs to be forgiven.' 'The adult people who have been molested need to offer forgiveness as well.'  Here we have another conservative Catholic that believes in compassion and forgiveness for pedophile priests.
\item Liberal bigotry against the Jewish began a long time ago.  Out damned spot, out.
\item The issue is why people feel the need to be able to detect gay people.  Over the years, many have claimed to have come up with ways to do this.  Why?  So people can discriminate against them?
\item Obama apologised in Cairo, was snubbed by Kenyan President for his gay agenda, was downgraded to a backdoor welcome in China, and was called 'Son of a W----' by president of Philippine. That speaks about his spine (or lack thereof).
\item Sigh.  Yes, DB-TA, protecting unpopular citizens like muslims from a government decision - in this case government decision by referendum.  That's exactly the kind of thing that Constitutions do, in Canada and elsewhere.
\item You're missing the point. Pastors,  Bakers and photographers don't want to do your gay wedding. That's their choice. Go somewhere else that WILL.   I'm perplexed why gay people would want to support a business that doesn't even support their gayness anyway lmao
\item Time to ban Islam from all western countries.
\item The 'citizens united' supreme court decision is a large part of the escalating \$\$\$ involved in American elections
\item I generally avoid engaging Odinsson Underbridge, or even directly reading his nonsense. However, you bring up a relevant point. Yes, there are indeed racist POC, antisemitic Jews, and even gender role intolerant GLBTQ. They are not a contradiction.
\item ...he had a prayer rug at work and took regular breaks for muslim prayers....'  That just means he discovered the hard way there's 10 different factions of Islam ,and they all hate and want to kill each other.  Assuming your statement is true , that is.
\item These are the Nazis of the Muslim world.  Like the Nazis they have destroyed  historical sites and statues representing views opposite of their own. Like the Nazis they indiscriminately kill those who they consider to be sub-human.  My condolences to the Spanish people.
\item Certainly a lot more then Trump is. Think about this, OUR Government has destroyed our country MUCH more then Islam could ever dream of doing. Think about it.
\item Israel: democracy for Jewish Israelis, discrimination ad second-class citizenship for Israeli Palestinians, and apartheid for Palestinians in the West Bank and Gaza. That is what is supporters defend.
\item Will you stop trying to put people into neat little boxes that fit your preconceptions? I am staunchly Conservative. I support the right to abortion.
\item Nonsense. You have any evidence for this claim or is it a religious belief on your part?
\item That is one of the differences between D’s And R’s.  R’s celebrate sexual assault with their orange messiah.  D’s cast aside the sexual predators.  Very Christian, the sexual assault that is
\item Today in France, the Jews no longer have to fear the Nazis. They are being attacked by the adherents of another ideology that is just as odious and violent - one based on the teachings of a Seventh Century pedophile.
\item Oh yeah, you gotta watch out for those cut throat Christian suicide bombers.
\item Thank you for the nugget from Breitbart. This is not an accurate rendering of the British Medical Association's guideline, which merely acknowledges that most people who get pregnant are obviously women but through language choice 'we can' include other people who may get pregnant (intersex or transgendered people).
\item I identify as  transgendered ladybug sandpaper. your opinion is hate speech to my gender fluid.
\item The article states 'trans gender Individuals,' which implies inclusivity for anyone who identifies as trans gender.
\item In all the times I've used public bathrooms, I've never been concerned nor saw a transgender using the women's bathroom.  I'm far more afraid of someone leaving their body fluid or poop on the toilet seat than I'm worried about someone's gender.
\item Pan, When Jesus was on earth, he was a dark skinned middle easterner not a ‘white’ European, i.e. he would be considered a ‘minority’ by current general standard.  So what are you going to answer when Jesus ask you 'Pan, Pan, why do you persecute Me?”
\item Everyone knows that the rich are hurting and need our financial assistance. 
\item But I bet you're equally against increased immigration.
\item These are simply forms of progressive Catholicism of a non-white culture.   Who are we to judge?
\item You think the USCCB would choose a transgender woman as a shill?
\item @quazz Your panties are in a bunch
\item Imam calling for Jews to be killed in sermon at Montreal mosque draws police complaint'
\item A commie Jew like (((Weintraub))) trying to restrict freedom of speech for the filthy goyim? I'm shocked, I tell you, shocked!
\item Guess men would be better off finding a feminist who enjoys sex then. You'd think we'd learn.
\item ridiculous, but it's OK to let and encourage 'children' about transgender......
\item They have another choice. They could leave Islam and religion altogether or convert to another faith.
\item Not really. Perhaps you might ask Jesus or Buddha or Krishna or Mohammad.
\item This will, of course, be used to try to shout down anybody who questions the number of Muslim immigrants and refugees that are let into the country.
\item I don't agree that they drive American was, but I do believe they are the source of a lot of trouble in this country.  most jews are crazy liberals and are constantly trying to be in control to achieve this.
\item Seriously? No.  Socrates was Greek, therefore a Greek was Socrates.  Socrates was a homosexual therefore a homosexual was Socrates.
\item In what universe is a wild bear 'cute and cuddly' And that's just the beginning of problems with your analysis.
\item FAKE news.  There's no such thing as a transgendered person who can live a good life and serve productively.  These are not real people!    /s
\item Thousands upon thousands of men and women out of work and she wants those unemployed to vote for her ????? What kind of job does she have for them???
\item Many parents are blinded by faith and these are the ones you have to be aware of. Parents that find out their kids are gay and then try and convert them or in some cases beat them.
\item Yep, 15 Russians on Facebook were able to counter the 24/7 bash Trump media that included CNN, ABC, NBC, CBS, and MSNBC.
\item Ummm, your Christianity has a bloody history as well. Any fear-based group is capable of violence -- be it by strapping a bomb to yourself or by voting for someone to do your bombing for you.
\item How do you feel about Obama pardoning a transgender traitor that cost taxpayers thousands of dollars for a sex change operation.  Knowing you probably pretty good.
\item Come on Kenney, quit attacking everything Trans and admit who you really are.  Albertans won't judge you too harshly.
\item Israeli press suppression behaviour should be publically denounced by all Jews. Israeli right-wing nationalist are now operating as the Fascist of old.
\item Would the transgendered adult male who now identifies as a prepubescent girl suffer from a psychological disorder in your opinion?
\item Eid holidays will be coming soon and Easter will be gone.  The collateral damage will be on women and homosexuals.
\item I think a narrow government role is what we're getting now. Doesn't seem to be working.
\item Married man here, not a priest.  Simple question though: who do you think Jesus would say has fuller participation in His Church?  The power hungry cleric or the ignorant farmer receiving Communion?
\item How does Miller justify this sudden conversion to 'libertarianism' with his 'I'm the Christianest Christian that ever Christianed'?  The guy is a huge. swallowing hypocrite.
\item Ridiculous. Tax bracket information is available to everyone.
\item May I ask what Viagra has to do with the Trans situation? And since you are talking about Viagra and costs, how much is spent on each trans person vs how much is spent on viagra per person?
\item I can't wait to read the Globe's torturous reasoning when they come to endorse Harper et al. at the next election.
\item Catholic pedophile priest is Judas Priest (judas iscariot) with lots of help from the Bishop.  There are million and millions of judas priests.
\item Yes, they both identical... Christians stone women all the time, and those honor killings..., but the GOP covers it up. Just for you.
\item No doubt these gay Chechens will be bringing their wife and children just in case anyone they know sees them in Canada and threatens their family back home in Chechnya.
\item The bible convinces you that you don't have to go to Church.....  Really?  how?
\item The audacity of claiming Clinton's campaign is running on insults from the team where all Mexicans are rapist, all Muslims are terrorist, et al is truly insulting.
\item Christian, Jewish, islam are the death religions. You have to die to reach heaven.
\item Harper's promise of greater transparency in government was a bunch of baloney. Why should Canadians believe in anything he says now.
\item I believe that the man was mentally incapacitated when he wrote his 1986 letter to the catholic bishops on the pastoral care [sic] of homosexual persons.
\item So we don't need drunk driving laws, speed limits, public health care, trade laws, minimum wage laws, etc? Think your theories through a little bit next time, buddy.
\item What is a trans woman is that man, I am confused.
\item jesus, you are taking this very hard
\item Isn't that amazing? The cognitive dissonance of his followers is stunning.  The guy's a huckster, non-Christian, corporatist, trust-fund brat (everything they claim to dislike) who has NOTHING in common with his followers but they love him.
\item Most of the people trying to kill me thought they were just white Christians doing God's will. The KKK is a Christian organization.
\item I wonder if they would turn away the help of gay paramedics, ambulance drivers, E.R. staff, or fire fighters.
\item How does allowing gays to marry affect straight marriages?  And you don't have to remind us that your knowledge of communism is nil. We already were quite aware. Incidentally, how does the 'traditional family' protect from 'tyranny and Communism'?
\item Ok Epnd, I'm curious, I'll bite.  Why the big hatred for Jews?
\item I read on three different places on the internet that Nick Travis is a transgender bathroom checker vigilante. Its out there, go do your own google search
\item may be allah should born all muslim's women without face . or they should stay in countries where these thing were invented like burka and all that crap. seems its not muslim women who are protesting it seems like politicians want muslim vote
\item NEVER UNDER ESTER MATE WHAT A CATHLIC JEW WILL DO
\item Ban transgender military personnel willing and able to serve,  …promote those who commit sexual assault.   (…not like sexual assault by drill sergeants is a new thing.)
\item on the other hand his toupee has always been a loyal follower
\item Such a weak attempt at diversion. How about Mr. Phillips is bigoted towards gays? Dislikes gay people and gay couples? Uses his religion as a sword and shield against gay people?
\item Once again Mr Saunders has managed to deflect Islamic problems in the West by claiming that the far-right is a greater threat to European Jews.He probably also thinks that white supremacists elected Donald Trump and British Skinheads were responsible for the Brexit vote.
\item You are pretty ignorant of what's going on if you think this is about protecting white people.  See my other posts on this article citing why affirmative action is BAD for Asians and Jews.
\item How do you know transgendered people are not using public restrooms now? Do you check their junk, when they walk in the door? These 'bathroom bills' are a solution in search of a problem.
\item Amen. Your decency shines through
\item So, turns out the anti-gay bigot is a pervert and kiddie rapist.  Of course the GOP stands up for him.  Being a pervert is only bad if you're a democrat.  Its a bonus if you're a republican.
\item I hope he'll gather his coalition of: birthers, evangelicals, white supremacists, conspiracy theorists, neo nazi's, commies, and some local tough guys, to go fight them.
\item Impeach Trump. He's a danger to the United States and all that it stands for.  Deprogram his deluded followers; they're as bad as the Germans who refused to see that millions of Jews were being killed right under their noses.
\item For liberals to use fear mongering and Islam bigotry to justify military procurement is just another sign of this governments loose relationship with ethics.
\item The Pulse nightclub shooter was motivated by Islam's traditional rage against homosexuals.  This I what you must come to grips with.
\item If you do not respect Canada as a constitutional monarchy, Do not become a Canadian.
\item Some of Ezra's supporters have asked for an example of his hate.  Google his article about the Roma Gypsy's.  If you don't think it's racist, then replace Gypsy with Jew and tell me what you really think.  It's a great exercise in exposing hypocrisy.
\item Florence is to gay males what Yachats is to lesbians.  Surely you know that.
\item wrong, you are typical of the problem in canada, this is not a federal responsibility , we dont need more government
\item FormerDougCo, Is the baker asking the gay couple for a cake? How are gay people discriminating against religious conservatives. If your religion says you are to kill me, but I kill you first in self-defense, is my killing of you discrimination?
\item Then that would be a question of evidence as to which was the real reason for the refusal.   Are you suggesting there have been cases of bakeries that refused to make gay wedding cakes because they reasonably feared the couple wouldn't pay the bill?
\item This does not represent the majority of liberals any more than using a gay slur represents the views of Trump supporters.
\item All the seniors with the 'good jobs' refuse to retire and so there is limited opportunity for those younger than them.
\item Clearly it is heresy to suggest that the Church not have total control over people's sex lives, because Jesus very clearly said, 'Love God and let my Church control your sex life.'
\item We obviously need to keep having the debate until people recognize the truth and the side that denies it.
\item Why the Chinese are brighter than the Jews
\item Memo to the Tory war room: there is really no need to run ads attacking Little Trudeau. He will disappear up his own behind soon enough.
\item Donny D'Bag is an illiterate Jewish nobody who wishes he had 1/10 of Trump's money.
\item Lol, sea monkey. If that website can't handle photoshop better than that, they deserve to have supporters like you.
\item any time is the time to uphold human rights. the saudis need the LAVs . trudeau will never be right
\item Mystery?Really?Anger and Islam are generally not very good combinations.
\item Regardless of where one stands on the transgender persons in the military issue, you have to admire someone who stands up  for their convictions when it is difficult.  I'm glad Ken bucked the system, and that trumps politics any day.
\item This is the stupidest thing Traitor Dan has done, since he signed that open letter to the leaders of the Islamic Republic of Iran.
\item Its what progs do. They love to fix that which isn't broken.
\item They don't like ostentatious expressions of personal religious beliefs, especially of thousand-year-old homophobic, misogynist, anti-science dogma. That makes them more logical than insular.
\item As the wife of the prime minister she deserves help with their three small children and for the many organizations that ask for her help. She is not a shill for the Liberal party but represents all of us. I support giving her the help she deserves.
\item I hope those professors are just as vociferous in supporting those who are critical of islamic doctrine. Will they leap up to defend those falsely accused of being islamophobic?
\item For anyone who wants to help the transgender community fight intolerance, here's a GoFundMe campaign for an awesome nonprofit I've supported in the past:  https://www.gofundme.com/help-save-gender-justice-nevada
\item give it a rest people the story is toast find something better to talk about like the provincial liberals they should all be in jail
\item Indeed. The Tories are playing fast and loose with the Charter these days. We especially need to protect the freedom of expression of those people whose views are considered offensive by many.
\item You know in everyone's life there is grief, stress and anxiety, but most people have no choice but to keep going each day and there is no organization encouraging them to come forward and be taken care of.
\item not an argument.
\item Hey Roach, Like yours, the Harper reputation will be like that of the Tea Party rednecks in the US who controlled him 100\%.
\item Why bother with this silly article; we already know how he will handle this. Can't understand why the bias media keep calling this a Muslim ban when 87\% of them worldwide are not affected. Silly, stupid and disgusting.
\item I think, but I'm not certain, that it says that the more women in government thebetter, regardless of their integrity, morals or political views.
\item If it promotes standard politically-correct orthodoxy, and if it sticks a blade into an elderly Jewish professor, then yes.
\item Meanwhile, Trump is up early to tweet about transgender in the military.  The man has the attention span of a gnat.
\item . "Stephen Harper is a nasty man" - Former Conservative Newfoundland/Labrador Premier Danny Williams .
\item It is unfortunate for Kang that he was not caught, tried and convicted while Obama was in office.  He could have then claimed to be a transgender and might have received a pardon like Obama gave another spy, traitor and transgender named Bradley Manning.
\item 30 yrs ago that small number of malcontents were gays
\item How so? None of us believe Tulsi's shift on gay marriage was genuine, so don't even go there. What else?
\item What a hypocritical editorial!
\item What garbage.  She isn't a girl. It will be interesting when teen age boys declare themselves transgender so they can explore the bodies in the girls locker room.  We can at least drop sex ed classes from schools now
\item Human rights 'advancing' is precisely why we have most of the problems we have today. Everybody has a right to have the gov take care of them while taking no reposibility for themselves. It is quite ridiculous.
\item J'accuse !  Witch! Counter revolutionary! Jew! Appropriator!
\item Butinski, here is another theory.  The person at the helm was a transgender who was distracted while putting on his make up.
\item Then why don't you seek SOCIAL JUSTICE from the private sector employers who have sacrificed their workers' benefits while the corporate executives retain theirs and rake in ever increasing salaries and bonuses?
\item Hey the voter should know eh what are the Lieberals hiding about him ?
\item Easy:  1) They won't allow female elders (church leaders responsible for decisions) 2) They condemn co-habitation AND marriage between homosexuals. Can't get much plainer than that!
\item Did this commission include black trangendered womxn, Black non-binary persons and black intersex bodies? Or did this commission exclude this marginalised and oppresssed group from these particular sex and gender conversations and policies?
\item The defence claimed self-defence, not stand-your-ground.
\item Not the same as being gay, just having alter boys more at hand. Hopefully the modern number is small enough that the sample is small too. There are no reports of Vatican abuse, where the Lavender Mafia has its turf.
\item Using the name of a historic figure from 1300 years ago noted for killing muslims and driving them out of Europe is pretty obvious, don't you think? One reason I use Alceste is irony, skyofblue. Are you concerned about it?
\item You do remember what Paul Martin had to do in the 1990's remember? You realize he had to do that because of a massive mountain of debt built up over the years preceding him. Ridiculous to say that red ink doesn't matter.
\item The sanctity of horse is ingrained, because they are animals that perform a service to humans, and are also pets. Can't compare them to cows and cattle.
\item Oh, so if someone comes out as gay, it might mean that he has an aversion to sex acts between people of the same sex?  Please.
\item What's the matter with your world?'  Sessions is a closet transgender.
\item Transgender people to not vote Republican in 2020
\item Wow, that Goldy is seriously racist.  It appears that Levant is a self-hating  Jew out to torment his brothers and sisters.  The Rebel is promoting hatred and division and Canada and should be investigated by the RCMP.
\item Except that most of the Republican hierarchy have failed to serve their country in times of war....Bush, Cheney, Rove, Trump etc. And the American values you speak of are exclusive of white Christian right wing folk....a minority in this country today, and are the values of hatred and bigotry.
\item No longer needing Jewish votes, Mr. Obama was free, finally, to punish the Jewish state in a way no previous President has done.  Can there by any doubt…any doubt whatsoever…regarding the real purpose of…the Iranian nuclear deal?!?
\item The only way LGBT lives are 'hell' is due to the effect of the  blatant bigotry on the part of this 'Prince of the Sect.'
\item Somebody should explain to President Trump that we defend our country with more than rifles and cannons. Our complex weapon systems now demand brains and training. On these requirements our transgender soldiers amply fit the bill. Indeed, more so.
\item I hold the governing association responsible, not this transgender boy. He asked to wrestle with the boys and was denied. There is little question about the advantage he had over his female opponents by taking testosterone but, had he wrestled with boys, it would not have been an issue.
\item So, let us assume that Milo has an excuse for his views on the gay love. I  wonder what's Bill Maher's or Samantha Bee's excuse for being crude and hateful?
\item Gays  are not imprisoned and flogged in Israel as in Gaza, Iran, Saudi Arabia etc.   Pride parades in Israel  None from Morocco across north africa to Pakistan
\item Another 'commentator' from central Canada that doesn't know thing one about which he speaks.
\item More accurately the Church of Jesus Christ of the Latter Day Saints reiterated its teaching that engaging in same sex activity is prohibited, and restating the consequences of flouting that teaching. Nothing here to see folks, move along.
\item who knows, God may very well exist... I just don't think he's visited for quite a while
\item Now maybe he will have to answer to his extremist views on women and gays.
\item You have demonstrated your ignorance of the Catechism.   Canon 915 certainly applied to Tim Kaine due to the fact abortion is intrinsically evil verses the issues of prudential judgement.  It's too bad there are uneducated Catholics like you and Bishop McElroy destroying this Church.
\item Hypothetical... your daughter is a boxer, she's the champ... and the undefeated top contender is a Trans Female... you cool with it?
\item Jesus blowing freaks are a curse on education.
\item Your stupidity rises so high I can't see it from down here. 
\item if it is a reasonable search warrant, the courts could compel the defendant to provide the relevant password or hold them in contempt of court until they comply
\item UOIT is a rapidly growing university winning respect for its academic programs, particularly in the sciences. Try to keep up.
\item No such thing as transgender - just males, females, and people with abnormal brain scans. Brain scans are abnormal among those who claim that they are really their own body's biological opposites.
\item Black, exactly what do you suggest that the government should do? Be precise.
\item One comment...WHO CARES?  What are there, maybe two transgender students in the state??
\item Marginalizing people', that's a laugh. You're the one to marginalize gay people. You also label people all the time. So, since you don't like homophobe, 'gay hater' will have to do.
\item One wonders how many of these French are Jewish, escaping the rising wave of Judenhass that has swept France. Regardless, the result is to the betterment of Canada and PQ. Bienvenue, et Santé!
\item If Trudeau's government pushes forward with this, and the items mentioned in the 'open government' article, I will have massive respect for him and the federal Liberals. That they are promising to do this is very, very encouraging.
\item Are you suggesting that when we meet a Muslim woman we should arrange to conduct our conversation on a telephone to get over the issue of not being able to see her face?
\item This shameless vote is probably the last episode of Obama's 'Arab Spring' - radicalization Muslims everywhere and replacing moderate Muslim regimes with militant extremists.
\item The purity of the blood eh? Where oh where have I heard that before?
\item This is Liberal policy. Would Justin force all of his MPs to vote in favour? Would they have to be Pro-Euthanasia to even run for the Liberals? Would he accept any limitations at all, or would it be 'on demand' ?
\item It's not racial rights, it's legal rights in the treaties stemming from the Royal Proclamation of 1763. You might want to learn some of this nations history, JB0713, and accept your responsibility to observe the law.
\item All 'western' countries need to get their freaking act together and send lovely Muslims back to the middle east.  Let them fight it out for eternity.  Their problems are not our problems.
\item Yeah, well ... Justin may be completely abusing his position, but Harper was literally the anti-Christ. Plus ... uhhh ... conservatives are bad and evil.   So leave Justin alone.   (Submitted simply to save some time for the usual apologists.)
\item Only partially facetious I blame that purple dinosaur, Barney. Where no one loses
\item Bravo. Let tolerance, equity and freedom be our passwords, and let them trump fear and hatred.
\item In the U.K. the word used was 'sissy'. It described boys who were unusually timid. Nothing sexual was intended as no one knew about homosexuality.
\item exactly first is was 'Who am I to judge?' about gays  then later he does not want gay priests  all platitudes like Justin Trudeau
\item Transgenderism is a guaranteed way of getting some attention when a youngster gets none at home.
\item Oh those poor criminals just trying to get free stuff
\item Yes let's have free votes for culture war issues such as SSM, abortion, gun rights, prostitution, church and state, corporate lobbying, pipelines, whatever. It's more democratic that way.
\item Most Americans Support Open Transgender Military Service
\item There is no such thing as secular values. Maybe that's why?
\item Please mind you bigotry. We arent doing the 'gay equality is bad because of my god derp derp' stuff here.
\item Talmud is a Jewish text.  Jews tend to be Democrats, not tRump supporters and stood with and marched with blacks during civil rights - so puh-lease get your name straight without insulting a whole group of people.  You were responding to 'tulimd'.
\item There's some truth here... but as long as some Christians are pushing anti-science notions like 'intelligent design', it will be tough for the rest of us to take them seriously.  Personally. I think diversity is highly over-rated.
\item stoner' - a word with such positive connotations!
\item Stupid as saying all Christians are responsible for paving the middle east over the years when it has been mostly the US and Britain
\item IRT Boots - You my friend are factually wrong. There has never been a study that concluded any person with X\&Y chromosomes did any better as a woman. In fact the leading pioneer in transgender research has stated emphatically; 'the change more often does long term harm.'
\item Spoken by an expert in 'brown lipstick'.
\item Ya where is the gender equality there??
\item Well it didn't take danepol too long to drag out that old canard - anti zionist = anti semitism! In fact I think Manjra is an equal opportunity phobe. His Islamophobia is positively shocking! And in Feinsteins casecase it is anti zionist=anti Semite=self hating non practising Jew!
\item If the day comes when a LGBTQ  or Islamic university exists, and they forbid Christians from becoming students, unless they are silent about their faith, will the government be so interventionist? Will Christians even be allowed to attend?
\item excellent, Quinn is a complete dolt.
\item Yes. If this was reported in a unbiased newspaper, it would read:  'Black Man with Ties to Alt-left arrested for Threats on Jews'.  but....wow...there is Just Too Much truthful, disturbing facts! -it Must be 'spun', it must be 'softened'. Disgusting!
\item I choose not to be gay, and I am a bad actor.
\item Beyond hypocritical article. Obama has befriended rogue, anti-human rights, anti-gay enemies of democracy like Iran. Get over your fake news-based obsession with Russia and Trump, liberals.
\item Conservative? I don't think conservatives make bomb threats to Jewish community buildings, I think Nazis do.
\item If there's a bad choice available, Trump will make it! His latest pick of David Friedman as ambassador to Israel will most certainly not bring peace to the middle east. Does he want more Muslim extremists? Because that is how you get more Muslim extremists.
\item So, people being 'believers' or transgender are legitimate concerns of yours? Mississippi would probably love to have you. P.S. I think the irritation in the back of your throat is probably just BS.
\item Yeah all cops strive for the day they can shoot and kill somebody! You really have no idea.....
\item Delusions, hallucinations, fairy tales, religion. Not one ounce of evidence for any of it. Why is belief in Thor, Ramses and Zeus scoffed at?Religion is the last bastion of the ignorant.
\item The headline makes it sound like it's the School Board promoting hate. Not cool. It should read 'Ontario School Board's support prompts anti-Muslim backlash.' The school board is not fueling this hate. The hate is coming from bigotry and racism.
\item Islam permits true believers to dissemble in order to protect their beliefs and faith.
\item If you are openly gay, does that mean you are sexually active?  Because that would merit suspension all by itself.
\item The fundies' war on gay marriage is ironic. They ought to welcome any support for a declining institution.
\item Details, details RealistLon ... you must trust the Liberal Force, or be swallowed whole by the Dark Side. How else can a fledgling personality cult get a start?
\item And Palestinian's are the UN's chosen people in their objective of eliminating Israel and eradicating Jews from the region. Personally, I prefer God.
\item I agree the law should. But adding gays to if won't do that. Elimination of the law will.
\item I might suggest looking up 'The Lords Resistance Army'  They are very much Christian terrorists.  I might also suggest looking at the terrorism perpetrated by the IRA, again, Christians.
\item Trump cited no credible source indicating that transgendered troops are a detriment to the effectiveness of the U.S. military.  It appears he is making statements like this to solidify his homophobic core supporters.
\item Im offended at your homophobic thoughts- you know its ok for one guy to like another guy.... even though that guy might be transgender-
\item As your post demonstrates, Civil Comments has disabled the civility filter for the folks who were complaining about too many Catholic posts. Along with adding blocking, that puts things more or less back where they were with Disqus.
\item Trudeau and Harper are relatively close in age. You realize that right? Harper just looks older... and fatter.
\item As long as he doesn't watch it, he can say: Still haven't actually seen video of the 'Jews will not replace us' thing. Sounds like an urban legend. Willful ignorance.
\item and yet here you are accusing the Jewish Zionists of mere 'excesses' against non-Jews in Israel and saying absolutely nothing about Israel's barbaric, genocidal treatment of ten million Palestinians since at least 1935.
\item I wonder what would happen if the Pentagon brass decided that tweets are not official orders, and simply waited for Trump's milliseconds-long attention span to be diverted elsewhere? 'General Dunford, is the transgender issue taken care of?' 'Yes, sir!' 'Fine. Carry on.'
\item Rep. Hensarling will say it was gay people's fault.
\item Maybe Mary was bodily assumed into heaven because Jesus wanted to keep the Church from pawing at her bones?
\item What's your point - that this is normal and our climate is not changing? Wake up! The trend is clear based upon evidence. We are in a time of serious climate disruption with devastating consequences if we refuse to act to stop fossil emissions.
\item And just how would that ever be enforced with any confidence of integrity whatsoever! Your post is the perfect example of why our rights and freedoms are disappearing. You rationalize it for them (and for us). No thank you mog\_man!
\item I suppose you're right. If it ends up being a Muslim who carried out the attack we can just call it muslim on muslim shooting. or Muslim Terrorist attack?
\item arab culture do not compliment western culture there will be many many problems to come
\item His supporters with racist aliases. Mexicans are rapists. Ban Muslims.
\item And fear and loathing of gays.
\item Someday Lorna is going to tell us how important Christians among us - yes, even our most eminent churchgoing government leaders - practice the ethics and moral purpose that they take from the good book. But I will not hold my breath in the interval.
\item that commitment and ethic will bode well for the future........good luck
\item The usual sane analysis from Mr. Heinbecker.
\item Can we say Islam is bad? Islam is threat to Canada? It's illegal to say such thing?   Can we discuss this topic:    if Muslim becomes majority in Canada, or even 20\%, What kind of Canada will become?
\item The suicide rate for homosexuals is 4x greater (CDC stat).  Use of psychoactive drugs high.  Gay in this sense is a huge misnomer.
\item Canadian politicians promised to be nice to one another after the Jan 2011 shooting of Senator Gabrielle Giffords in Arizona. Like most promises from politicians, they are soon forgotten.
\item ...cannot be burdened with the tremendous medical costs...Again, our President is correct.' The military spends more on Viagra than transgender medical costs. The military has spent less on transgender medical costs than the country has spent on Donald's golfing hobby the last seven months. Your President is wrong again.
\item Killing is always a good thing...just ask Jesus in prayer.
\item you can knowingly infect someone with aids and it's ok. you can go to jail if you don't use the proper pronoun when speaking to the transgenders. are the flames hot enough yet.
\item This just in: Mass shooters are mentally ill. Wow. Really? Who'd a' thunk it?
\item Good start, but don't forget about indigenous, visible minority and trans-gender. I'm not making fun.  These and other categories follow closely on attempts to correct imbalances politically.
\item Sure, because such medieval nonsense has absolutely no bearing on having faith in Christ and following his teachings. Why dabble in this extra-biblical nonsense which, as we have seen, so easily lends itself to abuse, corruption and distraction?
\item Protestants? Jews?
\item This must be the work of Satan.  They probably rejected Christianity as being a 'white man's religion'.
\item Black Pride = being black and proud Gay Pride = being gay and proud White Pride = NAZI! - Hypocrisy is a greater crime than racism.
\item Since my prostate surgery so do I, but I do it in the proper gender assigned bathroom unlike the mentally deficient phony group calling themselves 'trans people'. You are as you came into the World, and even assignment surgery does not change fact to fiction.
\item A one legged, multilingual ,trans, first nations, marxist should be appointed.
\item I am sorry to hear that you were homophobic and hope you have overcome it. As a Catholic I am not and have never been homophobic so I have never had the need for such an examination.
\item I am white. Not a single one of my rights is threatened by my Muslim or Chinese neighbours. On the other hand, I do feel threatened by ignorant people who see immigrants and people of colour as the enemy.
\item her grandfather was a Nazi , or a Nazi collaborator and  clearly  a propagandist.  Basic fact .   Her  grandfather helped kill Jews in the millions  Has she ever admitted this  fact while attacking Russia today and defending Nazi collaborators in her own family ???
\item It's a simple fact that there is no mention of a sexual encounter in the report. It's a quick read, you should check it out. By your logic, is everyone who does not support her a homophobe? I am neither a lesbian nor a homophobe, nice attempted troll though.
\item Nancy Pelosi is right. She is the top Democrat fundraiser so black, liberal and transgender Democrats should best shut up and stop complaining. It's her party and she is the boss.
\item I've already popped the pop corn. How will Francis deal with this magna cappa pirate. (There is gay humor lurking in this analogy somewhere!)
\item Here are Kristin Beck's (a transgender ex Navy SEAL) own words to Trump:  ''Let's meet face to face and you tell me I'm not worthy,' Kristin Beck, a 20-year veteran of the Navy SEALs, told Business Insider on Wednesday. 'Transgender doesn't matter. Do your service.'  http://www.businessinsider.com/kristin-beck-trump-transgender-ban-2017-7
\item These warlock Dems did not deny Catholics when president Kennedy won they just killed him.  May God forgive them.
\item Islamophobia is completely justified because Islam is the religion of the Quran of which the unbeliever or infidel is to be killed in the most brutal means and  sharia law imposed.
\item Except there is no God.
\item Arguing in neo-Marxist platitudes? Yes, that person was born a he, so it seems nature is 'anti-trans microaggressing,' according to your neo-Marxist Critical Gender Theory beliefs.
\item For the Gay community and the Black community, both whom have been successfully pressing for broad inclusion to exclude the police whom the vast majority of people strongly support, is more than ironic.  It's just plain wrong.  Count me out his year.
\item You must be a Republican.  Swirling black hole where your heart should be ... Hatriotism!!  Praying hard to the money gods while calling yourself a Christian, but we all know by now today's Christian is a 'christian'.  Super fakey!
\item The gays need colonoscopy.
\item And don't forget that their version of Islam throws gays off buildings.
\item Yeah, it's clearly too hard. Let's just give up and let the carnage continue.
\item That was simply an excuse... The average German soldier will claim they never fought to exterminate the Jews....
\item The Pharisees are the predecessors of rabbinical Judaism. Isn't it way past time Christians dropped the whole 'you killed our Lord!' talk?
\item Americans know something Canadians don't. No one really wants to look at a Muslim woman.
\item Amen brother
\item Considering transgender bathrooms 'fringe' is what will get you tarred and feathered in a modern university.  You are an 'old-fashioned Marxist' stuck in the 60s.
\item So what is the percentage of the 3 out of 1000 people that are transgendered that want to enter the military? Maybe the transgendered should pick other battles.
\item Lesbian reject men so why should men protect them?
\item oh please, you think the session moderated by Independent Jewish Voices, a notoriously Israel and jew-hating organization, is going to be a fair and balanced discussion on human rights?  What utter nonsense.
\item Knowledge is power. Less knowledge for the public means more power for the government and the elites. The powerful become more powerful, the powerless become more powerless. That's the way the powerful want it.
\item Oh great, thanks to Trudeau Canadians are now effectively forced to buy Middle Eastern oil and to fund islamist terrorism whether they like it or not. Meanwhile, Paul Martin's shipping company can continue to lavishly profit from the tanker trade. Coincidence?
\item Fake Senator, Fake Tories, Fake Christians...
\item Could we have a list of acts of terrorism committed by Syrians in North America? Or anywhere?
\item This clarifies the situation - or does it? Is the Queen gay?
\item The law is cowardly.  These same Quebec Liberals went to the funerals of 6 dead Quebec City mosque members back on January, 2017.  Ten months later, they make a law that targets Muslims.  I guess for Quebec Liberals, the grieving period was over.
\item This is a huge mistake and a setback for acceptance of the gay community. If I lived in Toronto I would boycott the parade after this decision.
\item Maybe they should have a transgender division - the current system doesn't seem fair.
\item That explains all those Jews getting put to death in Israel for cursing their parents.../s
\item I have to call bs here. I'm a churchgoing Christian, and there is nothing in our teachings that says it's okay to prey on young girls. These people are lunatics. It's not okay to generalize. There are lunatics in every faith (or non-faith).
\item London, as well as most of Europe, is deteriorating rapidly.  London now has a Muslim mayor which shows how they have infiltrated all levels of government.
\item You conveniently don't mention your cohorts who call for extermination of Jews and Blacks. With guys like IQ006, IQ22, and the rest in your corner, well, I wouldn't call you  loathsome or deplorable like them but I think ' imbecile' has some merit for your selectivity.
\item Is  LBB  Barry  back  from  his  gay  sex romp  in   the  south  seas  yet?   When  he  left Moochelle at  home?
\item At least in that they continue the traditions of the Church, as Saint Pope John Paul II the Great was a firm believer in protecting pedophile clergy.
\item Muslim prayers are certainly something to be afraid of.
\item You are still saying that two deaths are better than one. Which is 'pro-death', not 'pro-life'.   You claim I am not a proper Catholic, which shows your innate arrogance.
\item Really? I guess you could just flood your data base with fictitious information and aliases but heaven help you if one of your aliases turns up being wanted by law authorities. Maybe the trans world where you can be 'fluid' has some merit (eyes rolling).
\item Patsi writes:  'Tommy went out of his way to attack Paul Godfrey of the National Post for being Jewish. '  -  No, I've attacked him for being a failure as a CEO.  Never mentioned that he is Jewish.  Try harder to be accurate, Patsi.
\item Transgender people allowed in militaries of 18 countries' So what? The USA isn't one of them.
\item ***And for my next comment, I will channel Roy's justification for everything***  You want Trump to fire someone just because he doesn't like Jews?  What is this? Nazi Germany?
\item It doesn't make sense from a military perspective to ban transgender service members.  Trump tweeted it to shore up the homophobic sector of his base of supporters, which also includes racists, xenophobes, Islamophobes, and sexists.
\item The Democrats use Antifa like the Muslim community uses radicals. They turn a blind eye to it until it is pointed out to them, then they shrug, throw up their hands and complain there is  nothing they can do.
\item You do realize that segregation of the sexes is not limited to Islam right? What about Orthodox Judaism? It's just as sexist. Come to think of it Catholicism is pretty sexist too.
\item Dual citizen ship is a No No. One can not serve two masters. When one bows to master one its but is facing master two and vice versa. You come to Canada embrace it. If one is sceptical, Just do not apply for citizen ship fair enough.
\item President Trump has been the most pro-Isreal president to date.. why would you hold him responsible for any anti-semitic acts? Why not blame the only people who still, to this day, hate jews? (im referring to the religion that literally preaches about killing jews.. and it rhymes with ShmIslam.)
\item That's funny. It's not like muslims have killed over 1,200 innocent people in terrorist attacks within the last month. Oh wait, yes they have.  https://www.thereligionofpeace.com/
\item The only false equivalence is on your side. Christians have killed and terrorized throughout history in the name of God. You know it. Stop pretending.
\item Gay pornography?
\item The Queen's kids should hold another one this week. Flip the bird to the insecure world.
\item You DO understand that the term 'progressive' and 'Conservative' are counter to each other, right? That is why they took it out to begin with. The proggy hate is string today.
\item That would be people from both parties , I know many democratic and republican White Christian Gun Nuts that vote , Some are not party drones .
\item Self-hating Jews subscribe to the Forward. Jews in name only. Artificial Jews. Other than being born to a Jewish mother, you wouldn't know they were Jewish.
\item So funny and so hypocritical - coming from such a pro-Muslim crowd of politicians.
\item Let's hope that the Liberals , by getting hit on the head by the 4 by 4 of reality, make some wise decisions... the ship of state was manouvered successfully through the global economic maelstrom by the previous government and now comes another.
\item The Israeli's like their combat females..a lot.  They also have no issues with transgendered military personnel.
\item Any adult who thinks he or she is a child suffers from some type of disorder. Most transgendered adults do not suffer from this disorder. I doubt there are too many baby-wannabes in the military.
\item After 44 years of the P.C.s and decades of Social Credit before that, Albertans have had enough of the 'right' for a while and are willing to give the NDP a chance. We'll see in three years if the NDP deserves another mandate.
\item Good move. Obama's LOVE for all things anti-American and communist was irrational. No reason to support a muderous regime. Now NIX the Iran deal....and Obama's love for all things anti-American and islamic.
\item Jesus had two dads .Seems there are a few people out there who think he turned out ok .There are more reports of elected officials abusing kids in bathrooms than transgender folks .
\item Dostoevsky is turning over in his grave that the likes of you has appropriated that name.
\item Racial hatred and white nationalism are the glue that hold the Trump coalition together.  It is the duty of every Christian to oppose it.
\item Stay far away ... and just keep your head in the sand and ignore the atrocities, the rapes, the killing. Yeah, that's a great plan.
\item Anti 'infidel' hate by Muslims has no place in MY Canada.
\item Why do they need to do your bidding for you? Were you out denouncing white guys who shoot people after Vegas and every other shooting? No, so why do Muslims need to do it?
\item  but to also dampen the traits of what makes America great, such as: compassion, inclusion, equal opportunity, fairness, equality, truth and justice.'-----------------------------In what fantasy world are they at?
\item Nope. We do NOT want to revisit the ideas of women's freedom and equality, thank you very much.
\item The 'liberals' trot out a family whose 'Muslim' son died defending your country and freedom and Trump continued the disrespect and insults afterwards. Case closed.
\item Maybe he is a neo-nazi. Is the homeless man he falsely accused Jewish? Strangely enough, I feel a little better knowing that this is a hoax and that there really isn't a mentally ill homeless person running around stabbing hallucinations.
\item The BBC has reported that this is a terrorist attack by a Pakistani Muslim.
\item and don't forget that the Jordanians destroyed Jewish houses of worship, religious artifacts (kind of like the Nazis). 1967 changed all of that
\item How kind of the noble to speak english....
\item skyofblue: Rio is a well known poster who posts almost exclusively on jewish or Israel related stories.  He clearly has an agenda and would be happy if jews were eradicated completely.
\item It is unlikely that many will ever go back. I agree that they should not have to endure the things you mentioned. However, it is also possible to protect them closer to home while ISIS is beaten back to the stone ages they belong.
\item Yeah ... you also said that about Trump's first Muslim ban.  How did that work out?
\item PIGL - Academics go where they can a job. If you teach political science or philosophy............
\item I wish gay men would just leave children alone.
\item George Victor, you may say I'm a dreamer, but I'm not the only one. I hope some day you will join us, and the world will live as ONE.
\item Is this 'Jewish diatribe' your best effort? Have a coffee and think out something better.
\item The fact Fr. Martin seems to be all about homosexuality all the time makes me think he is a left-wing version of Michael Voris.
\item Fully agree ! It is a disgrace to mankind that women fail to be respected and appreciated more.
\item That's true now because a dirty little secret is coming out about male orgasm.  Men can experience orgasm without an erection.  You need to think about this TomZ and how this relates to gay men as well as older couples.
\item  ... we are all super fakey 'christians' that vote for the war machine and will stab our neighbors in the back for a buck or bugger boys hooked on crack ... '  We all know what 'focus on the family' REALLY means ...
\item That was precisely what made me realize that St. Paul was mere man and Jesus was God. Jesus never said such a stupid discriminating talk!
\item Hasn't even been a decade since 2011... or is your numeracy as poor as your literacy?
\item Alabama people are too smart for the LEFTIST.. Thank you Judge Moore for running. They are scared of a Christian Conservative..A TRUE CONSERVATIVE. Sincerely,  Florida
\item Christian Supremacist. Now that is something Canadians should be concerned about.
\item My God, that pantsuit!  Is that Hill of Beans or a transgender from Saturday Night Fever.?
\item A tricky issue. 'Past homosexuals' are pretty much all dead of AIDS. And they have no descendants, so who do you apologize to?
\item Trouble is there are reasons why some muslims become radicalized.  The Donald's plan ignores all this and just was discrimination against muslims.  Pretty Dumb when you consider it is generally years before they become radicalized.
\item Same for me and he stands in a long line of good Catholic writers over the centuries who have used humor to point out the follies of the 'whitened sepulchers' who are destroying the church by their blinded eyes and hardened hearts.
\item As goes for all special interest groups. No more making private lives public. Hench no more gay pride parades, no more (fill in the blank) protest. Agree yes ?
\item Scot...you've missed a medication dose today?
\item I doubt the accuracy of your statement. Please give your reference. There is a lot of misinformation which is not helpful. Money would not be wasted if solid partnerships were formed. As Wab Kinew says it is not that saviours are needed it is allies.
\item Let me get this straight, There is no friend anywhere . . . because some Globe posters are opposed to Trump's executive orders, you hate muslims more?  And seven other posters agree with you?  That's a head-shaker.
\item They were assimilators, not invaders.'  Go tell that one to Palestinians.  The point of previous comments was about how Canada and the US turned the Jews back during the holocaust which we should all have learned a lesson from.  However, it appears that certain Trump supporters are quite incapable of learning.
\item I doubt if the imaginary sky-being that JT 'worships', is one that hates homosexuals, hates gay-marriage, believes there's a lake of fire for homosexuals later. But the radicals supporting scheer do so. So I'm as certain as you that it's a different zeus than yours and theirs.
\item The moral authority speaks, the robo's dance and vote.
\item Sure, run tranny Mike, see how badly she gets beat. Republicans would love it.
\item What's the matter, James, Hitler didn't kill enough Jews for your liking?
\item I provided many examples of transgender people going back for quite some time, thousands of years. Don't assume. Read the links. In India the Hijra have records going back 4000 years. The evidence is out there. It helps to read it.
\item What makes you an expert on using natural gas fired turbines for electrical generation? Have you ever designed or built one? Or are you just being your typical blowhard?
\item I am an older transgender person, I vigorously oppose this legislation. I have made a video on the topic that I hope people will watch: https://youtu.be/x-txjWzJQjU . The western world is quickly going absolutely insane.
\item Fedar is a Homo.
\item Its mostly run by lesbians now.
\item So has Christianity. This is one man, one case. There are a few boneheads but this is not 'widely abused'.
\item Wrong. None of the people at the vigil were involved in Reconstruction or the Indian Wars. To blame them for it is a RACIST statement. Kinda like blaming today's Jews for crucifying Jesus.
\item Happy to see you left Juneau for Anchorage Michae....One less homosexual is always good news.
\item Didn't think the police arm themselves to kill Jews, Blacks, and any other races opposed to white supremacy.
\item So?  They're all conditions which are managed individually based on their situation.  Why couldn't you do the same with transgendered? Jeez, they're people who WANT to serve their country, unlike our Commander in Chief...lol....
\item Too many left wing loons running this country. We are doomed.
\item Or it is heartbreaking for a segregationist American southerner that his Lord is much darker than him.  Plus most of those churches were built after Europeans had seen Jews. The original Jews were darker that the Europeans. Centuries of intermixing, rape, etc have made some Jews blonde and blue eyed.
\item Mulroney was personally responsible for destroying the PC's, such was the level of hatred towards him by all Canadians. Even Stephen Harper was able to leave the Conservative Party intact, with a good showing at the last election.
\item Homosexuals are men right?
\item ‘Do Sunni and Shia Muslims pray together in the Muslim prayer rooms in our Ontario public schools?’ I often wondered that myself. Doesn’t one sect call the other heretics?
\item It's ok. The guy wasn't Muslim, so no big deal.
\item Anti-gay training'......what sophistry !!  LOL
\item What a flimsy editorial built around a one-line quip that exactly characterized PM Stephen Harper's behavior and the idea that Canada has to do airstrikes because so many others are.
\item Natural law:   When a Church is filled with gay clergy, thousands of boys end up getting raped by these gay priests.  The Church has been right all along about homosexuality.   Trouble is, gay people have an inexplicable attraction to the RCC.
\item like when the Imam's spew hatred and citing scriptures against Jews and infidels.  We apparently have no problem with that.
\item truly an astounding feat that you managed to read all 500 words of this article and stay focused! That's a lot of hard work for someone like you. Keep it up!
\item Actually prayer before all of those activities you mentioned and many more is the way we should conduct our lives. What Prayer can do is open your perspective and it helps you see solutions that might not have been considered other wise
\item Hatred? Irrational or rational? Islamophobic?
\item When are they bringing Dr. Porter back to be a Conservative Senator. The world is so predictable. Mr. Harper ...resign. This si getting close. I hope the RCMP still have some honour enough to pursue the OINKERS to the top.
\item Seriously? A guy has to apologize for not being black or trans?  These are weird times indeed.
\item It's disgusting that any terror attack by muslims has comments closed.  free speech is dead in mainstream media.  I'm sure this will be deleted.
\item This is a great example of the sort of insensitive trans language usage that is twisting even people who agree that trans rights are human rights. ' ---------------------------- Agreed. There is a big danger that even sympathetic people will begin to feel alienated and push back.
\item Legally and factually dubious claims about the law became the platform to oppose equality for trans and gender non-binary Canadians, cloaking the underlying transphobia that animated the opposition.'  Wow. Do the authors really believe this about their opponents?
\item Look everyone, Muslims are great! Says the mainstream media narrative anyway. A Muslim a few days ago tried to behead people with a sword outside of Buckingham Palace in London but the MSM wouldn't reveal his identity because, again, Muslims are great!
\item Is this about Canada or the Conservative party? Perhaps some real generosity of spirit might make this noteworthy.
\item Pat Robertson is the man to call in:  http://politicot.com/pat-robertson-trumps-macho-groping-tape-orchestrated-god-show-americans-hes-definitely-not-gay/
\item Obama was good at the Propaganda he was given.  Like Billy Clinton he was a narcissist and borderline sociopath, and just read the scripts he was given while Wall Street fleeced America dry.  Funny how the feminists, socialists, communists, transgenderists and all the other -ists, like to pretend that didn't happen.
\item I'll be curious to see how Mr. Trump's Jewish son-in-law continues to 'advise' his father-in-law in view of the tsunami of anti-semitic hatred Trump's supporters are unleashing.
\item Agree completely. I think that if one reads the wisdom of the sages of every culture, from Seneca to Laotzu, one finds that stoicism in one form or another is the key.
\item I'm a lesbian trapped in a man's body.'  Might work.
\item It was also bound to get his base all tied up in some ridiculous hate of transgenderism.  You're being played.
\item The fact that the catholic church has paid it's victims millions of dollars shows it is corrupt. In Ireland it is murderous.
\item What's wrong with saying 'Happy Holidays' and honoring all Americans, plus giving a nod to New Years Day, another 'holiday', which we all celebrate?  I don't have anything against wishing Jewish people a happy holiday.
\item We all know what the problem is and the governments in the west wont admit it. Immigrants and welfare.
\item Yes, according to Catholic teaching.  A truly objective and persuasive reason.  Gimme a freaking break!
\item Naturally, in her usual rush to dismiss alternative energy Wente completely omits the enormous capital, operating, environmental, and human costs of fossil fuel production and use, which dwarf any expenditures on wind and solar.
\item What does Trump have to do to prove he is not anti-gay  Hold Justin's hand and march in 3 Pride Parades ?
\item Well this might not be that well written but as a life-long Vancouverite I think he's spot on. It also speaks to the thin-skinned nature of our city that so many are so offended.'But, but, we're so world-class!' Lol.
\item we have already charged that all, both Jews and Greeks, are under the power of sin, 10as it is written: ‘There is no one who is righteous, not even one'' -- Romans 3:9-10
\item Yes, Charlie. It was wrong to put the Cossacks out of work.
\item I never threaten.  Neither you nor your transgender 'wife'.
\item There will be little to debate as any study that questions transgenderism will never receive funding, and if somehow funded, will never be published.  When scientific debate and research is censored in this manner, we are entering scary times.
\item It's a dead heat so crooked Hillary is just as likely to lose as Trump. Let's hope Trump pulls it out and helps the middle class that have been forgotten.
\item those Kenyans!!!!! ...per capita metric tons of C02 emmisions stands at .3.....Canada stands at 17.....
\item Turing was persecuted because he was gay, even after his heroism in the war.  That is the type of society we had in the west when the Church had more 'leadership.'  The same ethic is trying to block women priest, but it is dying out.
\item My side won. Yours lost. The whining is from the very people who said Trump would never win.
\item Dumb and dumber?
\item screw islam n dummy troudeau you want more islamist dummy move to the desert build youre own outhousesn start building with your money not canadians most dont want more islamists bring more jews french greeks lebs forget the stupid bunch
\item Interesting point. Here again the left has step in it. I think it is the same, refusing is refusing. The because is the issue. And with the left the because is they agree with gays, and not with supremacists.
\item People of Canada and the world need to get behind Justin, Obama, Hillary and Premier Wynne in our fight against fascism, Islamophobia, homophobia, anti-semitism and discrimination against Transgenders!
\item Anyone but Justine in 2019!  If you're not a transgender, refugee on welfare well, you're not welcome in Justine's tent.
\item I won't be waiting. Liberals have turned fence sitting into an artform.
\item You are a mere 180 degrees off.
\item Hmm.  Gayness is great, right?
\item Sanity has been restored at the White House.  It is unfortunate that trans gender people think as they do, but it is ludicrous to force the majority of people to change social norms to accommodate how people think.
\item Unless you have some proof, you are deliberately trying to promote hatred against these people who have been repeatedly victimized.  Do you say the same about the Jews?
\item Canada, Sweden and Holland will be the only of 190 countries of the UN to have transgender soldiers . When captured by ISIS then what?  Putting transgender soldiers in danger . not very politically correct you can bet ISIS will have no  transgender prisons and no  transgender washrooms
\item Actual Marxists, who are generally atheists, could not care less about Quanta Cura. It is like having an Orthodox Jew caring about what the Bhagavad Gita has to say.  Catholics, on the other hand, assuming they have ever heard of QC, tend to ignore it.
\item Because he was getting out of the way of his cousin, the Christ. He deliberately spoke out against the sinfulness of the King.  He was not stupid, he knew the consequences.
\item Actually, they aren't making the law, they are following it. Unlike our Prime Minister who swore to uphold the law.
\item who cares
\item so that justifies the killing of Christians?
\item The teaching of Paul IV is more likely to have led many to hell -- or to have led them to construct a hell on earth for Jews. 'By their fruits you shall know them.'
\item You know this was an Obama supporter, ... how? Because conservative anti-Semite thugs are always so respectful of Jewish synagogues and cemeteries? And, ... don't get upset when people call Trump derogatory names.
\item The vast majority of white supremacists profess to be 'Christians.'
\item Can I sue a business owner who does not serve gays if they think I am gay but am not but refuse to provide a service to me?'  I think you probably can, and successfully.
\item I like ranked ballots because it reverse the narrowcasting that parties now do. I also think it comes closer to reflecting the wishes of the most voters. No more majorities? Good, lets start working together more often.
\item That one looks Jewish and that one's a coon. Who let all this riff raff into the room? There's one smoking a joint and another with spots. If I had my way I'd have all of you shot.'- Pink Floyd
\item And vice versa though...where are the defenders of the niqab? Why are they not also here, defending the religious right of Catholics to their beliefs?
\item And we must disrupt a church of princes with an ancient irrelevant theology that discriminates against women, gays, and people of other religions and abuses children while protecting abusers.
\item Yes that's why I used a balanced example of a white transgender female political figure and a half-black male political figure.    The pinata was brought to class by a student so I don't fault the teacher at all.
\item trudeaux father was still in kneepants when this incident occurred. why should this current pm nincompoop go stirring up history now? answer; he hopes it will get him more Jewish votes when this pathetic excuse for a leader is thrown out of office.
\item Just as an aside ....and truth be told the Jews did start killing every german they could find immediately after the war and by some estimates killed more germans than germans killed jews
\item Not to mention that Sharia Law is a central tenet of Islam, making it incompatible with our constitution. I'd rather see permanent western military bases over there creating safe zones so they can enjoy their home country rather than trying to subvert ours.
\item Beautifully stated! All people, both straight and gay, are capable of sinning sexually when we objectify our sexual partner, even if that partner is our lawfully wedded spouse. Thank you for pointing out the kind of sexual ethic that really matters - for everyone.
\item Don't white supremacists hate Jews? Trump is surrounded by Jews. His daughter is a convert and his son in law is Orthodox Jewish.
\item the homeless jew knows where he can buy a house for \$12,000......he would get a job but prison and jail made him to crazy to work......and there are not to meny places that will let him work becouse he is a voilent offender....so dose eney budy have \$12,000..... ???
\item NP, I think you misread Klastri's comment.  It said, 'fundamentally evil when it comes to LGBT folks and women's rights,' meaning as he relates to those issues, not on the whole as your interpretation.
\item Liberals have gone insane saying you can discriminate against people's feelings about themselves, and that is exactly what this transgender stuff is all about.
\item Really? Did you demand that Trump prove that Obama was a Kenyan Muslim?
\item Harper-crites unite!
\item there is no such thing as a trans anything, you are either a man or a woman, the only 2 possibilities.
\item It's easy to understand. The a**holes and smart-alecks here simply pretend not to, are blinded by malice and/or partisanship, and/or of subnormal intelligence. Your typical Conservative Party voter, in other words.
\item the homeless jew knows where he could buy a house for \$12,000......he would get a job but .....he has a long voilent crimele recorde....and prison and jail made him to crazy to work.....
\item Unlike Harpocrits he didn't take the money. Now crawl back into your box.
\item Omar is a Right Wing religious fundamentalist. There is always place in a Conservative Cabinet for that type. Reverse gay rights, abortion rights, minority rights, etc.
\item Did you know that president Trump's son-in-law is Jewish and his daughter Ivanka is a converted Jew?  I thought I would sprinkle a little 'truth' around.
\item Well, 'everyone' is wrong. ISIL is a sideshow. Assad is the greater evil and Canada should have no part of any deal that accepts any role for Assad.
\item How do you know that there was a medieval global warming. Did you personally experience it? Oh, scientists told you about it and you believe them. The same scientists who you disbelief when they talk about global warming.
\item Just rough gay sex getting a little out of hand.
\item Wow, if only we had elected officials who channeled their outrage over the transgender experiment toward fixing this issue maybe we could actually accomplish something.  While everyone focuses on the 'outrage' of Trump's tweet, we have people dying because of failed policy.
\item uhhh WHO CARES!  We are \$20 Trillion in debt and who cares about the 3 transgender people in this state
\item Give the finger to the society? Perhaps they choose the wrong society to live in.
\item A Jew can become a gentile and a gentile can become a Jew but a man cannot become a woman nor a woman a man.
\item My point?   You focused on his Jewish donors and his racial attributes - without saying why they're relevant.  Most people who do that are racists and/or bigots.  I didn't want to jump to that conclusion about you, so I asked you to clarify your comment.
\item MaryJay1, You sound like my kind of woman. We need to get together and unite the left. Do you believe in the hereafter? Then you know what I'm here after.
\item So does Trump hate Jews or is he in bed with Israel?  The media needs to make its mind up and have a consistent narrative to sell why we should hate Trump.   What a joke!
\item I wonder when will the children of Palestine go Gaza to give respect to their loved ones!
\item a bishop who enables a pedophile priest should be excommunicated and in a prison cell'  Is Law in a cell in the Vatican's prison?
\item Les, Yes and public places...Gay night clubs, Schools, Company parties, Shopping malls. The list is endless. We are not safe. We need huge government expansion.
\item Really, R.D?  How many transgendered persons do you know personally?
\item Orthotoxic faux Christianity NEEDS to be warred against.
\item Because they stand up and have pride in their province (Quebec), and stand against islamic/muslim tyranny . The rest of everyone in all of the other provinces are just sheeple. They've either succumbed to the inevitable, or just don't care anymore.
\item Because it is a necessary, but not sufficient condition. But supporting those conditions requires a collective effort.
\item It should not, but it should be careful in what it calls sin.  No one is rejecting the concept of sin.  Assaulting people because they are gay is always sinful, mortally so.
\item Jews are the least inclusive people I can think of. Try moving to Israel and see how inclusive they are.
\item Israel, and those that support it, pretend to hold higher standards.
\item There is no science that supports transgender. How can we scream at the climate science deniers and at the same time support government policy decisions that are based on personal agendas and not on science? If you are born male or female, that's what you are. Period
\item Well, aren’t we just a ray of frigging sunshine.
\item List of ' Christian terrorists' -  sorry this page is blank
\item What can be more 'balanced' than a white transgender female and a black straight male?
\item So you are complaining about human nature. Your argument seems to suppose that all the budget issues are the result of this self interest when the story shows that pretty much every voter has an element of self interest. So much for your argument.
\item But what is the intent behind the law? Are there really that many people wearing the niqab, which is uncommon even in most of the Islamic world? When I lived in the Middle East, it was either Saudi women or much older Arab women who normally wore it.
\item Keep telling yourself that the Palestinians firing rockets and missiles into civilian Jewish areas of a sovereign nation is not a violation of international law......you might convince yourself eventually.
\item The difference is that transgendered individuals are quite capable of performing their duties.  After all, 18 countries including Canada, Israel, Australia, Britain, Germany and France currently allow transgendered individuals to serve openly and it doesn't seem to have impacted their military readiness.
\item Richard, are you referring to the russian spetsnaz with advanced weaponry who portray themselves as 'regular' Ukrainians? Nice try comrade.
\item Some priests should be put out to pasture. I'm sorry that you ever had to hear such a wrong thing, John. The inability to have a perspective on what is really pro-life will kill what's left of this Church.
\item To the White Nationalists (Supremacists) in Wasilla: Upon Rapture you will all see a Black or nearly Black Jesus. Then what?
\item CGL can build pipelines in hell, rather than turn Earth into an inferno
\item What a hypocrite. Kenny, a 49 year old bachelor, when asked about his own sexual persuasion, has replied that he doesn't discuss his private life with journalists. http://www.canadalandshow.com/kd-lang-asks-jason-kenney-if-hes-gay/ So, it's monstrously unfair of him to breach the privacy of teens by recommending parents be told their kids have joined a gay-straight alliance.
\item The Royal Alexander? Did the Tsar visit TO in the 19th C. or are you being facetious?
\item I believe that within 15 or 20 years, people like you will be pretending they were people like us and wondering why people weren't shouting louder.
\item He should have condemned first and foremost the POTUS himself who, no later than last week at a press conference, broke loose on an Orthodox Jew journalist trying to ask him a question, qualifying twice his question (that the poor guy was unable to complete) as 'disgusting'.
\item The suffix 'Jr.' Should only be used when the son has the same first name as the father. Ironically, with your use of the word as an attempt to suggest he is a man of lesser competence you have demonstrated your own lack of competence.
\item At least Trump's wife is actually a woman and not a tranny like his predecessor's 'wife' is.
\item That's pretty presumptive and not very Christian of you, you hater.
\item HI:'Muslims have the most to lose from Barcelona' NO. The people that lost their lives and loved ones have the most to loose. Why is their answer/solution death????
\item Having a gay husband?
\item This is Muslims doing what Muslims do.  Why do they expect anything different from Islam?  Do they not look at history?
\item The owner was willing to sell them a standard off-the-shelf cake, but he refused to discuss designing any cake -- solely because the couple was gay. It is one thing to object to a specific design. It's quite another to refuse to discuss any design.
\item Disgusting excuse for progressive Catholic journalism that smears most of America as racist.  Hateful, worthless, stupid, harmful, irresponsible, and untrue.
\item Good Lord Jack***, did you just say Iran has never threatened the US? That's right, you did, in the third sentence.  But 'Death to America' daily chants by angry Iranians, ARENT a threat?  Jack, I believe you are practicing Taqiyya and a closet Muslim.
\item Cultural Darwinism at work. The weaker culture is moved aside by the stronger.
\item Liberal progressive democrats are the pathetic masses of whom Stalin had often referred to as useful idiots.   The indoctrination is complete, free speech is dead with the democrats.  If you're right of lgbtq communists transgenders, then you're a NAZI...
\item I've heard this claim before but haven't been able to substantiate it. Could you help and provide your source that proves the Prime Minister made the offer of help?
\item Looks like Assad and the Rusians know how to deal muslim terrorists
\item In Toronto anti-Islamophobia protesters outnumbered anti-Muslim protesters by a ratio of 30-1.  Just remember that Islamophobic bloggers. You will never win. Canadian society is tolerant and inclusive and Muslims will be welcome here.
\item Gays got a whole tale.
\item National Post article 10 days ago regarding UN resolution. Jewish donors feel betrayed by Obama.
\item Since when is it 'shunning' to deny Communion? Another poster claimed Paprocki had ordered all gay people to be buried in 'unmarked graves.' Insanity!
\item White is more controlling than is Catholic. Nothing new here.
\item Just think...if it was Hilary under the bridge, she could have arranged abortions for all the pregnant nanny goats and sex-reassignment surgery for the trans-goats.
\item Surely the catholic church should concentrate on it's dwindling numbers and paedophiles
\item Don’t ever trust Labradors, they will always betray you
\item This election in Alberta will come down to jobs vrs transgendered bathrooms.   Even the  lgbt community needs jobs.    Kenney will win handily except in Edmonton and central Calgary.
\item Margaret, what do you mean by 'some'? All transgender activists are denying science. There is no science to support this belief.
\item Jesus said the 2nd greatest commandment is love thy neighbor as thyself, the Golden Rule, which Mr Phillips and the rest of the fake Christians like him violate regularly.
\item so, you like making people sick, then. you're in safe hands.
\item None of these other religions force women to wear scarves or cover themselves.  None of these other religions murders gays and lesbians. None of these other religions treats women as second class subjects.
\item The 'violence against conservatives' comment is ludicrously hypocritical when one considers the rash of horrific violent crimes commited by right wing extremists like Robert Dear, Dylan Roof, and Jeremy Christian.
\item Threats are crimes. Do you think the Jews in the synagogue in Charlotsville felt threatened when the Nazis marched past chanting their hateful slogans or do you think they were snowflakes?
\item ya thats it blame the jews for living in thier own land, what bs
\item National security' is only important to Trump if it means keeping those dang Muslim and Mexican furriners out of the US. Hiring Flynn, an unhinged conspiracy theorist and compromised liar, as national security advisor is fine, of course.
\item These attacks on the gay community have to stop
\item Why did our PM choose to present that image' ? The same reason that snakes slither. He can't not make everything about himself and his self importance.
\item It's not the ban on sex outside marriage that is discriminatory, as it applies equally to everyone.    What's discriminatory is that that married straight students are allowed to have sex while married gay students are not.
\item Lets just combine the Catholic church and the Boy Scouts organizations into one entity.    They both have been doing the same thing FOREVER,  ABUSING and having Intestinal Intercourse with young boys.
\item As usual you missed the point. Trump and Clinton are playing by different rules. He gets to be a the new guy in town that everybody wants to watch and she's old news unless she's tripped up. Women are held to a much higher standard.
\item No. Strict enforenforcement is the only way. Trans people deserve no less.
\item Good. It's about time Russia and Russians got their comeuppance for supporting anti-Semitic and anti-Israel motions at the UN, thereby putting Jews and Israelis in the line of fire from inveterate international anti-Semites who wish nothing more than the demise of Jews and Israelis.
\item Latino's for tRump is like Jews for Hitler....
\item Justin and Adams deserve each other - political opportunists
\item Classical lies. Nobody is threatening to bomb Jewish kids people.   The call came from within the office. This isn't some sophisticated prank. Its typical Zio behavior.
\item I think MikeAA is an embarrassment to the Catholic Faith.  Certainly he doesn’t know what he’s talking about.
\item You don't understand international finance do you fatty.
\item He speaks to my wife in English, with a Brooklyn Jewish accent.
\item Just say NO to all religion, everywhere! It's archaic teachings with no basis in truth or reality are are just an indoctrination of fear to control the masses. If a so-called 'Jesus' was immortal, how can his death be a sacrifice? Circular bible logic at it's finest!
\item Thanks for a thoughtful comment. We need to get back to government that does 'what's good for Canada' rather than 'what's good for the party'.
\item israel is surrounded by muslims that are committed to its destruction ( including Iran)
\item Nice if you would mention the women too.
\item Catholic' scholars? A laughable assertion, that. Thank goodness no one reads or listens to the National 'Catholic' Reporter anymore.
\item I had no doubt you would see it that way...A Lesbian who has an affair, allegedly on school property doing school hours is not enough smoke to assume there is a fire ? Would you be interested in buying the Fairy Street Bridge ?
\item Trump was going to ball all the transgender people? Who knew he had it in him?
\item Have you ever worked for extended periods in Japan?  I have. Discrimination against the Gaijin is intense, if cleverly understated in the public domain. If you're going to make derogatory comments about a group of people, Christians for example, try not to look silly doing so.
\item Being masculine, caring and respectful have never been mutually exclusive.
\item Muslims would absolutely never allow their children to be taught comparative religion That could lead to questions and that could lead to e apostasy which is punishable  by death.
\item Bibi has alot of friends in Hollywood with Geffen records maybe Bibi could make a few phone calls. Trump Loves Bibi and Putin. Traditional Jewish music with a slice of Cossack dancers. Menu; Kosher food with Russian Vodka.
\item The question was : 'Please name one country where 'gaiety' is punishable by death.'  Your response was about gays and had nothing to do with gaiety.
\item Funny how you failed to acknowledge the other half of the statement--that Trumpty-Dumpty is every bit an amoral sham as Hillory the Blood Countess.  Kind of like how bigoted Christians justify their arrogance by quoting the bible out of context.
\item Where is the money coming from to pay for all the transgender bathrooms we will be ordered to build?
\item White Christians perhaps; not white evangelicals who are definitely not the majority!
\item Who cares what the Downtown Toronto Cocktail Party Circuit thinks.? The PM is right. The people stand with him.
\item This is the problem with transgendered people.  /s
\item The lives of 'thousands' of transgender people have been thrown into 'chaos' because they now can't openly join the military - give me a break.
\item Yeah, socialists want to exterminate Jews, like that Jewish guy Bernie wants to do.  I'd say the level of ignorance and lack of education is comical, except it's so detrimental to our country. Read a book sometime.
\item Sure Nathan - going to the Muslim war zone aka Xinjing where Saudi funded terrorists are routinely blowing themselves up , and trying to interview the terrorist sympathizers to do a story on 'oppression' is such an great idea. You deserve full of it.
\item If justice has no expiry date world history would come to a dead stop and God could not create enough lawyers to untie the knot !!!
\item Trump will probably blame some Muslim guy for getting him drunk.
\item Mr. Bernier’s team said the Scheer victory was due to the social-Conservative vote and the strong showing of candidate Brad Trost, who expressed his discomfort during the race with “the whole gay thing” ....... ======= Yeah, you can't be a conservative by that ....
\item HOw much did Frank Giustra give the globe to get this crap written. Obama, the gay coke addict did more harm than anyone before him.
\item It's not a Muslim ban, it's a ban against countries known to support/protect/harbor terrorists and non-Muslim countries are in that list like North Korea and soon The Banana Republic of Hawaii will be added to it despite being an actual US state! LOL
\item your name is redundant.
\item ... isn't that what 'christians' like yourself do, 'hide the perverts' within the Church all while fudging paperwork as to what is really going on ... always more money to tithe to support the efforts/paying out lawsuits!!  :)
\item I have to be careful not to disparage a practice that allows a man to divorce by uttering some word 3 times? Even by phone or text? What are you smoking?
\item Canadian patriotic fervor = Good. American patriotic fervor = Bad. Well, anything American is bad.
\item Nobody but socialists, Liberals,  Democrats and people in the news media believe  Muslims.
\item Doctors should practice medicine, not morality. They are professionals; they should keep to their profession in their work.
\item More sitting republicans have gone be found to be being creepy in bathrooms than the entire trans community.   Maybe we need to ban Republicans males from bathrooms?
\item Let's not jump to conclusions ... Aaaaaaannnddddd it's ISLAM
\item A clear case of putting it's people first shows me that our Trudeau government is on the right track.
\item Huh.  I wonder how the Jews in Germany in the 1930s would have fared had they had automatic weapons.  Don't be naive; not everyone is a pacifist.
\item ... 'christians' have that mastered ...
\item Jews are doing what any other people would do: resist terrorism. Palestinians are doing what no one else would do: engaging in terrorism and stabbing innocent civilians.
\item Like Tim Tebrow , Kapernick is a Christian activist. Go for the obvious , white Tebrow is a national hero and black Kapetnick needs to learn his place on the plantation.
\item Yer transgender phobia is unwarranted fake Beaver.
\item If you believe that no lawyer should represent someone you (or they) feel is guilty, then you have no right to comment on our system of justice. You know nothing about it. Educate yourself a little before you next vote, please.
\item One problem is that the Jewish community is too tied up with supporting Israel. Do they have allegiance to Israel 1st and Canada 2nd?  'The Jewish Federation of Greater Vancouver referred a request for comment to the Centre for Israel and Jewish Affairs.'
\item Ooh, an opinion by the Post.  I must immediately change my views.  Hillary could burn down an orphanage filled with transgendered children of color and beat them with Gibson guitars as they came running out and the Post would still giver her their support.
\item Wombat, despite my strong opposition to transgendered people serving in the military, I have to agree with you on every single point mentioned here.  Although I agree with Trump on many points, he himself is an idiot.
\item Holy mother of god what a dunce
\item uh ...it is well known that she has had a string of lesbian affairs and even fathered a child of Web Hubbels
\item but still an Islamic terrorist
\item Too funny.
\item I'm sure in your mind this has something to do with transgender people serving in the armed forces of the United States.  WOW!
\item I disagree with mandating gay Boy Scout leaders when we have decades of perverts using the Boy Scouts as grooming locations.  Not all homosexuals are pedophiles; but, the hundreds who have been convicted in Boy Scout Troops of abuse is justification to prohibit them.
\item Rapeing ancient cultures the hobby of the corporate Christian lobby.
\item Typical liberal Jew. Where is Hitler when we need him?
\item Hey pal, it's LGBTQ2S, not LGBTQQ2S - what sort of homophobic monster are you?
\item The biggest losers will be people living in Scarborough. So be it.
\item LMAO! I'm sure christian nutjobs praying in islamic countries  at a public school(!)  would be murdered if they did this
\item Muslims are not coming to Canada  to supplement us, but to supplant us.
\item Patterning makes the pederasts. In the seminaries, some gay men simply come out while others adopt the asexual ideal imposed on them as a way of regaining latency.
\item Deception is an integral part of the Muslim Brotherhood's modus operandi.
\item Considering how badly the church treats them, it's amazing that there are any women -- let alone nuns -- who remain in the church. May G\_D bless them because their church doesn't much care about them.
\item I had relatives killed by fellow Christians in Ireland during 'the Troubles''  Liar.
\item Does pointing out that a growing majority of Americans support adultery (abortion, same sex marriage, even theft), change God's law an iota?
\item In think let Biko also know that his sons Andile Mngxitama and BLF are obnoxious racists and antisemites who makes fun of the Holocaust and how Jews were 'turned into soap' by the Nazis. But would you expect of an intrinsically and explicitly racist ideology.
\item The Inquisition is not the only alternative to tossing gay men off buildings.   There are a lot of other options.
\item So you're down with female mutilation and executing homosexuals eh Len?  http://www.cnn.com/2017/04/22/health/detroit-genital-mutilation-charges/
\item Do your jewish friends know that you 'like' online comments that say that 'the zionists' control Canada?
\item Mr Harper has been around just about ten years, it's time to go, then we need to lobby for term limits and a PR voting system so we can return to real democracy.
\item Transgender athletes..... Transgender students.....  This is what feminism gets you in society.  This was unheard of only a short 20 years ago.
\item Thanks for the little dose if common sense
\item Wearing swastikas, making zeig heil salutes, shouting 'blood and soil' and 'Jews will not replace us' and championing an ideology that executed millions of civilians is a more accurate definition of fascism. Unless of course you're a Nazi apologist...
\item Conservatives have raised fears about men or boys claiming to be transgender in order to spy or prey on women or girls in public restrooms.' -Well then those 'conservatives' should be more concerned about the president being in any room with a woman or girl.
\item What a sterile argument.  Remember Canon 1083 \#3: 'sterility neither nullifies nor prohibits marriage.'  If sterile straights can get married and have sterile sex then so can loving gay couples. There really is no difference, Ken.
\item Trudeau, nice hair, good smile. Complete lack of substance on issues. Way to go.
\item Peace in our time!
\item Ericnorstog, speak for yourself, (We are all that homeless Jew).     Not me... If you are a slime ball and shoplift or are otherwise a useless piece of human being,  then you have chosen your destiny..........
\item This is an example of the arrogance and ignorance that exemplifies Anchorage and is the same as a bunch of ugly racist and bigoted White Nationalist Americans moving to Israel and then have the gall to tell Israelis, 'Jews, you're lucky we let you stay here.'
\item Precisely. He's forever sulking about how gay people have (mis)appropriated the use of words like 'gay' and 'LGTB' while he's doing his level best to re-appropriate the use of scary words 'sodomy' and 'sodomite.' Sadly for him, it isn't working.
\item We don't elect a leader. Trudeau wasn't/isn't crazy. All three were competent. Your comparison simply isn't relevant.
\item And since it wasn't transgender, they refused to use it!
\item My thought exactly when I read that he frequented gay nightclubs. I don't know whether you saw but even two days ago, someone posted here that this would turn out to be like the clinic arson.
\item You say vengeance, I say justice.
\item self servingnaked ambitionbad temperament... Anyone on the left may be just once consider writing a puff piece on HRC? Lie to me!
\item The (in)famous 1917 Balfour Declaration to Baron Rothschild on Palestine (as it was then called) perfectly encapsulates the root of the conflict: a colonial power pledging to European Jews land that belongs to neither.  That Canada continues to effectively support this travesty is shameful.
\item I have long learned to eschew the bigotry, hypocrisy, and ignorance of the libtard generation. Israel is the Jewish answer to the Holocaust. One of the most successful nations on earth, fool.
\item real amercins are pro immagrioshen.....jews what to move to usa ....death to trump.....death to greeddy capitlist.....
\item I'm sorry, but people who are so easily offended need to grow thicker skins.  They cheerfully go on about damning disbelievers to Hell or talking about killing gay people or cutting the hands off thieves, but they get offended by THIS?
\item How many times do I have to tell you? He didn't say he was open and transparent, he said that he was open to trans parents.
\item You live next to a base, which of course, makes you an expert. Based on this post, I can see that you are indeed an expert. Clearly, you have a PhD... Proctology I presume.
\item What is wrong with these crazy anti-racists and ridiculous pro-transgender nuts? Don't they know the revolution is about stopping classism?
\item So you go out of your way to see films about gay people. Most actual straight guys I know don't do that. They couldn't care less. You seem to care an awful lot for a 'straight' guy. Just sayin'.
\item Shouting hateful slogans about Jews, using Nazi language, can't be considered a 'peaceful' march. Regardless of what happened after and how, the march was violent in purpose and meaning.
\item You mean it wasn't a blonde blue eyed baptist yelling 'alluh akbar'   SHOCKING.  Radical Islamic Terror? Again?   (I bet by the end of day all of the ISIS apologists and sympathizers will be all over this wall defending radical Islam)  It's like Christmas everday with President Trump.
\item One thing I do know is that our Lord would most certainly 'have a problem' with a Clinton presidency which would have opened the floodgates to infanticide and homosexual unions.
\item It's Mass!!!  Jeez, Catholics can't even spell it correctly!  Always a capital M!  Always!
\item The biggest problem with the residential school system was allowing the Catholic church to get involved. We all know what perverts those priests can be with little children.
\item Like I've been saying, Trump is not a racist with a Jewish son in law, convert daughter and Jewish grandchildren. Along with a black friend Dr. Ben Carson. Honesty? Who is the bigger liar, Hillary or Trump? I will say Hillary.
\item If you believe in Jesus and live with that belief, you will find that you have a perfect peace continuously regardless of what life throws at you and that you enjoy living every day with a joy which cannot be described. You should try it some time.
\item There lies the difference.   Jesus and Christianity teaches love.    Islam teaches hate.
\item He was an excellent marksman. Was he Muslim? I hope, otherwise we cannot blame them.
\item Today's realities'... please, these realities were imposed upon these people who were doing just fine and would continue to thrive not for our destructive intervention. Now it is the duty of Canadians to make these people whole.
\item It foments anti-Muslim animus.
\item He was an atheist who hated Christians. He might as well have been ISIS.
\item The anti-discrimination protection law talks about male and female.  Please do not take this as the wrong way, but which one would a transgender fall under?  Self identified or by chromosomes?    For one or the other will cover them in the male female legal classification.
\item What a wonderful and inspiring display of spontaneous outrage.  Where was the spontaneous outrage when children were being molested?  The Church of Jesus sure could have used some then.  Maybe next year there should be a Fortnight for Hypocrisy.
\item >>Canada is showing support to Poland, a nation that was raped by both the Nazis and the SovietsAnd where was Canada when Poland was invaded by the USSR? Canada was an ally of the Soviet Union and supported the invasion.
\item Homosexual 'marriage' is a public sinful act, recognized as such by the Canon Law and leading de facto to excommunication
\item Richard you have no way to know how many transgender people you have dealt with throughout your life.  You would be surprised to find out.
\item I am 65, my wife 62. We have been married for 41 years (high school sweethearts). And yes, I love her more than yesterday, but not as much as tomorrow.
\item If a black student made a 'joke' about a holocaust victim or something jewish, no one would be commenting here - that student would be gone.
\item The \$90 million per year the US spends on its soldiers' sexual health covers 1.3 million active service members. The (say) \$5 million the US spends on transgender issues covers perhaps a couple hundred individuals. Do you not see where the greater cost effectiveness lies?
\item I wasn't aware that there were anti-Semite Jews.  Interesting news.
\item I don't know whose more clueless: the reporters or the counter protesters. Study Islamic law before you open your mouths.
\item The latest chapter in the Globe's never-ending hatchet job on Harper. Wonder what comparisons are coming next? Hitler? Stalin?
\item I totally agree, we need that conversation. And the sooner the better. ( I also support helping refugees abroad with humanitarian aid )
\item No, it has happened.  The liberal media just won't report it cause they're covering for the trannies.
\item Lawyer Kim In-sook said the military penal code, which makes homosexual activity punishable by up to two years in prison, was unconstitutional because it tramples on basic human rights and dignity.  Yes, chomping on someone’s genitalia is really dignified.
\item Trump's been upset about this ever since he found out Melania is transgender.
\item How many parents abuse their kids for not following Christian values?
\item How is a gay couple a federally protected class? Federal protected classes include:  •Race. •Color. •Religion or creed. •National origin or ancestry. •Sex. •Age. •Physical or mental disability. •Veteran status. •Genetic information. •Citizenship.
\item Twenty-four hours before Russia invaded Crimea, the Russian ambassador to Canada stated that Russia would not invade Ukraine. These are all KGB/FSB people.
\item condolences to the family of rob ford.
\item Mark, byline has no hyphen and people are listed 'in,' not 'on.' Isn't picking flysh*t out of pepper just tons of fun!
\item All your generation has to do is vote, and in large numbers, for the most sympathetic leader to your cause. Harper has had his chance, so it's not him. Our country is led my those who vote.
\item Indeed, one would think that if the hierarchy is so concerned with keeping gays out of 'the club' they should certainly be concerned with cleaning out those already there.
\item The yobs in Charlottesville were chanting 'Jews will not replace us.'
\item I've yet to see one Catholic progressive here say that violence is unacceptable.   Instead, many here are saying that millions of Americans are fascists and racists, and this implies that they believe these Americans are criminals who should be defeated by any means necessary.
\item It puts an end to the old socialist lie that women are inherently superior to men in how they yield public office. But now they are still pushing the agenda that women are inherently superior to men in the board rooms of big business.
\item Damn lies.
\item Muslim Terrorist Attack.
\item [... it appears officials were unaware of the incidents uncovered by The Globe]As Upton Sinclair said, 'It is difficult to get a man to understand something when his salary depends on his not understanding it.'
\item The average age of the victims was 10.5 for girls and 11.5 for boys.' - from the Commission's statistics as reported by the BBC  So much for the tired claim that this was mostly gay priests and their teen lovers.
\item Poor poor Ontario. I feel for you. What a serious deficit of leadership this province has endured for decades. The spiral downwards continues.
\item How can a Twit explain any-thing?
\item Why isn't the United States sanctioning Saudi Arabia that does not even have a constitution. Saudi Arabia has only the Quran and laws that encourage child rape while severly punishing people  for reading the Christian BIble? So much hypocrisy!
\item Sarah,  Very articulate article; well written, incisive, well supported, thoughtful.   Without the usual tabloid pseudo-english and irrelevant anecdotes. Whether you agree with trans-people being in the military or not; it is just another example of Trump's M.O.: find a minority, pick on them.
\item Donna Trump?  News Flash:  Trump is Transgender!
\item Read it again Trans. Or have it translated into a language you can understand.
\item 90\% of people imprisoned for hate crimes come from public schools. Yep, sounds like there is no problem with the schooling system there hey!
\item Would you want a citizen of the Republic of France to negotiate a trade deal with Europe on Canada's behalf? The Leader of HM Loyal Opposition has a dual loyalty.
\item All Canadian are created equal... some however more equal than others! Tick tick tick ... 2015.... election....ABC
\item Ahhh.....a Jewish conspiracy is it?  LOL!!!
\item I would consider that I am already demonstrating that I am the better man. ..... I make love, not war.
\item It's an especially dumb move when Trump claims we are being menaced by hostile Muslim movements from outside the country to declare war on a group of fully acculturated, motivated people who support democratic norms of gubmit.
\item That's easy. Republicans love the 'People of Israel' when they're in Israel. It fits in with their apocalyptic Christian eschatology. Next door, not quite so much.
\item No, I am perfectly correct. Paprocki's statement shows fear and loathing of gays. Pandora supports Paprocki's statement. Pandora ALWAYS supports conservative bishops when they are criticized -- always.   Once again, I speak the facts that Pandora would like to brush off.
\item Good for our PM.  The apology is long overdue and if the Pope has any morals he will apologize and beg forgiveness for the terror and horrific abuses inflicted on innocent children by the Catholic church.
\item What??? The Germans didn't fight to create the 'master race'?  They didn't kill Jews, Gypsies, etc. because they believed that white Germans were the master race?  Where did you get your education? From Nazi propaganda publications?
\item Here's the truth, Sheema Khan. There may be a God although it seems very unlikely to me. But one thing I am certain of is that, if there is, it is by grace alone that we are redeemed.
\item I'm really worried about his last two:  Two women (one of whom is Native American) and a black!  That is ominous!  And he wants his Jewish son-in-law to have a major role in his administration!   If Hillary appointed that ethnicity. there would be balloons and champagne!
\item Some of what you write is not true. You can advocate, your directors can advocate your members can advocate. Individually they can go to a town meeting and speak out and mention which group they belong to.
\item Canadians have a reputation for being poor tippers.
\item Most mass shootings are committed by home-grown white males, many of them Christian-affiliated. This is true of both the US and Canada.
\item ...and trans people should be given bingo cards that have numbers that are not in the hopper. That's the way to stay happy and blessed.
\item BURKE - the face of Roman Catholic Fascism!
\item Throughout Latin America there is little or nothing for Catholics to apostatize FROM.
\item The church hesitates to expose its criminal priests because it fears its enemies would exploit the situation'; so instead the institutional Church covers the crimes up, not understanding that it will look worse when the crimes are found out.
\item In his pre-cardinal days, Burke was an arrogant, imperious and tyrannical despot. Oh, he's sweet, smarmy and so pious, bedecked in splendor at his Tridentine recreations, but he loves power. He's running for pope as we speak. Simply put, he wants the pope dead...or at least destroyed.
\item Islamic Terrorism is entrenched in the Muslim communities  of Canada and spreading with rich funding through mosques.  But Shhhh... don't talk about it.
\item You appear to have the same damn mentality that the  German people had when Hitler murdered six million Jews and Polish people; buried their heads so only their butt was sticking out.
\item Support for traditional families, community and Christian values. Not something you see much of here in Canada lately.
\item Seems a bit early for a gay pride parade?
\item Your comment makes sense if you ignore the mainstream Republican view of the LGBTQ community and if you dismiss the anti-transgender legislation proposed and enacted by them.
\item Dont feign ignorance, you are casting the state of Israel in a bad light intentionally, so know what I mean.  Anti-Semetic means anti Jewish, dont feign ignorance on one post and talk about your amazing grades in another....
\item Can we stop with this nonsense of who the middle class is and just assess both plans on their merits.
\item And yet over 60\% of Catholics voted for this hateful clown.  Why?
\item The Holy Spirit selects the Pope. The Pope must be listened to. Except I don't like this Pope and what he's teaching. The Holy Spirit obviously doesn't choose the Pope after all.
\item How about you get your facts straight. Vancouver does not pump raw sewage into the environment.
\item A PRAYER FOR ATHEISTSMay atheists be tolerant and not hate People of ReligionMay atheists preach tolerance and practise itMay atheists love People of Religion who love atheistsAmen
\item  ..how Canada's aboriginal culture actually forms the basis of many aspects of Canada's political/legal structure..'Total nonsense !
\item Look up the word 'purport' JB, clearly you don't know what it means or have the ability to read my full sentence. You either have an amazing ability to hear exactly what you want to hear, or you are incredibly intellectually dishonest.
\item Yeah, transgenders stay up all night plotting and planning about how they're going to assault unsuspecting citizenry.  Transphobia won't be the new normal.  The US Supreme Court put that nail in homophobia and transphobia.
\item For most people against this, the issue is not transgenders.  The issue is perverts pretending to be transgenders so they can go into bathrooms with members of the opposite sex, especially children.
\item Science has no place in a Wente rant.
\item Health care is a fat cow that must be trimmed constantly. The feds will force that, which is a good thing.
\item I never 'gave up' on 'opposite relationships'. I knew I was gay from the time I was 11 years old. It was not a 'choice'. The ignorance you assert here is simply unacceptable.
\item Its nice to see Trump focus on Islamic terrorists instead of treating the American People as the \#1 threat like Obama did.
\item people created as gay by God in the first trimester of gestation'.   Can you provide any scientific evidence to support this claim?
\item this will trigger another wave of jewish suicide bombers on the world...
\item You think talking about romantic relationships are synonymous with sex and oral sex? So I'm assuming that Christians that wait to have sex until they are married aren't in a romantic relationship until they're married? Your ignorance is truly undeniable.
\item LotL has a bogus theory about the transgendered, which he presents with NOTHING to support it.
\item According to the left America is a racist and homophobic land where success is guaranteed if you are a white, Christian, heterosexual male but otherwise you'll slave away for starvation wages. I'm surprised these people would want to come here. I guess they haven't gotten the message yet.
\item 115 House Dems want proof Trump coordinated transgender military ban with Pentagon'  Meanwhile, the rest of the country wants Dems to stop mindless obstruction and do something positive for the country but they refuse.  Why is that?
\item It is absolutely stunning to the point of journalistic malpractice that this isn't acknowledged.  It does predate Islam and is possibly pagan in origin.  To claim it as Islamic is to do no less than categorize Islam as a cargo cult.
\item Umm, they were both Muslim terrorists no? Just sayin..
\item I was banned from FB for a month because I dared to associate Palestinian students  burning the flag of Israel with Nazis burning books by Jewish authors. As far as I am concerned they are the same thing.
\item Tranny rights are human rights and human rights are tranny rights!  LOL. Just F kidding.
\item why is it that you hate jews so much?
\item And the Danes are known as the happiest folks in the world because you don't live there.
\item gawd... you again. how many times have you posted your pathetic petition this time?
\item I never respond to you on principle but I must correct the notion that there is any more 'sex' at a Gay Pride than there is at Mardi Gras. Kids attend. Our prime minister attends several across the country and takes his kids. You're full of it.
\item Wow--conversion therapy.  How sad that Mr. Gabriel is so woefully uninformed about this issue. Perhaps he is unaware of the suicide rate among young people who identify as transgender? Or the need for support of what is definitely not a lifestyle choice among teens? Makes me sad.
\item I was amused to note how long it took for Ontario to admit a woman to the bar after ruling that Jews could become lawyers- 60 years! And that she would be a rabidly anti-Semitic woman at that plates the irony with gold.
\item Coren's position has been the official position of the Church since Vatican II (which incidentally John TOry copied in his ill fated electoral campaign), so its no surprise.
\item There is no “transgender”; that is a sick libtard construct.  There is only male and female:  all else is mistake of nature or freak!
\item Classic Zio lies. '...the caller ID made it seem as if the call was coming from our own office...' Im sure it did.   Nobody is calling Jews with bomb threats folks. Pathetic.
\item I'm not really sure there was a transgender policy 50 years ago. That would be 1967?
\item The Japanese do not want to destroy their country and culture to an invasion of colonists who consume but do not provoke anything for themselves or society.
\item The Canadain government supports Islamic terrorism, their leadership is not a reliable ally.
\item Nothing is stopping the florist from exercising her freedom of speech by putting a hugh sign in her window 'WE DON'T SERVE GAY WEDDINGS' - why doesn't she?
\item well gee, I guess I'm just all confused, and here I thought the UN gave Israel to the Jews.
\item ya buddy... its those cats.... its not the pollution or the chemicals.. its the cats..
\item It seems to me  transgender is faulty wiring in the brain bordering psychosis of people that are otherwise healthy. a weirdness just like fetischism .
\item Talk to people in UK whose way of life is being changed. Young girls being raped. Cities being taken over by muslims with their sharia law.  Young girls sexually mutilated. Married at 6 years of age to an old pervert. Feel sick talking about these animals.
\item Take it from me (a bi guy who prefers men to women) not in a million years.  Like a straight guy once said, 'if gays want to get married and be miserable like the rest of us, then go for it.'  To me, that sums it up.
\item Shaista,  you might get less push back if you were also prepared to talk about and acknowledge the existence of radical Islamist terror, jihadists, and the role of radical clerics who manipulate and create these young terrorists.
\item Why fo gay guys always think they can get away with misogyny?
\item Tip:  Better to just use emojis to make your point, like DonfromKansas.   That's progressive Catholic rhetoric at its finest.
\item If we really want to honour the fallen. Give the money to veterans who are not getting it from the federal government or adds and lobbying to get the government to live up to it's responsibilities
\item Quebec can do what they want. I support them.
\item The whole ridiculousness of Transgender Sex is obviously here!
\item Muslims are obligated to implement Allah's orders to fulfil an Islamic State. The Quran states that it is not permissible to choose.
\item God bless you.
\item oh perk up at least now you can use a transgendered bathroom.
\item You should be poisoned and murdered. 
\item True political leadership is admitting you took a bribe.
\item Real problems are too difficult... Next up...transsexual perverts in the Washroom!
\item Dana, you asked whether or not these women at the SF airport would have made similar comments about veiled Muslim women. I think they would. Bigotry and prejudice knows no boundaries when it involves any person described as 'other' than one's self.
\item That Trump is patholigical is not news. Nor is it news that EWTN and National Catholic Register put party above sanity.  It is amazing that the Vatican is now more progressive than the Alt-Right Catholic media.
\item Before you spot off about discrimination you should ask if they voted against having a cemetery  next door to them or against a Muslim cemetery .  You don't know and neither does anyone else.
\item If the Mayor says that he has gay friends - I'd bet dollars to donuts they are involved in the drug trade.
\item Kinda like the Westboro Baptist folks who protest gay everything - by showing up at every gay function imaginable.
\item Do you know what 'transgender' means? It's not 'in between male and female', it's going from one to the other.  I see you did not address the fear and loathing towards our LGBT neighbors expressed by the society.
\item when dose the homeless jew get a grant for a month in a motlele??????\$1,500....puts the homeless jew into a motlele for a month
\item They probably trying to escape hungry Muslims hiding in the woods.   LOL
\item the only TGs trump wants in the military are those Moscow trannies in the hitler youth outfits who pissed on him in his hotel room
\item Hagiography ....HA !!Too funny.
\item Rogue Catholic knows, he just knows, that the Spanish tragedy was perpetrated by 'brown skinned people.' Disgusting.
\item No. Just anti-Russian. Not anti- Jews.
\item Read up on the facts concerning Abuses of the Temporary Foreign Worker Program \& current investigations in the Food Industry; Educate oneself to the facts instead of swallowing this half-baked Opinion G\&M gaseous-fluff -- wholesale...
\item What is Jewish response Bernie??   Oy Vey!!!
\item Transgenderism is an arbitrary sex change, a lifestyle enabled by modern medicine.
\item This is a major problem with diversity.  It mandates that everyone needs to be special.  Special groups now need their unique culture and issues protected.  This leads to constant friction between al the special groups. Even the gay community has become fractured.
\item Sorry for all the facts upsetting your bull...
\item In your effort to balance gender you have given up competency.'I'd love your take on which ministers you believe are 'not competent'. This cabinet is filled with competent and talented people.
\item You're right. Some of them are Republicans. (Sorry, couldn't help it!) I was referring to the rant: 'Agirlwhoknowsherownmind To put it bluntly, the war on Christmas has been led by Jewish organizations, financed by Jewish financiers.....' The condensed version would be: 'Jesus. The Reason for the Season'
\item He's a horrible man with his hate propaganda against homosexuals and his association with that portable toilet, the Poo Tin.
\item Wow. Jews really do get blamed for everything.
\item He may have attended Robert E. Lee High. He thinks it's free speech only if one can get away with yelling' Kill the Jews and Blacks'. If you yell ' Kill the Nazis and White Supremacists', that's not protected by free speech.
\item I can't stand the orange man; can't see why any of you idiots (who also voted for bush/cheney) voted for him;  but I'm thankful he started his speech tonight condemning the violence against Jews across the nation.
\item Since when the US government has as priority to defend and expand the homosexual agenda? Why the state dept. take side with a nazi corrupted man like Soros? Nobody need to be a genious to know the answer.
\item The Old Testament is also a Christian holy book.
\item Because it undermines some racist tendencies.  He hates Jews.  Then he discovers that he has genetic markers for being partially Jewish.  Now what?
\item His birthright is Canadian and should we remove anyone's citizenship due to the actions of the parents or vice versa then we would be deporting entire families of muslims where one has been involved with ISIS or other terrorist acts.
\item I just about choked when i saw this headline! Walk through any campus and you see rich diversity on display everywhere. Then my second thought was how do you compile stats on gender at a time when so many identify as transgendered?
\item This is the best comment I've read on a fairly obnoxious article re-hashing equally obnoxious, condescending media drivel about men and all their flaws (imagine if you can an article in the Globe focused on women and all their inadequacies).  Never been a better time to be gay.
\item A Church that refuses to accept women as priests will also negate gay priests. Misogyny is a sin.
\item TO's BML should be marching in Nigeria's gay pride next year under the Boko  Haram vail where most of their leadership's birthplace originates from.
\item But there is evidence that Judge supported same-sex acts by self-identifying as 'gay,' as opposed to one who has same-sex attraction, which does not imply any opinion on same-sex acts.'  And your evidence to support this conclusion is what?
\item How long have you been Gay?
\item The inerrant word of our saviour. With all of his infinite wisdom. Praise The Lord.
\item Shisaisama, you're back! Did you imagine that Jesus asked you to go back on Civil Beat to blaggard gay people again?
\item Good. Russia votes for a clearly anti-Israel resolution that serves to contribute to anti-Semitic sentiment and further attacks on and stabbings of innocent Israeli Jews by Palestinians.  Karma is right.
\item And now you see how the right wing uses the term political correctness to label their enemies.
\item I think the left actually wants to characterize most of the Catholic moral teaching as having to do with sexuality.'  Really, R.D.?  When I ever hear some self-described 'orthodox' Catholic talk about morality, it is always sexual morality.
\item All fine and dandy until a wanted psychopath gets dressed up or decided he is transgender and kills someone.You should be identified by your birth name for security reasons.WHY are these mentally ill people getting preferred treatment like Black Lives Matter and left wing nuts in general?
\item A 'fascist' has a Jewish son-in-law?  Black members of his administration?  Supports Israel?  What am I missing here?
\item attempt suicide or commit suicide?  I think the 43\% would be the \% of trans people who attempt it.
\item 7. Everyone has the right to life, liberty and security of the person and the right not to be deprived thereof except in accordance with the principles of fundamental justice.' Any other questions?
\item Sure, because 'very fine people' march with nazis and white supremacists carrying torches, chanting 'we will not be replaced by jews!'
\item Why not call hm what he is - a white christian terrorist?
\item Make America Gay Again'?  When were we ever a gay nation?
\item The 32\% of deplorables still adore him, and the evangelicals think he’s the second coming of JC, lol
\item Really, R.D.?  So white racism doesn't exist?  Did you happen to notice that white supremacist rally in Charlottesville.  Also, if priestly sex abuse never happens, how come the Catholic Church is paying out billions of \$ in settlements to victims?
\item That is very, very not smart. Illegal invaders are not a protected class.  Gays are a part of a protected class in Colorado, but that does not mean they are afforded extra rights, that is silly. If this were a test you would have failed.
\item Christ said give unto Cesar what is Caesar's. Pay your taxes like the rest of us suckers.
\item Aspirational self-identified gender? Griping about how two marginalized populations i.e. Native Hawaiians and transgender individuals tick the boxes sounds like you are an intolerant racist white male. You are a petty man.
\item Amazing indeed. She worked in the US illegally as a model and lied about it on her visa application. She lied about her university degree. She plagiarized her convention speech. She posed nude in lesbian themed soft-porn pix. Real classy. http://nypost.com/2016/08/01/melania-trumps-girl-on-girl-photos-from-racy-shoot-revealed/
\item If the Jews are eliminated, then the Nazis are OK (?)
\item Catholic trolls...who knew?
\item Reagan a hero, hahahahaha, it is people like you who aided trumps win.
\item Sask. corruption hmmm \& half of Devines cabinet thrown in jail... but yeah, Montreal \& Toronto got big problems... glad I'm here in Vanc.
\item Oh, please, another 'back in my day' story. Did you have to walk 2 hours a day to get t school too? The kids are alright.
\item Your islamophobic statement has been reported under M-103.  Referring to your Muslim brothers and sisters as 'suckers', in light of the recent attack, is not only intolerant, but it is hateful.  Don't you respect all faiths, or is it just one?
\item I summarized from the book and you were unsatisfied, therefore I directed you to the source, which by the way, won the freaking Pulitzer Prize.  Trad historiography: if history is unflattering to the Catholic Church, the historian is therefore anti-Catholic.  I can't take you seriously.
\item MINSHALL  i think a JEW would be a better assemblyman than you !
\item They could be transgender. I am so funny.
\item Pride in publishing dissent, heteroxy , attacks on teachings and faithful Catholics. Yes truly a great legacy and so exemplary of Jesuit inspired false spirit if VII 'catholicism'
\item Throw in a couple scenes of female genital mutilation and you have a ' How to Behave ' documentary for Muslim dominated countries.
\item Probably not the first time.' Speculation is not proof. I see nobody claiming that being Jewish confers any sort of free pass. On the contrary, there is a consensus that he said a stupid thing. There is not consensus, though, on whether this was a firing offence or not.
\item Well, the whole of the CI (Catholic Institution) start from Pope F., the Vatican prelates, Bishops are weeds, it needs to be plow under.  Any one rooted in Christ will flower after the plow since nothing can destroy the one who loves God.
\item Not true at all they would actually be guaranteed a strong permanent voice since they always get a good 30\% of support
\item robert reich is a sawed off stubby with an inferior complex that is a mile deep he is what the DNC palms off as an intellectual reich is a pig-me-me-me as the Jews would say - unclean goes bone deep
\item Thank you. The vast majority of people are very supportive of the real transgender community..although there is concern about some issues eg Caster Semenya running as a female. But they do NOT support genital mutilation for those with no chromosomal abnormalities.
\item Every member of the USCCB should be strapped to a lie detector at their next meeting and asked if they are a homosexual.
\item Ok, so there are diagnostic criteria for gender dysphoria which are not meet by simply being transgender. No one asked for, and no one cares what your personal opinions are.
\item All forms of racism must be eliminated, forms of Islamophobia, Anti-Semitism, Homophobia and discrimination against transgenders. People need to support Justin, Obama, Hillary and Premier Wynne in this fight against evil.
\item Attempts to go along have never panned out well for Israel.  Jewish intolerance?  LOL
\item Civil marriage is NOT a religious thing. Not one syllable of 'God-talk' is required to be civilly married. Religionism poisons everything it touches.
\item You are being really fucking nasty about this
\item The Brits won't learn until it's to late.   Gotta get ride of all those Muslims.
\item Khan and co knew the place was a rathole and firetrap for years but did nothing about it.  Shows Khan's true colors, most of those living there were poor muslims. Khan is just another champaign socialist
\item So, deny payments for the surgery if he's that upset over something that would amount to one one-hundredth of one percent of the Defense budget. But don't kick all transgender people out of the military. You're a perfect example of Trump's famous 'Fifth Avenue' quote.
\item Depends. The churches enjoy tax-exempt status and are therefore subsidized by all of us. They're ripe for human rights complaints and lawsuits, I say. Discriminate against gays and women in Canada in 2017--because your magic stories declare them sinners or inferiors--and you deservew what you get.
\item And what did you cancel when Obama dropped tons of bombs on innocent Muslim civilians.....or when he invoked, by presidential order the termination of Iraqi civilian immigration?!
\item He is gay, so he's imminently qualified to hold the portfolio of Minister of Virtue-Signalling and Identity Politics.
\item @progressive: those aren't the average schools though. the average american education experiance is CRAP. even the Americans admit it
\item from the Business Insider:  A 2016 study by the Rand Corporation found the maximum annual medical costs for transgender services would be around \$8.4 million. By comparison, the military spent \$84 million on erectile dysfunction medications such as Viagra and Cialis in 2014, the Military Times reported.    http://www.businessinsider.com/pentagon-transgender-medical-comparison-2017-7
\item Seems to me that the violence in Turkey has rapidly escalated since the anti secular, pro fundamentalist  Erdogen took office.  Could there be a link between violence and fundamentalist Islam?
\item I am totally shocked and deeply disturbed that abuse of minors is still happening in the Catholic Church. Are you? If you are not shocked and disturbed then you are part of the problem.
\item I mean, obviously... basketball players are taller than average
\item Yea, but is she going to toe the party line and promote transgendered, sexual dysphoria to our first graders?
\item Your bathroom? Are trans people coming into you house and using YOUR bathroom? I thought we were talking about PUBLIC bathrooms, which by definition are for the PUBLIC, not for your personal and exclusive use.
\item Let's be clear- Transgender Justin and Gerald Take-it-up-the-Butts don't care about asylum seekers, international borders, human rights, overtaxed Canadians or anything other than staying popular and staying elected.   It's pure smoke, mirrors, selfies \& 3x weekly hair salon visits.
\item Since he presumably honors his public vow of celibacy what difference would it make if he were gay?
\item ...............celebrate the birth of the god Mithras (or the new sun).
\item People can't join with psoriasis but lets reset all medical, physical training, tactical and operational standards for a transgender?'  I haven't seen anyone, not in these comments or anywhere else, propose that. Reset standards for transgendered? That's your straw man. Logic fail.
\item So, what does all that have to do with transgender?
\item I agree entirely which is why Christians who claim to be patriots are liars.
\item If you are implying  that the pope approves of transgender ideology, yes I do have a problem with your comment.
\item Pride Parade will. Santa is gay in the new Progressive world. Get with the times.
\item Funny thing is: Most of the populist movements in Europe are headed or supported by Catholics.   I guess the pope doesn't want to mingle with and smell like his sheep.   Hypocritical?   Yes.
\item When is the homeless Jew going some grant money?????
\item Keep in mind that medical personnel have families too. They work hard all year and want to enjoy some family time as well.
\item Breitbart? I bypass to snopes.  https://www.snopes.com/miguel-martinez-transgender-bathroom-controversy/
\item Democracy includes protection of minority rights. After all, the Nazis had the mandate of the majority to persecute the Jews.
\item Gender neutral EH. What is the point of photo ID if does not have gender and allows transgender cross dressing.
\item Christianity had a reformation? When did that happen exactly? And tieing atheist to communism is pure nonsense.
\item Now that is persecution, not telling a farmer he is not welcome at a market because he opposes gay civil marriage for religious reasons.
\item Thank you, bookmark... will spread... Cheers Miles,
\item Need a citation that Muslim terrorists are still being allowed to enter the country. Do you mean like that girls science team from Afghanistan for whom Trump told his administration to overrule the Muslim travel ban?
\item There is no Muslim cemetery in Quebec.
\item You are a re-take on the movie 'I'm All Right Jack.'
\item You are right, of course. Some Pharisees were indeed friends of Jesus, but most weren't. In fact, they repeatedly conspired with the Saducees to entrap Jesus, make him look a disobedient fool, and, ultimately, to have him executed. Hence the pejorative use of the word 'Pharisee'.
\item Oh, we're back on the Russia thing again?  What happened to Trump being a white supremacist, having a Jewish son-in-law, a convert daughter, and Jewish grandchildren?  Oh, and a black friend named Dr. Ben Carson.
\item Yeah, he'll put the UN in its place, just like he'll ban travel from Muslim countries and revoke Obamacare?
\item Give them a big Liberal hug and free heroin every day and they won't want to hurt other people
\item The Globe buries every article that is critical of the Liberals. It moves from the front page to hidden corners before noon.
\item Comparing someone to Trump ,like its a bad thing. Globe and mail is home to so much entitled cucks.
\item So then who made homosexuals? We are taught that God made us all.
\item Easy. The transgendered don't know who to molest.
\item inappropriate parties... this is a joke. I'll take my God to a more suitable location for my gay wedding.
\item Parasites.'  The word Hitler used over and over to describe Jews. Any time you find yourself speaking of other human beings in those terms, you need to back up and figure out where you went wrong.  Trump is unable to do that, but most normal people can.
\item ...but they're not in the Constitution. And which of those Judeo-Christian principles do you suppose compelled those good Christians to slaughter and persecute all those Native Anericans while expanding the empire?
\item I lost interest when i read the word, 'Muslim'.
\item You don't even realize how stupid your comment is ---- do you? LOL You are clueless about who the indictments were for or you would not have made the comment you did.
\item Leftist ideology gave women the vote. It also gave minorities the vote. Rightwing ideology backed segregation. It opposed gay marriage. It backed slavery.  Scheer is finished before he started.
\item You don't know what you're talking about, whatever-your-name-for-the-day is. You can't stay on point and have no understanding of scripture or history, and certainly no understanding of Judaism. So forgive me if I prefer what I learned in Rome to what you're trying to pass off here. Bye.
\item So? Islam has been encroaching on and invading Europe since the 7th century.  There can be no peace until Constantinople is returned to Christendom .   REMEMBER 1453 AND THE GOLDEN HORN:  NIL IUSTE  NIX PACE
\item Does that mean Jews are cannibals?
\item a lot of big words there professor. stick with your textbooks and living off the public dole.
\item The Viagra must be why the President has a hard-on against transgender troops. Hopefully he will soon cum to his senses or reconsider his position, I mean “and reconsider his decision”.
\item To Factcheck why? so that no doctor need violate his Conscience every man's conscience is sacred to him remember you love 'diversity' let's have diversity of conscience
\item AT: Your explanation reminds me of the excuses the 'good Germans' gave for why they didn't ask, where did the Jews disappear to?
\item You are too kind
\item Really?  And I suppose if your child is sexually abused by a priest/clergy member/preacher then it is all fine because the abuser is 'Christian'?  Grow up and start thinking.
\item But Trudeau is dancing pretty in Paris. Nevermind the taxes.
\item Lesbian chicks are OK as long as they are HOT!  This one appears to be marginal.  Anybody got any tapes?
\item So, it's gay people's fault. Don't worry, I'm sure you're on the priority list of people to be Raptured
\item Because it was a great place to be when posters like 'Harper is a fat fascist' (actual name) ruled??? My, are we not tolerant, and open minded...
\item No, we don't have a problem. We have the First Amendment. I didn't mention your religion. You are free to celebrate gay marriage.
\item Harvey as a name really sets off my gaydar.
\item Look at the guy in the picture who didn't doff his cap.  Someone should have knocked it off.  Or maybe he's just not a good Christian.
\item Don't set yourself up as being so special. Evangelical, Anglican, Presbyterian, Catholic, Muslim, Hindu, Shamanism, Buddhist, Sun Worshipers and Kardashian Fans. It makes no difference. They are all equally worthless.
\item And all the arguments used are valid.
\item I agree with y2, and there are more extremists on this board than there are in the average city.
\item My reading of the early chapters of this research, dealing with history, is that the predominant issue bedeviling the Church has been that of homosexual men abusing one another and teenage boys.
\item Perhaps this young man should have stayed in Syria. Where it is safe!!!!!
\item Oh, and if you think talk of tax cuts isn't pandering to the Toronto Sun and to the Libertarians of Lanark, you haven't been watching.
\item Wise observation waynes2.  Joshua Boyle may be another untrustworthy Islamic presence in Canada.
\item Thank you Barry. A comment from someone with actual experience and therefore credibility. I'm assuming if a female-in arms sacrificed their life or body part for you or another male colleague(s) on the field she would be respected like any other.
\item Show some grace Globe... I'm paying you \$20/month---I think you owe and other readers the courtesy of a serious thoughtful refection on what your support has done.
\item @ Expectation ManagerYour compassion and understanding is truly underwhelming. I hope you never find yourself needing support from the state if your circumstances change for the worse, or you become dependent in your old age.
\item but he's jewish right?  that must matter to some degree
\item In typical Globe and Mail fashion, nobody takes credit for this piece of crap article. Whitey is very afraid, and rightly so.
\item The baker should just put a sign out front that says, 'We refuse to serve gays for religious reasons.'  He should move to a state where it is legal to discriminate against gays.
\item Kenai assembly! Denounce your false Jewish man-god and accept Cthulhu as your dark savior! Only through Him can you escape this silly position in which you have put yourself. Repent of your godly works and your sins will be justified forevermore.
\item I love the ultra-christian right winger standing in a gas chamber warning us about ultra right wing christians from Europe some 70 odd years ago in order to advance his re-election efforts.  Hypocrtie.  Coward.
\item It's time to hit pause on immigration and direct all efforts and funds towards those in THIS country who desperately need support.
\item Greetings......Being a Christian I cannot really in all good conscience feel that voting for either Clinton or Trump is morally ethical. Clinton is not a  caring progressive as she says....but a Pro Choice Republican and Trump is off the charts as a greedy Narcisstic Fascist
\item Bad ideas should be mocked and ridiculed because, otherwise, they tend to infect later generations. That's why we have Christians today.
\item I don't understand the 'racial component' comment.   Whites split their votes more than any other race.  Hispanics, blacks, Jews, Asians all vote more racially, and more racially cohesive, than whites to.  Why isn't this ever criticized?   A:  hypocrisy.
\item Don't worry, not one cent of your tax dollars will end up in the hands of women or gay men.... unless they are called 'President', 'Minister' or 'General'
\item I can say 'Orthodox Jews'  I can also say Sharia law, burka, honor killings, Assad soldiers raping women, Isis raping women.
\item Hang on, let's not to be to hasty, we still have some groups, transgender for example, that need to be in cabinet, experience and know how will just have to wait.
\item What attitude would that be now? The one about traitors? Or the one about a traitor suddenly becoming transgender to escape a full prison sentence?
\item False, they have no sees to teach in or minister to.  They are now just old Catholic guys.  Their opinions are as valid as yours and mine.
\item ‘I assure you, as often as you did it for one of my least brothers, you did it for me.’ (Mat 25:40)   God weeps because the Catholic clergies rape him in Children!!!!!!!!!!! I can't understand how on earth clergies do not know this!
\item You have to remember that to Tridentinus, any Catholic who disagrees with HIM on anything is a heretic. Trid is extremely arrogant in his belief that he and only he represents orthodoxy.
\item What if Jesus were bisexual as a hermaphrodite?  Would that make a difference? Is being a woman less human than being a man? (St. Thomas said a woman was an 'ill-made man.'
\item I see they have Jews doing damage control
\item If a pedophile is male and abuses a boy, why is he not gay?  I never have understood that.  When the lgbt want gay leaders in the boy scouts and then beat up the boy scouts when a male abuses one of the boys.
\item You have no citations for your comments, so there is no reason to believe them, but there was a nice article stating that we spend more on Viagra fro servicemen than we would ever spend on gender reassignment.  Admit it, transgendered people just scare you.
\item The Catechism is wrong.
\item Initially, the Nazis too wanted to send the Jews out of Europe. The Final Solution was proposed later.  And providing smallpox infected blankets to the natives does suggest genocidal plans, knowing that they had no cure for that terrible disease.
\item This is illogical thinking.  Viagra costs (which should be paid by the individual) are spread across the millions ho serve.  Sex change drugs would apply only to the tiny minority who are 'trans'  -- so naturally the Viagra cost would be far greater.
\item This story highlights what I've know for years, 'christians' are totally screwed in the head and need to be fought at every turn.  They can't even protect THEIR OWN DAUGHTER ... from this 'religious' monster.  Yikes!!!
\item you are saying that the Jews will be responsible for a future genocide that will exterminate them.  interesting that the Globe watchdogs feels this comment is within their bounds of civility.
\item Yes...the Democrats made the neo-Nazis rally.... Just like the Jews made Hitler invade Poland.....it wasn't racial hatred...really... The Democrats made that boy run over those people and kill that girl.... The Democrats made Mr. Trump condone the behavior.... Darn Democrats...
\item There's nothing wrong with birds of a feather flocking together unless you're white - this is a big no-no. Complaints about lack of diversity etc will be cried out at the drop of a hat.
\item now we got some jap guy who thinks trump is hitler? good god people stop the drama please. trump wants to kick out bomb throwing muslims. real americans are all for it. get on board or get run over.
\item We can form the world's only predominately gay nation and Trudeau will have a majority government forever.
\item I can't imagine a transgender female going in to a men's restroom.
\item VanMorty - that's because all your friends are on these G\&M web- boards. Try talking to people and you'll see there's a lot of support for Enbridge and our energy producers generally than you'd ever guess reading this columnist.
\item Yup.... that's right. Go after the successful people. You know..... the ones that build large companies that create jobs, pay for peoples' mortgages and kids' educations. What did the Beatles do when their tax rate reached over 90\%...... they moved (along with their record label).... to the USA. Think it through, folks!
\item All speculation designed to convince the gullible that homosexual behaviour is perfectly normal and natural.
\item Fanatics'?  'Lunatics who hate Christians and conservatives'?  Rather strong words to describe those who believe that personal freedoms as long as they do no harm to others should be preserved and that corporations should not have equal standing with citizens.
\item Agirl:  SORRY, I just can NOT accept the Catholic organization because of their Raping  Priests.  Look at the Magnitude of Mental Anguish that they INFLICT on their Victims, and these Victims are messed up the rest of their lives.  Same with the Boy Scoundrel Scouts.........
\item Alleviate the suffering the best you can. That's what most Canadians want.
\item Ya sure but does he renounce Allah and Muslims now who want your neck ? Can you get that he wanted to kill you and  does he now according to the Quran?
\item There should be a law for posting on the internet the same as driving a car. If I have to read another one of these uninformed posts from a naive 15 year old on their lunch break I'd go ask my neice. 
\item He's the kind of pervert we have to worry about in our kids bathroom not transgender folks
\item You mean 'The Sociopathic Business Party'.But religion is just one of their crowd control techniques.
\item  Muslims are being harassed and assaulted in the streets. '  Source?
\item A vacuous comment from a simple mind.
\item And of course the same rules should apply to the unions. i am sure you agree..
\item Once a lower court legally recognizes a transgender petitioning for a legal name and sex change, there's nothing anyone can do about it (i.e. Chasity Bono and Bruce Jenner).  Try and stop either of these people from using a public access shower or bathroom.
\item We hope Lazeelink that the 4 people are literate enough to "get" her message even if it's entirely out of place this Canada Day :) Maybe those four will tip you better too when they return for a visit!
\item Last time I checked diabetes was an illness. Are you suggesting that transgenderism is also an illness?
\item What a perfectly 'christian' thing to do ... more of the SAME Fear and Loathing from 'christian' Republicans.
\item I'm sure all the Good Christian people of Alabama will be clutching their pearls in Outrage over Dump's use of foul un-Jesusy language.  Whatever Will We Tell The Children
\item How do your comments apply to Muslims. I know many and they are not interested at all in 'taking over the world.' What nonsense you spout. Get an education and then make some Muslim friends. You're the problem, not the solution.
\item Public affairs are secular. Period.
\item Dude, this is just a math problem lol. Literally 7800. Did it under 10 seconds. Do you not learn math in school anymore? Is this why the millennials are complaining life is so hard? Let me guess, math was racist so it got replaced with gender studies?
\item No Catholic is obliged to answer a call to violence even if uttered by one of the Church’s bishops.
\item Agreed. I think Colorado is open-minded enough to elect a gay politician, but I'm not sure. Might depend on whether the GOP nominates a moderate. Knowing them, they might nominate someone who was against same sex marriage.
\item A gender based tax policy? Sounds very complicated and very unfair. And what about transgendered? This is just another can of worms being opened.
\item Alabama is not a state known for producing intellectuals, but rather clueless Christian conservatives like Sessions.
\item I can't see why.  Gay people are just as responsible as everyone else to pay the societal costs associated with unwanted pregnancies.  But I guess a hater gotta' hate.
\item You fell far short of making any excuse for the lack of values inherent in so-called 'christian' Republicans.
\item Transgender like the  traitor 'Chelsea' Manning who was  pardoned by Obama.
\item Well said as usual... simple compassion what a concept...
\item It is called following the constitution. Certain powers are federal and certain are provincial. Nowhere does it specify that the centre of the universe is Toronto.
\item I wonder why?  Answer:  Because AIPAC likes it when they bomb Muslims.
\item As somebody else pointed out, the Danes also have one of the highest rates of suicide. Bash religion all you want, but you have to admit it gives people purpose in life.
\item Trump announces ban on transgender people serving in U.S. military'  How is that biased?
\item Homosexual is now gay,' And, gay people are out of the closet! They're in the military! Run for your life!
\item The new law, which ludicrously requires transgender people to use the restroom consistent with the sex on their birth certificates,'  Yeah, how dare we ask people to use the bathroom that fits their sex !!  How 'ludicrous' !
\item If the media had done its job of fairly criticizing both candidates, Trump's shorthand exaggerations would not have been necessary to get his points across.
\item If that was the case every one would claim they were a conscientious objector and get a draft deferral. And since that didn't happen it wouldn't happen to claim you were 'transgender' and get a deferral either.
\item They also predominantly marry relatives in Egypt, often first cousins. This has negative results for the population.
\item Do notice the assumption of gender differences.  How will this article read after a decade of same-sex marriage?  Oh, to heck with natural law.  We are too smart for our own good.
\item The holohoax (sic) didn't happen, but the holocaust, in which the NAZI's gassed, starved and shot 6 million Jews did indeed happen. You can admit this irrefutable truth and still be proud of your German heritage, Mr. Groth.
\item Lock her up until Trump resigns. The charge: An accomplice in crimes against humanity, denial of health care, anti transgender and no regard for refugees.
\item By comparing Trump to Hitler, you cheapen the death of 6 million Jews/5 million non Jews.
\item He was shouting God's name as he killed which is common for Islamic terrorists.. That might indicate his motivation
\item If Cosby was Muslim the comments would be closed   ;)
\item What's up, Doc? Don't forget the shemozzle at Red River College in Winnipeg. Nyaaah, what a maroon!
\item To R W Ranked ballot - second choice do you think Conservatives and NDP are so dumb as to give Second Choice to the Liberals Strategic voting they will give Second choice to smaller parties like Green etc ABL = anybody buy Liberals
\item thoughs and prayers - yeah that'll save a lot of lives
\item Thank God I am gay and dont have to deal with women.
\item I didn't know Donald Trump is transgendered!
\item Great work on the part of the Arcy MP! Great timing! I'm thrilled to know that our law enforcement officers support Adolph Harper's overthrow of what I once thought was an ideal country. The ideologues have us!
\item One of the loveliest ironies of this is that according to most historians, Tchaikovsky was gay. And we know how Russia treats its gay citizens, don't we?
\item As it always has been, the issue us the voluntary act, not the involuntary attraction.  'Gay' means same-sex attraction AND the unrepentant acceptance of engaging in sodomy.  So, when you 'tell' someone that you're 'gay,' you are telling them both things.
\item The non-progressive side never deserves even minimal respect.' Sure. And calling the author silly and an idiot shows a lot of respect for her views too.
\item Thank you for your courage, and for the beautiful article. The thoughts and prayers of millions of people around the world are with you.
\item I agree that he probably didn't mean it as it sounded, but it definitely sounded as though he meant that guns would solve the problem.
\item Only until he got elected.
\item Most advocates will be lesbians.
\item So Bush, Clinton and Obama became president because the nation is as you described top heavy with fake Christians etc. etc. etc.?
\item Ronster People are strongly affected by propaganda. Germans became killers of Jews through propaganda. Canadians have become killers of Canadians through propaganda.
\item The solicitors general should have to tell the police that they are supposed to enforce the law. They should know it already.
\item It seems it's OK when it's a Democrat doing the deed.
\item So Chinese people are the best judges of human rights for all of humanity? That is what you are saying, which is, of course absurdly arrogant and ignorant. You do know what human rights actually entail, right? Right?
\item we dont need transphobic left wing fanatics here. thanks.
\item Not here for a semantics debate, especially when the meanings and connotations of words change rather quickly nowadays.  Hope you have a gay day.
\item The Evangelicals hang on to Trump and Playboy disowns him.  That about says it for the Christian integrity of this current group of Evangelical political prostitutes.
\item Because it isn't about a solution. It is about the death and destruction of the Jews. Next question.
\item What does that have to do with transgender people in the military?
\item How ignorant can these rainbows be?  Islam forbids homosexual acts under penalty of death.  These maroons want to support and protect their enemy.
\item Systemic racism' brought about by those who kill and main in the name of Islam and you don't understand why.
\item I think Margaret Wente did a wonderful job in pointing out how malicious feminists can be; and the need for a reasonable approach in dealing with this matter
\item Take care! Hope the best for you.
\item You sir are, quite simply, wrong. Put your cracked pot away and join the 21st century. Science is not a hoax.
\item moon howler missed the Globe's mini-article yesterday, in which it listed its own record of endorsing Conservatives at election times: 9 times out of 12 elections in the last 40 years, including 2011. That's some 'Liberal bias.'
\item Given that their father assisted a lunatic who baked Jews in gas chambers, I would guess not.  http://www.huffingtonpost.com/entry/koch-refinery-nazis\_us\_569e9870e4b00f3e9863266c  https://www.nytimes.com/2016/01/12/us/politics/father-of-koch-brothers-helped-build-nazi-oil-refinery-book-says.html?\_r=0  Not sure what about the above two facts is funny, but it appears that G\&M threads are populated by a fair few sociopaths.  Wag the dog.
\item People like you.....'  So easy to tell the racists and sexists So what proof do you have that it was a 'transgender' that caused both ship accidents?
\item No, Tridentinus.  I come here for reasonable discussion of the issues both ecclesiastic and non-eclessiastic.   If your idea for a reasonable discussion is that someone has to leave the Catholic Church if they don't agree with you, then you are a troll.
\item Well, why doesn't the terrorist suspect hand himself in to police? Explain that one?  Of course his wallet would be either on himself or beside him while he committed his ISIS act of terror. Not too surprising either that the Islamist coward would flee the truck and forget his wallet.
\item Since the apostles were all Jews, then gentiles cannot be ordained. That is EXACTLY the same argument as the one about the apostles being all men, therefore women cannot be ordained.
\item Simply, why would the Liberals tie themselves to a sinking (NDBBQ) ship? The Liberals have far more upside, and the NDBBQ has only downside....come the next election..
\item <<I am curious what I look like thru 'hairy eyeballs.'>>  It seems I wasn't explicit enough: You look like a Catholic fascist.  But I didn't mean to derail the thread by throwing out a bit of snark.
\item Young and bright....' are there no older homosexuals?
\item The Chinese LOVE using the words co-operation and mutual trust. Believe me, I've done business with these folks and the co-operation and mutual trust only go one way. YOU co-operate and trust them, they will never extend the same courtesy to you.
\item 70,000 years'? How do you depict a transgender person with a cave drawing?
\item Sample needs a remedial course in catholic moral theology.  SAD!
\item Aspirin came from plants until it was isolated and put into medicinal form. What's your point? Digitalis is also deadly, hence the benefits from isolating it and controlling it purity, dosage, and usage.
\item really?  Should we kick out the Jews, the Irish, the Italians, the Sikhs, and anyone else you don't like?
\item Phew...and here I thought in 2017 that making fun of gays was wrong.  I guess the key is to be a progressive...
\item Nor is it okay for anyone to use the term ?you guys? (sexist).'Never mind the real world where groups of only women will use it in reference to each other.
\item Ultra-Orthodox Jews do not kill other Jews or Arabs and are not dangerous to anyone.
\item Just so you know, it's possible for people of all races to be racist. There are racist Asians, blacks, whites, Jews, Hispanics, aboriginals, and east Indians.
\item Hmm..my remark was certainly not uncivil.    But I'll change it just a bit.  Using your logic then...no one gets to make that accusation unless one is homosexual? So...what does that mean about those who make the allegations?  That they must be homosexual?
\item Sure...right after the IRS investigates all those left-wing Negro ministers and left-wing Jew rabbis.
\item Can you find the actual quotation, please? Because it was, in fact, an Israeli Prime Minister -- Itzhak Rabin -- who was assassinated by a Jewish-Israeli extremist for signing an agreement with the Palestinians.
\item Two questions: 1. Why Pope F. become a symbol of light instead of a pitch dark bottomless hole regarding clergy sex abuse of children? 2.  Is Pope F. consider as a Christian since he is hiding condoning his clergies rape children?
\item Who exactly are 'these people' that you speak of?  Do you mean all Muslims?  If so, then stop hiding and come right out with your bigoted, ignorant and baseless views.
\item The terrorists want a Christian right wing leader. It helps them recruit.   Their nightmare is the liberal, warm hearted and open minded leader. He makes it harder for them to recruit.
\item What's the difference between a Catholic Priest and a pimple? The pimple waits until after puberty before it comes on your face.
\item Gay men are not pedofiles but if you're a man who preys on boys, you're gay and a pedofile.  The gay community can try to argue otherwise but that is the way it is.
\item What a bigoted and discriminatory policy!  There is no mention at all of the trans-gendered, non-binary or 2-spirited in this policy.  Why is York U. openly discriminating against these groups?  Of course, I'm outraged.
\item like the nazis: those that were considered 'lesser than' the ideal. in their case Jews, Roma, Africans, and Slavs, the mentally retarded, the imperfect. we can add the old, the sick, with socialized medicine.
\item The Church shouldn't be ordaining anyone; that only confirms and feeds the clerical culture. Lay people -  female, male, trans, whoever -  should be empowered to preside at Mass. What makes an 'ordained' person any more worthy than anyone else?
\item i know women who live in Toronto and they tell me the best looking and stable men are mostly Gay.
\item @ Register-Guard, putting someone's name in triple parentheses is a white-supremacist means of targeting jewish people. It is hate speech. Please remove.
\item I wonder why the left continues to fight for allowing men in girls bathrooms and locker rooms? Seems strange behavior considering there are more pervs then transgenders.
\item What Canadians 'feel' is not relevant to the 100, 000 Canadians who have died in WWI, WWII, and Korea, to name a few. THAT is history, not current 'feelings' by a few.
\item and Christians do?  Guess you have selective use for free speech.  Sad.
\item For anyone who wants to help the transgender community fight intolerance, here's a GoFundMe campaign for an awesome nonprofit fighting the good fight:  https://www.gofundme.com/help-save-gender-justice-nevada
\item Deviance at its best means abnormal. At its worst means sexually perverted and compulsive. Not words to use when talking about transgender people.  Delusion is thinking there are only straight boys and straight girls and anything else is somehow abnormal or 'less than'.
\item ... ain't you Republicans all about restricting Freedoms and Liberties of others??!!  Ask a transgender VET to their faces.  Dare ya.
\item Transgender folks have always existed. It's just that most people are ignorant about it.
\item People claiming to be Christians are using our adopted religion to their evil benefit....
\item And we prosper.
\item When Obama was in office, only 30\% of white evangelicals would forgive a president's immoral behavior.   Now it's 72\%.   https://t.co/c6FlHbziMi
\item Unfounded.  Our military is not weakened by transgender people. Your example above is a fiction. Nobody is telling the military that they need to let anyone into any position regardless of performance.   You're insulting and dehumanizing people who are serving their country and it's sick.
\item Leadership, PMZ, Ohhhh hahahahah..
\item the government will make it illegal for a white man and a white women to breed as well the way it is going.   only question is will that come before the mandatory homosexuality laws.
\item Or any of the Islamist countries that treat women like second class citizens, demanding absolute submission to male authority under the guise of religious piety.
\item Canada ranks as one of the worse countries when it comes to vacation time. Leave the banked sick days alone.
\item McMaster university won't be getting any donations from me after what happened to the trans language prof. Agree with him or not but don't prevent him from speaking
\item Jocabe...... it is about having a qualified leader for the opposition. He is dangerous having no resume for the job. Garneau was so accomplished and probably brilliant and the Liberals rejected him over pretty boy Justin with the name.
\item Good grief, the thing has found an opening for its drool.
\item She is in the same line like her Grandfather! Granpda news said Russians and Jews were dirty animals and she still abhorres Russian. I don't know her feelings on Jews though.
\item I would believe that he is against it. I am hoping that he will deal with it and that many, many bishops and priests will be asked to leave (or retire) and then I hope that they are arrested and tried and jailed. Let's watch him. Let's pray for him.
\item Of course I wouldn't, but it wouldn't be because of transgender people; it would be because of a possible priest in there.
\item I suppose you've never heard of the Security Council, or why membership is important. But go ahead and maintain your ignorance, as Harper would want you to do.
\item Didn't Trudeau wag his finger and scold China,  Japan and Korea about how few women and transgendered persons are in the boardrooms of their national industries ?
\item Respect for people, not for ideologies.
\item I am not supporting Zille's thoughtless remarks, but to me the author's analogy with her tweets to colonialism that 'today’s Jews benefited from scientific advances made during the Holocaust' is unsustainably idiotic.
\item sylvia, All the Palestinians and Arabs had to do was not attacking Israel. Now the Jew-haters continue their terrorist tactics instead of negotiating. A topsy-turvy world, too difficult to research an issue when you can just ignore reality. Ever wonder how trump got in?
\item Got screwed by the liberals more than once. They became the LIEBERALS.
\item True sign of a cowardly bully is picking on weaker states while oozing out of office and never standing up to ISIS,terrorism,Communist China, and real issues.....bye... bye.... 'obummer'....Muslim plant,5th columnist,and worst President in U.S. history!
\item Anyone who professes to be a christian and supports Donald Trump is both a hypocrite and an idiot.
\item Bill C-51 threatens the rights of all Canadians, period.
\item That's a lot of words.   TL;DR version: I'm afraid my child will catch The Gay.
\item Whew - good thing this orange-glazed cracker wasn't President when the Jews were fleeing the Nazis.   Although, the USA, like Canada, did turn away one ship of refugees.
\item Catholic Social Services and City Government created cesspool.
\item All parishes need to become 'social justice' parishes.   The attitude of the institutional hierarchy is painfully obvious. They are becoming more and more irrelevant by their pathetic response to such Christian activities to help our poor and marginalised.
\item Leroy and Quinn,  look at her support from convicted felon Tom Anderson.  A guy who took bribes from a guy who was having sex with an under age Native Girl.  But hey,  they're both Christians, right?
\item We have not degraded the church as a moral guide, the church historically has degraded itself in horrific demented behavior. This is an excellent example; while white European Christians called us savages because of our gods, white PC liberals are calling us uncivil savages because of our mascots.
\item Americans don't ban Muslim women from wearing facial coverings. As far as I know it's not even on their radar. So why are Canadians so hyped up about it?
\item Bannon will go to war with people in Trump's circle that he sees as Globalists...and Jews. Get ready for a vicious cat fight on the right...grab the popcorn and watch the fur fly!
\item Danica Roem, elected to Virginia’s House of Delegates, became Virginia’s first openly transgender elected official . . . '  The right and proper response from a society that deems itself gender identity enlightened is 'Yeah, yeah, nice.  Is 'Pawn Stars' new or a rerun tonight?'
\item This article is a worthless rant... lets get on.
\item The media, the Liberal party, and the Canadian public 'suddenly discovered compassion', in Trudeau's words, after seeing the boy's picture. Of course there is no limit until their sin is redeemed.
\item Entirely anecdotal, but I've never had a bad experience in a public restroom. Ever. And to imply transgender people as perverted dudes in skirts is not accurate.
\item Other than one instance in Virginia all cases of vehicular mass murder are Muslim. But our media will never let us get over Vigina while never mentioning the full truth of the other 99.99999\% of cases.
\item The court does NOT create law - it just tells the politicians to rewrite the laws MORE CLEARLY. And they do and the system works - until some wing nut decides politicians should be dictators beholden to no outside scrutiny. Stupid move, wing nut!!
\item but I thought this was about children. Does bullying mall boys with a 'low masculine quotient' make them any less likely to grow into active homosexuals? - unless it kills them.
\item SayeSo Sayeth Martin, the Liberal uber-apologist.After the 'shock and awe' of Trump's victory, I'm surprised that he isn't still hiding in his 'safe space'.....
\item You're lonely yes, gay no.
\item Thanks for your support.
\item Well that settles it. All those scientists are wrong and HTexmes knows the truth. Thanks for letting us know. Perhaps you could have spoken up sooner and saved us a lot of angst, but at least now we know that there's nothing to this CO2 thing.
\item Wente's mistake. It was NOT the Israeli flag. It was a Star of David ( a Jewish not Israeli symbol ) on the Pride flag.
\item As is a trans women being a lesbian.
\item could of bot the homeless jew downtown a house with that money....but he wanted to be a big shot
\item Some aside...you tell such outrageous lies and now it's, 'jews by some estimates killed more germans than germans killed jews.'. I find your posts to be mostly phony BS but this one is simply disgusting. 'Have you no decency, sir?'  Two words - The Holocaust.
\item So Jews should be forbidden entry on the grounds of Psalm 137:8-9.
\item I seriously doubt that gay refugees are interested in that, given that they are fleeing anti-gay religions and cultures. Andrew --------------- what are these  anti-gay religions they are fleeing? Do these anti gay religions not also exist in Canada?
\item So headlines that include 'dangerous faggots' 'renegade jews' or 'muslin rape culture' aren't racist???
\item Oh well. Muslims doing what Muslims do.  Why do they hate each other so?
\item So all the preaching  in the mosque about extermination of Jews doesn't bother him?
\item How is this any different from the Kentucky clerk who refused to issue marriage licenses to gay couples?  If your religious beliefs are so against the gay community, then you had better not get a job or into a profession that is obligated to serve ALL people.
\item This sounds like a high school essay. Lots of platitudes and no substance.
\item Should tope pigmented people have problems? There are no people of any variety of pigment that are free of problems.
\item BROohthor  As Christians, are we are not called to stand opposed to ALL (euthanasia) of what is going on with this.  kevin your brother In Christ
\item His letter really is the definition of intolerance, a basket full of deplorables no? I would propose that far more Americans identify as Christians than 'Liberals'. That's a lot of hate and moral superiority from the left. Nothing new.......
\item I'm not sure you understand what I'm saying at all.   1. What laws are you referring to? 2. How am I being permissive of sexual misconduct over one orientation or the other? I've made it pretty clear that gay or straight: sexual misconduct is wrong.
\item Morality is always arguable . . .'  Let me understand:  The morality of, say, exterminating 6 millions Jews is arguable?
\item To imagine that the action of Baird and Harper had on recent events in Iran is quite delusional..
\item And making sure there's plenty of tranny solders and they can be assigned to the new Space Cadet Corps where they can be called Star Ship Trannies.
\item The Germans are going to love that.
\item Worst idea ever, you would be hurting the very people you profess to help.
\item The Father of Secularism was a medieval Muslim. Ibn Rushd, aka Averroes, lived in the 12th century. He was a brilliant scientist, philosopher, and Islamic theologian.
\item Good thing you're around to bring people together... I'd rather have lunch with the current head of Al Qaeda than spend time with you.
\item Can we stop calling it a 'Muslim ban'?'  No.
\item C'mon, Wente! If these privileged no name celebs weren't sticking their nose in others' business, what would they do with all that dead air time?
\item Yes, crime is always justified when committed by the regressive right. I bet you think the Jews in Germany also deserved it in the 1930s?
\item I have no regard for Trump, but not to worry, the left wing media will shamelessly shill for Clinton. No less than the Canadian media shills for the left.
\item There were probably a lack of trans gender people so our government boycotted the meeting
\item Tri, don't use their language.  'Homophobia' ostensibly implies a fear or persecution of a person; whereas those who are concerned with those who self-identify as 'gay' do not fear or persecute the person.
\item You make two good points. but neither excuse the fact that :  many  Ukrainians  helped the Nazi's kill Jews, and  the  Kremlin choreographed secession of the Crimea was ultra vires   and simple state thuggery
\item Which is why Christians like having sex with 13 year olds, right? I mean, that is how your good lord intended it, right?
\item what would he be bragging about?! People brag about accomplishments.  What kind of sick and deranged human being would brag about kiling her? Be proud of killing a Catholic priest child molester Be proud of killing Ted Bundy.  But her?
\item Lol, i love when people talk like this, not raging at you gary, but. It shows how ignorant you are. You can't just become transgender. There is soooo much you have to do, and prove. Years, even decades can pass before everything is done.
\item The following countries BAN any Israeli Jew from even entering their country: Syria Iran Iraq Yemen Libya  Algeria Bangladesh Brunei Kuwait Lebanon Malaysia Oman Pakistan Sudan Saudi Arabia United Arab Emirates
\item When we see gay people arguing for reverse conversion therapy to turn straight people gay, and black people working to systematically disenfranchise and deport white people, then we can talk.
\item her beliefs are misogynistic, anti-semitic, anti-gay, and anti-science so her hurt feelings really dont mean that much to me.
\item Considering a govt can get elected with only 39\% of the popular vote eliminating the views of 20\% of the population is just stupid.  Transgendered people represent less than 1\% of the population so from your comment they can be ignored as well.
\item Being a Mob Boss is one thing, ordering the murder, extortion, prostitution, money laundering, drug dealing, et'c are sins.  Being a homosexual man or woman is not a sin.
\item Peterson is pretty clearly a bigot - not because of refusal to use the 31 customized pronouns, but because of his public statements that transgender people don't deserve to be recognized as existing at all.
\item Exactly. The US passed the Magnitsky Act, and they're at the table. Dion simply caved and cravenly sucked up to Putin. End of story.
\item And we also have the duty to avoid prostituting our Catholic identity by appeals to phony dialogue that mask an abdication of our moral witness.'  (Archbishop Chaput 2009)  What a nasty comment!
\item Maybe if the Democrats would stop pandering to every identifiable special interest group they would have a chance to be seen as serious people. When your message is aimed mostly at people who care about transgender bathroom access and microagressions, you are going to lose more than you gain.
\item Terrorism is a modest, immediate threat to the United States.' Tell that to the 911, Boston Marathon, and San Bernardino families. The writer is a racist, blaming Jews. Shame on the RG for allowing this Holocaust-supporting writer to express his hatred.
\item I think a lot of so called Christians missed those verses.  They are more into the prosperity gospel.
\item Probably not so much a transgender agenda as much as a higher-ratings-play agenda.
\item When will the Iroquois nation pay back the surviving Huron natives for the genocides of the 18th Century? That reparation and reconciliation should be worth a few billion by now in today's money.
\item But more can always be done'  I agree, I would like to see the 'peaceful' Muslim community band together and create a revised Quran, that deletes the passages that advocate violence and killing. I feel confident that Alah would not object, given that ISIS has even been attacking other Muslims.
\item I correct myself... In other worlds, all people (not all Muslims) must follow their divine leaders teachings that say: join them or die!
\item Wait till they find out she is a black transsexual , then watch them spin
\item Fred you are than Islamoprobic who hate Islam and moslim. Islam is than peaceful religion. Terrorist arenot moslim.
\item As you know, I support the LGBT cause and object to the notion that gay marriage is a sin.
\item It is you who are mocking Christ and His Church by attempting to separate Him from his Church. Trent rescued Christ's Church from the errors of Protestantism yet you want to drag us back there again.
\item So another gobbet of bile as a substitute for any kind of argument - well done
\item Are you seriously calling the abuse of thousands of young people'fun for the gay clergy'?  What a totally disgusting comment!
\item Uhm Laureen put in a ten hour day yesterday, stop being a Union liar...
\item A bureaucrat's job is to advise, it is up to the politicians to make the decision.
\item I find it hard to take this congresswoman clown serious, she looks like a transgendered cowboy/girl. What a joker!
\item No one cares. 
\item So why isn't the attack on the mosque a 'terrorist attack'? Is it only'terrorism' when muslims attack others?
\item You're being ridiculous. A trans gendered woman (formerly male) would simply be considered a woman, and women can be in the military. Are you now arguing that women shouldn't be allowed in the military?
\item Is this a GOP party fundraiser or one of Pence's gay conversion clinics? Don't get me wrong, I think both are equally horrible and a huge waste of time and money ....
\item It is not a Muslim ban.  It affects non-Muslims also from the six countries.  And 90\% of world's Muslims from fifty odd countries are still allowed. But the lying media continue  jihad against President Trump on so called 'Muslim ban'
\item One yearns for a time when Canada as a nation can concentrate on what we can achieve together, all of us working towards a future where we have one equal citizenship for all.
\item Hitler  wasnt targeting Jews either.
\item And then what have you to say of the LGBT and trans 'forcing' the acceptance of their life style onto those religious people ?
\item how old are you? you can’t be over 12
\item with respect, far too many of those 'intelligent, articulate' members of the conservative party do themselves a disservice by demonstrating neither quality.
\item Who is this 'true' Christian? The one who bragged about  sexually assaulting Women and surrounds himself with the KKK, Neo Nazis and called Mexicans 'rapists and killers?' Don't be shy now.
\item Stephen ? Which are you ? a proud Homophobe ? Xenophobe ? Racist ? Or another closeted gay Republican ?  wear it loud and proud, get a big ' L' tattooed on your forehead.
\item 50 years? It has been 65 years since the european invaders seized Palestine. Put an end to the Nakba and unite Palestine from the Jordan River to the Mediteranean Sea! Put and end to the zionist scourge!
\item Canada has more than enough challenges right here at home. While I feel for the Chechnyan gays, they are simply not a priority for our tax dollars.
\item The prime minister (much less the cabinet) can not be elected directly because ours is a responsible government system. You'd have to change the constitution absolutely entirely if you wanted presidential-style elections.
\item Why to care about birth rate (which is the major characteristics of good government) if the government of Canada is more concerned with expanding homosexuality and immigration?
\item Surprisingly there is mention of any dialogue about US access to Canada's transgender washrooms.
\item What a waste of time this guy is...very inexperienced in he needs a reality check..
\item I've never met anyone who blamed their lack of success on 'nasty females, queers, coloured  folks'....obviously we move in different circles.
\item Go cry to mommy.
\item We're not distinct from America. Get serious. They should erase that border so we can align our economic interests instead of Canada being the backwater that it is. Grow up.
\item Merely proof that the Roman Empire policy of ' Bread and Circuses' for the proletariat was sufficient governance .....
\item I would like to attend a gay, white supremacist wedding, just out of curiosity.'  So..you think it's impossible for a homosexual to be racist? You don't get out much..do you? The Little Guy
\item Are you so naïve that you think the Muslims in this country really care what we think?  They just up their birth rate and bide their time.
\item for all of you who dont know, Michelle Obama was born a male.  She is the first transgender spouse of any president.  Joan rivers was killed during THROAT surgery after speaking out about this.
\item These foul bast@\#ds traffic in blatant lies and outrageous conspiracy theories and pretend to be Christian. My god but we are in the midst of some dangerous times. When people can no longer separated the wheat from the chaff we no longer have a democracy.
\item when you confuse  Anti-Muslim hate for  Anti-Radical Islam hate therein lies the confusion
\item Instead of restrooms, we'll only have porta potties installed.  Problem solved.  Transgender friendly restrooms.
\item Check ignition ....and may God's love be with you
\item The liberal FAKE NEWS media doesn't want to report about the anti-semitism directed at conservative jews.  Oh no. That doesn't help their neo nazi narrative.
\item This person came from a settlement that, in the eyes of the U.N., was illegal. Nothing to do with Jews - except for Jews who steal other people's land.
\item To see a preview of 'Fractured Land' or to donate to it's production: www. indiegogo.com/fracturedland
\item Well now that oil prices are down, he should probably just prorogue parliament. The Christmas break can't come soon enough, eh Harpo?!
\item Limit the PMO to 2 mil per annum in salaries. 1500 people is crazy.
\item After January 20th, Muslims will become (to use your favourite term) untouchables in the US. Not allowed to use schools, airports, hotels, restaurants along with their white counterparts.   Kind of like African Americans had to go through segregation. Bet you support that too!
\item Headline.............'Konrad should show a little understanding of reality!'
\item What if it was a child molester?' Then you would be a priest and be covered?  However, the catholic church has harbored 1000s of these ppl
\item Is the Pope Catholic?  Of course gun reforms will help curb gun violance.  Look at Australia.  Stupid to just continue to ignore this problem so that big business can make a few bucks.
\item maybe.  this is a continuation of a robo call to Jewish centres throughout North America.  Not sure why but I would suggest Trump has unleashed the worst in people.
\item Oh a trans-woman would be the wet dream. Its called 'intersectional victimhood', wherein you get to claim victim status for more than one thing. I wonder if you can get merit badges to sew into your vest, to show how many ways the patriarchy oppresses you?
\item My wife is Chinese and I'm White. This fact is almost never brought up between us. My wife told me the other day she forgets that I'm not Chinese. What goes on in these bitter people's minds?
\item threatening a person and name calling are substantively different. while both are uncivil only one is criminal
\item Very, very funny and really reflects Mr. Harper's weird way in which he is unable to answer any question given to him. I can see that 4thot is already upset at the accurate representation of our Prime Minister.
\item A Russian Ambassador is murdered by a Turkish Islamist and already the press in both Turkey and Russia are blaming the West in general and the US in particular.
\item But Trump will appoint judges who will protect fetuses and stop gay marriage, so it's all good - or so we've been told.
\item Tell that to the Ukrainian Catholics and the other Eastern Catholic churches that do not use Latin and never have.
\item Psychology is post-christian-rubbish.
\item How nice of Wohlforth and the Dispatch----they allow us to comment on this story , but to heck with what we think concerning his gay issue story .  Wohlforth and the Dispatch are against and ban free speech when matters dear to their heart are written about.
\item Knowing Donald Trump, he will ban Muslims from carrying laptops onto US-bound planes...
\item Of course 'all thy sons' should be dropped. It's 2016.'All of us,' though, is not very poetic 'All our hearts' is better: True patriot love in all our hearts command.
\item the Nazi and the Vichy French were involved with the killing of jews
\item ACPeds?  You mean the politically-motivated anti-LGBT hate group that's a fraction of the size of the well-respected American Academy of Pediatrics that supports trans kids?  Oh.  Those 'experts' in damaging children's health.
\item We must tolerate what we regard as barbaric cultural practices that do not break any laws. Thus we should tolerate the burka but not 'family honour' violence. So an immigrant who admits to having a strong sense of family honour should be screened.
\item Yes, let's end the insanity!  No more trans people! No more boys kissing boys! No more rock n roll music! Let's get back to the good ol' days of the 1950s!
\item Oh, I see, Alexvega... so, In other words, guilty until proven innocent, hmm? Yup... quite simple. Except that our justice system works on the reverse premise. Next...
\item Portapotties are transgender public-use toilets, as are airplane lavatories. All public use toilets should be one-at-time, one room, one-holers. People who think about sex in  a public toilet room are super gross.
\item Khadr is a real Canadian Hero after undergoing torture at the hands of the Civilized Americans and spending years of illegal incarceration at their offshore Black Hole prison in Cuba.
\item Think if Justin trudeau was PM he would make the rounds of all the Arab states ring kissing.
\item Vatican II was supposed to 'fix' the product and the Church went from good to bad.
\item Slanderous comment from The Great Malumba.
\item I'm not referring to the CBC as an entity but what it accomplish in connecting us as an nation.
\item This is the Catholic bishops dream - women as cows.'  A truly sick, bovine thought.
\item You mean that laughable double standard where 'blacks' and 'Jews' have historically oppressed 'whites'? Yeah, so laughable.
\item He refused to design ANY kind of wedding cake from the moment he heard the wedding was for a gay couple. This is all about religious conservatives wanting the absolute right to discriminate against gay couples while still being protected by the civil rights laws from discrimination against them.
\item SJWs at U of T have made laughing at trans-gender pronouns an actual criminal act,   punishable  by arrest, imprisonment  and fines.
\item I assume the transgender athletes are all taking hormones and/or steroids?  I don't know how you can call the Olympics clean when different people have different rules. . Not that they are clean in any event ... but they don't seem to even try to appear clean anymore
\item She has the same right as every other person writing editorials in this paper.  Why would she have any less right becuase she happens to be a Muslim?    You probably also believe that women belong in the kitchen, you misogynist bigot.
\item What's weird is the must be gay accusation only plays to right wingers.
\item Evidently, Layla is perfectly fine with the LGBTQ community not being represented in any manner.  But fortunately, the Supreme Court is not.
\item What, you think guys with effeminate characteristics like Martin and other gay men are new in society?
\item You might recall that six men were shot to death recently while at prayer in a mosque because they were Muslim.
\item It looks like the K brand poverty pimps just write other columns occasionally here at the Globe ... giving us a 'balanced' perspective. Wonder if they are paid for their columns, and where that money goes?
\item ...or more accurately 'some animals never got to be equal.. yet'. Our First Nations need a little more time and consideration to be considered equal in a lot of Canadians' eyes.
\item Republican party FILTHY w super fakey 'christians'.  They'll stab in you in the back for a buck, wave a flag, then kick you in the face ...
\item I'm much-more concerned with her wardrobe.  Where does she get those outfits?  Doesn't she know any gay people?
\item Who is this evil Catholic woman enterpreneur who does  not pay her workers properly? Can we name some names?
\item wow you are a fool
\item It's also about time that you and your parents and relatives who have settled on lands belonging to the native peoples begin to evacuate and leave just as the UN resolution demands of Jews living in the West Bank. Get moving, you racist hypocrite!
\item I think it is time for Justin to name to the court the first trans indigenous person...why?  Because it's 2017 silly....
\item The Fleur de Lis is a religious symbol.
\item Now I understand why you support Trump so fervently. You are incapable of logical or rational thought.
\item Not that long ago that Catholics had to cover their heads at mass (remember the ridiculous hanky thing?)! Most of the Muslim women I know do not cover their hair- let us not get crazy about this.
\item I include you Elaine in my nightly prayers, I pray that everyone of your Grandchildren is healthy, happy and gay.
\item Close the MSM down, get rid of the jews that run them..they are the problem
\item Oh please. This story is over 70 years old.  What about a write up on at least one Jew saving an Arab from their own government's continual holocaust of Palestinians happening today? No, never in the G\&M.
\item Oh yes it can!  Bishops do it all the time!  The surest way to suppress dogma is to EGNORE it, as the hierarchy has long been doing in reference to the Catholic clergy sex abuse crisis.  Did they skip Catholicism 101, or what?
\item Complaining that you might get blown up on the way to vacation is islamophobic.
\item Are the Muslim women protesting Islam and Muhammad for relegating them to lower status than men?
\item Because gays make up a large segment of the priesthood? Because sexual predisposition, by definition, does not appear only in certain categories of faith ?
\item What is your source for this statement since there are many examples of abuse of females, Marie being a prime example? Since bishops and cardinals used to be priests, how many are gay? A Goggle search will show many of them have offended against both male and female children.
\item GAR385 Less Americans voted for Trump than voted for Clinton. -------------- FEWER Americans voted for Trump than voted for Clinton. It would not hurt to bring back teaching grammar
\item Knew he wasn't a white Christian, or much of an American. When Americans do this this we use all kinds of guns, guns and more guns and lots of ammo. This guy clearly wasn't fully assimilated into our society.
\item A nation must have common values that bind people together. Canadians will need to have this discussion, but I can't see any existing party brave enough to suggest this.
\item Fine--why is he not condemning politicians --especially 'Catholic' politicians who support abortion with the same veracity?
\item This is a perfect example of the RG mocking Christianity..... by not making a simple grammar edit from 'feast'  to 'festival', they maliciously embarrass an obvious ESL christian.  Pathetic.  Any display of Christianity in Eugene nowadays will get you tased and jailed by the PC brownshirts.  /s
\item the Globes painful attempts to avoid the word Islam  ... what a clown show
\item Just as Bill Clinton claimed to be the first black president, Obama will claim to be the first trans president
\item Homophobia isn't fear of homosexual people, it's fear of homosexual feelings/attractions the person has inside their own mind. Thor has a semantic point.
\item Everyone in that crowd who was carrying tiki torches and chanting 'Jew will not replace us!' and 'blood and soil!' is a terrorist. Do your research.
\item Dump the monarchy, elect a president (keep calling him GG if you wish) and give that president-GG power and authority to protect parliament from government and PMO abuses. Oh, and dump the senmate.
\item The Jewish circumcision of male infants could be called 'barbaric'. And we're ashamed of the time we didn't welcome them here.
\item The KKK and Nazis hate Jews. Trump is surrounded by Jews. His daughter is a convert and his son in law is Orthodox Jewish. Trump's grandchildren are Jewish. Before you go there, Trump also has a black friend named Dr. Ben Carson.
\item No, I am not a sore/poor loser.  I think this so-called genital grabbing president has expressed bigoted views, backed people like Bannon, who hates Jews, and is a Putin lover.  Instead of being a unifying this country he is dividing it even more.
\item They should win - - as long as they can put shock-collars on the WildRose fascists to stop them spouting-off inane anachronisms; denouncing and hating: women, homosexuals. environmentalists, non-white Canadians, labour laws, and any person or activity that doesn't increase the profits of U.S. and foreign oil companies...
\item Is an 'independent mind' at liberty to breach a 'sacred trust'? -- especially a Pope's. We'll see if Benedict XVI is capable of producing more theological masterpieces in the future.
\item Yes - Canada is based on the fundamental principle of good government.
\item I guess that was a primary reason Canada didn't allow Jewish refugees during World War Two. It was very hard to cross check with Nazi records if any of the applicants was a mass murderer or a judge!
\item Yes, I did know that. But it's a tradition for us to ask presidential candidates this silly question. In past years, it's elicited the only non-scripted moment. Should I not have asked him because he is Jewish? No, I don't think so.
\item allow Military-grade assault weapons to be sold to anyone who isn't a Muslim or a known criminal?'   Specifically what 'military-grade assault weapons' are you referring to?  Not recalling any of that involved in recent situations.
\item True, but those who incite violence at 'rallies' do self-identify as both 'republican' and 'Christian.'  They did vote for Trump, and he did thank them.
\item I lived in a semi rural western town. They are more religious, anti-gay, and unlikely to vote for the Liberals and NDP. Luckily, they are declining as proportion of the population.
\item Given this president's insecurities, he likely feels that his manhood is threatened because there are transgender people that want to serve, while he couldn't run away from serving fast enough when it was his time.
\item It's just the staff writers and their multiple sockpuppet accounts that insult and harass you all the time.
\item 1) because of Islam, which is an all or nothing, fight to the death philosophy 2)  because of Islam, which is an all or nothing, fight to the death philosophy
\item Tell that to the Ethiopian Sephardic Jews
\item For an alternate view on 'generosity' toward refugees, see: http://montrealgazette.com/news/national/opinion-canada-can-and-should-do-better-on-syrian-refugees
\item In an attempt to be civil, I find great difficulty with the Jew Bernstein.  In my opinion, he has always be and will continue to be scum.
\item They should be worried. The liberalism in Europe has allowed for the emergence of another fascist ideology - political Islam. People have every right to be worried and the only party willing to talk about this issue is the right wing.
\item I'm holding out for the Transgender doll with mix and match body parts.
\item First you crazy Jesus freaks tell us everything on the Earth 'God' made.  Then, you claim that his, 'son' Jesus doesn't want us to use it?  Make up your mind, Ned Flanders.  'Let it grow...let it grow...greatly yield'!
\item Geez, a shame your school wasn't interested in teaching you how to read. Try re-reading it with both hands on top of your desk, westelca21.
\item But of course. That is why I never seek advice from people older than me about anything, since I know better than they do.
\item It is very sweet and normal to have a lasting relationship with someone that stretches into decades. Congratulations to anyone who sticks it out to the end.
\item Yes and these 'non-white' Catholics, as the race obsessed  are constantly drawing our attention to, bring their own prejudices and problems.  What's your point?
\item We all know your views on gay men.  Though I have to wonder, how does the life choices(which it's not a choice) of gay men effect you.  Are you at risk for HIV infection from either a gay man, or injection drugs?
\end{enumerate}

==> sections/methods.tex <==

\paragraph{Participants}
Our data collection process aimed to recruit a balanced set of annotators from eight geo-cultural regions, namely, Northern America, Latin America, Arab Cultures, Sinosphere, Oceania, Sub Saharan Africa, Indian Cultural Sphere, and Western Europe.\footnote{Our efforts for collecting data from Eastern Europe halted because of the Russia's war in Ukraine.} We recruited at least 450 participants from each region ($N_{participants}$ = 4309), %through the Qualtrics panel.\footnote{https://www.qualtrics.com/research-services/online-sample/}. 
represented by 2-4 countries, 
with at least 100 participants per country,
% balancing country representation within each region,
except for South Korea and Qatar where 
we managed to recruit only a smaller number of raters. See Table~\ref{tab_stats} for country-level statistics.
% we did not manage to achieve this quota.
While typical raters recruited through a dedicated annotation platform or service possess specialized training or experience that may influence how they complete tasks, most platforms feature a relatively limited degree of cultural representation within their pools. As a result, they are less appropriate for specifically and robustly evaluating cultural differences and their relationship to annotation judgments.



% For each region we controlled for balanced representation of binary genders (less than 60\% female, and less than 60\% male), and age (15\% over 50, 25\% between 30 and 50, 60\% between 18 and 30). Since the survey items were all in English, we controlled for participants’ proficiency in speaking and writing in English based on their self report.


\paragraph{Annotation}
Each participant was assigned to annotate offensiveness of 40 textual items with a value between 0 (not offensive at all) and 5 (extremely offensive). We asked participants to decide whether they perceived them as offensive, noting that ``whether something is offensive or not may depend on the context in which this message is exchanged, which we are not providing you in these questions. Please make the best assessment based on the information/context you have from the provided text.'' Moreover, half of the participants were provided with a note that defined \textit{extremely offensive language} as ``profanity, strongly impolite, rude or vulgar language expressed with fighting or hurtful words in order to insult a targeted individual or group.'' Other participants were expected to label items based on their own definition of offensiveness. Participants’ common understanding of offensiveness was tested by 5 (non-offensive) controlled questions randomly distributed among the 40-items annotation process. Participants with at least one wrong answer were excluded.




\paragraph{Stimuli}
Textual items were selected from Jigsaw's Toxic Comments Classification dataset \cite{Jigsaw-toxic}, and the Unintended Bias in Toxicity Classification dataset \cite{Jigsaw-bias}.
We set our data collection goal to increase the chance of evoking disagreements, and involving different moral judgments in annotations. To address the former, we randomly selected items from Jigsaw's Toxic Comments Classification dataset, prioritizing those with high disagreement levels. To measure disagreements on each item, we averaged annotators' toxicity scores ranging from 0 (lowest toxicity) to 1 (highest toxicity). We chose items with a normal distribution centered around a toxicity score of 0.5 (indicating highest disagreement) with a standard deviation of 0.2.
To select items that would potentially evoke moral reasoning we collected items from Jigsaw's Unintended Bias in Toxicity Classification dataset with moral sentiment, labeled by on a supervised moral foundation tagger trained on the Moral Foundations Twitter Corpus \cite{hoover2020moral}. We also collected a third set of items each mentioning at least one social group (this information is provided in the Jigsaw's raw data), to assess annotation of language that is potentially offensive toward different social groups.

\ifthenelse{\boolean{pnas}}{
%%%%%%%%%%%%%%%% PNAS FIGURE
\begin{table}[ht]
    \centering
    \scalebox{1}{
    \begin{tabular}{m{5em} m{18em} m{5em}}
    \toprule
        Foundation && $F$(7, 4287) \\\toprule
        Care & \includegraphics[width=.25\textwidth]{img/care-variance.png} & 34.477*  \\\hline
        Equality & \includegraphics[width=.25\textwidth]{img/equality-variance.png} & 13.368* \\\hline
        Propor. & \includegraphics[width=.25\textwidth]{img/propor-variance.png} & 51.240* \\\hline
        Authority & \includegraphics[width=.25\textwidth]{img/authority-variance.png} & 102.250* \\\hline
        Loyalty & \includegraphics[width=.25\textwidth]{img/loyalty-variance.png} & 158.300* \\\hline
        Purity & \includegraphics[width=.25\textwidth]{img/purity-variance.png} & 203.550* \\\hline
        \includegraphics[width=.45\textwidth]{img/title.png}&  &  \\\hline
    \end{tabular}}
    \caption{Distribution of the moral foundations scores and the results of one-way ANOVA analysis conducted for each moral foundation across regions. *means the $p$-value of the analysis is lower than .001}
    \label{tab:moral-region}
\end{table}}{
%%%%%%%%%%%%%%%% NEURIPS TABLE
\begin{table}[]
    \centering
    \scalebox{.72}{
    \begin{tabular}{m{1em} m{2em} m{1em} m{.5em} m{1em} m{2em} m{1em}}
    \toprule
        Foundation & Distribution & $F$(7, 4287) && Foundation & Distribution & $F$(7, 4287) \\\toprule
        Care & \includegraphics[width=.35\textwidth]{img/care-variance.png} & 34.48* && Authority & \includegraphics[width=.35\textwidth]{img/authority-variance.png} & 102.25* \\\hline
        Equality & \includegraphics[width=.35\textwidth]{img/equality-variance.png} & 13.37* && Loyalty & \includegraphics[width=.35\textwidth]{img/loyalty-variance.png} & 158.30*  \\\hline
        Propor. & \includegraphics[width=.35\textwidth]{img/propor-variance.png} & 51.24* && Purity & \includegraphics[width=.35\textwidth]{img/purity-variance.png} & 203.55*  \\\hline
        \multicolumn{7}{c}{
        \includegraphics[width=.9\textwidth]{img/title.png}} \\\hline
    \end{tabular}}
    \caption{Distribution of the moral foundations scores and the results of one-way ANOVA analysis conducted for each moral foundation across regions. *means the $p$-value of the analysis is lower than .001}
    \label{tab:moral-region}
\end{table}
}


\paragraph{Regions and Countries}
Our selected list of geo-cultural regions and countries within regions is not meant to be exhaustive, rather just to make sure that our study is done on a set of countries with diverse cultural histories. Each region listed has countries and sub-regions that have distinct cultural practices, and it is wrong to assume that the country we choose would comprehensively represent that region. Similarly, the countries listed are meant as likely places to collect data from, based on familiarity with previous data collection efforts, which potentially reflect the power structures existing within those regions. Also, each country is rarely a monolith in terms of culture (e.g., India has diverse subcultures, Australia being characterized as a ``Western'' culture erases the vibrant Australian Aboriginal culture). Data collected would also reflect the local disparities in who tends to be in the social strata that maximally overlaps with the data-collection workforce in those respective regions, and what subcultures they represent.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}





\paragraph{Moral Foundation Questionnaire-2}
After annotating items, participants were asked to fill out the Moral Foundation Questionnaire \citep{atari2022morality}, which includes 36 statements, each concerning one moral value by extending the the moral foundation theory \cite{graham2009liberals} (i.e., \textit{Care}, \textit{Equality}, \textit{Proportionality}, \textit{Loyalty}, \textit{Authority}, and \textit{Purity}). Participants' concerns regarding each item were captured on a 5-point Likert scale, and items where aggregated to calculate 6 moral scores for each participant.

\paragraph{Test Items}
We used participants' response to 5 test items to evaluate their understanding of offensiveness. These items (listed below) were unanimously labeled as \textit{not offensive at all} by authors and were used as an attention check to remove participants who annotated them otherwise. 

\begin{itemize}[noitemsep,nolistsep]
    \item Could you explain your point in a little more detail please.
    \item The NY Times yesterday had a rebuttal by the Iranian UN ambassador.
    \item Ditto to everything said here.
    \item Just looked at the link. Impressive and missed opportunity.
    \item Don't be so hard on yourself. Your life will go on.
\end{itemize}

\paragraph{Data Cleaning}
We selected thresholds for the amount of time needed to finish the survey and removed annotators who performed the task either quicker or slower than the expectation. Annotators with similar answers to all items were also removed from the data.

\paragraph{Mediation}
We perform the mediation analysis on the annotator level by aggregating annotation labels provided from each annotator. While annotators labeled different parts of the dataset (each annotating 35 out of the 5k items) equal number of annotators from each region were assigned to label the same set. In other words for each set of 35 items, there are 3 annotators from each region that labeled the whole set. 


% \paragraph{Analysis without China} Since the data from China seems to be particularly different from all other countries (even countries within Sinosphere) we repeated all analysis on all countries excluding China. This issue might be due to the country's particular regulations on speech. Analyzing how country-level regulations on language can affect annotators is an important question that needs further investigations, which is out of the scope of this work.

% Rerunning the mediation analysis shows that the effect of regions on annotation labels remains, with the mediation impact of Care (with $ACME$ = -0.043, $p$ < .001), and Purity ($ACME$ = -0.015, $p$ < .001).

%\paragraph{Jigsaw vs. Perspective API labels}
%An item-wise correlation test shows that while labels from Jigsaw and Perspective API are in moderate correlation (Pearson correlation of $0.48$), and they tend to have lower correlation with majority votes of different regions. It is important to note that the low correlation between Perspective API and Jigsaw labels are potentially due to the high disagreement in original annotations provided for our set of items in the Jigsaw dataset. As described previously, we have selected items with high disagreements from Jigsaw datasets, such that while the average inter-annotator disagreement on all Jigsaw items is 15.6\%, the average disagreement score on the set we selected is 62.7\%. Therefore, it is natural for Perspective API to not have high accuracy in predicting Jigsaw labels.


==> sections/morality.tex <==
\begin{enumerate}
    \item Caring for people who have suffered is an important virtue.
    \item The world would be a better place if everyone made the same amount of money.
    \item I think people who are more hard-working should end up with more money.
    \item  I think children should be taught to be loyal to their country.
    \item  I think it is important for societies to cherish their traditional values.
    \item  I think the human body should be treated like a temple, housing something sacred within.
    \item  I believe that compassion for those who are suffering is one of the most crucial virtues.
    \item  Our society would have fewer problems if people had the same income.
    \item  I think people should be rewarded in proportion to what they contribute.
    \item It upsets me when people have no loyalty to their country.
    \item I feel that most traditions serve a valuable function in keeping society orderly.
    \item I believe chastity is an important virtue.
    \item We should all care for people who are in emotional pain.
    \item I believe that everyone should be given the same quantity of resources in life.
    \item The effort a worker puts into a job ought to be reflected in the size of a raise they receive.
    \item Everyone should love their own community.
    \item I think obedience to parents is an important virtue.
    \item It upsets me when people use foul language like it is nothing.
    \item I am empathetic toward those people who have suffered in their lives.
    \item I believe it would be ideal if everyone in society wound up with roughly the same amount of
    money.
    \item It makes me happy when people are recognized on their merits.
    \item Everyone should defend their country, if called upon.
    \item We all need to learn from our elders.
    \item If I found out that an acquaintance had an unusual but harmless sexual fetish I would feel uneasy
    about them.
    \item Everyone should try to comfort people who are going through something hard.
    
    \item When people work together toward a common goal, they should share the rewards equally, even
    if some worked harder on it.
    \item In a fair society, those who work hard should live with higher standards of living.
    \item Everyone should feel proud when a person in their community wins in an international
    competition.
    \item I believe that one of the most important values to teach children is to have respect for authority.
    \item People should try to use natural medicines rather than chemically identical human-made ones.
    \item It pains me when I see someone ignoring the needs of another human being.
    \item I get upset when some people have a lot more money than others in my country.
    \item I feel good when I see cheaters get caught and punished.
    \item I believe the strength of a sports team comes from the loyalty of its members to each other.
    \item I think having a strong leader is good for society.
    \item I admire people who keep their virginity until marriage.
\end{enumerate}
